Certifiably Robust Policy Learning against Adversarial Communication in Multi-agent Systems

Communication is important in many multi-agent reinforcement learning (MARL) problems for agents to share information and make good decisions. However, when deploying trained communicative agents in a real-world application where noise and potential attackers exist, the safety of communication-based policies becomes a severe issue that is underexplored. Specifically, if communication messages are manipulated by malicious attackers, agents relying on untrustworthy communication may take unsafe actions that lead to catastrophic consequences. Therefore, it is crucial to ensure that agents will not be misled by corrupted communication, while still benefiting from benign communication. In this work, we consider an environment with $N$ agents, where the attacker may arbitrarily change the communication from any $C<\frac{N-1}{2}$ agents to a victim agent. For this strong threat model, we propose a certifiable defense by constructing a message-ensemble policy that aggregates multiple randomly ablated message sets. Theoretical analysis shows that this message-ensemble policy can utilize benign communication while being certifiably robust to adversarial communication, regardless of the attacking algorithm. Experiments in multiple environments verify that our defense significantly improves the robustness of trained policies against various types of attacks.

==> 1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% \draft{We study the attacks and defenses in communicative multi-agent reinforcement learning.


% Our contributions:
% 1. formulate the adversarial problem in CMARL.
% 2. propose a certifiable defense algorithm
% 3. empirical study in a simulated game and a market environment.
% }

% Recent years have witnessed significant advances in reinforcement learning (RL), especially deep reinforcement learning (DRL). Although vanilla RL considers the interaction between a single agent and the environment, many real-world applications have multiple agents involved, such as autonomous driving~\cite{shalev2016safe}, robotics~\cite{dudek1996taxonomy}, etc. 


% \ys{start from decision making?}
With the rapid improvement of deep reinforcement learning (DRL) techniques, neural network-based multi-agent reinforcement learning (MARL) has achieved significant advances in many real-world applications, such as autonomous driving~\cite{shalev2016safe,sallab2017deep}. In a multi-agent system, especially in a cooperative game, communication usually plays an important role. Through communication, each agent can obtain more information about the environment and other agents, and thus can learn a better policy. Many recent works~\cite{foerster2016learning,hausknecht2016cooperation,sukhbaatar2016learning} have shown that feeding communication messages to RL networks can result in better decision makers.

However, neural networks are shown to be vulnerable to adversarial attacks~\cite{goodfellow2014explaining}, i.e.,
% , especially network-based RL policies~\cite{huang2017adversarial} \fh{network-based RL policies are not a special case of neural networks. So the logic here is a bit unsmooth.}, 
a well-trained network may output a wrong answer if the input to the network is slightly but deliberately perturbed.
% if the inputs to the network are slightly but deliberately perturbed, the network, although well-trained on clean datasets \fh{rather than datasets, shall we say unattacked environment or safe environment, since RL is not necessarily trained on a ``dataset''?}, may output a wrong answer. 
As a result, although a policy can obtain a high reward by taking in the messages sent by other agents, it may also get drastically misled by inaccurate information or even adversarial communication from malicious attackers. 
For example, when several drones execute pre-trained policies and exchange information via wireless communication, it is possible that some malicious attacker eavesdrops on their communication and intentionally perturbs some messages to a victim agent via cyber attacks. 
Moreover, even if the communication channel is protected by advanced encryption algorithms, an attacker may also hack some agents and alter the messages before they are sent out (e.g. hacking IoT devices that usually lack sufficient protection~\cite{naik2017cyber}). Figure~\ref{fig:diagram} demonstrates an example of communication-attack, where the attacker may lure the agent to a dangerous location through malicious message propagation and cause fatal damage.

\begin{figure*}[!t]
\vspace{-2em}
    \centering
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{figs/train.pdf}
         \vspace{-0.5em}
         \caption{Training time}
         \label{sfig:train}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{figs/test.pdf}
         \vspace{-0.5em}
         \caption{Test time (in deployment)}
         \label{sfig:test}
     \end{subfigure}
     \vspace{-0.5em}
    \caption{An example of test-time communication attacks in a communicative MARL system. Agents can be heterogeneous as depicted by various icons. (a) During training, agents are trained collaboratively in a safe environment, such as a simulated environment. (b) In deployment, agents execute pre-trained policies in the real world which may susceptible to attacks that perturb communication messages. Malicious attackers may modify the benign messages into adversarial signals. In this figure, arrows denote communication channels among agents, {\color{darkpastelgreen}{green}} messages stand for benign communication, and {\color{red}{red}} messages stand for adversarial communication.}
    \label{fig:diagram}
\vspace{-1.5em}
\end{figure*}

Although adversarial attacks and defenses have been extensively studied in supervised learning~\cite{madry2018towards,cohen2019certified} and reinforcement learning~\cite{zhang2020robust,zhang2021robust,oikarinen2020robust}, there has been little discussion on the robustness issue against adversarial communication in MARL problems. 
Therefore, in order to safely apply communication to more high-stakes multi-agent scenarios, it is crucial to robustify MARL policies against adversarial attacks.
% \textcolor{red}{Defending against the adversarial communication while still utilizing the benign communication}\fh{needs rewording. Maybe: Achieving high performance in a multi-agent cooperative game through inter-agent communication while remain robust to adversarial communication attacks} 
Achieving high performance in a multi-agent cooperative game through inter-agent communication while being robust to adversarial communication attacks is a {challenging problem} due to the following reasons. 
\textbf{Challenge I}: The attacker may construct malicious messages in various ways, so that they are hard to be distinguished from benign messages. For example, the malicious messages shown in Figure~\ref{sfig:test} are in the same form as the benign messages and also make semantic sense. \textbf{Challenge II}: A strong attacker can even be \textit{adaptive} to the victim agent and significantly reduce the victim's total reward. For instance, for a victim agent who moves according to the average of GPS coordinates sent by others, the attacker may learn to send extreme coordinates to influence the average.
% the attacker may learn an RL policy to send sequential misleading messages. \fh{This point is not very clear.}
\textbf{Challenge III}: There can be more than one attacker (or an attacker can perturb more than one message at one step), so that they can collaborate to mislead a victim agent.

Tu et al.~\cite{tu2021adversarial} apply adversarial training~\cite{madry2018towards} to improve model robustness against communication perturbation. But they focus on the $\ell_p$ threat model (perturbation with small $\ell_p$ norm), which do not solve many attack scenarios such that the attack in Figure~\ref{sfig:test}.
Some recent works~\cite{blumenkamp2020emergence,xue2021mis,mitchell2020gaussian} recognize the existence of adversarial communications in MARL and propose several defending methods, e.g. a trained message filter~\cite{xue2021mis}. However, these heuristics-based defenses, although are the first step to investigate adversarial communication in MARL, do not fully address the aforementioned challenges, and are not guaranteed to be robust, especially under adaptive attacks. 
% \textcolor{purple}{PH: all communication attacks, any communication attack? YS: should be all, thanks} 
%\textcolor{purple}{PH: Is it clear what we mean by adaptive attacks? In challenge 2 we are kind of defining it. Would it make sense to make the \textit{adaptive} italic in challenge 2 to stand out? YS: Sure! Good point}

In contrast, we address all aforementioned challenges by proposing \textit{a certifiable defense named \textbf{\oursfull (\ours)} that can guarantee the performance of agents against multiple adversarial communication messages}.
% \fh{Our proposed defense addresses all three aforementioned challenges.}
% \fh{should not overclaim. mention this is for communication attacks only}. 
The main idea is to construct an \emph{ensemble policy} which makes decisions based on multiple different subsets of communication messages (i.e., ablated messages). 
Specifically, for a list of messages coming from different agents, we train a \emph{base policy} that takes in a subset of messages and outputs a \emph{base action}. 
Then we obtain an ensemble policy by aggregating multiple base actions coming from multiple different message subsets. For a discrete action space, the ensemble policy takes the majority of the multiple base actions obtained, while for a continuous action space, the ensemble policy takes the median of these base actions. \ours is a generic framework that works for any agent that observes multiple messages from different sources, as long as the agent receives more benign communication messages than adversarial ones. We also show in Section~\ys{todo} that \ours can be used in many other scenarios beyond defending against MARL communication attacks.
% Therefore, \ours can be extended to defend against 
% \ys{flexibility, as discussed later}

Our contributions can be summarized as below:\\
\textbf{(1)} We formulate the problem of adversarial attacks and defenses in communicative MARL (CMARL).\\
\textbf{(2)} We propose a novel defense method, \ours, 
% \SF{perhaps introduce ``ablation" terminology in the previous paragraph so readers become familiar with it at this point}
% based on randomized ablation on communication messages. \ours 
that is provably robust against arbitrary perturbations of up to $C<\frac{N-1}{2}$ communication channels, where $N$ is the number of agents. \\
% both in discrete action space and in continuous action space. \fh{I feel the contribution is not that we include both discrete or continuous action space, but rather, we can achieve very strong results in the discrete space, as well as good results in the continuous space. I feel the current wording sounds a bit off the path.}\\
\textbf{(3)} Experiment in 3 multi-agent environments shows that \ours obtains significantly higher reward than baseline methods under both non-adaptive and adaptive attackers. 
% The agent trained with \ours achieves similar 
% \SF{add a bit more details here; what environments; discrete or cont; what gains do we achieve?}. 
% \fh{maybe some numbers in terms of performance improvement etc}



==> 2_relate.tex <==
% \vspace{-0.5em}
\section{Related Work}
\label{sec:relate}
% \fh{I don't think we need this related work to be at the beginning to explain our method. Shall we move it here?}

% \ys{add more papers for arxiv. if else command}

\textbf{Communication in MARL}\quad
Communication is crucial in solving collaborative MARL problems. There are many existing studies learning communication protocols across multiple agents. \cite{foerster2016learning} are the first to learn differentiable communication protocols that is end-to-end trainable across agents. Another work by~\cite{sukhbaatar2016learning} proposes an efficient permutation-invariant centralized learning algorithm which learns a large feed-forward neural network to map inputs of all agents to their actions. 
It is also important to communicate selectively, since some communication may be less informative or unnecessarily expensive. To tackle this challenge, \cite{das2020tarmac} propose an attention mechanism for agents to adaptively select which other agents to send messages to. \cite{liu2020who2com} introduce a handshaking procedure so that the agents communicate only when needed. Our work assumes a pre-trained communication protocol and does not consider the problem of learning communication mechanisms.

\textbf{Adversarial Attacks and Defenses in CMARL}\quad
The investigation of adversarial communication in MARL problems is a relatively new topic, and has recently attracted increasing attention.  
\cite{blumenkamp2020emergence} show that in a cooperative game, some self-interest agents can learn manipulative communication policies and hurt other agents' performance. 
% To accommodate multiple agent objectives, they propose \change{Aggregation}\fh{aggregated? is aggregation GNN a terminology? I've not heard of it.} Graph Neural Networks to model and learn an inter-agent communication policy. 
To achieve robust communication, \cite{mitchell2020gaussian} use Graph Neural Networks to model the communication architecture and adopt a Gaussian Process-based probabilistic model to compute the posterior probabilities that whether each partner is truthful. 
\cite{tu2021adversarial} investigate the vulnerability of multi-agent autonomous systems against communication attacks. 
% \change{multiple aspects} \fh{?}.
\cite{xue2021mis} present an algorithm to defend against one adversarial communication message by an anomaly detector and a message reconstructor, which is trained with groundtruth labels and messages. In comparison, our work proposes a provably robust defense mechanism that has certifiable performance even when near to half of the communication messages are corrupted.
% formulates adversarial attacks in a general \fh{are previous works not generic? Why?}communicative MARL (CMARL) setting, and 
% \fh{Is \cite{xue2021mis} attack agnostic? The current description doesn't answer this question.}.

\textbf{Adversarial Robustness of RL Agents}\quad
As RL techniques have been applied to more and more applications, the robustness of agents under environment noise or adversarial attacks becomes an emerging research topic. 
For a single-agent problem, there are many recent works on adversarial state perturbation~\cite{huang2017adversarial,zhang2020robust} and action perturbation~\cite{tan2020robustifying,tessler2019action}. In a multi-agent system, the interplay among agents introduces more uncertainty to the environment. \cite{gleave2020adversarial} point out that a well-trained agent can be completely misled by adversarial behaviors of another agent. Although adversarial training (i.e., introducing adversarial agents to the system during training~\cite{pinto2017robust,phan2021resilient}) can empirically improve agents' robustness, such robustness is not guaranteed to hold under all possible attackers.


\textbf{Certifiable Defense}\quad
There is an important line of work studying guaranteed robustness of neural networks~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness} while the input data is perturbed within an $\ell_p$ norm ball. In an effort to certify RL agents' robustness, \cite{lutjens2020certified} and \cite{oikarinen2020robust} utilize convex relaxation of Q networks to improve the worst-case performance of agents. \cite{kumar2021policy} and \cite{wu2021crop} follow the idea of randomized smoothing~\cite{cohen2019certified} and smooth out the policy by adding Gaussian noise to the input.
To the best of our knowledge, our \ours is the first certifiable defense in MARL against communication attacks. Moreover, we consider a strong threat model where up to half of communication messages can be arbitrarily corrupted. 
\ys{flexibility}
% This threat model can cover many realistic attacking scenarios that the $\ell_p$ model does not solve.

% This paper \myst{is also closely related to} \fh{bears some similarities with}~\cite{gleave2020adversarial}, which studies the effects of adversarial actions in an MARL problem. In contrast, our work aims to defend against communication attacks that can be more stealthy in practice.
% Randomized ablation is proposed by~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification problems, in which the classifier is trained by randomly ablating pixels of images. 
% We are the first to extend the idea of randomized ablation to MARL and to achieve action and reward certificates against communication attacks.
% Note that the number of pixels in an image and the number of agents in an MARL problem are in different scales. Also, a classifier outputs discrete labels, while a policy may have discrete or continuous output space. Therefore, our problem setup, methodology and theoretical results are significantly different from~\cite{Levine_Feizi_2020} and are novel.

% \textbf{parameter sharing} Sharing parameters are a common way to take advantage of centralized training \cite{lowe2017multi,foerster2016learning} by learning a single shared critic network for multiple agents. \cite{gupta2017cooperative} uses single-agent RL methods to learn policies in cooperative environments.

==> 3_setup.tex <==
\section{Problem Formulation}
\label{sec:setup}

% \fh{Shall we change the section title to Problem Formulation?}

% \subsection{Basic Notations}
% For an interger $N$, let $[N]$ denote the set $\{1,2,\cdots,N\}$.
% We use $X_{1:N}$ as a shorthand notation of the list $[X_1,\cdots,X_N]$.
% % , and $X_{-i}$ as a shorthand notation of the list $[X_1,\cdots, X_{i-1}, X_{i+1}, \cdots, X_N]$.
% Let $\mathcal{H}(N,k)$ denote the set of all the unique $k$ indices out of $N$, so $|\mathcal{H}(N,k)|=\binom{N}{k}$, and let $\mathcal{U}(N,k)$ denote the uniform distribution over $\mathcal{H}(N,k)$.
% Let $\mathcal{T}=\{i_1, i_2,...,i_k\}\sim \mathcal{U}(N,k)$ be the random variable that denotes the collection of $k$ out of $N$ dimensions. 
% For a list of $N$ elements $m=[m_1, m_2, \cdots, m_n]$, $\mathsf{Ablate}(m, \mathcal{T}) = [m_{i_1}, \cdots, m_{i_k}]$. 
% For any random variable $X \sim \mathcal{D}$ ($\sim \mathcal{D}$ is omitted below for simplicity) and a real-valued function $f(X)$, define a function $\mathsf{Med}_{X}(f(X))$ as 
% $$
% \mathsf{Med}_{X}(f(X)) := \inf \{ c\in\mathbb{R}: \mathbb{P}_X [ f(X) \geq c ] \geq 0.5 \}.
% $$
% For a vector-valued function $F = [f_1(X), \cdots, f_l(X)]^\top$, the $\mathsf{Med}$ function is extended as the element-wise median value, i.e.,
% $$
% \mathsf{Med}_{X}(F(X)) = [\mathsf{Med}_{X}(f_1(X)), \cdots, \mathsf{Med}_{X}(f_l(X))]^\top.
% $$



\subsection{Communicative Muti-agent Reinforcement Learning}
\label{sec:setup_cmarl}

% \textbf{Dec-POMDP Model.}\quad
% We consider a Decentralised Partially Observable Markov Decision Process (Dec-POMDP)~\cite{oliehoek2012decentralized,oliehoek2015concise,das2020tarmac} which is a multi-agent generalization of the single-agent POMDP models. 
% A Dec-POMDP can be modeled as a tuple $\langle \mathcal{D}, \mathcal{S}, \mathcal{A}, \mathcal{O}, O, P, R, \gamma, \rho_0 \rangle$. 
% $\mathcal{D}=\{1,\cdots,N\}$ is the set of $N$ agents.
% $\mathcal{S}$ is the underlying state space. $\mathcal{A}=\times_{i\in\mathcal{D}}\mathcal{A}_i$ is the \emph{joint} action space. $\mathcal{O}=\times_{i\in\mathcal{D}}\mathcal{O}_i$ is the \emph{joint} observation space, with $O$ being the observation emission function.
% $P: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \Delta(\mathcal{S}) $ is the state transition function\footnote{$\Delta(\mathcal{X})$ denotes the space of probability distributions over space $\mathcal{X}$.}.
% $R: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \mathbb{R}$ is the immediate reward function.
% $\gamma$ is the shared discount factor, and $\rho_0$ is the initial state distribution.

% \textbf{Communication in Dec-POMDP}\quad
% At every step $t$, each agent $i\in[N]$ observes its local observation $o_i\step$ and sends a communication message $m_{i \to j}\step := F(i,o_i\step,j)\in\mathcal{M}$ to agent $j$ for all $j\neq i$. 
% Here $m_{i \to j}\step$ denotes a message sent from agent $i$ to $j$ in step $t$. For notation simplicity, we will omit ${}\step$ when there is no ambiguity. 
% A message $m_{i \to j}$ can be a scalar or a vector, e.g., signal of GPS coordinates. 
% For notation simplicity, we assume that agents are fully connected for communication, although our algorithm directly applies to partially connected communication graphs. That is, at each step, every agent sends $N-1$ messages (1 for each agent other than itself), and receives $N-1$ messages from others.
% We use $\mtoi$ to denote the list of messages received by agent $i$, i.e., $\mtoi:=\{m_{j \to i} | 1\leq j \leq N, j\neq i \}$. 



\ys{reminder: communicative stochastic game}
We consider a \textit{Communicative Multi-agent Reinforcement Learning (CMARL)} problem, where the environment is modeled as a tuple 
% \fh{$\mathcal{M}$ used for both the MAC-MDP and the message space}
$\langle N, \mathcal{S}, \mathcal{A}, \mathcal{O}, \mathcal{M}, P, R, B, F, \gamma, \rho_0 \rangle$.
% \fh{Could we add $f_i: \mathcal{O}_i \to \mathcal{M}_1\times\cdots \mathcal{M}_{i-1}\times  \mathcal{M}_{i+1}\times \cdots \mathcal{M}_N$ or just $\{f_i\}_{i=1}^N$ to the tuple to indicate that we consider $f_i$ as part of the environment rather than part of our strategy?}
$N$ is the number of agents;
$\mathcal{S}$ is the underlying common state space;
$\mathcal{A}=\mathcal{A}_1\times\mathcal{A}_2\times\cdots\times\mathcal{A}_N$ is the \emph{joint} action space;
$\mathcal{O}=\mathcal{O}_1\times\mathcal{O}_2\times\cdots\times\mathcal{O}_N$ is the \emph{joint} observation space;
$\mathcal{M}$ is the message space;
$P: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \Delta(\mathcal{S}) $ is the state transition function\footnote{$\Delta(\mathcal{X})$ denotes the space of probability distributions over space $\mathcal{X}$.};
$R: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \mathbb{R}^N$ is the \emph{joint} reward function that returns a list of rewards for all agents;
$B: \mathcal{S} \to \Delta(\mathcal{O}_1) \times \Delta(\mathcal{O}_2) \times \cdots \times \Delta(\mathcal{O}_N)$ is the observation emission probability function;
$F$ is the communication protocol, with $F(i,o_i,j) \in\mathcal{M}$ being the communication signal/message sent from agent $i$ to agent $j$ when $i$ observes $o_i\in\mathcal{O}_i$;
$\gamma$ is the shared discount factor; $\rho_0$ is the initial state distribution.

The above formulation is generic and can model many real-world scenarios. 
(1) The reward function $R$ can output the same values for all agents (\textit{fully-cooperative} setting), or output different values for heterogeneous agents (\textit{self-interested} setting). Note that although communication is usually considered in cooperative problems~\cite{foerster2016learning,ghavamzadeh2004learning}, self-interested agents can also benefit from communication. For example, auto-driving cars can avoid collision by sharing their routes with each other. 
(2) The communication protocol $F$ can be \textit{hand-coded} or \textit{learned}~\cite{foerster2016learning}. In deployment, agents follow a fixed communication protocol or execute a trained communication model/policy.
Our goal is to defend against perturbed communication messages as detailed in Section~\ref{sec:setup_adv}, regardless of how communication is generated.
Most existing multi-agent environments can be regarded as special cases of this CMARL formulation. For example, the reward function $R$ maps the current state and all current agent actions to a reward vector, containing the rewards received by each individual agent. If all agents get the same reward at every step, then the environment degenerates to a fully-cooperative one. 

\textbf{Communication Message $\boldsymbol{m}$}\quad
% In a CMARL problem, agents can communicate based on a protocol $F$, which can be either pre-defined or learned as discussed in prior works~\cite{foerster2016learning}. In this paper, we consider a pre-defined communication protocol $F$ and learning $F$ is out of our scope.
At every step $t$, each agent $i\in[N]$ observes its local observation $o_i\step$ and sends a communication message $m_{i \to j}\step := F(i,o_i\step,j)\in\mathcal{M}$ to agent $j$ for all $j\neq i$. 
Here $m_{i \to j}\step$ denotes a message sent from agent $i$ to $j$ in step $t$. For notation simplicity, we will omit ${}\step$ when there is no ambiguity. 
A message $m_{i \to j}$ can be a scalar or a vector, e.g., signal of GPS coordinates. 
For notation simplicity, we assume that agents are fully connected for communication, although our algorithm directly applies to partially connected communication graphs. That is, at each step, every agent sends $N-1$ messages (1 for each agent other than itself), and receives $N-1$ messages from others.
We use $\mtoi$ to denote the list of messages received by agent $i$, i.e., $\mtoi:=\{m_{j \to i} | 1\leq j \leq N, j\neq i \}$. 

% \textcolor{purple}{PH: I know we said we omit $(t)$ when there is no ambiguity, but for consistency of notation, shall we keep or omit $(t)$ in both $\mtoi$ and $m_{j \to i}$ in the definition $:=$? YS: Yes, this is a typo, I fixed it.}
% _{j\neq i:j=1}^N
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
%     \mtoi := [m_{1 \to i}, \cdots, m_{(i-1) \to i}, m_{(i+1) \to i}, \cdots, m_{N \to i}].
% \end{equation*}

% The communication messages are generated by agents' private communication functions denoted as $\commfunc$ \fh{$\commfunc_i$ for an agent $i$}.
% To cover more real-world scenarios, we consider the case where agents  can share different information (\fh{based on their local observation}) with \textcolor{red}{different} \fh{their selected} recipients at each step.  Specifically, each agent $i$ generates communication \fh{messages} by function $f_i: \mathcal{O}_i \to \mathcal{M}_i^{N-1}$ \fh{need to define what does the superscript mean here.}. This function $f_i$ can be either pre-defined with domain knowledge, or trained with existing approaches~\cite{foerster2016learning}. \textcolor{red}{But note that learning advanced communication methods is not the focus of this paper, since we aim to defend against adversarial communication over any pre-defined or learned communication protocols.}
% \fh{In this paper, we do not focus on learning advanced communication methods $\{\commfunc_i\}_{i=1}^N$. Rather we aim to defend against adversarial communication over any pre-defined or learned communication protocols. In other words, we investigate defense mechanisms for adversarial perturbations to agent $i$'s messages $\commfunc_i(o_i\step):=\mathbf{m}_{i\to :}\step := [m_{i \to 1}\step, \cdots, m_{i \to (i-1)}\step, m_{i \to (i+1)}\step, \cdots, m_{i \to N}\step]$.} 

\textbf{Acting Policy $\boldsymbol{\pi}$}\quad
The goal of each agent $i\in [N] := \{1,2,\cdots,N\}$ is to maximize its discounted cumulative reward $\sum_{t=0}^\infty \gamma^t r\step_i$ by learning an acting policy $\pi_i: \mathcal{O}_i\times \mathcal{M}^{N-1} \to \mathcal{A}_i$, 
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
%     \pi_i: \mathcal{O}_i\times \mathcal{M}_1 \times\cdots \mathcal{M}_{i-1} \times \mathcal{M}_{i+1} \times \cdots \mathcal{M}_N \to \mathcal{A}_i,
% \end{equation*}
which maps the agent's current observation $o_i$ and all communication messages from other agents $\mtoi$ 
% \fh{$\{m_{j \to i}\step\}_{j\neq i:j=1}^N$} 
to an action for agent $i$, i.e., $a_i$.
% The underlying state of the environment is often not fully observable to an individual agent, i.e., $o_i$ usually does not contain all information needed to make optimal decisions.
% % the underlying state of the environment is not fully observable to an individual agent. 
% For example, the local view of a single drone does not cover the entire map for navigation. Therefore 
Communication messages from other agents are important for the acting policy to gain high rewards, especially in cooperative games~\cite{foerster2016learning,liu2018energy}. However, as will be discussed in Section~\ref{sec:setup_adv} below, communication can be a double-edge sword --- it expedites learning by information sharing but may make agents vulnerable to adversarial attacks.





% At every step $t$, an agent $i\in [N] := \{1,2,\cdots,N\}$ goes through the following process: \\
% \textbf{(1)} Agent $i$ observes its (local) observation $o_i\step \in \mathcal{O}_i$ (the environment has current state $s\step$ which is not visible to the agent). \\
% \textbf{(2)} Agent $i$ sends messages to other agents by the communication function $\mu_i: \mathcal{O}_i \to (\mathcal{M}_i \cup \{\mathsf{NULL}\})^{N-1}$, where $\mathsf{NULL}$ indicates that no message is sent to the corresponding receiver.
% % $\mu_i: \mathcal{O}_i \to \{0,1\}^{N-1} \times \mathcal{M}_i$, where $b \in \{0,1\}^{N-1}$ denotes a communication mask. If $b=[1,\cdots,1]$, the message is broadcasted to all other agents. If $b=[1,0\cdots,0]$, the message is only sent to the first agent. 
% Let $m_{i\to j}\step$ denote the message from agent $i$ to agent $j$ at step $t$.\\
% \textbf{(3)} Agent $i$ receives messages sent from all other agents 
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
%     \mtoi\step := [m_{1 \to i}\step, \cdots, m_{(i-1) \to i}\step, m_{(i+1) \to i}\step, \cdots, m_{N \to i}\step].
% \end{equation*}
% \fh{where each $m_{j \to i}\step$ is a vector of dimension ?}
% (If $j$ did not send a message to $i$, then $m_{j \to i}\step$ is empty.) \\
% \textbf{(4)} Agent $i$ takes action $a_i\step$ by its \emph{acting policy}  \fh{$\pi_i$ which considers its local observation as well as messages from other agents}
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
%     \pi_i: \mathcal{O}_i\times \mathcal{M}_1 \times\cdots \mathcal{M}_{i-1} \times \mathcal{M}_{i+1} \times \cdots \mathcal{M}_N \to \mathcal{A}_i.
% \end{equation*}

% \fh{Note that the acting policy doesn't specify the communication strategy of an agent. Should we talk about the communication strategy here, i.e., how to render the message?}
% \vspace{-1em}

% The communication function $\mu_i$ \fh{you never defined $\mu_i$. Typo.} can be either pre-defined or learned. Let $[R(s_t, a_1\step, \cdots, (a_N)_t))]_x$ \fh{$(a_N)_t$ not defined} denote the reward of agent $x \in [N]$ at step $t$. \fh{We need to make the notations clear here. What does this $[\cdot]_x$ mean? What does each $a_i\step$ denote? We should make it clear that each agent may have their own reward as explained in the model where we can there is a joint reward function. I feel this needs more explanation. Also I am thinking, shall we draw a simple 3-agent-diagram to depict MACRL if we have time?} \fh{In the previous descriptions, you use $i$ to denote agent id, now it is changed to $x$. Can we make them consistent?} Then, the goal of agent $x$ is to maximize its own cumulative reward, i.e.,
% {\small{
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:agent_obj}
% \tag{$Q$}
% \begin{aligned}
%     \min_{\pi_x} \fh{\max?} & \; \natobj^x := \mathbb{E} [ \sum_{t=0}^\infty \gamma^t [R(s\step, a_1\step, \cdots, a_N\step)]_{x} ] \\
%     \text{where } & \; a_i\step = \pi_i(o_i\step, \mtoi\step), \forall i\in [N], t=1,\cdots
% \end{aligned}
% \end{equation}
% }}

% $\pi_i: \mathcal{O}_i\times \mathcal{M}_1 \times\cdots \mathcal{M}_{i-1} \times \mathcal{M}_{i+1} \times \cdots \mathcal{M}_N \to \mathcal{A}_i$.
% Note that the $N$ agents can be heterogeneous, as each of them has its own observation space, action space, message space and reward function. 
% Many existing multi-agent environments can be regarded as special cases of the above formulation. For example, if there is no communication, then it is a normal MARL environment, equivalent to setting $\mathcal{M}_{1:N}$ to be empty sets. If all agents have the same reward ($R_1,\cdots,R_N$ are equal), then the environment degenerates to a fully-cooperative game. If agents further share the same observation space and action space, then they can be viewed as symmetric agents.
% Therefore, our above formulation of MACRL is generic and can model many real-world scenarios. 




\subsection{Communication Attacks in Deployment of CMARL}
\label{sec:setup_adv}

Communication attacks in MARL has recently attracted increasing attention~\cite{blumenkamp2020emergence,tu2021adversarial,xue2021mis} with different focuses, as summarized in Section~\ref{sec:relate}. 
In this paper, we consider a practical and strong threat model where malicious attackers can arbitrarily perturb a subset of communication messages in CMARL.

\textbf{Formulation of Communication Attack}\quad 
% \ys{I will re-write this section to make it less complicated and more clear}
During test time, agents execute well-trained policies $\pi_1,\cdots, \pi_N$. For any agent $i\in[N]$, it receives $N-1$ communication messages from other agents, but some of them can be adversarial messages that are perturbed arbitrarily.
Each agent receives no greater than $C$ adversarial messages at every step, among all $N-1$ messages.
The victim agent has no knowledge of which messages are adversarial, and the attacker may attack at different $C$ channels at each step.
% Here $C$ is a constant representing how many communication channels the attacker can manipulate at each step, and it 
Here $C$ is a reflection of the attacker's attacking power, which is usually limited in practice (i.e., $C$ is not too large).
Once the attacker has control over a communication channel (e.g. channel from $j$ to $i$), it is able to arbitrarily change the corresponding messages (e.g. $m_{j \to i}$ can be arbitrarily perturbed).
% Therefore, we consider a strong threat model where the attacker is allowed to send $C$ arbitrary adversarial messages, making it more challenging to design a defense as it has to be a strong defense as well. 
% This threat model is analogous to an $\ell_0$ attack on the policy's input, as detailed in Appendix~\ref{app:theory}.

To obtain theoretically guaranteed robustness, we make the following mild and realistic assumption.
\begin{assumption}
\label{assum:num}
The attacker is able to manipulate less than half of the communication channels, i.e.,
$C<\frac{N-1}{2}$.
% $C<\lfloor\frac{N}{2}\rfloor$. 
% \textcolor{purple}{PH: less than half of the communication channels?}
\end{assumption}
This is a realistic assumption because the attacker in practice usually has limited power, such that controlling the majority of agent communications is less likely. 

\textbf{Various Attack Algorithms}\quad
As formulated above, the attacker can perturb up to $C$ communication messages sent to any agent at every step. 
However, we do not make any assumption on what attack algorithm the attacker uses, i.e., how a message is perturbed. %\textcolor{purple}{PH: how it perturbs a message, or how a message is perturbed? }
In practice, an attacker may randomly change the communication signal, or learn a function to perturb the communication based on the current situation. 
% The attacker can either be white-box or black-box, based on whether it knows the victim agent's policy, as extensively studied in the field of adversarial supervised learning~\cite{chakraborty2018adversarial}. 
To achieve generic robustness under a wide range of practical scenarios, it is highly desirable for a defense to be agnostic to attack algorithms and work for arbitrary (including strongest/worst) perturbations. This is achieved by our defense which will be introduced in Section~\ref{sec:algo}. 
% Therefore, in the next section, we introduce a defense method against adversarial communication, that is provably robust against any attack algorithms which perturb up to $C$ communication messages at each time step. 

\paragraph{Comparison with Other Threat Models}\quad 
Many existing works on adversarial attack and defense assume that the perturbation is small in $\ell_p$ norm. However, there are many realistic attacks that can not be solved by the $\ell_p$ threat model. For example, the attacker may replace a word in a sentence, add a patch to an image, or permute the order of messages. In these cases, the $\ell_p$ distance between the clean value and the perturbed value is large, so that $\ell_p$ defenses do not work.
In contrast, we allow arbitrary perturbations of these $C$ messages for broader application and stronger robustness. 
% This type of limited attacking power assumption is common in adversarial learning, i.e.,  attack with bounded radius in $\ell_p$ norm. 

\textbf{Comparison with Observation Attacks}\quad
Recent study~\cite{huang2017adversarial,gleave2020adversarial,sun2021strongest} has revealed that a well-trained Deep RL policy are vulnerable to adversarial perturbation on the observations.
% test-time evasion attacks. That is, a malicious attacker can significantly reduce the reward of a victim agent by adding crafted 
% small perturbations to the victim's observations. Although most prior works consider observation attacks~\cite{huang2017adversarial,zhang2020robust,sun2021strongest}, it is not always feasible 
% \textcolor{purple}{PH: practical$->$feasible? since we say "in practice" in the same sentence}
However, it is not always feasible for an attacker to change an agent's observation in practice~\cite{gleave2020adversarial}. For example, a robot's observation is often captured by built-in sensors~\cite{pinkava1990towards}, which the attackers may not have access to. 
In contrast, an attacker can eavesdrop on and alter the messages propagated in a communication channel to influence a victim agent's decisions, which is relatively an easier and thus more practical attack than changing an agent's observations that are not easily modifiable. 
More importantly, since an acting policy $\pi$ takes in both its own observation and the communication messages, communication can be regarded as a subset of policy inputs, and thus is related to traditional adversarial defenses of deep neural policies. 
But different from most literature that consider $\ell_\infty$ or $\ell_2$ perturbations on the entire input vector, we focus on the case where a fraction of inputs can be totally corrupted, analogous to an $\ell_0$ attack (sparse attack) model as detailed in Appendix~\ref{app:theory}.
% More importantly, since communication is broadcast 
% \change{in a multi-agent world where agents are usually trained in a centralized way and executed in a decentralized way}\fh{
% in a multi-agent problem where agents expedite learning and make informed decisions through information sharing, adversarial attackers can exploit the vulnerabilities of such information exchange across agents to mislead decision-making.
% In particular, an attacker can eavesdrop on and alter the messages propagated in a communication channel to influence a victim agent's decisions, which is relatively an easier and thus more practical attack than changing an agent's observations that are not easily modifiable. 
% which are usually from sensors that are built in and not easily accessible. 
% A well-known real-world example is cyber attacks to communication channels. 

\textbf{Comparison with Action Attacks}\quad
Note that in a communication attack, the attacker only alters the communication and does not directly change the actions of any agent. Therefore, all agents are still following $\pi_1,\cdots, \pi_N$.
This is different from the multi-agent attacking scenario studied by~\cite{gleave2020adversarial}, where one agent becomes adversarial and behaves differently (i.e., executes a different policy) to attack the victim agent. 
% The communication attack model studied in our paper can be more practical since attacking a communication channel can be more feasible than attacking the observations of a built-in sensor or the policy that is stored in the machine (as described earlier).  
Compared with this type of attack that behaves abnormally to cause performance drop of the victim agent, the communication attack model studied in our paper can be more stealthy and harder to detect, as the other agents do not change their behaviors. For example, if a drone is hacked and controlled by an attacker to behave differently, it is relatively easy for humans to notice the abnormal agent. 
However, it can be hard to recognize adversarial communication signals. For instance, the adversarial messages in Figure~\ref{fig:diagram} look similar to benign messages and can be hard to detect. Furthermore, a learned communication message can be automatically generated by neural networks~\cite{foerster2016learning,tu2021adversarial} and are thus hard for humans to interpret. 
% especially the learned communication \fh{what is learned communication?} which can be uninterpretable.


\ys{Different forms of attacks.
directly perturbing the victim: not always feasible in hardware
attacking the victim via perturbing other agents: change the action of the other agent - influence its own reward. 
}





% % Without loss of generality, we look at a specific agent $i\in [N]$ .
% we suppose that the adversaries an victim agent $x \in [N]$ whose identity is unknown, but the formulation can be easily generalized to multiple victim attacks.
% Suppose there is an attacker manipulating communication messages from a subset of agents $\mathcal{Y}=\{ y_1, \cdots, y_C \}$ to $x$ ($x \notin \mathcal{Y})$, i.e., the attacker can control the communication channels to the victim from up to $C$ agents. \fh{Note that $C$ should be considered as a known hyperparameter, and we will provide more insight later in the paper about how to set $C$ in practice.} 
% As pointed out by some prior works~\cite{zhang2020robust,sun2021strongest}, the \textit{optimal attack} \fh{to an RL policy} can be learned by solving an RL problem:
% % {\small{
% \setlength\abovedisplayskip{-2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:adv_obj}
% \tag{$Q_A$}
% \begin{aligned}
%     \min_{\nu_1,\cdots,\nu_C} & \; \advobj^x :=  \mathbb{E} [ \sum_{t=0}^\infty \gamma^t [R(s\step, a_1\step, \cdots, a_N\step)]_{x} ] \\
%     \text{where } & \; a_i\step = \pi_i(o_i\step, \mtoi\step), \forall i\in [N], t \geq 0 \\
%      & \; m_{y_j \to x}\step = \nu_{j}(o_{y_j}\step), \forall j\in [C], t \geq 0
% \end{aligned}
% \end{equation}
% % }}

% % In other words, the attacker learns $C$ communication policies that collaboratively minimizes the reward of the victim agent $x$.
% The minimizer to Problem~\eqref{eq:adv_obj}, $\nu_1^*,\cdots,\nu_C^*$ , defines an optimal communication attacking strategy that is adaptive to victim $\pi_x$. 
% However, this is a theoretical optimal attack with white-box access to the victim's reward function, while a real-world attacker can be different \fh{unclear} and weaker \fh{this sentence seems to open a big problem that is not explained well. Needs to be reorganized.}.
% In this paper, we propose a provably robust defense that is agnostic to attacking strategies, including the ``optimal'' white-box adaptive attacker learned as Problem~\eqref{eq:adv_obj}.

% For illustration simplicity, we call the $C$ manipulated agents in $\mathcal{Y}$ as \textit{adversarial agents} against victim $x$, because $x$ receives adversarial communication from them \fh{although these manipulated agents can still maintain their own target and reward and execute their optimal acting policy (polish this)}.  
% We can show that the above communication threat model is analogous to an $\ell_0$ attack in the policy's input space, as illustrated in Appendix~\ref{app:theory}.
% Note that the attacker only changes the communication between other agents and the victim agent, while 
% not directly changing the actions of any agent. Therefore, all non-victim agents are behaving normally, different from the change-of-action attacks considered in~\cite{gleave2020adversarial}. 

% \fh{We need to discuss the descriptions of the threat models.}

% \fh{Shall we move the attacks subsection to a seperate section, outside of the problem formulation?}

% \subsection{Goal: Defending against Communication Attacks}
% \label{sec:setup_defense}

% Traditional MARL algorithms optimize the natural reward $\natobj$ without any attacks, as defined in Problem~\eqref{eq:agent_obj}. However, the learned policies are not necessarily robust against adversarial communications. That is, the attacked reward $\advobj$ can be made extremely low under learned attackers solved by Problem~\eqref{eq:adv_obj}, as verified by our experiments in Section~\ref{sec:exp}.

% Motivated by the fact that communication among agents may be noisy, unstable, and vulnerable to attacks, our goal is to train robust acting policies $\{ \pi_i, i \in [N] \}$, such that for any agent, $\natobj$ and $\advobj$ are both high, even when there are up to $C$ communication messages corrupted at every step. 
% More importantly, we aim to provide a defense mechanism and guarantee that the agents will not be significantly misled by adversarial communication messages during test time.

==> 4_algo_new.tex <==
\section{Provably Robust Defense for CMARL}
\label{sec:algo}

In this section, we present our defense algorithm, \textit{\oursfull (\ours)}, against test-time communication attacks in CMARL. 
% We first define some notations used throughout the paper and a key assumption for the robustness guarantee to hold. Then, we 
We first introduce the main idea of the algorithm in Section~\ref{sec:algo_overview}.
Then, in Section~\ref{sec:algo_dist} and Section~\ref{sec:algo_cont}, we provide detailed methodology and theoretical analysis for \ours robust policies in discrete action spaces and in continuous action spaces, respectively.
Section~\ref{sec:algo_partial} further extends the \ours algorithm by introducing a hyper-parameter for more efficient implementation in larger-scale problems, with corresponding theoretical guarantees.
\ys{generalize to decision making}

% For notation simplicity and with a little abuse of notation, 
% % we assume that there are $N+1$ agents in total, so that every agent can communicate with $N$ other agents in every step.
% assume all $N$ agents have identical observation space, action space and message space denoted as $\mathcal{O}, \mathcal{A}$ and $\mathcal{M}$. So that the joint observation/action/message space is $\mathcal{O}^{N}$/$\mathcal{A}^{N}$/$\mathcal{M}^{N}$.
% As is common is MARL~\cite{foerster2016learning}, we learn a single policy network that is shared across all agent. But note that this setting is only for illustration simplicity, our algorithm applies to heterogeneous agents with multiple policies.

\subsection{\oursfull (\ours): An Overview}
\label{sec:algo_overview}

% \SF{In the intro, we call the method ensemble policy; we should use the same terminology. I like AME} >> Sure, I added AME to the intro.
As characterized in Section~\ref{sec:setup}, in a CMARL game, every agent makes decisions based on not only its own observations, but also all received messages. If an agent trusts the communication from all other agents, it may fail when some communication is maliciously corrupted.
On the other hand, if an agent does not trust communication, it can not benefit from the useful information shared by other benign agents.
Therefore, there is a trade-off between natural performance (i.e., reward under no attack) and robustness (i.e., reward under attacks).
Our goal is to learn and execute a robust policy for any agent in the environment, so that the agent can perform well in both a non-adversarial environment and an adversarial environment.


% Traditional MARL algorithms optimize the natural reward $\natobj$ without any attacks, as defined in Problem~\eqref{eq:agent_obj}. However, the learned policies are not necessarily robust against adversarial communications. That is, the attacked reward $\advobj$ could be made extremely low under learned attackers solved by Problem~\eqref{eq:adv_obj}, as verified by our experiments in Section~\ref{sec:exp}.

% Motivated by the fact that communication among agents may be noisy, unstable, and vulnerable to attacks, our goal is to train robust acting policies $\{ \pi_i, i \in [N] \}$, such that for any agent, $\natobj$ and $\advobj$ are both high, even when there are up to $C$ communication messages corrupted at every step. 
% More importantly, we aim to provide a defense mechanism and guarantee that the agents will not be significantly misled by adversarial communication messages during test time.

\textbf{Main Idea}\quad
Intuitively, if an agent $i$ overly relies on the information given by agent $j$, then a strong adaptive attacker can easily mislead $i$ by perturbing the messages from $j$.
Moreover, the benign messages sent from other agents usually contain redundant/overlapping information.
% \myst{, as the goal of communication is to provide the agent additional information and to help the agent make better decisions. }
At each step, an agent receives a set of $N-1$ messages from all other agents, called a \emph{message set}.
% and the set has $N-1$ elements, each is a message received. 
The main idea of our defense is to make decisions based on multiple random subsets of the message set, called \emph{randomly-ablated message samples (or m-samples for short)}.
Under a carefully designed ablation mechanism, benign m-samples can outweigh malicious ones.
To be more specific, we propose to train a \emph{base policy} that makes decisions with one 
% \myst{randomly selected subset of the message set} 
m-sample at each step. 
Then, during test-time, the agent generates multiple m-samples at every step.
% One can design an ablation strategy which guarantees that a majority number of these m-samples contain no malicious messages.
Then the agent applies the trained base policy to  
% \myst{randomly ablated messages, and aggregate the base-policy actions by sampling multiple message combinations, so that the agent can make safe decisions with theoretical guarantees.}
each of these m-samples, getting multiple resulting actions where the majority of them are generated based on benign messages only. 
% The majority of these resulting actions are based on benign messages only and thus safe. 
Therefore, the agent is guaranteed to make a ``safe'' decision if it takes a collection of wisdom from the ensemble of all resulting actions, since the majority of these resulting actions are guaranteed to be guided by benign messages.
% \fh{Made lots of changes here. Can you check whether they are correct?}



A similar randomized ablation defense is used to defend against $\ell_0$ attacks in image classification~\cite{Levine_Feizi_2020}. 
% However, reinforcement learning is fundamentally different from image classification. 
But our defensive mechanism is fundamentally different from the method by~\cite{Levine_Feizi_2020} which provides a high-probability guarantee for discrete image label outputs, as our defense achieves both action and long-term reward certification (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output, which is non-trivial.
% \fh{Our proposed defensive mechanism is a non-trivial extension of the randomized ablation in image classification, as defenses in MDPs requires action certification as well as reward certification whereas defenses in image classification only requires label certification. (This description does not quite clearly explain why MDPs are much harder...)}



\textbf{Notations}\quad
\textbf{(1) Ablation function.} For a list $\mathbf{m}$ and a set of $k$ indices $T=\{j_1,j_2,\cdots,j_k\}$, define an \emph{ablation function} which removes all elements except for those in $T$: $\funabl(\mathbf{m}, T) = [m_{j_1}, \cdots, m_{j_k}]$.
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
%     \funabl(\mathbf{m}, T) = [m_{j_1}, \cdots, m_{j_k}].
% \end{equation}
\textbf{(2) Size-$k$ power subset.} For an integer $n>0$ and the index set $[n]:=\{1,\cdots,n\}$, let $\mathcal{H}(n,k)$ denote the set of all unique $k$ indices out of $[n]$, referred as size-$k$ power subset of $[n]$. That is, $\mathcal{H}(n,k)$ contains all size-$k$ elements in the power set of $[n]$, and thus  $|\mathcal{H}(n,k)|=\binom{n}{k}$. 
% \textcolor{purple}{PH: We have $T$ as the observation omission prob in Sec 2.1, and here as a set of indices. Perhaps we should change the one in Sec 2.1? YS: yes, indeed, I changed it to B}
% \textbf{(2) Power subset. \fh{what's the right terminology?}} For an integer $n>0$ and the indices set $[n]:=\{1,\cdots,n\}$, let $\mathcal{H}(n,k)$ denote the set of all unique $k$ indices out of $[n]$ \fh{known as power subset of size $k$}. That is, $\mathcal{H}(n,k)$ contains all \fh{sized $k$} subsets of $[n]$ \textcolor{red}{with cardinalities $k$} and thus  $|\mathcal{H}(n,k)|=\binom{n}{k}$.  
% Define $\mathcal{U}(n,k)$ as the uniform distribution over $\mathcal{H}(n,k)$. 
% \textbf{(3) \fh{A name for this?}} We let $\krv_{k,n}=\{j_1, j_2,...,j_k\}$ be a random variable taking values on the uniform distribution over $\mathcal{H}(n,k)$. \fh{Intuitively, $\funabl(\mathbf{m}, \krv_{k,n})$ denotes selecting a subset of messages indexed by a random realization $T$ of $\krv_{k,n}$, i.e. $\funabl(\mathbf{m}, T)$ where $T$ is a sized-$k$ index set drawn from $\krv_{k,n}$.} \fh{The problem is that we never defined $\funabl(input-1, input-2)$ when $input-2$ is not a set of indices, but rather a random variable.}
% over $\mathcal{U}(n,k)$. 

With the above intuition and notations, we introduce \ours, a generic defense framework that can be combined with any MARL algorithm with communication.
The training and defending strategies of \ours are provided in Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test}, respectively. 
% Note that the proposed defense is a generic framework that can be combined with any MARL algorithm. 
% Next, we explain the detailed design of these two algorithms. The training and executing procedures for all agents are identical, so we omit the subscript ${}_i$ of policies.

\textbf{Training a Base Ablation Policy $\boldsymbol\ablpolicy$ (Algorithm~\ref{alg:train})}\quad
During training time, every agent learns an \textit{ablation policy} $\ablpolicy_i: \mathcal{O}_i \times \mathcal{M}^k \to \mathcal{A}_i$ which maps an observation and $k$ messages to an action. Here $k$ is a user-specified hyperparameter satisfying
% in order for a successful defense against up to $C$ malicious messages:
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
    \label{eq:k_cond}
    \binom{N-1-C}{k} \geq \frac{1}{2} \binom{N-1}{k}.
\end{equation}
We will explain later that Equation~\eqref{eq:k_cond} plays an important role in our robustness guarantees (Theorem~\ref{thm:main_dist} \& Theorem~\ref{thm:main_cont}) for a successful defense against up to $C$ malicious messages.
% \fh{We will provide more details including the reasoning of such required condition for the choice of $k$ in Section~\ref{?}.} \fh{(Shall we talk about the selection of $k$ somewhere? )}
Note that all agents communicate according to the environment's communication protocol $F$, and attacks do not exist during training.
In every step, an agent randomly samples $k$ out of $N-1$ communication messages, and uses its current acting policy $\ablpolicy$ to react to its current observation and the selected $k$ messages (Line 7 in Algorithm~\ref{alg:train}).
That is, for agent $i$, we optimize and make decisions via $\ablpolicy_i(o_i, \mathsf{Ablate}(\mtoi, T))$, where $\mathsf{Ablate}(\mtoi, T)$ denotes the selected $k$ messages sent from other agents to agent $i$. 
\ys{communication being symmetric}
% and $\ablpolicy_i(o_i, \mathsf{Ablate}(\mtoi, T))$ returns the action the agent $i$ takes according to its current policy.
%$T$ is a random collection of $k$ indices out of $[N-1]$.
% $\krv_{k,N-1}$ is a random collection of $k$ indices out of $[N-1]$. \fh{Then, $\funabl(\mathbf{m}, \krv_{k,n})$ denotes selecting $k$ of the $N$ messages in $\mathbf{m}$ indexed by a set that is a random drawn of $\krv_{k,n}$.} 

% The ablation policy $\ablpolicy$ is trained in a normal environment without any attacks. But we will show that $\ablpolicy$ can be used to defend against test-time communication attacks with theoretical certification. 

\input{algo_train}
\input{algo_test}

\textbf{Defending with an Ensemble Policy $\boldsymbol\smpolicy$ (Algorithm~\ref{alg:test})}\quad
Once we have learned a reasonable ablation policy $\ablpolicy_i$ for agent $i$, we can execute it with ablation and aggregation during test time to defend against adversarial communication. 
Recall that there are up to $C$ malicious messages out of $N-1$ total messages, so the remaining $N-1-C$ messages are benign.
The defense objective is to make a \textit{safe decision} that is robust to malicious massages. 
The main idea is to sample multiple different message subsets out of all $N-1$ received messages, and to select an action suggested by the majority of those message subsets. 
$\smpolicy_i: \mathcal{O}_i \times \mathcal{M}^{N-1} \to \mathcal{A}_i$ is an \textit{ensemble policy} that outputs an action by aggregating the ablation policy's base actions on multiple message subsets (Line 5 in Algorithm~\ref{alg:test}).
The concrete definition of $\smpolicy_i$ depends on whether the action space $\mathcal{A}_i$ is discrete or continuous, which will be detailed in Section~\ref{sec:algo_dist} and Section~\ref{sec:algo_cont}, with corresponding theoretical guarantees on actions and rewards.
% \textcolor{purple}{PH: would it help mentioning $\smpolicy_i: \mathcal{O}_i \times \mathcal{M}^{N-1} \to \mathcal{A}_i$?}



\subsection{\ours in Discrete Action Space}
\label{sec:algo_dist}


Next, we provide the implementation of ensemble policy used in \ours and the corresponding theoretical robustness guarantees for agent $i$ when $\mathcal{A}_i$ is discrete. 
For notation simplicity, we only focus on one agent (although our defense works for multiple agents) and omit the subscript $i$. We further use $\mathbf{m}$ to denote the message list $\mtoi$ received by the current agent at the current step.
% At each step, an agent receives a \emph{message set} with $N-1$ elements, each being a message received. 
Our defense is to make decisions based on multiple size-$k$ random subsets of all messages in $\mathbf{m}$. 

% Recall that $\{ \funabl(\mathbf{m}, T_d)\}_{d=1}^D$ are $D$ different size-$k$ message subsets sampled from the $N-1$ received messages. 
% In a discrete action space, we define the \textit{ensemble policy} $\tilde{\pi}$ as below.

\begin{definition}[\textbf{Ensemble Policy for Discrete Action Space}]
\label{def:ensemble_dist}
For a trained ablation policy $\ablpolicy$, define $u_a$ as the number of times/votes such that the ablation policy $\ablpolicy$ renders action $a$ when taking each of the $\binom{N-1}{k}$ number of message subsets, i.e.,
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
\label{eq:vote}
    u_a := \sum\nolimits_{T\in\mathcal{H}(N-1,k)} \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T))=a].
\end{equation}
Then the ensemble policy $\smpolicy$ takes the action $\widetilde{a}$ which has the most votes, i.e.,
\begin{equation}
\label{eq:ensemble_pi_dist}
    \widetilde{a} = \smpolicy(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \; u_a
\end{equation}
% \fh{How about $\tilde{a} = \smpolicy\Big(o, \{\funabl(\mathbf{m}, T_d)\}_{d=1}^D\Big) := \mathrm{ argmax}_{a\in\mathcal{A}} \; u_a.$?}
\end{definition}
\textbf{Remarks.}
(1) The ensemble policy $\smpolicy$ takes the action suggested by the majority-vote of all size-$k$ message subsets. There are $\binom{N-1}{k}$ number of such size-$k$ subsets in total.
(2) In many practical multi-agent problems, $N$ is not very large, e.g., the number of drones in an area. Therefore, $\binom{N-1}{k}$ is relatively small and not expensive to compute. For example, when $N=10,k=2$, $\binom{N-1}{k}=36$.
% \fh{And we can defend against up to $C=?$ malicious messages.
% I added it to the discussion on ablation size k.
(3) In the case where $\binom{N-1}{k}$ is large, we also provide a variant of the algorithm which takes $D<\binom{N-1}{k}$ samples of message subsets whose certification guarantee is provided in Section~\ref{sec:algo_partial}.

At any step, let $o$ be the observation, $\goodmsg$ and $\advmsg$ be the benign message list before attack and the corrupted message list after attack, respectively.
% $\goodmsg$ be the benign messages (before attack), and $\advmsg$ be the messages after attack (with up to $C$ messages being corrupted). 
Note that $\goodmsg$ and $\advmsg$ both have $N-1$ messages while they differ by up to $C$ messages. 
With the above notation, we define a set of actions rendered by pure-benign message subsets in Definition~\ref{def:safeact_dist}. As the agent is likely to take these actions in a non-adversarial environment, they can be regarded as safe actions to take. 
\begin{definition}[Benign Action Set $\safeaction$]
\label{def:safeact_dist}
For any step, define $\safeaction \subseteq \mathcal{A}$ as a set of actions that $\ablpolicy$ may select under randomly sampled benign messages.
\begin{equation}
\label{eq:safeact_dist}
     \safeaction := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}
\end{equation}
\end{definition}


Next, we provide both action certificate and reward certificate for the above ensemble policy $\smpolicy$.

\textbf{Action Certificate}\quad
% $\safeactiondist \subseteq \mathcal{A}$ is a set of actions that $\ablpolicy$  may select at the current step under randomly sampled benign messages.
The following theorem suggests that the ensemble policy $\smpolicy$ always takes benign actions in $\safeaction$ under mild conditions, even when malicious information is present in the input.

% In this case, the following theorem suggests that the ensemble policy $\smpolicy$ is not influenced by the malicious messages under mild conditions.

\begin{theorem}[Action Certificate for Discrete Action Space]
\label{thm:main_dist}
% Assume that subset size $k$  and ensemble policy $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. 
Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees benign actions under $\advmsg$, i.e.,
\begin{equation}
    \widetilde{a} = \smpolicy(o, \advmsg) \in \safeaction,
    \label{eq:cert_dist}
\end{equation}
if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% where 
% \begin{equation}
%     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% \end{equation}
\end{theorem}
\textbf{Remarks.}
(1) Theorem~\ref{thm:main_dist} certifies that for every step of execution, $\smpolicy$ selects a benign action when the agent receives $\advmsg$ with up to $C$ malicious messages. 
% \fh{Is there a specific reason why we emphasize one step? Should the certification certify every step? Is it possible that the actions appears safe for this round, but not safe for the next round? Oh, maybe the concept of safe already guarantees long-term safety? I feel the emphasis on current-step may cause confusion. We either need to talk about this current-step guarantees long-term safety or we just talk about long-term safety without mentioning current-step?} 
(2) The condition $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ is easy to satisfy when $C \ll N$. This condition accounts for the worst-case scenario when the adversarial messages collaborate to vote for an unsafe action and outweigh benign messages in all base policies. 
But such a worst-case scenario is uncommon in practice, so our algorithm makes the agents robust without requiring this condition of $u_{\widetilde{a}}$, as verified in experiments. 
  
\textbf{Reward Certificate}\quad
Theorem~\ref{thm:main_dist} justifies that under sufficient majority votes $u_{\tilde{a}}$, the ensemble policy $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a benign action that is suggested by some benign message combinations even when the malicious messages are not identified.
Therefore, the ensemble policy $\smpolicy$'s action in every step falls into a benign action set, and thus its cumulative reward under adversarial communications is also guaranteed to be no lower than the worst natural reward the base policy $\ablpolicy$ can get under random benign message subsets. The detailed reward certification is shown in Corollary~\ref{cor:reward_dist} in Appendix~\ref{app:theory_dist}.

\textbf{Discussion on Ablation Size $\boldsymbol k$}\quad 
As an essential condition for the above certificates to hold, Equation~\eqref{eq:k_cond} implies that among all size-$k$ message subsets, there are more purely benign subsets than subsets that contain adversarial messages. This condition always has solutions for $k$ as $C<\frac{N-1}{2}$, and $k=1$ is always a feasible solution. In general, if $k$ is smaller, the ensemble policy is more robust. However, the base ablation policy with a smaller $k$ could gain lower reward as it throws away many messages. Therefore, there is a trade-off between robustness and accuracy, as is pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}.
In practice, if we know $C$ in advance, we can set $k$ to be the largest integer satisfying Equation~\eqref{eq:k_cond}. On the other hand, if $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Equation~\eqref{eq:k_cond}, which shows how many adversarial messages the policy can tolerate. 
For example, when $N=10$, \ours can tolerate up to $C=4$ with $k=1$, and up to $C=2$ with $k=2$. 
Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Equation~\eqref{eq:k_cond}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages, and when $C$ is small, we can use a larger $k$ such that the natural performance is not compromised much.
% 

\subsection{\ours in Continuous Action Space}
\label{sec:algo_cont}

In this section, we introduce the implementation of ensemble policy in \ours and the robustness guarantees in an $L$-dimensional continuous action space. 
Instead of majority voting that is used in a discrete action space, we now use the median statistics to make a robust decision. Define a median function $\funmed$ such that $\funmed(\mathbf{g})$ returns the median value of a list $\mathbf{g}$. If $\mathbf{g}$ is a list of $L$-dimensional vectors, then $\funmed(\mathbf{g})$ returns the element-wise median value, which is also an $L$-dimensional vector.

% \textbf{Additional Notations}\quad
% For any random variable $X$ and a real-valued function $f(X)$, define the median function $\funmed_{X}(f(X))$ as 
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
% \label{eq:med}
% \funmed_{X}(f(X)) := \inf \{ c\in\mathbb{R}: \mathbb{P}_X [ f(X) \geq c ] \geq 0.5 \}.
% \end{equation*}
% For a vector-valued function $F = [f_1(X), \cdots, f_l(X)]^\top$, the $\funmed$ function is extended as the element-wise median value, i.e.,
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
% \label{eq:med_func}
% \funmed_{X}(F(X)) = [\funmed_{X}(f_1(X)), \cdots, \funmed_{X}(f_l(X))]^\top.
% \end{equation*}


In a continuous action space, the ensemble policy $\smpolicy$ takes the median of base actions resulting from all message samples.
% \textcolor{purple}{PH: is this in the right place?  We introduce $D$ later in the section 3.4. Or do we mean to say: ... $\smpolicy$ takes the median of actions resulting from all ablated message samples of size $k$? }
\begin{definition}[\textbf{Ensemble Policy for Continuous Action Space}]
\label{def:ensemble_cont}
For a trained ablation policy $\ablpolicy$, define the ensemble policy $\smpolicy$ as
\begin{equation}
\label{eq:ensemble_pi_cont}
    \tilde{\pi}(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T): T\in\mathcal{H}(N-1,k) \}.
\end{equation}
% \small
% %\vspace{-1.5em}
% \textcolor{red}{
% \begin{equation}
% \label{eq:ensemble_pi_cont}
%     \tilde{\pi}(o, \mathbf{m}, \{T_d\}_{d=1}^D) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% }
% \fh{
% \begin{equation}
%     \resizebox{0.88\columnwidth}{!}{$\smpolicy\Big(o, \{\funabl(\mathbf{m}, T_d)\}_{d=1}^D\Big) =\funmed \Big(\{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D\Big)\label{eq:ensemble_pi_cont}.$}
% \end{equation}
% }
\end{definition}

% \vspace{-1em}
\textbf{Action Certificate}\quad
As in the discrete action case, the continuous ensemble policy will output an action $\widetilde{a}$ that follow the consensus of benign messages. But in a continuous action space, it is hard to ensure that $\widetilde{a}$ is exactly in $\safeaction$. Instead, $\widetilde{a}$ is guaranteed to be within the range of $\safeaction$, as detailed in the following theorem.

\begin{theorem}[Action Certificate for Continuous Action Space]
\label{thm:main_cont}
Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees benign actions under $\advmsg$, i.e.,
\begin{equation}
    \smpolicy(o, \advmsg) \in \mathsf{Range}(\safeaction) := \{a: \forall 1\leq l \leq L, \exists \underline{a}, \overline{a} \in \safeaction \text{ s.t } \underline{a}_l \leq a_l \leq \overline{a} \}.
    \label{eq:cert_cont}
\end{equation}
% then any dimension $l$ of $\smpolicy$'s output satisfies
% \begin{equation*}
%     \inf_{\krv} [\hat{a}]_l  
%     \leq [\smpolicy(o, \advmsg, \{T_d\}_{d=1}^D)]_l 
%     \leq \sup_{\krv} [\hat{a}]_l.
% \end{equation*}
% where $\hat{a} := \ablpolicy(o, \mathsf{Ablate}(m, \krv))$.
\end{theorem}

$\mathsf{Range}(\safeactioncont)$ is a set of actions that are coordinate-wise bounded by base actions resulted from pure-benign m-samples. It is reasonable to assume that actions in $\mathsf{Range}(\safeactioncont)$ are relatively safe. For example, if the action denotes the price a seller sells its product in a market, and the communication messages are the transaction signals in an information pool, then $\mathsf{Range}(\safeactioncont)$ is a price range that is determined based on uncorrupted messages. Therefore, the seller will set a reasonable price without being influenced by a malicious message. 


\textbf{Reward Certificate}\quad
Theorem~\ref{thm:main_cont} shows how the ensemble policy outputs an action that is coordinate-wisely bounded by the range of benign actions. Under mild assumptions, it can also lead to a reward guarantee, as detailed in Appendix~\ref{app:theory_cont}.

\subsection{Extension of \ours: Ensemble with Partial Samples}
\label{sec:algo_partial}

So far we have discussed the proposed \ours algorithm and the constructed ensemble policy that aggregates all $\binom{N-1}{k}$ number of message subsets out of $N-1$ messages. 
However, if $N$ is large, sampling all $\binom{N-1}{k}$ combinations of message subsets could be expensive. In this case, a smaller number of message-subset combinations can be used. That is, given a sample size $0<D\leq\binom{N-1}{k}$, we randomly select $D$ samples $\{T_d\}_{d=1}^D$ from $\mathcal{H}(N-1,k)$ (without replacement), and then we aggregate the ablation policy's decision on $\{\funabl(\mathbf{m}, T_d)\}_{d=1}^D$. 
In this way, we define a sampled version of the ensemble policy, namely \textit{$D$-ensemble policy} $\smpolicy_D$, formulated as below.
% , whose detailed definition is provided in Appendix~\ref{app:theory_sample}.
% define the $D$-ensemble policy $\smpolicy_D$ as the sampled version of $\smpolicy$
\begin{equation}
\label{eq:ensemble_pi_dist_d}
    \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
\end{equation}
for a discrete action space, and
\begin{equation}
\label{eq:ensemble_pi_cont_d}
    \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
\end{equation}\normalsize
for a continuous action space. 



In this case, we can still provide a high-probability robustness guarantee. Theorem~\ref{thm:sample_cont} shows the theoretical result for a continuous action space, while the result for a discrete action space is slightly different and is provided in Appendix~\ref{app:theory_sample}.
% in Theorem~\ref{thm:sample_dist} and Theorem~\ref{thm:sample_cont}. 

\begin{theorem}[General Action Guarantee for Continuous Action Space]
\label{thm:sample_cont}
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$,  under Assumption~\ref{assum:num}, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_cont_d} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, relation~\eqref{eq:cert_cont} holds with probability at least
\begin{equation}
\label{eq:p_sample_cont}
    p_D=\frac{\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n_1-n_2}{D-j}}{\binom{n_1}{D}},
\end{equation}
where $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$ and $\tilde{D} = {\lfloor \frac{D}{2} \rfloor}+1$. 
\end{theorem}
Therefore, for an arbitrary $D$, a benign action will be selected with high probability. The larger $D$ is, the higher the probability is. 
In Theorem~\ref{thm:sample_cont}, when $D=\binom{N-1}{k}$,  the probability $p_D$ is 1 and the result matches Theorem~\ref{thm:main_cont}. 
Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.


\subsection{More Discussion on Applicability and Flexibility of \ours}

\ys{general for any RL policy or decision-making model}

\ys{how a policy is trained}



\ys{training and testing hyperparameters}



==> 5_exp.tex <==
\section{Empirical Study}
\label{sec:exp}

\textbf{Environment Setup: FoodCollector}\quad
We design and implement a 2D particle environment named FoodCollector, adapted from the WaterWorld environment in PettingZoo~\cite{terry2020pettingzoo}. 
There are 9 agents (colored dots surrounded by black lines) relying on sensors (black lines around agents) to observe the world. Each agent's goal is to find the food (colored large dots) of the same color as itself, and avoid collision with poisons (black dots).
The action space can be either (1) discrete, with 9 actions including 8 moving directions and 1 no-move action, or (2) continuous, where the action is an acceleration decision, denoted by a 2-dimensional real-valued vector.
Due to the limited sensory range, each agent can only see the objects around it, and thus communication is helpful. We use a pre-defined protocol where agents share their observed food with each other. Figure~\ref{fig:food}(right) verifies the advantage of communication in FoodCollector. More details of the environment and the communication settings are shown in Appendix~\ref{app:exp_env}.



\textbf{Evaluation}\quad
To evaluate the effectiveness of our defense strategy, we seek to evaluate the performance of the ensemble policy under no attack and under various values of $C$ (for simplicity, we refer to $C$ as the \textit{number of adversaries}). 
Different from previous work~\cite{blumenkamp2020emergence} where the adversarial agent disrupts all the other agents, we consider the case where the attacker deliberately misleads a selected victim, which could evaluate the robustness of the victim under the harshest attacks. 
We use the following two attack methods:
(1) \textbf{non-adaptive attack} that randomly generates a message. Note that this is already a strong attack since a randomly generated message could be arbitrary and far from the original benign message;
% random attacks \fh{random looks too weak, can we justify this is a good attack? Can we give a better name to it?} 
(2) \textbf{learned adaptive attack} that learns the strongest/worst adversarial communication with an RL algorithm to minimize the victim's reward (a white-box attacker which knows the victim's reward). The learned attack can strategically mislead the victim (e.g., to a poison).
As shown in prior works~\cite{zhang2020robust,zhang2021robust,sun2021strongest}, the theoretically optimal attack (which minimizes the victim's reward) can be formed as an RL problem and learned by RL algorithms. 
We can regard this attack as a worst-case attack for the victim agents.
% Therefore, we train an RL attacker policy that maps adversarial agent's observations to adversarial communications. 
More details are in Appendix~\ref{app:exp_imple}.

\textbf{Implementation and Baselines}\quad
We compare our \ours with two baselines: (1) \textbf{(Vanilla)} vanilla training which learns a policy based on all benign messages. (2) \textbf{(AT)} adversarial training as in~\cite{zhang2021robust}, which alternatively trains an adaptive RL attacker and an agent. 
As is common in related work~\cite{lowe2017multi,gupta2017cooperative}, we use parameter sharing and train a shared policy network for all agents.
Our \ours and baselines are all trained with PPO~\cite{schulman2017proximal}, and more implementation details are provided in Appendix~\ref{app:exp_imple}.

\begin{figure}[t]
\vspace{-0.5em}
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{figs/foodcollector.png}
        \vspace{-0.5cm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figs/comm_dist_small}}
        \vspace{-0.5cm}
    \end{subfigure}
\vspace{-1em}
\caption{\textbf{Left:} The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. 
\textbf{Right:} Reward of agents trained with communication v.s. without communication in a discrete action space. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly. The result in a continuous action space is similar, as presented in Appendix~\ref{app:exp_env}.}
\label{fig:food}
\vspace{-1.5em}
\end{figure}

% \paragraph{Random Attacks} xxx

% \paragraph{Heuristic Attacks} xxx

% \paragraph{Optimal Attacks} Suppose there is an attacker manipulating communication messages from a subset of agents $\mathcal{Y}=\{ y_1, \cdots, y_C \}$ to $x$ ($x \notin \mathcal{Y})$, i.e., the attacker can control the communication channels to the victim from up to $C$ agents. \fh{Note that $C$ should be considered as a known hyperparameter, and we will provide more insight later in the paper about how to set $C$ in practice.} 
% As pointed out by some prior works~\cite{zhang2020robust,sun2021strongest}, the \textit{optimal attack} \fh{to an RL policy} can be learned by solving an RL problem:
% % {\small{
% \setlength\abovedisplayskip{-2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:adv_obj}
% \tag{$Q_A$}
% \begin{aligned}
%     \min_{\nu_1,\cdots,\nu_C} & \; \advobj^x :=  \mathbb{E} [ \sum_{t=0}^\infty \gamma^t [R(s\step, a_1\step, \cdots, a_N\step)]_{x} ] \\
%     \text{where } & \; a_i\step = \pi_i(o_i\step, \mtoi\step), \forall i\in [N], t \geq 0 \\
%      & \; m_{y_j \to x}\step = \nu_{j}(o_{y_j}\step), \forall j\in [C], t \geq 0
% \end{aligned}
% \end{equation}
% % }}
% \fh{ I tried to move something, but may not be complete and logic needs to be straightened out.}


% The minimizer to Problem~\eqref{eq:adv_obj}, $\nu_1^*,\cdots,\nu_C^*$ , defines an optimal communication attacking strategy that is adaptive to victim $\pi_x$. 
% In other words, the attacker learns $C$ communication policies that collaboratively minimizes the reward of the victim agent $x$.



\textbf{Experiment Results}\quad
As shown in Figure~\ref{fig:res_all}, the rewards of Vanilla and AT drastically drop under attacks, especially adaptive attackers. %(A random agent can gain reward -80.)
We find that AT does not achieve better robustness than Vanilla, since malicious messages can appear at any channel, and it is hard for AT to learn a general defense strategy, as explained in Appendix~\ref{app:exp_imple}.
% becomes too conservative as it is trained to adapt to adversarial messages from multiple channels, i.e., AT does not trust any communication, as detailed in Appendix~\ref{app:exp_imple}.
% , and thus AT cannot utilize well the benign messages.
% does not outperform Vanilla under communication attacks, because there are many communication channels and it is hard for the agent to adapt to all communication attacks.
% Note that the lowest possible reward in this environment is about -100, so in the discrete action case, 2 adaptive adversarial messages can already reduce the reward of Vanilla and AT to the lowest level.
In contrast, we use $k=2$ for our \ours, which provides performance guarantees against up to $C=2$ adversaries. We can see that the reward of \ours under $C=1$ or $C=2$ is similar to its reward under no attack, matching our theoretical analysis. 
The high performance of \ours verifies that it can utilize benign communication well while being robust to adversarial communication.
In both discrete and continuous action spaces, \ours achieves a significantly better performance than Vanilla and AT under various numbers of adversaries, even under 3 adversaries where the theoretical guarantees no longer hold. Therefore, \textit{\ours makes agents robust under varying numbers of adversaries.} 

\input{fig_food_res}

\input{fig_food_k_dist} 

% \textbf{Hyper-parameter Tests}\quad 
% % \ours requires a hyper-parameter $k$  which controls how many messages the base ablation policy relies on to output a base action. The partial-sample variant of \ours introduced in Section~\ref{sec:algo_partial} requires another hyper-parameter $D$, the number of message subset samples the ensemble policy uses. 
% To evaluate the effects of two hyper-parameters $k$ (ablation size) and $D$ (sample size, only used for partial-sample \ours introduced in Section~\ref{sec:algo_partial}), we train \ours with different $k$'s and $D$'s and plot the results in Figure~\ref{fig:res_k_dist} for discrete-action FoodCollector, and Figure~\ref{fig:res_k_cont} for continuous-action FoodCollector (in Appendix~\ref{app:exp_res}).
% \\
\textbf{Hyper-parameter Test of Ablation Size $\boldsymbol k$}\quad
As discussed in Section~\ref{sec:algo_dist}, the value of $k$ is related to the trade-off between natural performance and robustness. To see how $k$ influences the agent's performance, we evaluate \ours's natural reward and \ours's reward under $2$ adaptive adversaries with different ablation sizes $k$. The result in discrete-action FoodCollector is shown in Figure~\ref{fig:res_k_dist}(left), while the continuous-action result is similar and is in Appendix~\ref{app:exp_res}. We can see that increasing the ablation size $k$ improves the natural performance of the agent since each agent could gather more information from others. However, raising the ablation size $k$ also increases the risk of making decisions based on communication messages sent from an adversary. Therefore, \textit{increasing ablation size $k$ trades off robustness for natural performance.} 

\textbf{Hyper-parameter Test of Sample Size $\boldsymbol D$}\quad
We further evaluate the partial-sample variant of \ours introduced in Section~\ref{sec:algo_partial} using $k=2$ under $2$ adaptive adversaries, with $D$ varying from 28 (the largest sample size) to 1 (the smallest sample size). Figure~\ref{fig:res_k_dist}(right) shows the result in a discrete action space, and the continuous-action result is in Appendix~\ref{app:exp_res}. As $D$ goes down, \ours obtains lower reward under attackers, but it is still significantly more robust than baseline methods, even when $D=1$ where the agent makes decisions based on only 1 random message subset.

% Note that when $C=2$, the maximum $k$ such that our certificates hold is 2, according to Inequality~\eqref{eq:k_cond}. Figure~\ref{fig:res_k_dist} shows that, when $k$ increases from $1$ to $2$, the robust performance barely drops, which verifies again the effectiveness of our theoretical guarantees. In practice, to decide the ablation size $k$, we suggest first to estimate the number of attackers that one would like to defend and then choose the maximum $k$ satisfying the condition in Eq~\eqref{eq:k_cond} such that Theorem \ref{thm:main_dist} or \ref{thm:main_cont} hold.


% \begin{figure}[t]
% % \vspace{-0.1cm}
%  \centering
%  \hspace{-1em}
%  \begin{subfigure}[t]{0.42\columnwidth}
%   \input{figs/FoodCollector_Attacker_Dist}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.45\columnwidth}
%   \input{figs/FoodCollector_Ablation_k_2adv_dist}
%  \vspace{-1.5em}
%  \subcaption{Discrete Action Space} 
  
%  %\vspace{0.2cm}
%  \centering
%  \hspace{-1em}
%  \begin{subfigure}[t]{0.42\columnwidth}
%   \input{figs/FoodCollector_Attacker_Cont}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.45\columnwidth}
%   \input{figs/FoodCollector_Ablation_k_2adv_cont}
%  \end{subfigure}
%  \vspace{-1.5em}
%  \subcaption{Continuous Action Space}
% % \vspace{-0.5em}
% \caption{\textbf{Left}: Average return under different number of attackers for our Randomized Ablation defensive method against Adversarial Training and Vanilla Training. \textbf{Right}: Tradeoff between clean and robust performance through ablation size $k$}
% \vspace{-0.5em}
% \label{fig:n_attacker}
% \end{figure}

% \begin{figure}[h]
% \vspace{-0.2cm}
%  \centering
%  \begin{subfigure}[t]{1\columnwidth}
%  \centering
% \input{figs/FoodCollector_Ablation_k_2adv_dist.tex}
% \vspace{-0.2cm}
% \subcaption{Discrete Action Space}
% \end{subfigure}
% %\hfill
% \begin{subfigure}[t]{1\columnwidth}
%  \centering
% \input{figs/FoodCollector_Ablation_k_2adv_cont.tex}
% \vspace{-0.2cm}
% \subcaption{Continuous Action Space}
% \end{subfigure}
% \vspace{-0.4cm}
% \caption*{Tradeoff between clean and robust performance through ablation size $k$}
% \vspace{-0.3cm}
% \label{fig:ablation_k}
% \end{figure}


% \textbf{Increasing ablation sample size $D$ results in higher certification probability, which leads to higher robust performance}

% In the previous experiments, we used the full-sample ablation, i.e. $D=\binom{N-1}{k}$. However, in practice when the number of agents is large, it becomes too computationally expensive to compute all $\binom{N-1}{K}$ ablation combinations. In this case, theorem \ref{thm:main_cont} and \ref{thm:main_dist} provide a robust guarantee for partial-sample ablation when uniformly sampling $D$ combinations. To investigate the relationship between the certification probability $p_D$ provided in theorem 
% \begin{figure}[h]
% \vspace{-0.2cm}
%  \centering
% \input{figs/FoodCollector_Ablation_k_sample.tex}
% \vspace{-0.4cm}
% \caption{Effects of ablation sample size $D$ on robust reward and certification probability in Theorem\ref{thm:main_dist}}
% \label{fig:ablation_k_sample}
% \end{figure}

% \textit{Detection of Adversaries is possible with randomized ablation in continuous action space.}


% \begin{figure}[h]
% \vspace{-0.1cm}
%  \centering
% \input{figs/FoodCollector_Ablation_k_2adv_dist.tex}
% \vspace{-0.3cm}
% \caption{Attacker identification based on action bias $\nu_j$. Adv1 and Adv2 stands for Adversary 1 and 2. B1 up to B6 stands for 6 other benign agents.}
% \vspace{-0.5cm}
% \label{fig:detect_adv}
% \end{figure}



%\textbf{Baselines.}\quad

%\ys{todo: try other attacks?}

%\ys{In each environment, results we expect to show are:

%1. 
%clean reward and attacked reward (under different numbers of attackers) %for (1) (baseline) vanilla training, (2) (baseline) alternate adversarial %training, (3) ablation with a good choice of k

%2. [optional]
%different values of k

%3. [optional]
%different values of sample size, results with trustworthy scores

% \begin{figure}[!h]
%  \centering
%  \begin{subfigure}[b]{0.45\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{figs/attacker_1.jpg}
%     \caption{Under 1 attacker.}
%      \label{sfig:ablation_1}
%  \end{subfigure}
%  \hfill
% \begin{subfigure}[b]{0.45\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{figs/attacker_2.jpg}
%      \caption{Under 2 attackers.}
%      \label{sfig:ablation_2}
%  \end{subfigure}
% \caption{Simple randomized ablation vs. vanilla training under attacks in a 9-agent FoodCollector.}
% \label{fig:ablation}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figs/sampling.png}
%     \caption{Sample-based advanced randomized ablation vs. vanilla training under 2 attackers in a 9-agent FoodCollector. Note that sample size 1 is equivalent to the simple ablation method, and sample size 28 is equivalent to the exhausted ablation. }
%     \label{fig:ablation}
% \end{figure} 

==> 5_exp_arxiv.tex <==
\section{Empirical Study}
\label{sec:exp}

\subsection{Defending against Adversarial Position Messages in A Particle Domain}
\label{sec:exp_particle}

\textbf{Environment Setup}\quad We design and implement a practical 2D particle environment named FoodCollector, adapted from the WaterWorld environment in PettingZoo~\cite{terry2020pettingzoo}. 
There are 9 agents (colored dots surrounded by black lines) relying on sensors (black lines around agents) to observe the world. Each agent's goal is to find the food (colored large dots) of the same color as itself, and avoid collision with poisons (black dots).
The action space can be either (1) discrete, with 9 actions including 8 moving directions and 1 no-move action, or (2) continuous, where the action is an acceleration decision, denoted by a 2-dimensional real-valued vector.
Due to the limited sensory range, each agent can only see the objects around it, and thus communication is helpful. We use a pre-defined protocol where agents share their observed food with each other. Figure~\ref{fig:food} verifies the advantage of communication in FoodCollector. More details of the FoodCollector environment and the communication settings are shown in Appendix~\ref{app:exp_env}.


\textbf{Evaluation}\quad
To evaluate the effectiveness of our defense strategy, we seek to evaluate the performance of the ensemble policy under no attack and under various values of $C$ (for simplicity, we refer to $C$ as the \textit{number of adversaries}). 
Different from previous work~\cite{blumenkamp2020emergence} where the adversarial agent disrupts all the other agents, we consider the case where the attacker deliberately misleads a selected victim, which could evaluate the robustness of the victim under the harshest attacks. 
We use the following two attack methods:
(1) \textbf{non-adaptive attack} that randomly generates a message. Note that this is already a strong attack since a randomly generated message could be arbitrary and far from the original benign message;
% random attacks \fh{random looks too weak, can we justify this is a good attack? Can we give a better name to it?} 
(2) \textbf{learned adaptive attack} that learns the strongest/worst adversarial communication with an RL algorithm to minimize the victim's reward (a white-box attacker which knows the victim's reward). The learned attack can strategically mislead the victim (e.g., to a poison).
As shown in prior works~\cite{zhang2020robust,zhang2021robust,sun2021strongest}, the theoretically optimal attack (which minimizes the victim's reward) can be formed as an RL problem and learned by RL algorithms. 
We can regard this attack as a worst-case attack for the victim agents.
% Therefore, we train an RL attacker policy that maps adversarial agent's observations to adversarial communications. 
More details are in Appendix~\ref{app:exp_imple}.

\textbf{Implementation and Baselines}\quad
We compare our \ours with two baselines: (1) \textbf{(Vanilla)} vanilla training which learns a policy based on all benign messages. (2) \textbf{(AT)} adversarial training as in~\cite{zhang2021robust}, which alternatively trains an adaptive RL attacker and an agent. 
As is common in related work~\cite{lowe2017multi,gupta2017cooperative}, we use parameter sharing and train a shared policy network for all agents.
Our \ours and baselines are all trained with PPO~\cite{schulman2017proximal}, and more implementation details are provided in Appendix~\ref{app:exp_imple}.

\begin{figure}[t]
\vspace{-0.5em}
    \centering
    \begin{subfigure}[t]{0.32\columnwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{figs/foodcollector.png}
        \vspace{-0.5cm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figs/comm_dist_small}}
        \vspace{-0.5cm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figs/comm_cont}}
        \vspace{-0.5cm}
    \end{subfigure}
% \vspace{-1em}
\caption{\textbf{Left:} The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. 
\textbf{Middle/Right:} Reward of agents trained with communication v.s. without communication in discrete/continuous action space. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly. 
%The result in a continuous action space is similar, as presented in Appendix~\ref{app:exp_env}.
}
\label{fig:food}
\vspace{-1.5em}
\end{figure}

% \paragraph{Random Attacks} xxx

% \paragraph{Heuristic Attacks} xxx

% \paragraph{Optimal Attacks} Suppose there is an attacker manipulating communication messages from a subset of agents $\mathcal{Y}=\{ y_1, \cdots, y_C \}$ to $x$ ($x \notin \mathcal{Y})$, i.e., the attacker can control the communication channels to the victim from up to $C$ agents. \fh{Note that $C$ should be considered as a known hyperparameter, and we will provide more insight later in the paper about how to set $C$ in practice.} 
% As pointed out by some prior works~\cite{zhang2020robust,sun2021strongest}, the \textit{optimal attack} \fh{to an RL policy} can be learned by solving an RL problem:
% % {\small{
% \setlength\abovedisplayskip{-2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:adv_obj}
% \tag{$Q_A$}
% \begin{aligned}
%     \min_{\nu_1,\cdots,\nu_C} & \; \advobj^x :=  \mathbb{E} [ \sum_{t=0}^\infty \gamma^t [R(s\step, a_1\step, \cdots, a_N\step)]_{x} ] \\
%     \text{where } & \; a_i\step = \pi_i(o_i\step, \mtoi\step), \forall i\in [N], t \geq 0 \\
%      & \; m_{y_j \to x}\step = \nu_{j}(o_{y_j}\step), \forall j\in [C], t \geq 0
% \end{aligned}
% \end{equation}
% % }}
% \fh{ I tried to move something, but may not be complete and logic needs to be straightened out.}


% The minimizer to Problem~\eqref{eq:adv_obj}, $\nu_1^*,\cdots,\nu_C^*$ , defines an optimal communication attacking strategy that is adaptive to victim $\pi_x$. 
% In other words, the attacker learns $C$ communication policies that collaboratively minimizes the reward of the victim agent $x$.



\textbf{Robust performance Under Attacks}\quad
As shown in Figure~\ref{fig:res_all}, the rewards of Vanilla and AT drastically drop under attacks, especially adaptive attackers. %(A random agent can gain reward -80.)
We find that AT does not achieve better robustness than Vanilla, since malicious messages can appear at any channel, and it is hard for AT to learn a general defense strategy, as explained in Appendix~\ref{app:exp_imple}.
% becomes too conservative as it is trained to adapt to adversarial messages from multiple channels, i.e., AT does not trust any communication, as detailed in Appendix~\ref{app:exp_imple}.
% , and thus AT cannot utilize well the benign messages.
% does not outperform Vanilla under communication attacks, because there are many communication channels and it is hard for the agent to adapt to all communication attacks.
% Note that the lowest possible reward in this environment is about -100, so in the discrete action case, 2 adaptive adversarial messages can already reduce the reward of Vanilla and AT to the lowest level.
In contrast, we use $k=2$ for our \ours, which provides performance guarantees against up to $C=2$ adversaries. We can see that the reward of \ours under $C=1$ or $C=2$ is similar to its reward under no attack, matching our theoretical analysis. 
The high performance of \ours verifies that it can utilize benign communication well while being robust to adversarial communication.
In both discrete and continuous action spaces, \ours achieves a significantly better performance than Vanilla and AT under various numbers of adversaries, even under 3 adversaries where the theoretical guarantees no longer hold. Therefore, \textit{\ours makes agents robust under varying numbers of adversaries.} 

\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist_naive}}
  \vspace{-1.5em}
  \caption{Disc. \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist}}
  \vspace{-1.5em}
  \caption{Disc. \& Adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Cont_naive}}
  \vspace{-1.5em}
  \caption{Cont. \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\textwidth}{!}{ \input{figs/FoodCollector_Attacker_Cont}}
  \vspace{-1.5em}
  \caption{Cont. \& Adaptive}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Reward comparison between our \ours and baselines in FoodCollector with discrete/continuous action space, under no attacker or non-adaptive/adaptive attacks under varying numbers of adversaries. Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_all}
\end{figure}





\subsection{Defending against Adversarial Demand Messages in A Market Domain}
\label{sec:exp_market}

\textbf{Environment Setup}\quad 
We design a practical environment called \textit{MarketEnv} which simulates the real-world inventory management problem, where $N=10$ heterogeneous seller agents carry inventory for $M=3$ products. A population of $B=300$ buyers request a product from a randomly selected seller agent according to a demand distribution. Sellers manage their inventory by restocking products through interacting with the buyers. The game is episodic with horizon set to $50$. At the beginning of each episode, a realization of the demand distribution $\mathbf{p}$ is randomly generated and the agents' inventory for each product is randomly initialized from $[0, \frac{B}{N}]$, where $\frac{B}{N}$ is the expected number of buyers per seller. 
Sellers are penalized for mismatch between their inventory and the demand for a product, and they aim to restock enough units of a product at each step to prevent insufficient inventory without accruing a surplus at the end of each step. Sellers communicate with each other by exchanging their own demand observations, so that they can estimate the true demand distribution more accurately and manage stock better. More details of the Market environment and the communication settings are shown in Appendix~\ref{app:market_env}.


\textbf{Evaluation and Implementation}\quad
As in the FoodCollector environment, we compare \ours with Vanilla and AT against learned adaptive attacks and non-adaptive attacks. To simulate various types of practical attacks, we design multiple non-adaptive attack formulations: (1) \permute that randomly permutes the order of the demand observation of $M$ products; (2) \swap that swaps the highest demand and the lowest demand, the second highest demand with the second lowest demand and so forth; (3) \flip that flips the demand values with respect to the average demand observation. The agents and the adaptive attackers are both learned with PPO, detailed in Appendix~\ref{app:market_imple}. 


\paragraph{Robust performance Under Attacks} \quad
In this section, we evaluate robustness of the proposed \ours defense strategy in MarketEnv and compare it against Vanilla Learning and Adversarial Training. Figure~\ref{fig:res_all_market} shows the natural and robust performance of \ours with $k=2$, which provides performance guarantees against up to $C=2$ adversarial messages. The performance is compared with AT when the agents policy is alternatively trained against $2$ adversaries. We observe that there is a considerable reduction in the Vanilla and AT rewards under attacks, especially for the strong adaptive attack and \swap. Similar to the FoodCollector, adversarial training is not robust to adversarial communications in the MarketEnv such that for two or more adversarial messages the performance is close to or much lower than the reward achieved with no communications. However, as expected for $k=2$, \ours is able to achieve rewards comparable to the no-attack case  under $C=1$ and $C=2$ adversaries even for strong adversarial attacks. Moreover, \ours outperforms the baselines for $C=3$ for which the theoretical guarantees no longer hold. Even though the gap between natural and robust performance under the weak \permute is less for all three strategies, \ours achieves the highest reward. In  MarketEnv, \ours is able to preserve the communication gains arising from informative messages shared among the agents while being robust against adversarial communications.

  
\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
  \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_adaptive}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_permute}}
  \vspace{-1.5em}
  \caption{\permute}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_flip}}
  \vspace{-1.5em}
  \caption{\swap}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
  \resizebox{\linewidth}{!}{ \input{figs/MarketEnv/MarketEnv_Attacker_Dist_swap}}
  \vspace{-1.5em}
  \caption{\flip}
 \end{subfigure}
%  \vspace{-0.5em}
\caption{\textbf{MarketEnv}: Reward comparison between our \ours and baselines with continuous action space, under no attacker and varying numbers of adversaries for (a) adaptive and (b), (c), (d) non-adaptive attacks. Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_all_market}
\end{figure}




\subsection{Defending against Adversarial Communication in Multi-agent Image Classification}
\label{sec:exp_mnist}

\textbf{Environment Setup}\quad 
Communicative multi-agent learning is also used in vision tasks. For example, \cite{mousavi2019multi} use MARL for image classification in the MNIST dataset. There are multiple agents aiming to classify an image within  a limited time horizon. At every step, each agent observes a patch of the image, and can take an action to move to an adjacent patch, based on an LSTM policy. In the meanwhile, agents are allowed to exchange information (encoded local beliefs) with other agents to update their own beliefs. Therefore, different from the hand-coded communication protocols used in FoodCollector and MarketEnv, agents in this MNIST classification task use learned communication.

\textbf{Evaluation and Implementation}\quad 
Our implementation is based on \cite{mnistgithub} that reproduces the results of~\cite{mousavi2019multi}.
We first test the robustness of the original LSTM policies proposed by \cite{mousavi2019multi} under communication attacks, i.e., $C$ out of $N-1$ communication messages (encodings) are corrupted. Then, we equip the LSTM policy with \ours by message ablation and ensemble, and verify its robustness against random attacks and learned adaptive attacks. More environment description and implementation details are provided in Appendix~\ref{app:mnist}.


\textbf{Robust performance Under Attacks}\quad
Figure~\ref{fig:res_mnist} demonstrates the robust performance of the MARL algorithm proposed by~\cite{mousavi2019multi} without or with our \ours defense. We set $N=9$ and $k=2$ for all experiments.
Under learned adaptive attackers, the original MARL classifier~\cite{mousavi2019multi}  without \ours suffers from significant performance drop in terms of both precision and recall, while \ours considerably improves the robustness of agents across different numbers of attackers. 
Under random attacks, we find that the MARL classifier~\cite{mousavi2019multi} is moderately robust when a few communication signals are randomly perturbed. However, when noise exists in many communication channels (e.g. $C=6$), the performance decreases a lot. In contrast, our \ours still achieves high performance when $C=6$ communication messages are corrupted.

\begin{figure}[h]
% \vspace{-0.5em}
\hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/MNIST_Adaptive_Attacker_Precision}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MNIST_Adaptive_Attacker_Recall}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/MNIST_Random_Attacker_Precision}}
  \vspace{-1.5em}
  \caption{Non-adaptive Attack}
 \end{subfigure}
\hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MNIST_Random_Attacker_Recall}}
  \vspace{-1.5em}
  \caption{Non-adaptive Attack}
 \end{subfigure}
\vspace{-0.5em}
\caption{Precision and recall of MARL classification on MNIST without or with \ours, under learned adaptive attacks and non-adaptive random attacks. }
% \vspace{-1.5em}
\label{fig:res_mnist}
\end{figure}


\subsection{Hyper-parameter Tests}
\label{sec:exp_hyper}

\textbf{Hyper-parameter Test of Ablation Size $\boldsymbol k$}\quad
As discussed in Section~\ref{sec:algo_dist}, the value of $k$ is related to the trade-off between natural performance and robustness. To see how $k$ influences the agent's performance, we evaluate \ours's natural reward and \ours's reward under the same number ($C=2$) of strong adaptive adversaries with different ablation sizes $k$. 
The results in FoodCollector and MarketEnv are shown in Figure~\ref{sfig:hyper_k_food} and Figure~\ref{sfig:hyper_k_market}, respectively.
We can see that increasing the ablation size $k$ improves the natural performance of the agent since each agent could gather more information from others. However, raising the ablation size $k$ also increases the risk of making decisions based on communication messages sent from an adversary. Therefore, \textit{increasing ablation size $k$ trades off robustness for natural performance.} 


\textbf{Hyper-parameter Test of Sample Size $\boldsymbol D$}\quad
We further evaluate the partial-sample variant of \ours introduced in Section~\ref{sec:algo_partial} using $k=2$ under $C=2$ adaptive adversaries, with $D$ varying from $N-1 \choose k$ (the largest sample size) to 1 (the smallest sample size). Figure~\ref{sfig:hyper_d_food} and Figure~\ref{sfig:hyper_d_market} demonstrate the performance of different $D$'s in FoodCollector and MarketEnv. As $D$ goes down, \ours obtains lower reward under attackers, but it is still significantly more robust than baseline methods, even when $D=1$ where the agent makes decisions based on only 1 random message subset.

\begin{figure}[htbp]
% \vspace{-0.5em}
\hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_cont}}
  \vspace{-1.5em}
  \caption{FoodCollector}
  \label{sfig:hyper_k_food}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}}
  \vspace{-1.5em}
  \caption{MarketEnv}
  \label{sfig:hyper_k_market}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_sample_cont}}
  \vspace{-1.5em}
  \caption{FoodCollector}
  \label{sfig:hyper_d_food}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_K_sampleD}}
  \vspace{-1.5em}
  \caption{MarketEnv}
  \label{sfig:hyper_d_market}
 \end{subfigure}
\vspace{-0.5em}
\caption{Hyper-parameter tests of ablation size $k$ and sample size $D$. 
We show how natural reward and attacked performance change with \textbf{(a)} various $k$ in continuous-action FoodCollector, \textbf{(b)} various $D$ in continuous-action FoodCollector, \textbf{(c)} various $k$ in MarketEnv, and \textbf{(d)} various $D$ in MarketEnv. (Dashed green lines refer to the performance of Vanilla agent under $C=2$ attacks.) The result of discrete-action FoodCollector is similar as shown in Figure~\ref{fig:res_k_dist} in Appendix~\ref{app:exp_res}.}
\vspace{-1.5em}
\label{fig:res_hyper}
\end{figure}



% \textbf{Hyper-parameter Tests}\quad 
% % \ours requires a hyper-parameter $k$  which controls how many messages the base ablation policy relies on to output a base action. The partial-sample variant of \ours introduced in Section~\ref{sec:algo_partial} requires another hyper-parameter $D$, the number of message subset samples the ensemble policy uses. 
% To evaluate the effects of two hyper-parameters $k$ (ablation size) and $D$ (sample size, only used for partial-sample \ours introduced in Section~\ref{sec:algo_partial}), we train \ours with different $k$'s and $D$'s and plot the results in Figure~\ref{fig:res_k_dist} for discrete-action FoodCollector, and Figure~\ref{fig:res_k_cont} for continuous-action FoodCollector (in Appendix~\ref{app:exp_res}).
% \\





% \paragraph{Hyper-parameter Test of Ablation Size $\boldsymbol k$} 
% Figure~\ref{fig:res_k_cont_market}(left)  shows how the agent's natural performance and robustness varies with the ablation size $k$. We compare \ours’s natural reward and \ours’s reward under $C=2$ adversarial communication messages for adaptive and non-adaptive attacks  with different values of $k$. Similar to the FoodCollector, As the ablation size $k$ increase, the agent is able to improve its natural performance by utilizing information communicated by more agents. However, the agent becomes more vulnerable to adversarial communications which can impacts its decision-making for managing its inventory. Therefore, ablation size $k$ trades off robustness for natural performance. Additionally, we observe that the non-adaptive \swap which constructs the  adversarial communications strategically to mislead the victim agent is quite effective in reducing the victims reward compared to the \permute which communicates adversarial messages without tactically modifying the adversary's observed demands.
 
% \paragraph{Hyper-parameter Test of Sample Size $\boldsymbol D$}
% In Figure~\ref{fig:res_k_cont_market}(right), we evaluate the robustness of the partial-sample variant of \ours presented in Section~\ref{sec:algo_partial} against $C=2$  adversaries for ablation size $k=2$, when $D$  varies from $36$ (the largest sample size) to $1$ (the smallest sample size). It is shown that with lower $D$, \ours achieves lower rewards under adversarial communications, but is considerably more robust compared to the baseline method. When the agent makes decisions based on a single random message with $D=1$, the agent's average robust reward is higher than the Vanilla reward.


% \begin{figure}[h]
%  \centering
%  \begin{subfigure}[t]{0.49\textwidth}
%  \centering
%   \resizebox{0.6\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.49\textwidth}
%  \centering
%   \resizebox{0.6\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_K_sampleD}}
%  \end{subfigure}
% %  \vspace{-2em}
% %  \subcaption{Continuous Action Space}
% \vspace{-0.5em}
% \caption{\textbf{MarketEnv} Hyper-parameter test in continuous-action MarketEnv. \textbf{Left:}  Natural and robust performance with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. Dashed green line refers to Vanilla under $C=2$ attacks.}
% \vspace{-0.5em}
% \label{fig:res_k_cont_market}
% \end{figure}

==> 6_discuss.tex <==
\vspace{-0.5em}
\section{Conclusion and Discussion}
\label{sec:discuss}
% \vspace{-0.5em}

This paper formulates communication attacks in MARL problems, and proposes \ours, a certifiable defense against multiple arbitrarily perturbed adversarial communication messages, based on randomized ablation and aggregation. The idea of \ours can also be extended to detect attackers, by measuring the difference between the action suggested by any specific communication message and the ensemble policy's action, as empirically verified in Appendix~\ref{app:exp_detect}. 
\ys{flexibility of different $k$'s in training and test.}

==> a1_proof.tex <==
\section{Proofs of Main Theorems}
For the simplicity of the proof, we make the following definition.
\label{app:proof}
\begin{definition} (Safe Message Combination)
For a message combination $T\in \mathcal{H}(N-1, k)$, $\funabl(\textbf{m}, T)=[m_{j_1},...,m_{j_k}]$ is a \emph{safe message combination} iff for every $1\leq n\leq k$, $m_{j_n}$ is a benign communication message. Otherwise, it is  an \emph{unsafe message combination}. 

% \textcolor{purple}{PH: I think the terminology here may not be consistent with the main paper. 
% \begin{itemize}
%     \item $T$ is the index set of messages, but here we are referring to it as "combination message". Should we use $[m_{j_1}\dots, m_{j_k}]$?
%     \item  In section 2.2 [Formulation of Communication Attack] and Assumption 2.1, we talk about One attacker that can perturb $C$ of the communication messages (channels). However, here we are talking about $k$ benign/adversarial agents. Maybe we could say "iff $m_{j_n}$ is a benign communication message for every $1\leq n\leq k$"?
% \end{itemize}}
\end{definition}
For simplicity, we will refer to the indexes $T$ as a safe message combination iff $\funabl(\textbf{m}, T)$ is a safe  message combination. Note that the total  number of safe message combinations is $n_2=\binom{N-C-1}{k}$, and the total number of unsafe message combinations is $n_1-n_2=\binom{N-1}{k}-\binom{N-C-1}{k}$.

\subsection{Proofs in Discrete Action Space}
\begin{proof}[Proof of Theorem~\ref{thm:main_dist} and Theorem~\ref{thm:sample_dist}]
The majority voted action $\tilde{a}$ is a benign action, i.e., $\tilde{a}\in \safeactiondist$, if the ablation policy $\hat{\pi}$ renders action $\tilde{a}$ for
at least one safe message combination.  If $u_{\tilde{a}}>n_1-n_2$, since $n_1-n_2$ is exactly the total number of unsafe combinations, then it is guaranteed that there is at least one safe combination for which $\hat{\pi}$ renders $\tilde{a}$. Thus, $\tilde{a}\in \safeactiondist$.
%Here, the majority voted action $\tilde{a}\in \safeactiondist$ is equivalent to the condition that $\tilde{a}$ is chosen by at least one safe message combination. Therefore, if $u_{\tilde{a}}>n_1-n_2$, where $n_1-n_2$ is exactly the total number of unsafe combinations, then it is guaranteed that $\tilde{a}$ is chosen by at least one safe combination. Thus, $\tilde{a}\in \safeactiondist$ is a safe action.

However, if $u_{\tilde{a}}\leq n_1-n_2$, then in order for $\tilde{a}$ to be safe, among the $u_{\tilde{a}}$ message combinations resulting in $\tilde{a}$ there can be at most $u_{\tilde{a}}-1$ unsafe combinations.  % Therefore, the maximum number of votes coming from unsafe message combination is $u_{\tilde{a}}-1$. 
There are $ \sum_{j=0}^{u_{\tilde{a}}-1}\binom{n_1-n_2}{j}\binom{n_2}{D-j}$ such possibilities in terms of the sampling of $D$, and the total number of possibilities are $\binom{n_1}{D}$. Therefore, we get Equation \eqref{eq:p_sample_dist}.



The proof of Theorem~\ref{thm:main_dist} follows as a special case of Theorem~\ref{thm:sample_dist} when $D=\binom{N-1}{k}$. In this case, the only non-zero term left in the numerator of $p_D$ is $\binom{n_2}{j}\binom{n_1-n_2}{n_1-j}=\binom{n_2}{n_2}\binom{n_1-n_2}{n_1-n_2}=1$ ($j=n_2$), so $p_D=1$.

% Let $m_{:\to i}$ denote the message list communicated to agent $i$ by all other agents in the non-adversarial setting. In the adversarial setting, $K\in [n]$ is the set of malicious agents attacking agent $i$ ($K$ is not known to agent $i$), and $m_{:\to i}^\prime$ denotes the communicated message list in this setting. Then, 
% \begin{align}
% &\mathbb{P}(\hat{\pi}(o, m_{:\to i})=\hat{\pi}(o, m_{:\to i}^\prime))\\
% \geq& \mathbb{P}(\hat{\pi}(o, m_{:\to i})=\hat{\pi}(o, m_{:\to i}^\prime), \mathcal{T} \wedge K = \emptyset )\\
% =& \mathbb{P}(\hat{\pi}(o, m_{:\to i})=\hat{\pi}(o, m_{:\to i}^\prime)|\mathcal{T} \wedge K = \emptyset) \mathbb{P}(\mathcal{T} \wedge K = \emptyset)\\
% =& \mathbb{P}(\mathcal{T} \wedge K = \emptyset) 
% % \;\; (\text{Because}\; \hat{\pi}(o, m)=\hat{\pi}(o, m^\prime) \;\text{if}\;  \mathcal{T} \wedge K = \emptyset) 
% \\
% =& \frac{\binom{N-C}{k}}{\binom{N}{k}}
% \end{align}
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:reward_dist}]

Based on the definition of benign action set, $\smpolicy$ selects an action $\widetilde{a}$ if and only if there exists an index set $T$ such that the benign message combination $\funabl(\mathbf{m},T)$ makes the ablation policy $\ablpolicy$ select $\widetilde{a}$. Therefore, for any trajectory generated by $\smpolicy$ under attacks, there is a trajectory of $\ablpolicy$ with a list of indices sets $T_1,T_2,\cdots$ that renders the same cumulative reward under no attack.

\end{proof}


\subsection{Proofs in Continuous Action Space}

\begin{proof}[Proof of Theorem~\ref{thm:main_cont} and Theorem~\ref{thm:sample_cont}]
To understand the intuition of element-wise median operation in continuous action space, let us first start with an intuitive example: consider 5 arbitrary numbers $x_1$,...,$x_5$, if we already know 3 of them $x_1$,$x_2$,$x_3$, then it is certain that Min($x_1$,$x_2$,$x_3$)$\leq$Median($x_1$,...,$x_5$)$\leq$Max($x_1$,$x_2$,$x_3$). Applying this element-wise, when safe message combinations form the majority, the median action falls into the range of actions produced by safe messages. 

Concretely, in continuous action space,  $\tilde{a}\in \safeactioncont$ is equivalent to the condition that out of the $D$ sampled message combinations, safe message combinations make up the majority. There are $\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n1-n2}{D-j}$ such possibilities in terms of the sampling of $D$, where $\tilde{D}={\lfloor \frac{D}{2} \rfloor}+1$. Once again the total number of possibilities is $\binom{n_1}{D}$. Therefore, we get Equation \eqref{eq:p_sample_cont}.

The proof of Theorem~\ref{thm:main_cont} follows as a special case of Theorem~\ref{thm:sample_cont} when $D=\binom{N-1}{k}=n_1$. Same as above, in this case, the only non-zero term left in the numerator of $p_D$ is $\binom{n_2}{j}\binom{n_1-n_2}{n_1-j}=\binom{n_2}{n_2}\binom{n_1-n_2}{n_1-n_2}=1$ ($j=n_2$), so $p_D=1$.
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:reward_cont}]

Similar to the proof of Corollary~\ref{cor:reward_dist}, at any state $s$, the action $\widetilde{a}$ generated by $\smpolicy$ is always bounded by actions generated from $\ablpolicy$ with some indices set. Due to Assumption~\ref{assump:order}, there exists $a^\prime\sim\ablpolicy$ such that $R(s,a^\prime) \leq R(s,\widetilde{a})$. Therefore, the cumulative reward of $\smpolicy$ is lower bounded by the minimal cumulative reward of $\ablpolicy$ among all indices set lists.

\end{proof}

==> a2_theory.tex <==
\section{Additional Theoretical Definitions and Analysis}
\label{app:theory}

\textbf{Relation between Communication Attack and $\boldsymbol \ell_0$ Observation Attack}\quad
The communication threat model described in Section~\ref{sec:setup_adv} is analogous to a constrained $\ell_0$ attack on policy inputs. When agent $i$ is attacked, the input space of its acting policy $\pi_i$ is $\tilde{\mathcal{O}}_i := \mathcal{O}_i \times \mathcal{M}^{N-1}$. Therefore, when $C$ communication messages are corrupted, the original observation $\tilde{o}_i$ gets perturbed to $\tilde{o}_i^\prime$. Let $d$ be the dimension of a communication message, then $\tilde{o}_i$ and $\tilde{o}_i^\prime$ differ by up to $dC$ dimensions, which is similar to an $\ell_0$ attack constrained in certain dimensions. 



\subsection{Additional Analysis of \ours in Discrete Action Space}
\label{app:theory_dist}

Theorem~\ref{thm:main_dist} justifies that under sufficient majority votes $u_{\tilde{a}}$, the ensemble policy $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a safe action that is suggested by some benign message combinations even when the malicious messages are not identified.
Therefore, with ensemble policy $\smpolicy$, the agent's cumulative reward under adversarial communications would be similar to the natural reward of $\ablpolicy$ under no attacks, as justified in the following corollary.
% The corollary below shows the relationship between the attacked reward of $\smpolicy$ and the natural reward of $\ablpolicy$. Note that $\ablpolicy$ is the policy learned during training time in a clean (non-adversarial) environment, and it is easy for us to evaluate its natural cumulative reward. $\smpolicy$ is 
% \fh{I feel the current description doesn't make it easy to  distinguish between $\ablpolicy$ and $\smpolicy$.}

\begin{corollary}[Reward Certificate for Discrete Action Space]
\label{cor:reward_dist}
With ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} under adversarial communication satisfying Assumption~\ref{assum:num} is no lower than the lowest cumulative reward that the ablation policy $\ablpolicy$ can obtain with randomly selected message subsets under no attacks, i.e.,
\begin{equation}
\begin{aligned}
    \advobj(\smpolicy) \geq \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
\end{aligned}
\end{equation}
where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under attacks, and $\natobj(\ablpolicy|T_1,T_2,\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ whose message is ablated by index set $T_t$ at step $t>0$.
\end{corollary}

% \begin{corollary}[Reward Certificate for Discrete Action Space]
% \label{cor:reward_dist}
% \fh{Under sample size $D=\binom{N-1}{k}$, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with a message subset size $k$ satisfying Equation~\eqref{eq:k_cond} obtains a total reward no worse than that obtained by the base ablation policy $\ablpolicy$ using benign messages:
% \begin{align}
%   & \advobj\Big(\smpolicy\big(o, \{\funabl(\advmsg, T_d)\}_{d=1}^D\big)\Big) \geq \nonumber \\
%   & \min_{T} \natobj\Big(\ablpolicy\big(o, \funabl(\goodmsg, T)\big)\Big) \label{eq:reward_dist}
% \end{align}
% if the majority votes $u_{\tilde{a}}$ satisfies $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step.
% }
% \textcolor{red}{Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If $D=\binom{N-1}{k}$, and the majority votes satisfy 
% $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step, 
% then the total reward of $\smpolicy$ satisfies
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:reward_dist}
%     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy),
% \end{equation}}
% Here $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the \textcolor{red}{sampled message indices}\fh{indices of the message subsets?} used by $\ablpolicy$ at all steps. \fh{What does this mean? My equation doesn't use $\tau$, rather I use $T$.}
% \end{corollary}
Note that $\min_{\tau} \natobj(\ablpolicy)$ can be estimated by executing $\ablpolicy$ during training time, so that the test-time performance of $\smpolicy$ is guaranteed to be no lower than this value, even if there are up to $C$ corrupted messages at every step.




\subsection{Additional Analysis of \ours in Continuous Action Space}
\label{app:theory_cont}

% \begin{definition}[Q Value of Ablation Policy $\ablpolicy$]
% \label{def:q_abl}
% Suppose that agent $i$ is executing policy $\ablpolicy$, and all other agents are also executing fixed policies denoted as $\pi_{-i}$. Then, the action value of $\ablpolicy$ can be defined as below.
% \begin{equation}
% \label{eq:q_abl}
%     \hat{Q}^{\ablpolicy}(s,a):=\mathbb{E}_{\krv\step \sim \mathcal{U}(N-1,k), P, \pi_{-i}}[\sum_{t=0}^\infty \gamma^t r\step | s_0=s, a_0=a, a_t\sim\ablpolicy(o\step, \funabl(\mtoi\step, \krv\step))],
% \end{equation}
% where $r\step$ is the reward obtained by $i$ at step $t$.
% \end{definition}


Theorem~\ref{thm:main_cont} shows how the ensemble policy outputs an action bounded by safe actions. However, to obtain a reward certificate, an extra assumption about the reward structure is needed.
% Now we further discuss how it can lead to a reward certificate.
% Let $\preccurlyeq$ define the element-wise less than or equal to relation between two vectors.
% The following assumption is essential for obtaining a reward certificate, which suggests that a coordinate-wisely bounded action also has lower bounded reward.
\begin{assumption}
\label{assump:order}
Let $R: \mathcal{S} \times \mathcal{A} \to \mathbb{R}$ be the reward function of the current agent. For any state $s\in\mathcal{S}$, assume $R(s,a) \geq \min_{\hat{a}\in\mathsf{\safeaction}} R(s,\hat{a})$.
\end{assumption}
% \begin{assumption}[Ordered Action]
% \label{assump:order}
% For any state $s\in\mathcal{S}$, and any actions 
% $a_1\preccurlyeq a_2 \preccurlyeq a_3$, we have either $R(s,a_2) \geq R(s,a_1)$, or $R(s,a_2) \geq R(s,a_3)$, where $R$ is the reward function for the current agent.
% \end{assumption}

Assumption~\ref{assump:order} suggests that there is no ``caveat'' in the safe action set. 
This assumption is mild and practical in many real-life scenarios where actions have concrete meanings (e.g. price, speed, etc). For example, if driving at 40 mph and driving at 50 mph are both safe, then driving at 45 mph is also safe. 
Note that without the assumption of reward structure, there may exist extreme cases where some actions in $\safeaction$ could lead to low reward, which makes the reward not certifiable. In practice, we can usually expect this assumption to hold when the safe action range generated by the ablation policy is relatively narrow, i.e., the benign communication messages achieve agreements.

With Assumption~\ref{assump:order}, the following reward certificate holds.

\begin{corollary}[Reward Certificate for Continuous Action Space]
\label{cor:reward_cont}
Under Assumption~\ref{assump:order}, with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} under adversarial communication satisfying Assumption~\ref{assum:num} is no lower than the lowest cumulative reward the ablation policy $\ablpolicy$ can obtain with randomly selected message subsets under no attacks, i.e.,
\begin{equation}
\begin{aligned}
    \advobj(\smpolicy) \geq \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
\end{aligned}
\end{equation}
where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under attacks, and $\natobj(\ablpolicy|T_1,T_2,\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ whose message is ablated by indices set $T_t$ at step $t>0$.
\end{corollary}


% \begin{corollary}[Reward Certificate for Continuous Action Space]
% \label{cor:reward_cont}
% Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If Assumption~\ref{assump:order} holds, and $D=\binom{N-1}{k}$, 
% then the total reward of $\smpolicy$ satisfies
% \begin{equation}
% \label{eq:reward_cont}
%     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy)
% \end{equation}
% where $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the sampled message indices used by $\ablpolicy$ at all steps.
% \end{corollary}



\subsection{Additional Definitions for \ours with Partial Samples}
\label{app:theory_sample}

% The $D$-ensemble policy $\pi_D$ is defined as
% \begin{equation}
% \label{eq:ensemble_pi_dist_d}
%     \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
% \end{equation}
% for a discrete action space, and
% \begin{equation}
% \label{eq:ensemble_pi_cont_d}
%     \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% for a continuous action space. 

The following theorem shows a general guarantee for $D$-ensemble policy in a discrete action space.

\begin{theorem}[General Action Guarantee for Discrete Action Space]
\label{thm:sample_dist}
Let $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$. 
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$, under Assumption~\ref{assum:num}, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_dist_d} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, relation~\eqref{eq:cert_dist} holds deterministically if $u_{\tilde{a}}>n_1-n_2$. Otherwise it holds with probability at least
%\vspace{-0.1cm}
\begin{equation}
\label{eq:p_sample_dist}
    p_D=\frac{\sum_{j=0}^{u_{\tilde{a}}-1}\binom{n_1-n_2}{j}\binom{n_2}{D-j}}{\binom{n_1}{D}}.
\end{equation}
\end{theorem}

==> a3_exp.tex <==
\section{Additional Experiment Settings and Results in FoodCollector Environment}
\label{app:exp}

\subsection{Description of FoodCollector Environment}
\label{app:exp_env}

The FoodCollector environment is a 2D particle world shown by Figure~\ref{fig:food}(left). There are $N=9$ agents with different colors, and $N$ foods with colors corresponding to the $N$ agents. Agents are rewarded when eating foods with the same color. A big round obstacle is located in the center of the map, which the agent cannot go through. There are some poisons (shown as black dots) in the environment, and the agents get penalized whenever they touch the poison. Each agent has 6 sensors that detect the objects around it, including the poisons and the colored foods. 
The game is episodic, with horizon set to be 200. In the beginning of each episode, the agents, foods and poisons are randomly generated in the world. 
At every step, each agent will receives a negative reward $-0.5$ if it has not eaten all its food. Therefore, every agent should explore the environment and eat all food as fast as possible.
% Every time an agent eats a food, the food disappears, and the world re-generate a food with the same color in a random position. Therefore, an agent is supposed to explore the world and to eat as many foods as possible within limited number of steps.

Each of the 6 sensors can detect the following values when the corresponding element is within the sensor's range:\\
(1) (if detects a food) the distance to a food (real-valued); \\
(2) (if detects a food) the color of the food (one-hot); \\
(3) (if detects an obstacle) the distance to the obstacle (real-valued); \\
(4) (if detects the boundary) the distance to the boundary (real-valued); \\ (5) (if detects another agent) the distance to another agent (real-valued).\\
The observation of an agent includes an agent-identifier (one-hot encoding), its own location (2D coordinates), its own velocity, two flags of colliding with its food and colliding with poison, and the above sensory inputs. So, the observation space is a ($7N+30$)-dimensional vector space. 

The action space can be either \textit{discrete} or \textit{continuous}. For the discrete version, there are 9 actions including 8 moving directions (north, northwest, west, southwest, south, southeast, east, northeast) and 1 no-move action. For the continuous version, the action is an acceleration decision, denoted by a 2-dimensional real-valued vector, with each coordinate taking values in $[-0.01,0.01]$. 

\begin{figure}[h]
% \vspace{-1em}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/foodcollector.png}
    % \vspace{-0.5em}
    % \caption{The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. }
    % \label{fig:food}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{figs/comm_dist}
        % \vspace{-0.1cm}
        \caption{Discrete action space}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{figs/comm_cont}
        % \vspace{-0.1cm}
        \caption{Continuous action space}
    \end{subfigure}
% \vspace{-0.5em}
\caption{Reward of agents trained with communication v.s. without communication. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.}
\label{fig:food_comm}
% \vspace{-0.4cm}
\end{figure}

Due to the limited sensory range, every agent can only see the objects around it and thus only partially observe the world. Therefore, communication among agents can help them find their foods much faster. Since our focus is to defend against adversarially perturbed communications, we first define a valid and beneficial communication protocol, where an agent sends a message to a receiver once it observes a food with the receiver's color. For example, if a red agent encounters a blue food, it can then send a message to the blue agent so that the blue agent knows where to find its food. 
% The communication follows the protocol below. Once agent $i$ detects the location of some food or poison from its sensors, it will update the communication channel to every other agent with the latest sensor observation containing its position and its sensory data, which contains the relative location of the food and/or poison. 
To remember the up-to-date communication, every agent maintains a list of most recent $N-1$ messages sent from other $N-1$ agents.
A message contains the sender's current location and the relative distance to the food (recorded by the 6 sensors). Therefore, a message is a $8$-dimensional vector, and each agent's communication list has $8(N-1)$ dimensions in total.

During training with communication, we concatenate the observation and the communication list of the agent to an MLP-based policy, compared to the non-communicative case where the policy only takes in local observations.
As verified in Figure~\ref{fig:food_comm}, communication does help the agent to obtain a much higher reward in both discrete action and continuous action cases, which suggests that the agents tend to rely heavily on the communication messages for finding their food. 
% \fh{Since we will consider the communication protocol as part of the environment, shall we describe the protocol concretely here in this foodcollector experiment?}




\subsection{Implementation Details}
\label{app:exp_imple}

\textbf{Implementation of Trainer}\quad
In our experiments, we use the Proximal Policy Optimization (PPO) \cite{schulman2017proximal}  algorithm to train all  agents as well as the  attackers. Specifically, we adapt from the elegant OpenAI Spinning Up \cite{SpinningUp2018} Implementation for PPO training algorithm. On top of the Spinning Up PPO implementation, we also keep track of the running average and standard deviation of the observation and normalize the observation.

For the policy network, we use a multi-layer perceptron (MLP) with two hidden layers of size 64. Because the action space of our environment is bounded between -0.01 and 0.01, we parameterize the policy as a Beta distribution, which has been proposed in previous works to better solve reinforcement learning problems with bounded actions  \cite{pmlr-v70-chou17a}. In particular, we parameterize the shape parameteres of the Beta distribution as $\alpha=\log(1+e^{\alpha_{\theta}(s)})+1$ and $\beta=\log(1+e^{\beta_{\theta}(s)})+1$ (1 is added to make sure that $\alpha, \beta\geq 1$). $\pi(a|s)=f(\frac{a-h}{2h};\alpha, \beta)$, where $h=0.01$, and $f(x;\alpha, \beta)=\frac{\Gamma(\alpha+\beta)}{\Gamma(\alpha)\Gamma(\beta)}x^{\alpha-1}(1-x)^{\beta-1}$ is the density function of the Beta Distribution.
For the value network, we also use an MLP with two hidden layers of size 64. 

In terms of other hyperparameters used in the experiments, we use a learning rate of 0.0003 for the policy network, and a learning rate of 0.001 is used for the value network. We use the Adam optimizer with $\beta_1=0.99$ and  $\beta_2 = 0.999$. For every training epoch, the PPO agent interacts with the environment for 4000 steps, and it is trained for 500 epochs in our experiments.

% \textcolor{purple}{PH: before describing the  type of attackers, should we mention what an attacker is training. For example, we say below that " The action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1." Perhaps we can state it here to make it more clear the attacker is learning a communication policy and not taking over the actions of agents?}


\textbf{Attacker}\quad
An attacker maps its own observation to the malicious communication messages that it will send to the victim agent. Thus, the action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1. 
\vspace{-0.5cm}
\begin{itemize}
\item \emph{Non-adaptive Attacker}\quad
We implement a fast and naive attacking method for the adversary. At every dimension, the naive attacker randomly picks 1 or -1 as its action, and then sends the perturbed message which consists entirely of 1 or -1 to the victim agent. 
\vspace{-0.2cm}
\item \emph{Adaptive RL Attacker}\quad
We use the PPO algorithm to train the attacker, where we set the reward of the attacker to be the negative reward of the victim. The attacker uses a Gaussian policy, where the action is clipped to be in the valid communication range. The network architecture and all other hyperparameter settings follow the exact same from the clean agent training.
\end{itemize}
\vspace{-0.2cm}

\textbf{Implementation of Baselines}\quad
\vspace{-0.2cm}
\begin{itemize}
\item \emph{Vanilla Learning}\quad
For Vanilla method, we train a shared policy network to map observations and communication to actions. Note that the messages are symmetric (of the same format), we shuffle the messages before feeding them into the policy network, to reduce the bias caused by agent order. We find that shuffling the messages helps the agent converge much faster (50\% fewer total steps).
\vspace{-0.2cm}
\item \emph{Adversarial Training (AT)}\quad
For adversarial training, we alternate between the training of attacker and the training of the victim agent. Both the victim and attackers are trained by PPO. For every 200 training epochs, we switch the training, where we either fix the trained victim and train the attacker for the victim or fix the trained attacker and train the victim under attack. We continue this process for 10 iterations. Similar to Vanilla, the victim also shuffles the communication messages to obtain higher reward and converge faster.
\end{itemize}
\vspace{-0.2cm}


\emph{Adversarial Training does not improve agent's robust performance.}
As we observed in Figure \ref{fig:res_all}, adversarial training does not improve the robustness of the agent in both discrete and continuous action space, although AT achieves good robustness against observation attacks in a single-agent environment~\cite{zhang2021robust}. 
We hypothesize that it is due to (1) the large number of total agents, and (2) the uncertainty of adversarial message channels. 
To be more specific, during the training of AT, we alternately train the agent and the attacker, and the attacker can change the channels it controls among iterations. As a result, the agent might not be able to distinguish adversarial messages and benign messages. 
% We hypothesize that it is due to the communication shuffling of the agent. In fact, this is also similar to another practical scenario where at different time steps, the attacker might hijack different agents. As a consequence, in both scenarios, malicious messages could randomly appear in any part of the agent's input vector. 
Therefore, simply training the agent and attacker together cannot make the agent learn how to detect the malicious messages and ignore them. 


\subsection{Additional Experiment Results}
\label{app:exp_res}

In addition to Figure \ref{fig:res_k_dist}, we also provide the plot for Hyper-parameter test in continuous-action FoodCollector in Figure \ref{fig:res_k_cont}. 
\input{fig_food_k_cont}






==> a6_market.tex <==
\section{Additional Experiment Settings and Results in Market Environment}
\label{app:market}

% \textcolor{red}{we need to mention in the main text that we have additional experiments on MarketEnv in the Appendix} 

\subsection{Description of Market Environment}
\label{app:market_env}
The \textit{MarketEnv} environment is an inventory management setup, where $N=10$ heterogeneous seller agents carry inventory for $M=3$ products. A population of $B=300$ buyers request a product from a randomly selected seller agent according to a demand distribution $\mathbf{p}=[p_1,\dots,p_M]$. We denote the demand realization for seller $i$ with $\mathbf{d_i}=[d_{i,1},\dots,d_{i,M}]$. Sellers manage their inventory by restocking products through interacting with the buyers. The game is episodic with horizon set to $50$. At the beginning of each episode, a realization of the demand distribution $\mathbf{p}$ is randomly generated and the agents' inventory for each product is randomly initialized from $[0, \frac{B}{N}]$, where $\frac{B}{N}$ is the expected number of buyers per seller. %\ys{describe the initial inventory in every episode?} 
Sellers are penalized for mismatch between their inventory and the demand for a product, and they aim to restock enough units of a product at each step to prevent insufficient inventory without accruing a surplus at the end of each step.  %\ys{defining the reward function by math?}
\begin{itemize}
    \item State observation: A seller agent's observation includes its inventory for each product, and the products that were requested by buyers during the previous step. The observation space is a $2M$-dimensional vector.
    
    \item Agent action: Sellers manage their inventory by restocking new units of each product or discarding part of the leftover inventory at the beginning of each step. Hence, agents take both positive and negative actions denoted by an $M$-dimensional vector, and the action space can be either discrete or continuous. In our experiments, we use continuous actions assuming that products are divisible and sellers can restock and hold fractions of a product unit.
    
    \item Agent reward function: During each step, agent $i$'s reward is defined as $r_i = - || \max( \mathbf{I}_i+\mathbf{a}_i, 0) - \mathbf{d}_i||_2$, where $\mathbf{I}_i$ denotes the agents initial inventory vector, and $\mathbf{a}_i$ denotes the inventory restock vector from action policy $\pi_i$.  
    
    
    \item Agent communication: Sellers learn the demand distribution and optimize their inventory by interacting with their own customers (i.e., portion of buyers that request a product from that seller). Sellers would benefit from sharing their observed demands with each other, so that they could estimate the demand distribution more accurately for managing inventory. At the end of each step, a seller communicates an $M$-dimensional vector reporting its observed demands to all other agents. In the case of adversarial communications, this message may differ from the agents' truly observed demands.
    
    During training with communication, messages received from all other agents are concatenated to the agent's observation, which is used to train an MLP-based policy, compared to the non-communicative case where the policy is trained using only local observations. As observed from Figure \ref{fig:marketenv_comm}, communication helps agents obtain  higher rewards since they are able to manage their inventory based on the overall demands observed across the population of buyers rather than their local observation. Results are reported by averaging rewards corresponding to $5$ experiments run with different training seeds.
\end{itemize}
 
\begin{figure}[h]
\vspace{-0.1cm}
 \centering
\resizebox{.4\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_comm_dist}}
\vspace{-0.1cm}
\caption{\textbf{MarketEnv}: Reward of agents trained with communication v.s. without communication. %Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.
} 
\label{fig:marketenv_comm}
\end{figure}
 
 



\subsection{Implementation Details}
\label{app:market_imple}
\textbf{Implementation of Trainer}\quad 
As in the FoodCollector experiments, we use the PPO algorithm to train all agent action policy as well as adversarial agent communication policies. We use the same MLP-based policy and value networks as the FoodCollector but parameterize the policy as a Gaussian distribution. The PPO agent interacts with the environment for $50$ steps, and it is trained for $10000$ episodes. The learning rate is set to be 0.0003 for the policy network, and 0.001 for the value network.
% All other hyper-parameters are set similar to the FoodCollector experiments.


\textbf{Attacker}\quad 
The attacker uses its observations to communicate malicious messages to  victim sellers, and its action space is the communication space of a benign agent.  We consider the following non-adaptive and adaptive attackers:
\begin{itemize}
    \item \textit{Non-adaptive Attacker}: The attacker's goal is to harm the victim agent by misreporting its observed demands so that the victim seller under-estimates or over-estimates the restocking of products. In our experiments, we evaluate the effectiveness of defense strategies against the following attack strategies:
    \begin{itemize}
     \item{\permute}: The communication message is a random permutation of the true demand vector observed by the attacker.
    \item {\swap}: In order to construct a communication vector as different as possible from its observed demand, the attacker reports the most requested products as the least request ones and vice versa. Therefore, the highest demand among the products is interchanged with the lowest demand, the second highest demand is interchanged with the second lowest demand and so forth.
    \item{\flip:} Adversary $i$ modifies its observed demand $\mathbf{d}_i$ by mirroring it with respect to $\eta=\frac{1}{M}\sum_{j=1}^M d_{ij}$, such that products demanded less than $\eta$ are reported as being requested more, and conversely, highly demanded products are reported as less popular.
    \end{itemize}
   
    
    \item \textit{Adaptive Attacker}: The attacker communication policy is trained using the PPO algorithm, and its reward is set as the negative reward of the victim agent. The attacker uses a Gaussian policy with a softmax activation in the output layer to learn a adversarial probability distribution across products, which is then scaled by the total observed demands $\sum_{j=1}^M d_{ij}$ to construct the communication message.

\end{itemize} 


 

\textbf{Implementation of Baselines}\quad 
\begin{itemize}
    \item \textit{Vanilla Learning}: In the vanilla training method with no defense mechanism against adversarial  communication, we train a shared policy network using agents' local observations and their received communication messages.
     \item \textit{Adversarial Training (AT)}: We alternate between training the agent action policy and the victim communication policy, both using PPO. For the first iteration we train the policies for $10000$ episodes, and then use $1000$ episodes for $5$ additional training alteration iterations for both the action policy and the adversarial communication policy. For more efficient adversarial training, we first shuffle the received communication messages before feeding them into the policy network. Consequently, the trained policy  treats communications received from different agents in a similar manner, and we are able to only train the policy with a fixed set of adversarial agents rather than training the network on all possible combinations of adversarial agents. We do not shuffle the  communication messages being input to the policy trained with vanilla learning as we did not observe improved convergence, as in the FoodCollector environment. %\ys{maybe mention the communication permuting here? and explain why permutation is not used for vanilla (performance no better than vanilla). }

\end{itemize}


 


\subsection{Experiment Results in Market Environment}
\label{app:market_res}

\paragraph{Robust performance Under Attacks} \quad
In this section, we evaluate robustness of the proposed \ours defense strategy in MarketEnv and compare it against Vanilla Learning and Adversarial Training. Figure~\ref{fig:res_all_market} shows the natural and robust performance of \ours with $k=2$, which provides performance guarantees against up to $C=2$ adversarial messages. The performance is compared with AT when the agents policy is alternatively trained against $2$ adversaries. We observe that there is a considerable reduction in the Vanilla and AT rewards under attacks, especially for the strong adaptive attack and \swap. Similar to the FoodCollector, adversarial training is not robust to adversarial communications in the MarketEnv such that for two or more adversarial messages the performance is close to or much lower than the reward achieved with no communications. However, as expected for $k=2$, \ours is able to achieve rewards comparable to the no-attack case  under $C=1$ and $C=2$ adversaries even for strong adversarial attacks. Moreover, \ours outperforms the baselines for $C=3$ for which the theoretical guarantees no longer hold. Even though the gap between natural and robust performance under the weak \permute is less for all three strategies, \ours achieves the highest reward. In  MarketEnv, \ours is able to preserve the communication gains arising from informative messages shared among the agents while being robust against adversarial communications.

  
 
\input{fig_market_res}

\paragraph{Hyper-parameter Test of Ablation Size $\boldsymbol k$} 
Figure~\ref{fig:res_k_cont_market}(left)  shows how the agent's natural performance and robustness varies with the ablation size $k$. We compare \ours’s natural reward and \ours’s reward under $C=2$ adversarial communication messages for adaptive and non-adaptive attacks  with different values of $k$. Similar to the FoodCollector, As the ablation size $k$ increase, the agent is able to improve its natural performance by utilizing information communicated by more agents. However, the agent becomes more vulnerable to adversarial communications which can impacts its decision-making for managing its inventory. Therefore, ablation size $k$ trades off robustness for natural performance. Additionally, we observe that the non-adaptive \swap which constructs the  adversarial communications strategically to mislead the victim agent is quite effective in reducing the victims reward compared to the \permute which communicates adversarial messages without tactically modifying the adversary's observed demands.
 
\paragraph{Hyper-parameter Test of Sample Size $\boldsymbol D$}
In Figure~\ref{fig:res_k_cont_market}(right), we evaluate the robustness of the partial-sample variant of \ours presented in Section~\ref{sec:algo_partial} against $C=2$  adversaries for ablation size $k=2$, when $D$  varies from $36$ (the largest sample size) to $1$ (the smallest sample size). It is shown that with lower $D$, \ours achieves lower rewards under adversarial communications, but is considerably more robust compared to the baseline method. When the agent makes decisions based on a single random message with $D=1$, the agent's average robust reward is higher than the Vanilla reward.

\input{fig_market_k_dist} 



 

==> a7_exp_arxiv.tex <==


\section{Additional Implementation Details and Results in FoodCollector}
\label{app:exp}

\subsection{Description of FoodCollector Environment}
\label{app:exp_env}

The FoodCollector environment is a 2D particle world shown by Figure~\ref{fig:food}(left). There are $N=9$ agents with different colors, and $N$ foods with colors corresponding to the $N$ agents. Agents are rewarded when eating foods with the same color. A big round obstacle is located in the center of the map, which the agent cannot go through. There are some poisons (shown as black dots) in the environment, and the agents get penalized whenever they touch the poison. Each agent has 6 sensors that detect the objects around it, including the poisons and the colored foods. 
The game is episodic, with horizon set to be 200. In the beginning of each episode, the agents, foods and poisons are randomly generated in the world. 
At every step, each agent will receives a negative reward $-0.5$ if it has not eaten all its food. Therefore, every agent should explore the environment and eat all food as fast as possible.
% Every time an agent eats a food, the food disappears, and the world re-generate a food with the same color in a random position. Therefore, an agent is supposed to explore the world and to eat as many foods as possible within limited number of steps.

Each of the 6 sensors can detect the following values when the corresponding element is within the sensor's range:\\
(1) (if detects a food) the distance to a food (real-valued); \\
(2) (if detects a food) the color of the food (one-hot); \\
(3) (if detects an obstacle) the distance to the obstacle (real-valued); \\
(4) (if detects the boundary) the distance to the boundary (real-valued); \\ (5) (if detects another agent) the distance to another agent (real-valued).\\
The observation of an agent includes an agent-identifier (one-hot encoding), its own location (2D coordinates), its own velocity, two flags of colliding with its food and colliding with poison, and the above sensory inputs. So, the observation space is a ($7N+30$)-dimensional vector space. 

The action space can be either \textit{discrete} or \textit{continuous}. For the discrete version, there are 9 actions including 8 moving directions (north, northwest, west, southwest, south, southeast, east, northeast) and 1 no-move action. For the continuous version, the action is an acceleration decision, denoted by a 2-dimensional real-valued vector, with each coordinate taking values in $[-0.01,0.01]$. 

% \begin{figure}[h]
% % \vspace{-1em}
%     \centering
%     % \includegraphics[width=0.5\columnwidth]{figs/foodcollector.png}
%     % \vspace{-0.5em}
%     % \caption{The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. }
%     % \label{fig:food}
%     \centering
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \input{figs/comm_dist}
%         % \vspace{-0.1cm}
%         \caption{Discrete action space}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \input{figs/comm_cont}
%         % \vspace{-0.1cm}
%         \caption{Continuous action space}
%     \end{subfigure}
% % \vspace{-0.5em}
% \caption{Reward of agents trained with communication v.s. without communication. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.}
% \label{fig:food_comm}
% % \vspace{-0.4cm}
% \end{figure}

Due to the limited sensory range, every agent can only see the objects around it and thus only partially observe the world. Therefore, communication among agents can help them find their foods much faster. Since our focus is to defend against adversarially perturbed communications, we first define a valid and beneficial communication protocol, where an agent sends a message to a receiver once it observes a food with the receiver's color. For example, if a red agent encounters a blue food, it can then send a message to the blue agent so that the blue agent knows where to find its food. 
% The communication follows the protocol below. Once agent $i$ detects the location of some food or poison from its sensors, it will update the communication channel to every other agent with the latest sensor observation containing its position and its sensory data, which contains the relative location of the food and/or poison. 
To remember the up-to-date communication, every agent maintains a list of most recent $N-1$ messages sent from other $N-1$ agents.
A message contains the sender's current location and the relative distance to the food (recorded by the 6 sensors). Therefore, a message is a $8$-dimensional vector, and each agent's communication list has $8(N-1)$ dimensions in total.

During training with communication, we concatenate the observation and the communication list of the agent to an MLP-based policy, compared to the non-communicative case where the policy only takes in local observations.
As verified in Figure~\ref{fig:food}, communication does help the agent to obtain a much higher reward in both discrete action and continuous action cases, which suggests that the agents tend to rely heavily on the communication messages for finding their food. 
% \fh{Since we will consider the communication protocol as part of the environment, shall we describe the protocol concretely here in this foodcollector experiment?}




\subsection{Implementation Details}
\label{app:exp_imple}

\textbf{Implementation of Trainer}\quad
In our experiments, we use the Proximal Policy Optimization (PPO) \cite{schulman2017proximal}  algorithm to train all  agents as well as the  attackers. Specifically, we adapt from the elegant OpenAI Spinning Up \cite{SpinningUp2018} Implementation for PPO training algorithm. On top of the Spinning Up PPO implementation, we also keep track of the running average and standard deviation of the observation and normalize the observation.

For the policy network, we use a multi-layer perceptron (MLP) with two hidden layers of size 64. Because the action space of our environment is bounded between -0.01 and 0.01, we parameterize the policy as a Beta distribution, which has been proposed in previous works to better solve reinforcement learning problems with bounded actions  \cite{pmlr-v70-chou17a}. In particular, we parameterize the shape parameteres of the Beta distribution as $\alpha=\log(1+e^{\alpha_{\theta}(s)})+1$ and $\beta=\log(1+e^{\beta_{\theta}(s)})+1$ (1 is added to make sure that $\alpha, \beta\geq 1$). $\pi(a|s)=f(\frac{a-h}{2h};\alpha, \beta)$, where $h=0.01$, and $f(x;\alpha, \beta)=\frac{\Gamma(\alpha+\beta)}{\Gamma(\alpha)\Gamma(\beta)}x^{\alpha-1}(1-x)^{\beta-1}$ is the density function of the Beta Distribution.
For the value network, we also use an MLP with two hidden layers of size 64. 

In terms of other hyperparameters used in the experiments, we use a learning rate of 0.0003 for the policy network, and a learning rate of 0.001 is used for the value network. We use the Adam optimizer with $\beta_1=0.99$ and  $\beta_2 = 0.999$. For every training epoch, the PPO agent interacts with the environment for 4000 steps, and it is trained for 500 epochs in our experiments.

% \textcolor{purple}{PH: before describing the  type of attackers, should we mention what an attacker is training. For example, we say below that " The action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1." Perhaps we can state it here to make it more clear the attacker is learning a communication policy and not taking over the actions of agents?}


\textbf{Attacker}\quad
An attacker maps its own observation to the malicious communication messages that it will send to the victim agent. Thus, the action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1. 
% \vspace{-0.2cm}
\begin{itemize}
\item \emph{Non-adaptive Attacker}\quad
We implement a fast and naive attacking method for the adversary. At every dimension, the naive attacker randomly picks 1 or -1 as its action, and then sends the perturbed message which consists entirely of 1 or -1 to the victim agent. 
% \vspace{-0.2cm}
\item \emph{Adaptive RL Attacker}\quad
We use the PPO algorithm to train the attacker, where we set the reward of the attacker to be the negative reward of the victim. The attacker uses a Gaussian policy, where the action is clipped to be in the valid communication range. The network architecture and all other hyperparameter settings follow the exact same from the clean agent training.
\end{itemize}
\vspace{-0.2cm}

\textbf{Implementation of Baselines}\quad
% \vspace{-0.2cm}
\begin{itemize}
\item \emph{Vanilla Learning}\quad
For Vanilla method, we train a shared policy network to map observations and communication to actions. Note that the messages are symmetric (of the same format), we shuffle the messages before feeding them into the policy network, to reduce the bias caused by agent order. We find that shuffling the messages helps the agent converge much faster (50\% fewer total steps).
% \vspace{-0.2cm}
\item \emph{Adversarial Training (AT)}\quad
For adversarial training, we alternate between the training of attacker and the training of the victim agent. Both the victim and attackers are trained by PPO. For every 200 training epochs, we switch the training, where we either fix the trained victim and train the attacker for the victim or fix the trained attacker and train the victim under attack. We continue this process for 10 iterations. Similar to Vanilla, the victim also shuffles the communication messages to obtain higher reward and converge faster.
\end{itemize}
\vspace{-0.2cm}


\emph{Adversarial Training does not improve agent's robust performance.}
As we observed in Figure \ref{fig:res_all}, adversarial training does not improve the robustness of the agent in both discrete and continuous action space, although AT achieves good robustness against observation attacks in a single-agent environment~\cite{zhang2021robust}. 
We hypothesize that it is due to (1) the large number of total agents, and (2) the uncertainty of adversarial message channels. 
To be more specific, during the training of AT, we alternately train the agent and the attacker, and the attacker can change the channels it controls among iterations. As a result, the agent might not be able to distinguish adversarial messages and benign messages. 
% We hypothesize that it is due to the communication shuffling of the agent. In fact, this is also similar to another practical scenario where at different time steps, the attacker might hijack different agents. As a consequence, in both scenarios, malicious messages could randomly appear in any part of the agent's input vector. 
Therefore, simply training the agent and attacker together cannot make the agent learn how to detect the malicious messages and ignore them. 


\subsection{Additional Experiment Results}
\label{app:exp_res}

In addition to Figure \ref{fig:res_hyper}, we also provide the plot for Hyper-parameter test in discrete-action FoodCollector in Figure \ref{fig:res_k_dist}. 
\input{fig_food_k_dist}




\section{Additional Implementation Details and Results in MarketEnv}
\label{app:market}

% \textcolor{red}{we need to mention in the main text that we have additional experiments on MarketEnv in the Appendix} 

\subsection{Description of Market Environment}
\label{app:market_env}
The \textit{MarketEnv} environment is an inventory management setup, where $N=10$ heterogeneous seller agents carry inventory for $M=3$ products. A population of $B=300$ buyers request a product from a randomly selected seller agent according to a demand distribution $\mathbf{p}=[p_1,\dots,p_M]$. We denote the demand realization for seller $i$ with $\mathbf{d_i}=[d_{i,1},\dots,d_{i,M}]$. Sellers manage their inventory by restocking products through interacting with the buyers. The game is episodic with horizon set to $50$. At the beginning of each episode, a realization of the demand distribution $\mathbf{p}$ is randomly generated and the agents' inventory for each product is randomly initialized from $[0, \frac{B}{N}]$, where $\frac{B}{N}$ is the expected number of buyers per seller. %\ys{describe the initial inventory in every episode?} 
Sellers are penalized for mismatch between their inventory and the demand for a product, and they aim to restock enough units of a product at each step to prevent insufficient inventory without accruing a surplus at the end of each step.  %\ys{defining the reward function by math?}
\begin{itemize}
    \item State observation: A seller agent's observation includes its inventory for each product, and the products that were requested by buyers during the previous step. The observation space is a $2M$-dimensional vector.
    
    \item Agent action: Sellers manage their inventory by restocking new units of each product or discarding part of the leftover inventory at the beginning of each step. Hence, agents take both positive and negative actions denoted by an $M$-dimensional vector, and the action space can be either discrete or continuous. In our experiments, we use continuous actions assuming that products are divisible and sellers can restock and hold fractions of a product unit.
    
    \item Agent reward function: During each step, agent $i$'s reward is defined as $r_i = - || \max( \mathbf{I}_i+\mathbf{a}_i, 0) - \mathbf{d}_i||_2$, where $\mathbf{I}_i$ denotes the agents initial inventory vector, and $\mathbf{a}_i$ denotes the inventory restock vector from action policy $\pi_i$.  
    
    
    \item Agent communication: Sellers learn the demand distribution and optimize their inventory by interacting with their own customers (i.e., portion of buyers that request a product from that seller). Sellers would benefit from sharing their observed demands with each other, so that they could estimate the demand distribution more accurately for managing inventory. At the end of each step, a seller communicates an $M$-dimensional vector reporting its observed demands to all other agents. In the case of adversarial communications, this message may differ from the agents' truly observed demands.
    
    During training with communication, messages received from all other agents are concatenated to the agent's observation, which is used to train an MLP-based policy, compared to the non-communicative case where the policy is trained using only local observations. As observed from Figure \ref{fig:marketenv_comm}, communication helps agents obtain  higher rewards since they are able to manage their inventory based on the overall demands observed across the population of buyers rather than their local observation. Results are reported by averaging rewards corresponding to $5$ experiments run with different training seeds.
\end{itemize}
 
\begin{figure}[h]
\vspace{-0.1cm}
 \centering
\resizebox{.4\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_comm_dist}}
\vspace{-0.1cm}
\caption{\textbf{MarketEnv}: Reward of agents trained with communication v.s. without communication. %Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.
} 
\label{fig:marketenv_comm}
\end{figure}
 
 



\subsection{Implementation Details}
\label{app:market_imple}
\textbf{Implementation of Trainer}\quad 
As in the FoodCollector experiments, we use the PPO algorithm to train all agent action policy as well as adversarial agent communication policies. We use the same MLP-based policy and value networks as the FoodCollector but parameterize the policy as a Gaussian distribution. The PPO agent interacts with the environment for $50$ steps, and it is trained for $10000$ episodes. The learning rate is set to be 0.0003 for the policy network, and 0.001 for the value network.
% All other hyper-parameters are set similar to the FoodCollector experiments.


\textbf{Attacker}\quad 
The attacker uses its observations to communicate malicious messages to  victim sellers, and its action space is the communication space of a benign agent.  We consider the following non-adaptive and adaptive attackers:
\begin{itemize}
    \item \textit{Non-adaptive Attacker}: The attacker's goal is to harm the victim agent by misreporting its observed demands so that the victim seller under-estimates or over-estimates the restocking of products. In our experiments, we evaluate the effectiveness of defense strategies against the following attack strategies:
    \begin{itemize}
     \item{\permute}: The communication message is a random permutation of the true demand vector observed by the attacker.
    \item {\swap}: In order to construct a communication vector as different as possible from its observed demand, the attacker reports the most requested products as the least request ones and vice versa. Therefore, the highest demand among the products is interchanged with the lowest demand, the second highest demand is interchanged with the second lowest demand and so forth.
    \item{\flip:} Adversary $i$ modifies its observed demand $\mathbf{d}_i$ by mirroring it with respect to $\eta=\frac{1}{M}\sum_{j=1}^M d_{ij}$, such that products demanded less than $\eta$ are reported as being requested more, and conversely, highly demanded products are reported as less popular.
    \end{itemize}
   
    
    \item \textit{Adaptive Attacker}: The attacker communication policy is trained using the PPO algorithm, and its reward is set as the negative reward of the victim agent. The attacker uses a Gaussian policy with a softmax activation in the output layer to learn a adversarial probability distribution across products, which is then scaled by the total observed demands $\sum_{j=1}^M d_{ij}$ to construct the communication message.

\end{itemize} 


 

\textbf{Implementation of Baselines}\quad 
\begin{itemize}
    \item \textit{Vanilla Learning}: In the vanilla training method with no defense mechanism against adversarial  communication, we train a shared policy network using agents' local observations and their received communication messages.
     \item \textit{Adversarial Training (AT)}: We alternate between training the agent action policy and the victim communication policy, both using PPO. For the first iteration we train the policies for $10000$ episodes, and then use $1000$ episodes for $5$ additional training alteration iterations for both the action policy and the adversarial communication policy. For more efficient adversarial training, we first shuffle the received communication messages before feeding them into the policy network. Consequently, the trained policy  treats communications received from different agents in a similar manner, and we are able to only train the policy with a fixed set of adversarial agents rather than training the network on all possible combinations of adversarial agents. We do not shuffle the  communication messages being input to the policy trained with vanilla learning as we did not observe improved convergence, as in the FoodCollector environment. %\ys{maybe mention the communication permuting here? and explain why permutation is not used for vanilla (performance no better than vanilla). }

\end{itemize}


 


% \subsection{Experiment Results in Market Environment}
% \label{app:market_res}

% \paragraph{Robust performance Under Attacks} \quad
% In this section, we evaluate robustness of the proposed \ours defense strategy in MarketEnv and compare it against Vanilla Learning and Adversarial Training. Figure~\ref{fig:res_all_market} shows the natural and robust performance of \ours with $k=2$, which provides performance guarantees against up to $C=2$ adversarial messages. The performance is compared with AT when the agents policy is alternatively trained against $2$ adversaries. We observe that there is a considerable reduction in the Vanilla and AT rewards under attacks, especially for the strong adaptive attack and \swap. Similar to the FoodCollector, adversarial training is not robust to adversarial communications in the MarketEnv such that for two or more adversarial messages the performance is close to or much lower than the reward achieved with no communications. However, as expected for $k=2$, \ours is able to achieve rewards comparable to the no-attack case  under $C=1$ and $C=2$ adversaries even for strong adversarial attacks. Moreover, \ours outperforms the baselines for $C=3$ for which the theoretical guarantees no longer hold. Even though the gap between natural and robust performance under the weak \permute is less for all three strategies, \ours achieves the highest reward. In  MarketEnv, \ours is able to preserve the communication gains arising from informative messages shared among the agents while being robust against adversarial communications.

  
 
% \input{fig_market_res}

% \paragraph{Hyper-parameter Test of Ablation Size $\boldsymbol k$} 
% Figure~\ref{fig:res_k_cont_market}(left)  shows how the agent's natural performance and robustness varies with the ablation size $k$. We compare \ours’s natural reward and \ours’s reward under $C=2$ adversarial communication messages for adaptive and non-adaptive attacks  with different values of $k$. Similar to the FoodCollector, As the ablation size $k$ increase, the agent is able to improve its natural performance by utilizing information communicated by more agents. However, the agent becomes more vulnerable to adversarial communications which can impacts its decision-making for managing its inventory. Therefore, ablation size $k$ trades off robustness for natural performance. Additionally, we observe that the non-adaptive \swap which constructs the  adversarial communications strategically to mislead the victim agent is quite effective in reducing the victims reward compared to the \permute which communicates adversarial messages without tactically modifying the adversary's observed demands.
 
% \paragraph{Hyper-parameter Test of Sample Size $\boldsymbol D$}
% In Figure~\ref{fig:res_k_cont_market}(right), we evaluate the robustness of the partial-sample variant of \ours presented in Section~\ref{sec:algo_partial} against $C=2$  adversaries for ablation size $k=2$, when $D$  varies from $36$ (the largest sample size) to $1$ (the smallest sample size). It is shown that with lower $D$, \ours achieves lower rewards under adversarial communications, but is considerably more robust compared to the baseline method. When the agent makes decisions based on a single random message with $D=1$, the agent's average robust reward is higher than the Vanilla reward.

% \input{fig_market_k_dist} 


\section{Additional Implementation Details of MARL-MNIST Environment}
\label{app:mnist}

\subsection{Description of MARL-MNIST Environment}

We use the environment setup proposed by~\cite{mousavi2019multi}, where agents collaboratively classify an unknown image by their observations and inter-agent communication. 
More specifically, we use $N=9$ agents in the MNIST dataset of handwritten digits~\cite{lecun1998gradient}.  The dataset consists
of 60,000 training images and 10,000 testing images, where
each image has $28 \times 28$ pixels. 
There are $h=5$ steps in an episode. In the beginning, all agents start from a pre-determined spatial configuration. At every step, each agent observes a local $5 \time 5$ patch, performing some local data processing, and communicating the result with neighboring agents (we use a fully connected communication graph). 
With given observation and communication, each agent outputs an action in $\{Up, Down, Left, Right\}$. By each movement, the agent is translated in the desired direction by $5$ pixels. In the end of an episode, agents make predictions, and all of them are rewarded by $- prediction_loss$. 


\subsection{Implementation Details}

We use the same network architecture and hyperparameter setting as~\cite{mousavi2019multi}, which are implemented in~\cite{mnistgithub}. 

\textbf{Network Architecture}\quad
Concretely, at every step, the input of every agent contains 3 components: (1) an encoded observation with two convolutional layers followed by vectorization and a fully connected layer; (2) the average of all communication messages from other agents; (3) a position encoding computed by feeding the current position into a single linear layer.
These 3 components are concatenated and passed to two independent LSTM modules, one is for an acting policy, another is for a message generator. 
In the end of an episode, every agent uses its final cell state to generate a prediction using a 2-layer MLP. Then we take the average of the output logits of all agents, and use a softmax function to obtain the final probabilistic label prediction. The reward is the opposite number of the L2 difference between the prediction and the one-hot encoding of true image label.

\textbf{Hyperparameters}\quad
In our experiments, we follow the default hyperparameter setting in~\cite{mnistgithub}. We use $N=9$ agents. The size of LSTM belief state is 128. The hidden layers have size 160. The message size is set to be 32. The state encoding has size 8. We use an Adam optimizer with learning rate 1e-3. We train the agents in the MNIST dataset for 40 epochs.

\textbf{Attackers}\quad
Since the communication messages are learned by neural networks, we perturb the $C$ messages received by each agent. To make sure that the messages are not obviously detectable, we clip every dimension of the perturbed message into the range of $[-3,3]$. The non-adaptive attacker randomly generates a new message. The adaptive attacker learns a new message generator based on its own belief state, which is trained with learning rate 1e-3 for 50 epochs.


\section{Additional Discussion on the Choice of Ablation Size $\boldsymbol k$}
\label{app:hyper}

In our proposed \ours defensive mechanism, the most crucial hyperparameter is the ablation size $k$. 
% Decreasing the ablation size $k$ trades off natural performance under no attack for robust performance under attack. 
Choosing a smaller $k$ could make the agents more robust, but could also potentially hurt their natural performance since the agents would have access to less information shared by others. Based on the previous experimental results, it is crucial to set $k$ such that condition $\eqref{eq:k_cond}$ is satisfied so that the agent could have performance certificate and thus remains robust under attack. 


In practice, if we have an estimate of the number of attackers that we would like to defend against, then we could choose the maximum $k$ satisfying Equation \eqref{eq:k_cond}. If not, based on the total number of agents, we could say that \ours could certifiably defend up to maximum $C$ attackers. So there is an interdependence between three parameters: total number of agents $N$, number of attackers $C$, and the ablation size $k$. In Figure \ref{fig:ablation_cnk} we visualize their relationship by fixing one variable at a time. From these figures, we can see an obvious trade-off between $C$ and $k$ --- if there are more attackers, $k$ has to be set smaller. But when $C$ is small, e.g. $C=1$, $k$ can be relatively large, so the agent does not need to compromise much natural performance to achieve robustness. 
% Importantly, when $C$ is much smaller than $N$, e.g. $C=1, N=30$, $k$ can be set relatively large, e.g. 15. Therefore, the natural performance is not compromised too much to achieve robustness. \textcolor{purple}{PH: not a big deal, but $K$ in the figures (title and legend) is upper case rather than lowercase $k$ used in the paper YS: fixed!}

\begin{figure*}[h]
\vspace{-0.1cm}
 \centering
    \begin{subfigure}[t]{0.31\textwidth}
    \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_C&K}}
     \label{sfig:C&K}
     \vspace{-0.5cm}
      \subcaption{$C$ vs. $k$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_N&C}}
     \label{sfig:N&C}
     \vspace{-0.5cm}
      \subcaption{$N$ vs. $C$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_N&K}}
     \label{sfig:N&K}
     \vspace{-0.5cm}
     \subcaption{$N$ vs. $k$}
    \end{subfigure}
% \vspace{-0.3cm}
\caption{Relationship between the total number of agents $N$, number of attackers $C$, and ablation size $k$. \textbf{(a)}: Maximum certifiable ablation size $k$ under different number of attackers. \textbf{(b)}: Maximum defensible number of attackers $C$ with different total number of agents $N$. \textbf{(c)}: Maximum certifiable ablation size $k$ with different total number of agents $N$.}
\label{fig:ablation_cnk}
\vspace{-0.1cm}
\end{figure*}
\label{app:exp}


 \section{Discussion: Detecting Malicious Messages with Ablation}
\label{app:exp_detect}

Theorem~\ref{thm:main_dist} and Theorem~\ref{thm:main_cont} provide strong theoretical guarantees for the proposed \ours defense. For the theorems to hold, one has to choose a $k$ to satisfy Equation \eqref{eq:k_cond}. As shown in Figure~\ref{fig:ablation_cnk}, to defend against a larger $C$, one has to choose a relatively small $k$ for certifiable performance. However, Figure \ref{sfig:hyper_k_food}, Figure \ref{sfig:hyper_k_market} and Figure~\ref{fig:res_k_dist} suggest that a small $k$ also sacrifices the natural performance of the agent to obtain higher robustness. This is known as the trade-off between robustness and accuracy~\cite{tsipras2018robustness,zhang2019theoretically}. Can we achieve better robustness while not sacrificing much natural performance, or obtain higher natural reward while not losing robustness?

We point out that with our proposed \ours defense, it is possible to choose a larger $k$ than required by condition~\ref{eq:k_cond} without sacrificing robust performance by identifying the malicious messages beforehand. We hypothesize that given a well-trained victim policy, malicious messages should mislead the victim agent to take an action that is "far away" from a "good" action that the victim is supposed to take.

To verify this hypothesis, we first train the agent $i$ with a randomized ablation policy of $k=1$. Then for every communication message that another agent $j$ sends, we compute the action $a_j$ that the victim policy $\pi_i$ chooses based on all message subsets containing message $m_{j\to i}$, i.e. $a_j = \ablpolicy(o, m_{j\to i})$ (note that $k=1$ so $\ablpolicy$ only takes in one message at a time). We then define the \emph{action bias} as $\nu_j=\|a_j-\funmed\{a_k\}_{k=1}^{N}\|_1$. Based on our hypothesis, an agent which has been hacked by attackers should induce a significantly larger action bias since they are trying to mislead the victim to take a completely different action. Here, we execute the policy of two hacked agents together with six other good agents for twenty episodes and calculate the average action bias for each agent.
As shown in in Figure \ref{fig:detect_adv}, the agents hacked by attackers indeed induce a larger action bias compared to other benign agents, which suggests the effectiveness of identifying the malicious messages by action bias. 

% Note that although there is no theoretical guarantee for identifying the adversarial communication messages, 
After filtering out $A$ messages, one could compute the required $k$ by Equation~\ref{eq:k_cond} based on $C-A$ malicious messages and $N-A$ total messages, which can be larger than the largest $k$ induced by $C$ malicious messages out of $N$ total messages. For example, if $N=30$, $C=3$, then the largest $k$ satisfying Equation~\ref{eq:k_cond} is 5, but when 1 adversarial message is filtered out, the largest $k$ that can defend against the remaining 2 adversarial messages is 8. Although the adversary identification is not theoretically guaranteed to be accurate, Figure \ref{fig:detect_adv} demonstrates the effectiveness of the adversarial message detection, which, combined with \ours with larger $k$'s, has the potential to achieve high natural performance and strong robustness in practice.
% one could still apply Theorem \ref{thm:main_cont} with $C-A$ malicious messages and $N-A$ good messages in total.
\begin{figure}[h]
\vspace{-0.1cm}
 \centering
\input{figs/Attacker Identification.tex}
\vspace{-0.3cm}
\caption{Attacker identification based on action bias $\nu_j$. Adv1 and Adv2 stands for two agents hacked by the attacker. B1 up to B6 stands for six other benign agents.}
\vspace{-0.5cm}
\label{fig:detect_adv}
\end{figure}

==> backup_algo.tex <==
%%% Old version of algorithm theory


\textbf{Action Certificate}\quad
First, we define a set of actions rendered by random combinations of benign messages. As the agent is likely to take these actions in a non-adversarial environment, they can be regarded as safe actions to take.
\begin{definition}[Discrete Safe Action Set $\safeactiondist$]
\label{def:fsafeact_dist}
For any step, define $\safeactiondist \subseteq \mathcal{A}$ as a set of actions that $\ablpolicy$ may select under randomly sampled benign messages.
\begin{equation}
\label{eq:safeact_dist}
     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}
\end{equation}
\end{definition}
% $\safeactiondist \subseteq \mathcal{A}$ is a set of actions that $\ablpolicy$  may select at the current step under randomly sampled benign messages.
The following theorem suggests that the ensemble policy $\smpolicy$ always takes safe actions in $\safeactiondist$ under mild conditions, even when malicious information is present in the input.


% In this case, the following theorem suggests that the ensemble policy $\smpolicy$ is not influenced by the malicious messages under mild conditions.

\begin{theorem}[Action Certificate for Discrete Action Space]
\label{thm:main_dist}
% Assume that subset size $k$  and ensemble policy $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. 
Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees safe actions under $\advmsg$, i.e.,
\begin{equation}
    \widetilde{a} = \smpolicy(o, \advmsg) \in \safeactiondist,
    \label{eq:cert_dist}
\end{equation}
if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% where 
% \begin{equation}
%     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% \end{equation}
\end{theorem}
\textbf{Remarks.}
(1) Theorem~\ref{thm:main_dist} certifies that for every step of execution, $\smpolicy$ selects a safe action when the agent receives $\advmsg$ with up to $C$ malicious messages. 
% \fh{Is there a specific reason why we emphasize one step? Should the certification certify every step? Is it possible that the actions appears safe for this round, but not safe for the next round? Oh, maybe the concept of safe already guarantees long-term safety? I feel the emphasis on current-step may cause confusion. We either need to talk about this current-step guarantees long-term safety or we just talk about long-term safety without mentioning current-step?} 
(2) \change{The condition $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ is for the worst-case consideration, which ensures robustness even if the adversarial messages collaborate to vote for an unsafe action and outweigh benign messages in all base policies. 
But in practice, our algorithm works well without requiring such a condition as verified in experiments. }
% \textcolor{red}{select some bad action} \fh{they don't have the freedom to choose actions, maybe change to something like:craft sophisticated malicious messages}
% Also, this condition is mild since $C$ is usually much smaller than $N$.


% \change{
% \textbf{Action Certificate}
% The following theorem suggests that the ensemble policy $\smpolicy$ always takes ``safe'' actions resulting from pure benign messages under mild conditions, even when malicious information is present in the input.
% \begin{theorem}[Action Certificate for Discrete Action Space]
% \label{thm:main_dist}
% Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees safe actions under $\advmsg$, i.e.,
% \begin{equation}
%     \widetilde{a} = \smpolicy(o, \advmsg) \in \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\} =: \safeactiondist,
%     \label{eq:cert_dist}
% \end{equation}
% if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% % where 
% % \begin{equation}
% %     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% % \end{equation}
% \end{theorem}
% \textbf{Remarks.}
% (1) $\safeactiondist$ is a set of actions rendered by random combinations of benign messages. As the agent is likely to take these actions in a non-adversarial environment, they can be regarded as ``safe'' actions to take.
% (2) Theorem~\ref{thm:main_dist} certifies that for every step of execution, $\smpolicy$ selects a safe action when the agent receives $\advmsg$ with up to $C$ malicious messages. 
% (3) The condition $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ is for the worst-case consideration, which ensures robustness even if the adversarial messages collaborate to vote for an unsafe action and outweigh benign messages in all base policies. 
% But in practice, our algorithm works well without requiring such a condition as verified in experiments. }



%%% Continuous action

\textbf{Action Certificate}\quad
As in the discrete action case, we first define the safe action set in the continuous action case $\safeactioncont$ as the set of actions that do not exceed the ``safe action range'' resulting from all combinations of $k$ benign messages.
% \ys{explain the safe action set with more intuition}
\begin{definition}[Continuous Safe Action Set $\safeactioncont$]
\label{def:safeact_cont}
For every $a\in \mathcal{A}\subseteq \mathbb{R}^L$, $a\in \safeactioncont$ iff for every coordinate $1\leq l\leq L$,
\vspace{-1.5em}

\small
\begin{equation}
\label{eq:safeact_cont}
\begin{aligned}
    \min\nolimits_{T\in\mathcal{H}(N-1,k)} [\ablpolicy(o, \funabl(\goodmsg, T))]_l
    \leq a_l 
    \leq 
    \max\nolimits_{T\in\mathcal{H}(N-1,k)} [\ablpolicy(o, \funabl(\goodmsg, T))]_l
\end{aligned}
\end{equation}\normalsize
\end{definition}
\vspace{-0.5em}

% We first define the safe action set in continuous-action case $\safeactioncont$ as the set of actions that does not exceed ``safe action range'' resulted by all possible combinations of benign messages. That is, in the current step, an action $a$ is in $\safeactioncont$ iff each coordinate $l \in L$ satisfy
% \begin{equation}
% \begin{aligned}
%     \inf_{T\in\mathcal{H}(N-1,k)} [\ablpolicy(o, \funabl(\goodmsg, T))]_l
%     \leq a_l \\ 
%     \leq 
%     \sup_{T\in\mathcal{H}(N-1,k)} [\ablpolicy(o, \funabl(\goodmsg, T))]_l
% \end{aligned}
% \end{equation}

$\safeactioncont \subseteq \mathcal{A}$ is a set of actions inside the range of $\ablpolicy$ under randomly sampled benign messages in the current step. 
It is reasonable to assume that actions in $\safeactioncont$ are relatively safe. For example, if the action denotes the price a seller sells its product in a market, and the communication messages are the transaction signals in an information pool, then $\safeactioncont$ is a price range  that is determined based on uncorrupted messages. Therefore, the seller will set a reasonable price without being influenced by a malicious message. 
With this definition, the following action certificate holds.
\begin{theorem}[Action Certificate for Continuous Action Space]
\label{thm:main_cont}
Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees safe actions under $\advmsg$, i.e.,
\begin{equation}
    \smpolicy(o, \advmsg) \in \safeactioncont 
    \label{eq:cert_cont}
    % \textcolor{purple}{PH: \advmsg or  \mathbf{m}?}
\end{equation}
% then any dimension $l$ of $\smpolicy$'s output satisfies
% \begin{equation*}
%     \inf_{\krv} [\hat{a}]_l  
%     \leq [\smpolicy(o, \advmsg, \{T_d\}_{d=1}^D)]_l 
%     \leq \sup_{\krv} [\hat{a}]_l.
% \end{equation*}
% where $\hat{a} := \ablpolicy(o, \mathsf{Ablate}(m, \krv))$.
\end{theorem}

==> cmarl/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% \draft{We study the attacks and defenses in communicative multi-agent reinforcement learning.


% Our contributions:
% 1. formulate the adversarial problem in CMARL.
% 2. propose a certifiable defense algorithm
% 3. empirical study in a simulated game and a market environment.
% }

% Recent years have witnessed significant advances in reinforcement learning (RL), especially deep reinforcement learning (DRL). Although vanilla RL considers the interaction between a single agent and the environment, many real-world applications have multiple agents involved, such as autonomous driving~\cite{shalev2016safe}, robotics~\cite{dudek1996taxonomy}, etc. 


% \ys{start from decision making?}
With the rapid improvement of deep reinforcement learning (DRL) techniques, neural network-based multi-agent reinforcement learning (MARL) has achieved significant advances in many real-world applications, such as autonomous driving~\cite{shalev2016safe,sallab2017deep}. In a multi-agent system, especially in a cooperative game, communication usually plays an important role. Through communication, each agent can obtain more information about the environment and other agents, and thus can learn a better policy. Many recent works~\cite{foerster2016learning,hausknecht2016cooperation,sukhbaatar2016learning} have shown that feeding communication messages to RL networks can result in better decision makers.

However, neural networks are shown to be vulnerable to adversarial attacks~\cite{goodfellow2014explaining}, i.e.,
% , especially network-based RL policies~\cite{huang2017adversarial} \fh{network-based RL policies are not a special case of neural networks. So the logic here is a bit unsmooth.}, 
a well-trained network may output a wrong answer if the input to the network is slightly but deliberately perturbed.
% if the inputs to the network are slightly but deliberately perturbed, the network, although well-trained on clean datasets \fh{rather than datasets, shall we say unattacked environment or safe environment, since RL is not necessarily trained on a ``dataset''?}, may output a wrong answer. 
As a result, although a policy can obtain a high reward by taking in the messages sent by other agents, it may also get drastically misled by inaccurate information or even adversarial communication from malicious attackers. 
For example, when several drones execute pre-trained policies and exchange information via wireless communication, it is possible that some malicious attacker eavesdrops on their communication and intentionally perturbs some messages to a victim agent via cyber attacks. 
Moreover, even if the communication channel is protected by advanced encryption algorithms, an attacker may also hack some agents and alter the messages before they are sent out (e.g. hacking IoT devices that usually lack sufficient protection~\cite{naik2017cyber}). Figure~\ref{fig:diagram} demonstrates an example of communication-attack, where the attacker may lure the agent to a dangerous location through malicious message propagation and cause fatal damage.

\begin{figure*}[!t]
\vspace{-2em}
    \centering
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{figs/train.pdf}
         \vspace{-0.5em}
         \caption{Training time}
         \label{sfig:train}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{figs/test.pdf}
         \vspace{-0.5em}
         \caption{Test time (in deployment)}
         \label{sfig:test}
     \end{subfigure}
     \vspace{-0.5em}
    \caption{An example of test-time communication attacks in a communicative MARL system. Agents can be heterogeneous as depicted by various icons. (a) During training, agents are trained collaboratively in a safe environment, such as a simulated environment. (b) In deployment, agents execute pre-trained policies in the real world which may susceptible to attacks that perturb communication messages. Malicious attackers may modify the benign messages into adversarial signals. In this figure, arrows denote communication channels among agents, {\color{darkpastelgreen}{green}} messages stand for benign communication, and {\color{red}{red}} messages stand for adversarial communication.}
    \label{fig:diagram}
\vspace{-1.5em}
\end{figure*}

Although adversarial attacks and defenses have been extensively studied in supervised learning~\cite{madry2018towards,cohen2019certified} and reinforcement learning~\cite{zhang2020robust,zhang2021robust,oikarinen2020robust}, there has been little discussion on the robustness issue against adversarial communication in MARL problems. 
Therefore, in order to safely apply communication to more high-stakes multi-agent scenarios, it is crucial to robustify MARL policies against adversarial attacks.
% \textcolor{red}{Defending against the adversarial communication while still utilizing the benign communication}\fh{needs rewording. Maybe: Achieving high performance in a multi-agent cooperative game through inter-agent communication while remain robust to adversarial communication attacks} 
Achieving high performance in a multi-agent cooperative game through inter-agent communication while being robust to adversarial communication attacks is a {challenging problem} due to the following reasons. 
\textbf{Challenge I}: The attacker may construct malicious messages in various ways, so that they are hard to be distinguished from benign messages. For example, the malicious messages shown in Figure~\ref{sfig:test} are in the same form as the benign messages and also make semantic sense. \textbf{Challenge II}: A strong attacker can even be \textit{adaptive} to the victim agent and significantly reduce the victim's total reward. For instance, for a victim agent who moves according to the average of GPS coordinates sent by others, the attacker may learn to send extreme coordinates to influence the average.
% the attacker may learn an RL policy to send sequential misleading messages. \fh{This point is not very clear.}
\textbf{Challenge III}: There can be more than one attacker (or an attacker can perturb more than one message at one step), so that they can collaborate to mislead a victim agent.

Tu et al.~\cite{tu2021adversarial} apply adversarial training~\cite{madry2018towards} to improve model robustness against communication perturbation. But they focus on the $\ell_p$ threat model (perturbation with small $\ell_p$ norm), which do not solve many attack scenarios such that the attack in Figure~\ref{sfig:test}.
Some recent works~\cite{blumenkamp2020emergence,xue2021mis,mitchell2020gaussian} recognize the existence of adversarial communications in MARL and propose several defending methods, e.g. a trained message filter~\cite{xue2021mis}. However, these heuristics-based defenses, although are the first step to investigate adversarial communication in MARL, do not fully address the aforementioned challenges, and are not guaranteed to be robust, especially under adaptive attacks. 
% \textcolor{purple}{PH: all communication attacks, any communication attack? YS: should be all, thanks} 
%\textcolor{purple}{PH: Is it clear what we mean by adaptive attacks? In challenge 2 we are kind of defining it. Would it make sense to make the \textit{adaptive} italic in challenge 2 to stand out? YS: Sure! Good point}

In contrast, we address all aforementioned challenges by proposing \textit{a certifiable defense named \textbf{\oursfull (\ours)} that can guarantee the performance of agents against multiple adversarial communication messages}.
% \fh{Our proposed defense addresses all three aforementioned challenges.}
% \fh{should not overclaim. mention this is for communication attacks only}. 
The main idea is to construct an \emph{ensemble policy} which makes decisions based on multiple different subsets of communication messages (i.e., ablated messages). 
Specifically, for a list of messages coming from different agents, we train a \emph{base policy} that takes in a subset of messages and outputs a \emph{base action}. 
Then we obtain an ensemble policy by aggregating multiple base actions coming from multiple different message subsets. For a discrete action space, the ensemble policy takes the majority of the multiple base actions obtained, while for a continuous action space, the ensemble policy takes the median of these base actions. \ours is a generic framework that works for any agent that observes multiple messages from different sources, as long as the agent receives more benign communication messages than adversarial ones. We also show in Section~\ys{todo} that \ours can be used in many other scenarios beyond defending against MARL communication attacks.
% Therefore, \ours can be extended to defend against 
% \ys{flexibility, as discussed later}

Our contributions can be summarized as below:\\
\textbf{(1)} We formulate the problem of adversarial attacks and defenses in communicative MARL (CMARL).\\
\textbf{(2)} We propose a novel defense method, \ours, 
% \SF{perhaps introduce ``ablation" terminology in the previous paragraph so readers become familiar with it at this point}
% based on randomized ablation on communication messages. \ours 
that is provably robust against arbitrary perturbations of up to $C<\frac{N-1}{2}$ communication channels, where $N$ is the number of agents. \\
% both in discrete action space and in continuous action space. \fh{I feel the contribution is not that we include both discrete or continuous action space, but rather, we can achieve very strong results in the discrete space, as well as good results in the continuous space. I feel the current wording sounds a bit off the path.}\\
\textbf{(3)} Experiment in 3 multi-agent environments shows that \ours obtains significantly higher reward than baseline methods under both non-adaptive and adaptive attackers. 
% The agent trained with \ours achieves similar 
% \SF{add a bit more details here; what environments; discrete or cont; what gains do we achieve?}. 
% \fh{maybe some numbers in terms of performance improvement etc}



==> cmarl/2_relate.tex <==
% \vspace{-0.5em}
\section{Related Work}
\label{sec:relate}
% \fh{I don't think we need this related work to be at the beginning to explain our method. Shall we move it here?}

% \ys{add more papers for arxiv. if else command}

\textbf{Communication in MARL}\quad
Communication is crucial in solving collaborative MARL problems. There are many existing studies learning communication protocols across multiple agents. \cite{foerster2016learning} are the first to learn differentiable communication protocols that is end-to-end trainable across agents. Another work by~\cite{sukhbaatar2016learning} proposes an efficient permutation-invariant centralized learning algorithm which learns a large feed-forward neural network to map inputs of all agents to their actions. 
It is also important to communicate selectively, since some communication may be less informative or unnecessarily expensive. To tackle this challenge, \cite{das2020tarmac} propose an attention mechanism for agents to adaptively select which other agents to send messages to. \cite{liu2020who2com} introduce a handshaking procedure so that the agents communicate only when needed. Our work assumes a pre-trained communication protocol and does not consider the problem of learning communication mechanisms.

\textbf{Adversarial Attacks and Defenses in CMARL}\quad
The investigation of adversarial communication in MARL problems is a relatively new topic, and has recently attracted increasing attention.  
\cite{blumenkamp2020emergence} show that in a cooperative game, some self-interest agents can learn manipulative communication policies and hurt other agents' performance. 
% To accommodate multiple agent objectives, they propose \change{Aggregation}\fh{aggregated? is aggregation GNN a terminology? I've not heard of it.} Graph Neural Networks to model and learn an inter-agent communication policy. 
To achieve robust communication, \cite{mitchell2020gaussian} use Graph Neural Networks to model the communication architecture and adopt a Gaussian Process-based probabilistic model to compute the posterior probabilities that whether each partner is truthful. 
\cite{tu2021adversarial} investigate the vulnerability of multi-agent autonomous systems against communication attacks. 
% \change{multiple aspects} \fh{?}.
\cite{xue2021mis} present an algorithm to defend against one adversarial communication message by an anomaly detector and a message reconstructor, which is trained with groundtruth labels and messages. In comparison, our work proposes a provably robust defense mechanism that has certifiable performance even when near to half of the communication messages are corrupted.
% formulates adversarial attacks in a general \fh{are previous works not generic? Why?}communicative MARL (CMARL) setting, and 
% \fh{Is \cite{xue2021mis} attack agnostic? The current description doesn't answer this question.}.

\textbf{Adversarial Robustness of RL Agents}\quad
As RL techniques have been applied to more and more applications, the robustness of agents under environment noise or adversarial attacks becomes an emerging research topic. 
For a single-agent problem, there are many recent works on adversarial state perturbation~\cite{huang2017adversarial,zhang2020robust} and action perturbation~\cite{tan2020robustifying,tessler2019action}. In a multi-agent system, the interplay among agents introduces more uncertainty to the environment. \cite{gleave2020adversarial} point out that a well-trained agent can be completely misled by adversarial behaviors of another agent. Although adversarial training (i.e., introducing adversarial agents to the system during training~\cite{pinto2017robust,phan2021resilient}) can empirically improve agents' robustness, such robustness is not guaranteed to hold under all possible attackers.


\textbf{Certifiable Defense}\quad
There is an important line of work studying guaranteed robustness of neural networks~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness} while the input data is perturbed within an $\ell_p$ norm ball. In an effort to certify RL agents' robustness, \cite{lutjens2020certified} and \cite{oikarinen2020robust} utilize convex relaxation of Q networks to improve the worst-case performance of agents. \cite{kumar2021policy} and \cite{wu2021crop} follow the idea of randomized smoothing~\cite{cohen2019certified} and smooth out the policy by adding Gaussian noise to the input.
To the best of our knowledge, our \ours is the first certifiable defense in MARL against communication attacks. Moreover, we consider a strong threat model where up to half of communication messages can be arbitrarily corrupted. 
\ys{flexibility}
% This threat model can cover many realistic attacking scenarios that the $\ell_p$ model does not solve.

% This paper \myst{is also closely related to} \fh{bears some similarities with}~\cite{gleave2020adversarial}, which studies the effects of adversarial actions in an MARL problem. In contrast, our work aims to defend against communication attacks that can be more stealthy in practice.
% Randomized ablation is proposed by~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification problems, in which the classifier is trained by randomly ablating pixels of images. 
% We are the first to extend the idea of randomized ablation to MARL and to achieve action and reward certificates against communication attacks.
% Note that the number of pixels in an image and the number of agents in an MARL problem are in different scales. Also, a classifier outputs discrete labels, while a policy may have discrete or continuous output space. Therefore, our problem setup, methodology and theoretical results are significantly different from~\cite{Levine_Feizi_2020} and are novel.

% \textbf{parameter sharing} Sharing parameters are a common way to take advantage of centralized training \cite{lowe2017multi,foerster2016learning} by learning a single shared critic network for multiple agents. \cite{gupta2017cooperative} uses single-agent RL methods to learn policies in cooperative environments.

==> cmarl/3_setup.tex <==
\section{Problem Formulation}
\label{sec:setup}

% \fh{Shall we change the section title to Problem Formulation?}

% \subsection{Basic Notations}
% For an interger $N$, let $[N]$ denote the set $\{1,2,\cdots,N\}$.
% We use $X_{1:N}$ as a shorthand notation of the list $[X_1,\cdots,X_N]$.
% % , and $X_{-i}$ as a shorthand notation of the list $[X_1,\cdots, X_{i-1}, X_{i+1}, \cdots, X_N]$.
% Let $\mathcal{H}(N,k)$ denote the set of all the unique $k$ indices out of $N$, so $|\mathcal{H}(N,k)|=\binom{N}{k}$, and let $\mathcal{U}(N,k)$ denote the uniform distribution over $\mathcal{H}(N,k)$.
% Let $\mathcal{T}=\{i_1, i_2,...,i_k\}\sim \mathcal{U}(N,k)$ be the random variable that denotes the collection of $k$ out of $N$ dimensions. 
% For a list of $N$ elements $m=[m_1, m_2, \cdots, m_n]$, $\mathsf{Ablate}(m, \mathcal{T}) = [m_{i_1}, \cdots, m_{i_k}]$. 
% For any random variable $X \sim \mathcal{D}$ ($\sim \mathcal{D}$ is omitted below for simplicity) and a real-valued function $f(X)$, define a function $\mathsf{Med}_{X}(f(X))$ as 
% $$
% \mathsf{Med}_{X}(f(X)) := \inf \{ c\in\mathbb{R}: \mathbb{P}_X [ f(X) \geq c ] \geq 0.5 \}.
% $$
% For a vector-valued function $F = [f_1(X), \cdots, f_l(X)]^\top$, the $\mathsf{Med}$ function is extended as the element-wise median value, i.e.,
% $$
% \mathsf{Med}_{X}(F(X)) = [\mathsf{Med}_{X}(f_1(X)), \cdots, \mathsf{Med}_{X}(f_l(X))]^\top.
% $$



\subsection{Communicative Muti-agent Reinforcement Learning}
\label{sec:setup_cmarl}

% \textbf{Dec-POMDP Model.}\quad
% We consider a Decentralised Partially Observable Markov Decision Process (Dec-POMDP)~\cite{oliehoek2012decentralized,oliehoek2015concise,das2020tarmac} which is a multi-agent generalization of the single-agent POMDP models. 
% A Dec-POMDP can be modeled as a tuple $\langle \mathcal{D}, \mathcal{S}, \mathcal{A}, \mathcal{O}, O, P, R, \gamma, \rho_0 \rangle$. 
% $\mathcal{D}=\{1,\cdots,N\}$ is the set of $N$ agents.
% $\mathcal{S}$ is the underlying state space. $\mathcal{A}=\times_{i\in\mathcal{D}}\mathcal{A}_i$ is the \emph{joint} action space. $\mathcal{O}=\times_{i\in\mathcal{D}}\mathcal{O}_i$ is the \emph{joint} observation space, with $O$ being the observation emission function.
% $P: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \Delta(\mathcal{S}) $ is the state transition function\footnote{$\Delta(\mathcal{X})$ denotes the space of probability distributions over space $\mathcal{X}$.}.
% $R: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \mathbb{R}$ is the immediate reward function.
% $\gamma$ is the shared discount factor, and $\rho_0$ is the initial state distribution.

% \textbf{Communication in Dec-POMDP}\quad
% At every step $t$, each agent $i\in[N]$ observes its local observation $o_i\step$ and sends a communication message $m_{i \to j}\step := F(i,o_i\step,j)\in\mathcal{M}$ to agent $j$ for all $j\neq i$. 
% Here $m_{i \to j}\step$ denotes a message sent from agent $i$ to $j$ in step $t$. For notation simplicity, we will omit ${}\step$ when there is no ambiguity. 
% A message $m_{i \to j}$ can be a scalar or a vector, e.g., signal of GPS coordinates. 
% For notation simplicity, we assume that agents are fully connected for communication, although our algorithm directly applies to partially connected communication graphs. That is, at each step, every agent sends $N-1$ messages (1 for each agent other than itself), and receives $N-1$ messages from others.
% We use $\mtoi$ to denote the list of messages received by agent $i$, i.e., $\mtoi:=\{m_{j \to i} | 1\leq j \leq N, j\neq i \}$. 



\ys{reminder: communicative stochastic game}
We consider a \textit{Communicative Multi-agent Reinforcement Learning (CMARL)} problem, where the environment is modeled as a tuple 
% \fh{$\mathcal{M}$ used for both the MAC-MDP and the message space}
$\langle N, \mathcal{S}, \mathcal{A}, \mathcal{O}, \mathcal{M}, P, R, B, F, \gamma, \rho_0 \rangle$.
% \fh{Could we add $f_i: \mathcal{O}_i \to \mathcal{M}_1\times\cdots \mathcal{M}_{i-1}\times  \mathcal{M}_{i+1}\times \cdots \mathcal{M}_N$ or just $\{f_i\}_{i=1}^N$ to the tuple to indicate that we consider $f_i$ as part of the environment rather than part of our strategy?}
$N$ is the number of agents;
$\mathcal{S}$ is the underlying common state space;
$\mathcal{A}=\mathcal{A}_1\times\mathcal{A}_2\times\cdots\times\mathcal{A}_N$ is the \emph{joint} action space;
$\mathcal{O}=\mathcal{O}_1\times\mathcal{O}_2\times\cdots\times\mathcal{O}_N$ is the \emph{joint} observation space;
$\mathcal{M}$ is the message space;
$P: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \Delta(\mathcal{S}) $ is the state transition function\footnote{$\Delta(\mathcal{X})$ denotes the space of probability distributions over space $\mathcal{X}$.};
$R: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \mathbb{R}^N$ is the \emph{joint} reward function that returns a list of rewards for all agents;
$B: \mathcal{S} \to \Delta(\mathcal{O}_1) \times \Delta(\mathcal{O}_2) \times \cdots \times \Delta(\mathcal{O}_N)$ is the observation emission probability function;
$F$ is the communication protocol, with $F(i,o_i,j) \in\mathcal{M}$ being the communication signal/message sent from agent $i$ to agent $j$ when $i$ observes $o_i\in\mathcal{O}_i$;
$\gamma$ is the shared discount factor; $\rho_0$ is the initial state distribution.

The above formulation is generic and can model many real-world scenarios. 
(1) The reward function $R$ can output the same values for all agents (\textit{fully-cooperative} setting), or output different values for heterogeneous agents (\textit{self-interested} setting). Note that although communication is usually considered in cooperative problems~\cite{foerster2016learning,ghavamzadeh2004learning}, self-interested agents can also benefit from communication. For example, auto-driving cars can avoid collision by sharing their routes with each other. 
(2) The communication protocol $F$ can be \textit{hand-coded} or \textit{learned}~\cite{foerster2016learning}. In deployment, agents follow a fixed communication protocol or execute a trained communication model/policy.
Our goal is to defend against perturbed communication messages as detailed in Section~\ref{sec:setup_adv}, regardless of how communication is generated.
Most existing multi-agent environments can be regarded as special cases of this CMARL formulation. For example, the reward function $R$ maps the current state and all current agent actions to a reward vector, containing the rewards received by each individual agent. If all agents get the same reward at every step, then the environment degenerates to a fully-cooperative one. 

\textbf{Communication Message $\boldsymbol{m}$}\quad
% In a CMARL problem, agents can communicate based on a protocol $F$, which can be either pre-defined or learned as discussed in prior works~\cite{foerster2016learning}. In this paper, we consider a pre-defined communication protocol $F$ and learning $F$ is out of our scope.
At every step $t$, each agent $i\in[N]$ observes its local observation $o_i\step$ and sends a communication message $m_{i \to j}\step := F(i,o_i\step,j)\in\mathcal{M}$ to agent $j$ for all $j\neq i$. 
Here $m_{i \to j}\step$ denotes a message sent from agent $i$ to $j$ in step $t$. For notation simplicity, we will omit ${}\step$ when there is no ambiguity. 
A message $m_{i \to j}$ can be a scalar or a vector, e.g., signal of GPS coordinates. 
For notation simplicity, we assume that agents are fully connected for communication, although our algorithm directly applies to partially connected communication graphs. That is, at each step, every agent sends $N-1$ messages (1 for each agent other than itself), and receives $N-1$ messages from others.
We use $\mtoi$ to denote the list of messages received by agent $i$, i.e., $\mtoi:=\{m_{j \to i} | 1\leq j \leq N, j\neq i \}$. 

% \textcolor{purple}{PH: I know we said we omit $(t)$ when there is no ambiguity, but for consistency of notation, shall we keep or omit $(t)$ in both $\mtoi$ and $m_{j \to i}$ in the definition $:=$? YS: Yes, this is a typo, I fixed it.}
% _{j\neq i:j=1}^N
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
%     \mtoi := [m_{1 \to i}, \cdots, m_{(i-1) \to i}, m_{(i+1) \to i}, \cdots, m_{N \to i}].
% \end{equation*}

% The communication messages are generated by agents' private communication functions denoted as $\commfunc$ \fh{$\commfunc_i$ for an agent $i$}.
% To cover more real-world scenarios, we consider the case where agents  can share different information (\fh{based on their local observation}) with \textcolor{red}{different} \fh{their selected} recipients at each step.  Specifically, each agent $i$ generates communication \fh{messages} by function $f_i: \mathcal{O}_i \to \mathcal{M}_i^{N-1}$ \fh{need to define what does the superscript mean here.}. This function $f_i$ can be either pre-defined with domain knowledge, or trained with existing approaches~\cite{foerster2016learning}. \textcolor{red}{But note that learning advanced communication methods is not the focus of this paper, since we aim to defend against adversarial communication over any pre-defined or learned communication protocols.}
% \fh{In this paper, we do not focus on learning advanced communication methods $\{\commfunc_i\}_{i=1}^N$. Rather we aim to defend against adversarial communication over any pre-defined or learned communication protocols. In other words, we investigate defense mechanisms for adversarial perturbations to agent $i$'s messages $\commfunc_i(o_i\step):=\mathbf{m}_{i\to :}\step := [m_{i \to 1}\step, \cdots, m_{i \to (i-1)}\step, m_{i \to (i+1)}\step, \cdots, m_{i \to N}\step]$.} 

\textbf{Acting Policy $\boldsymbol{\pi}$}\quad
The goal of each agent $i\in [N] := \{1,2,\cdots,N\}$ is to maximize its discounted cumulative reward $\sum_{t=0}^\infty \gamma^t r\step_i$ by learning an acting policy $\pi_i: \mathcal{O}_i\times \mathcal{M}^{N-1} \to \mathcal{A}_i$, 
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
%     \pi_i: \mathcal{O}_i\times \mathcal{M}_1 \times\cdots \mathcal{M}_{i-1} \times \mathcal{M}_{i+1} \times \cdots \mathcal{M}_N \to \mathcal{A}_i,
% \end{equation*}
which maps the agent's current observation $o_i$ and all communication messages from other agents $\mtoi$ 
% \fh{$\{m_{j \to i}\step\}_{j\neq i:j=1}^N$} 
to an action for agent $i$, i.e., $a_i$.
% The underlying state of the environment is often not fully observable to an individual agent, i.e., $o_i$ usually does not contain all information needed to make optimal decisions.
% % the underlying state of the environment is not fully observable to an individual agent. 
% For example, the local view of a single drone does not cover the entire map for navigation. Therefore 
Communication messages from other agents are important for the acting policy to gain high rewards, especially in cooperative games~\cite{foerster2016learning,liu2018energy}. However, as will be discussed in Section~\ref{sec:setup_adv} below, communication can be a double-edge sword --- it expedites learning by information sharing but may make agents vulnerable to adversarial attacks.





% At every step $t$, an agent $i\in [N] := \{1,2,\cdots,N\}$ goes through the following process: \\
% \textbf{(1)} Agent $i$ observes its (local) observation $o_i\step \in \mathcal{O}_i$ (the environment has current state $s\step$ which is not visible to the agent). \\
% \textbf{(2)} Agent $i$ sends messages to other agents by the communication function $\mu_i: \mathcal{O}_i \to (\mathcal{M}_i \cup \{\mathsf{NULL}\})^{N-1}$, where $\mathsf{NULL}$ indicates that no message is sent to the corresponding receiver.
% % $\mu_i: \mathcal{O}_i \to \{0,1\}^{N-1} \times \mathcal{M}_i$, where $b \in \{0,1\}^{N-1}$ denotes a communication mask. If $b=[1,\cdots,1]$, the message is broadcasted to all other agents. If $b=[1,0\cdots,0]$, the message is only sent to the first agent. 
% Let $m_{i\to j}\step$ denote the message from agent $i$ to agent $j$ at step $t$.\\
% \textbf{(3)} Agent $i$ receives messages sent from all other agents 
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
%     \mtoi\step := [m_{1 \to i}\step, \cdots, m_{(i-1) \to i}\step, m_{(i+1) \to i}\step, \cdots, m_{N \to i}\step].
% \end{equation*}
% \fh{where each $m_{j \to i}\step$ is a vector of dimension ?}
% (If $j$ did not send a message to $i$, then $m_{j \to i}\step$ is empty.) \\
% \textbf{(4)} Agent $i$ takes action $a_i\step$ by its \emph{acting policy}  \fh{$\pi_i$ which considers its local observation as well as messages from other agents}
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
%     \pi_i: \mathcal{O}_i\times \mathcal{M}_1 \times\cdots \mathcal{M}_{i-1} \times \mathcal{M}_{i+1} \times \cdots \mathcal{M}_N \to \mathcal{A}_i.
% \end{equation*}

% \fh{Note that the acting policy doesn't specify the communication strategy of an agent. Should we talk about the communication strategy here, i.e., how to render the message?}
% \vspace{-1em}

% The communication function $\mu_i$ \fh{you never defined $\mu_i$. Typo.} can be either pre-defined or learned. Let $[R(s_t, a_1\step, \cdots, (a_N)_t))]_x$ \fh{$(a_N)_t$ not defined} denote the reward of agent $x \in [N]$ at step $t$. \fh{We need to make the notations clear here. What does this $[\cdot]_x$ mean? What does each $a_i\step$ denote? We should make it clear that each agent may have their own reward as explained in the model where we can there is a joint reward function. I feel this needs more explanation. Also I am thinking, shall we draw a simple 3-agent-diagram to depict MACRL if we have time?} \fh{In the previous descriptions, you use $i$ to denote agent id, now it is changed to $x$. Can we make them consistent?} Then, the goal of agent $x$ is to maximize its own cumulative reward, i.e.,
% {\small{
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:agent_obj}
% \tag{$Q$}
% \begin{aligned}
%     \min_{\pi_x} \fh{\max?} & \; \natobj^x := \mathbb{E} [ \sum_{t=0}^\infty \gamma^t [R(s\step, a_1\step, \cdots, a_N\step)]_{x} ] \\
%     \text{where } & \; a_i\step = \pi_i(o_i\step, \mtoi\step), \forall i\in [N], t=1,\cdots
% \end{aligned}
% \end{equation}
% }}

% $\pi_i: \mathcal{O}_i\times \mathcal{M}_1 \times\cdots \mathcal{M}_{i-1} \times \mathcal{M}_{i+1} \times \cdots \mathcal{M}_N \to \mathcal{A}_i$.
% Note that the $N$ agents can be heterogeneous, as each of them has its own observation space, action space, message space and reward function. 
% Many existing multi-agent environments can be regarded as special cases of the above formulation. For example, if there is no communication, then it is a normal MARL environment, equivalent to setting $\mathcal{M}_{1:N}$ to be empty sets. If all agents have the same reward ($R_1,\cdots,R_N$ are equal), then the environment degenerates to a fully-cooperative game. If agents further share the same observation space and action space, then they can be viewed as symmetric agents.
% Therefore, our above formulation of MACRL is generic and can model many real-world scenarios. 




\subsection{Communication Attacks in Deployment of CMARL}
\label{sec:setup_adv}

Communication attacks in MARL has recently attracted increasing attention~\cite{blumenkamp2020emergence,tu2021adversarial,xue2021mis} with different focuses, as summarized in Section~\ref{sec:relate}. 
In this paper, we consider a practical and strong threat model where malicious attackers can arbitrarily perturb a subset of communication messages in CMARL.

\textbf{Formulation of Communication Attack}\quad 
% \ys{I will re-write this section to make it less complicated and more clear}
During test time, agents execute well-trained policies $\pi_1,\cdots, \pi_N$. For any agent $i\in[N]$, it receives $N-1$ communication messages from other agents, but some of them can be adversarial messages that are perturbed arbitrarily.
Each agent receives no greater than $C$ adversarial messages at every step, among all $N-1$ messages.
The victim agent has no knowledge of which messages are adversarial, and the attacker may attack at different $C$ channels at each step.
% Here $C$ is a constant representing how many communication channels the attacker can manipulate at each step, and it 
Here $C$ is a reflection of the attacker's attacking power, which is usually limited in practice (i.e., $C$ is not too large).
Once the attacker has control over a communication channel (e.g. channel from $j$ to $i$), it is able to arbitrarily change the corresponding messages (e.g. $m_{j \to i}$ can be arbitrarily perturbed).
% Therefore, we consider a strong threat model where the attacker is allowed to send $C$ arbitrary adversarial messages, making it more challenging to design a defense as it has to be a strong defense as well. 
% This threat model is analogous to an $\ell_0$ attack on the policy's input, as detailed in Appendix~\ref{app:theory}.

To obtain theoretically guaranteed robustness, we make the following mild and realistic assumption.
\begin{assumption}
\label{assum:num}
The attacker is able to manipulate less than half of the communication channels, i.e.,
$C<\frac{N-1}{2}$.
% $C<\lfloor\frac{N}{2}\rfloor$. 
% \textcolor{purple}{PH: less than half of the communication channels?}
\end{assumption}
This is a realistic assumption because the attacker in practice usually has limited power, such that controlling the majority of agent communications is less likely. 

\textbf{Various Attack Algorithms}\quad
As formulated above, the attacker can perturb up to $C$ communication messages sent to any agent at every step. 
However, we do not make any assumption on what attack algorithm the attacker uses, i.e., how a message is perturbed. %\textcolor{purple}{PH: how it perturbs a message, or how a message is perturbed? }
In practice, an attacker may randomly change the communication signal, or learn a function to perturb the communication based on the current situation. 
% The attacker can either be white-box or black-box, based on whether it knows the victim agent's policy, as extensively studied in the field of adversarial supervised learning~\cite{chakraborty2018adversarial}. 
To achieve generic robustness under a wide range of practical scenarios, it is highly desirable for a defense to be agnostic to attack algorithms and work for arbitrary (including strongest/worst) perturbations. This is achieved by our defense which will be introduced in Section~\ref{sec:algo}. 
% Therefore, in the next section, we introduce a defense method against adversarial communication, that is provably robust against any attack algorithms which perturb up to $C$ communication messages at each time step. 

\paragraph{Comparison with Other Threat Models}\quad 
Many existing works on adversarial attack and defense assume that the perturbation is small in $\ell_p$ norm. However, there are many realistic attacks that can not be solved by the $\ell_p$ threat model. For example, the attacker may replace a word in a sentence, add a patch to an image, or permute the order of messages. In these cases, the $\ell_p$ distance between the clean value and the perturbed value is large, so that $\ell_p$ defenses do not work.
In contrast, we allow arbitrary perturbations of these $C$ messages for broader application and stronger robustness. 
% This type of limited attacking power assumption is common in adversarial learning, i.e.,  attack with bounded radius in $\ell_p$ norm. 

\textbf{Comparison with Observation Attacks}\quad
Recent study~\cite{huang2017adversarial,gleave2020adversarial,sun2021strongest} has revealed that a well-trained Deep RL policy are vulnerable to adversarial perturbation on the observations.
% test-time evasion attacks. That is, a malicious attacker can significantly reduce the reward of a victim agent by adding crafted 
% small perturbations to the victim's observations. Although most prior works consider observation attacks~\cite{huang2017adversarial,zhang2020robust,sun2021strongest}, it is not always feasible 
% \textcolor{purple}{PH: practical$->$feasible? since we say "in practice" in the same sentence}
However, it is not always feasible for an attacker to change an agent's observation in practice~\cite{gleave2020adversarial}. For example, a robot's observation is often captured by built-in sensors~\cite{pinkava1990towards}, which the attackers may not have access to. 
In contrast, an attacker can eavesdrop on and alter the messages propagated in a communication channel to influence a victim agent's decisions, which is relatively an easier and thus more practical attack than changing an agent's observations that are not easily modifiable. 
More importantly, since an acting policy $\pi$ takes in both its own observation and the communication messages, communication can be regarded as a subset of policy inputs, and thus is related to traditional adversarial defenses of deep neural policies. 
But different from most literature that consider $\ell_\infty$ or $\ell_2$ perturbations on the entire input vector, we focus on the case where a fraction of inputs can be totally corrupted, analogous to an $\ell_0$ attack (sparse attack) model as detailed in Appendix~\ref{app:theory}.
% More importantly, since communication is broadcast 
% \change{in a multi-agent world where agents are usually trained in a centralized way and executed in a decentralized way}\fh{
% in a multi-agent problem where agents expedite learning and make informed decisions through information sharing, adversarial attackers can exploit the vulnerabilities of such information exchange across agents to mislead decision-making.
% In particular, an attacker can eavesdrop on and alter the messages propagated in a communication channel to influence a victim agent's decisions, which is relatively an easier and thus more practical attack than changing an agent's observations that are not easily modifiable. 
% which are usually from sensors that are built in and not easily accessible. 
% A well-known real-world example is cyber attacks to communication channels. 

\textbf{Comparison with Action Attacks}\quad
Note that in a communication attack, the attacker only alters the communication and does not directly change the actions of any agent. Therefore, all agents are still following $\pi_1,\cdots, \pi_N$.
This is different from the multi-agent attacking scenario studied by~\cite{gleave2020adversarial}, where one agent becomes adversarial and behaves differently (i.e., executes a different policy) to attack the victim agent. 
% The communication attack model studied in our paper can be more practical since attacking a communication channel can be more feasible than attacking the observations of a built-in sensor or the policy that is stored in the machine (as described earlier).  
Compared with this type of attack that behaves abnormally to cause performance drop of the victim agent, the communication attack model studied in our paper can be more stealthy and harder to detect, as the other agents do not change their behaviors. For example, if a drone is hacked and controlled by an attacker to behave differently, it is relatively easy for humans to notice the abnormal agent. 
However, it can be hard to recognize adversarial communication signals. For instance, the adversarial messages in Figure~\ref{fig:diagram} look similar to benign messages and can be hard to detect. Furthermore, a learned communication message can be automatically generated by neural networks~\cite{foerster2016learning,tu2021adversarial} and are thus hard for humans to interpret. 
% especially the learned communication \fh{what is learned communication?} which can be uninterpretable.


\ys{Different forms of attacks.
directly perturbing the victim: not always feasible in hardware
attacking the victim via perturbing other agents: change the action of the other agent - influence its own reward. 
}





% % Without loss of generality, we look at a specific agent $i\in [N]$ .
% we suppose that the adversaries an victim agent $x \in [N]$ whose identity is unknown, but the formulation can be easily generalized to multiple victim attacks.
% Suppose there is an attacker manipulating communication messages from a subset of agents $\mathcal{Y}=\{ y_1, \cdots, y_C \}$ to $x$ ($x \notin \mathcal{Y})$, i.e., the attacker can control the communication channels to the victim from up to $C$ agents. \fh{Note that $C$ should be considered as a known hyperparameter, and we will provide more insight later in the paper about how to set $C$ in practice.} 
% As pointed out by some prior works~\cite{zhang2020robust,sun2021strongest}, the \textit{optimal attack} \fh{to an RL policy} can be learned by solving an RL problem:
% % {\small{
% \setlength\abovedisplayskip{-2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:adv_obj}
% \tag{$Q_A$}
% \begin{aligned}
%     \min_{\nu_1,\cdots,\nu_C} & \; \advobj^x :=  \mathbb{E} [ \sum_{t=0}^\infty \gamma^t [R(s\step, a_1\step, \cdots, a_N\step)]_{x} ] \\
%     \text{where } & \; a_i\step = \pi_i(o_i\step, \mtoi\step), \forall i\in [N], t \geq 0 \\
%      & \; m_{y_j \to x}\step = \nu_{j}(o_{y_j}\step), \forall j\in [C], t \geq 0
% \end{aligned}
% \end{equation}
% % }}

% % In other words, the attacker learns $C$ communication policies that collaboratively minimizes the reward of the victim agent $x$.
% The minimizer to Problem~\eqref{eq:adv_obj}, $\nu_1^*,\cdots,\nu_C^*$ , defines an optimal communication attacking strategy that is adaptive to victim $\pi_x$. 
% However, this is a theoretical optimal attack with white-box access to the victim's reward function, while a real-world attacker can be different \fh{unclear} and weaker \fh{this sentence seems to open a big problem that is not explained well. Needs to be reorganized.}.
% In this paper, we propose a provably robust defense that is agnostic to attacking strategies, including the ``optimal'' white-box adaptive attacker learned as Problem~\eqref{eq:adv_obj}.

% For illustration simplicity, we call the $C$ manipulated agents in $\mathcal{Y}$ as \textit{adversarial agents} against victim $x$, because $x$ receives adversarial communication from them \fh{although these manipulated agents can still maintain their own target and reward and execute their optimal acting policy (polish this)}.  
% We can show that the above communication threat model is analogous to an $\ell_0$ attack in the policy's input space, as illustrated in Appendix~\ref{app:theory}.
% Note that the attacker only changes the communication between other agents and the victim agent, while 
% not directly changing the actions of any agent. Therefore, all non-victim agents are behaving normally, different from the change-of-action attacks considered in~\cite{gleave2020adversarial}. 

% \fh{We need to discuss the descriptions of the threat models.}

% \fh{Shall we move the attacks subsection to a seperate section, outside of the problem formulation?}

% \subsection{Goal: Defending against Communication Attacks}
% \label{sec:setup_defense}

% Traditional MARL algorithms optimize the natural reward $\natobj$ without any attacks, as defined in Problem~\eqref{eq:agent_obj}. However, the learned policies are not necessarily robust against adversarial communications. That is, the attacked reward $\advobj$ can be made extremely low under learned attackers solved by Problem~\eqref{eq:adv_obj}, as verified by our experiments in Section~\ref{sec:exp}.

% Motivated by the fact that communication among agents may be noisy, unstable, and vulnerable to attacks, our goal is to train robust acting policies $\{ \pi_i, i \in [N] \}$, such that for any agent, $\natobj$ and $\advobj$ are both high, even when there are up to $C$ communication messages corrupted at every step. 
% More importantly, we aim to provide a defense mechanism and guarantee that the agents will not be significantly misled by adversarial communication messages during test time.

==> cmarl/4_algo_new.tex <==
\section{Provably Robust Defense for CMARL}
\label{sec:algo}

In this section, we present our defense algorithm, \textit{\oursfull (\ours)}, against test-time communication attacks in CMARL. 
% We first define some notations used throughout the paper and a key assumption for the robustness guarantee to hold. Then, we 
We first introduce the main idea of the algorithm in Section~\ref{sec:algo_overview}.
Then, in Section~\ref{sec:algo_dist} and Section~\ref{sec:algo_cont}, we provide detailed methodology and theoretical analysis for \ours robust policies in discrete action spaces and in continuous action spaces, respectively.
Section~\ref{sec:algo_partial} further extends the \ours algorithm by introducing a hyper-parameter for more efficient implementation in larger-scale problems, with corresponding theoretical guarantees.
\ys{generalize to decision making}

% For notation simplicity and with a little abuse of notation, 
% % we assume that there are $N+1$ agents in total, so that every agent can communicate with $N$ other agents in every step.
% assume all $N$ agents have identical observation space, action space and message space denoted as $\mathcal{O}, \mathcal{A}$ and $\mathcal{M}$. So that the joint observation/action/message space is $\mathcal{O}^{N}$/$\mathcal{A}^{N}$/$\mathcal{M}^{N}$.
% As is common is MARL~\cite{foerster2016learning}, we learn a single policy network that is shared across all agent. But note that this setting is only for illustration simplicity, our algorithm applies to heterogeneous agents with multiple policies.

\subsection{\oursfull (\ours): An Overview}
\label{sec:algo_overview}

% \SF{In the intro, we call the method ensemble policy; we should use the same terminology. I like AME} >> Sure, I added AME to the intro.
As characterized in Section~\ref{sec:setup}, in a CMARL game, every agent makes decisions based on not only its own observations, but also all received messages. If an agent trusts the communication from all other agents, it may fail when some communication is maliciously corrupted.
On the other hand, if an agent does not trust communication, it can not benefit from the useful information shared by other benign agents.
Therefore, there is a trade-off between natural performance (i.e., reward under no attack) and robustness (i.e., reward under attacks).
Our goal is to learn and execute a robust policy for any agent in the environment, so that the agent can perform well in both a non-adversarial environment and an adversarial environment.


% Traditional MARL algorithms optimize the natural reward $\natobj$ without any attacks, as defined in Problem~\eqref{eq:agent_obj}. However, the learned policies are not necessarily robust against adversarial communications. That is, the attacked reward $\advobj$ could be made extremely low under learned attackers solved by Problem~\eqref{eq:adv_obj}, as verified by our experiments in Section~\ref{sec:exp}.

% Motivated by the fact that communication among agents may be noisy, unstable, and vulnerable to attacks, our goal is to train robust acting policies $\{ \pi_i, i \in [N] \}$, such that for any agent, $\natobj$ and $\advobj$ are both high, even when there are up to $C$ communication messages corrupted at every step. 
% More importantly, we aim to provide a defense mechanism and guarantee that the agents will not be significantly misled by adversarial communication messages during test time.

\textbf{Main Idea}\quad
Intuitively, if an agent $i$ overly relies on the information given by agent $j$, then a strong adaptive attacker can easily mislead $i$ by perturbing the messages from $j$.
Moreover, the benign messages sent from other agents usually contain redundant/overlapping information.
% \myst{, as the goal of communication is to provide the agent additional information and to help the agent make better decisions. }
At each step, an agent receives a set of $N-1$ messages from all other agents, called a \emph{message set}.
% and the set has $N-1$ elements, each is a message received. 
The main idea of our defense is to make decisions based on multiple random subsets of the message set, called \emph{randomly-ablated message samples (or m-samples for short)}.
Under a carefully designed ablation mechanism, benign m-samples can outweigh malicious ones.
To be more specific, we propose to train a \emph{base policy} that makes decisions with one 
% \myst{randomly selected subset of the message set} 
m-sample at each step. 
Then, during test-time, the agent generates multiple m-samples at every step.
% One can design an ablation strategy which guarantees that a majority number of these m-samples contain no malicious messages.
Then the agent applies the trained base policy to  
% \myst{randomly ablated messages, and aggregate the base-policy actions by sampling multiple message combinations, so that the agent can make safe decisions with theoretical guarantees.}
each of these m-samples, getting multiple resulting actions where the majority of them are generated based on benign messages only. 
% The majority of these resulting actions are based on benign messages only and thus safe. 
Therefore, the agent is guaranteed to make a ``safe'' decision if it takes a collection of wisdom from the ensemble of all resulting actions, since the majority of these resulting actions are guaranteed to be guided by benign messages.
% \fh{Made lots of changes here. Can you check whether they are correct?}



A similar randomized ablation defense is used to defend against $\ell_0$ attacks in image classification~\cite{Levine_Feizi_2020}. 
% However, reinforcement learning is fundamentally different from image classification. 
But our defensive mechanism is fundamentally different from the method by~\cite{Levine_Feizi_2020} which provides a high-probability guarantee for discrete image label outputs, as our defense achieves both action and long-term reward certification (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output, which is non-trivial.
% \fh{Our proposed defensive mechanism is a non-trivial extension of the randomized ablation in image classification, as defenses in MDPs requires action certification as well as reward certification whereas defenses in image classification only requires label certification. (This description does not quite clearly explain why MDPs are much harder...)}



\textbf{Notations}\quad
\textbf{(1) Ablation function.} For a list $\mathbf{m}$ and a set of $k$ indices $T=\{j_1,j_2,\cdots,j_k\}$, define an \emph{ablation function} which removes all elements except for those in $T$: $\funabl(\mathbf{m}, T) = [m_{j_1}, \cdots, m_{j_k}]$.
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
%     \funabl(\mathbf{m}, T) = [m_{j_1}, \cdots, m_{j_k}].
% \end{equation}
\textbf{(2) Size-$k$ power subset.} For an integer $n>0$ and the index set $[n]:=\{1,\cdots,n\}$, let $\mathcal{H}(n,k)$ denote the set of all unique $k$ indices out of $[n]$, referred as size-$k$ power subset of $[n]$. That is, $\mathcal{H}(n,k)$ contains all size-$k$ elements in the power set of $[n]$, and thus  $|\mathcal{H}(n,k)|=\binom{n}{k}$. 
% \textcolor{purple}{PH: We have $T$ as the observation omission prob in Sec 2.1, and here as a set of indices. Perhaps we should change the one in Sec 2.1? YS: yes, indeed, I changed it to B}
% \textbf{(2) Power subset. \fh{what's the right terminology?}} For an integer $n>0$ and the indices set $[n]:=\{1,\cdots,n\}$, let $\mathcal{H}(n,k)$ denote the set of all unique $k$ indices out of $[n]$ \fh{known as power subset of size $k$}. That is, $\mathcal{H}(n,k)$ contains all \fh{sized $k$} subsets of $[n]$ \textcolor{red}{with cardinalities $k$} and thus  $|\mathcal{H}(n,k)|=\binom{n}{k}$.  
% Define $\mathcal{U}(n,k)$ as the uniform distribution over $\mathcal{H}(n,k)$. 
% \textbf{(3) \fh{A name for this?}} We let $\krv_{k,n}=\{j_1, j_2,...,j_k\}$ be a random variable taking values on the uniform distribution over $\mathcal{H}(n,k)$. \fh{Intuitively, $\funabl(\mathbf{m}, \krv_{k,n})$ denotes selecting a subset of messages indexed by a random realization $T$ of $\krv_{k,n}$, i.e. $\funabl(\mathbf{m}, T)$ where $T$ is a sized-$k$ index set drawn from $\krv_{k,n}$.} \fh{The problem is that we never defined $\funabl(input-1, input-2)$ when $input-2$ is not a set of indices, but rather a random variable.}
% over $\mathcal{U}(n,k)$. 

With the above intuition and notations, we introduce \ours, a generic defense framework that can be combined with any MARL algorithm with communication.
The training and defending strategies of \ours are provided in Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test}, respectively. 
% Note that the proposed defense is a generic framework that can be combined with any MARL algorithm. 
% Next, we explain the detailed design of these two algorithms. The training and executing procedures for all agents are identical, so we omit the subscript ${}_i$ of policies.

\textbf{Training a Base Ablation Policy $\boldsymbol\ablpolicy$ (Algorithm~\ref{alg:train})}\quad
During training time, every agent learns an \textit{ablation policy} $\ablpolicy_i: \mathcal{O}_i \times \mathcal{M}^k \to \mathcal{A}_i$ which maps an observation and $k$ messages to an action. Here $k$ is a user-specified hyperparameter satisfying
% in order for a successful defense against up to $C$ malicious messages:
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
    \label{eq:k_cond}
    \binom{N-1-C}{k} \geq \frac{1}{2} \binom{N-1}{k}.
\end{equation}
We will explain later that Equation~\eqref{eq:k_cond} plays an important role in our robustness guarantees (Theorem~\ref{thm:main_dist} \& Theorem~\ref{thm:main_cont}) for a successful defense against up to $C$ malicious messages.
% \fh{We will provide more details including the reasoning of such required condition for the choice of $k$ in Section~\ref{?}.} \fh{(Shall we talk about the selection of $k$ somewhere? )}
Note that all agents communicate according to the environment's communication protocol $F$, and attacks do not exist during training.
In every step, an agent randomly samples $k$ out of $N-1$ communication messages, and uses its current acting policy $\ablpolicy$ to react to its current observation and the selected $k$ messages (Line 7 in Algorithm~\ref{alg:train}).
That is, for agent $i$, we optimize and make decisions via $\ablpolicy_i(o_i, \mathsf{Ablate}(\mtoi, T))$, where $\mathsf{Ablate}(\mtoi, T)$ denotes the selected $k$ messages sent from other agents to agent $i$. 
\ys{communication being symmetric}
% and $\ablpolicy_i(o_i, \mathsf{Ablate}(\mtoi, T))$ returns the action the agent $i$ takes according to its current policy.
%$T$ is a random collection of $k$ indices out of $[N-1]$.
% $\krv_{k,N-1}$ is a random collection of $k$ indices out of $[N-1]$. \fh{Then, $\funabl(\mathbf{m}, \krv_{k,n})$ denotes selecting $k$ of the $N$ messages in $\mathbf{m}$ indexed by a set that is a random drawn of $\krv_{k,n}$.} 

% The ablation policy $\ablpolicy$ is trained in a normal environment without any attacks. But we will show that $\ablpolicy$ can be used to defend against test-time communication attacks with theoretical certification. 

\input{algo_train}
\input{algo_test}

\textbf{Defending with an Ensemble Policy $\boldsymbol\smpolicy$ (Algorithm~\ref{alg:test})}\quad
Once we have learned a reasonable ablation policy $\ablpolicy_i$ for agent $i$, we can execute it with ablation and aggregation during test time to defend against adversarial communication. 
Recall that there are up to $C$ malicious messages out of $N-1$ total messages, so the remaining $N-1-C$ messages are benign.
The defense objective is to make a \textit{safe decision} that is robust to malicious massages. 
The main idea is to sample multiple different message subsets out of all $N-1$ received messages, and to select an action suggested by the majority of those message subsets. 
$\smpolicy_i: \mathcal{O}_i \times \mathcal{M}^{N-1} \to \mathcal{A}_i$ is an \textit{ensemble policy} that outputs an action by aggregating the ablation policy's base actions on multiple message subsets (Line 5 in Algorithm~\ref{alg:test}).
The concrete definition of $\smpolicy_i$ depends on whether the action space $\mathcal{A}_i$ is discrete or continuous, which will be detailed in Section~\ref{sec:algo_dist} and Section~\ref{sec:algo_cont}, with corresponding theoretical guarantees on actions and rewards.
% \textcolor{purple}{PH: would it help mentioning $\smpolicy_i: \mathcal{O}_i \times \mathcal{M}^{N-1} \to \mathcal{A}_i$?}



\subsection{\ours in Discrete Action Space}
\label{sec:algo_dist}


Next, we provide the implementation of ensemble policy used in \ours and the corresponding theoretical robustness guarantees for agent $i$ when $\mathcal{A}_i$ is discrete. 
For notation simplicity, we only focus on one agent (although our defense works for multiple agents) and omit the subscript $i$. We further use $\mathbf{m}$ to denote the message list $\mtoi$ received by the current agent at the current step.
% At each step, an agent receives a \emph{message set} with $N-1$ elements, each being a message received. 
Our defense is to make decisions based on multiple size-$k$ random subsets of all messages in $\mathbf{m}$. 

% Recall that $\{ \funabl(\mathbf{m}, T_d)\}_{d=1}^D$ are $D$ different size-$k$ message subsets sampled from the $N-1$ received messages. 
% In a discrete action space, we define the \textit{ensemble policy} $\tilde{\pi}$ as below.

\begin{definition}[\textbf{Ensemble Policy for Discrete Action Space}]
\label{def:ensemble_dist}
For a trained ablation policy $\ablpolicy$, define $u_a$ as the number of times/votes such that the ablation policy $\ablpolicy$ renders action $a$ when taking each of the $\binom{N-1}{k}$ number of message subsets, i.e.,
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
\label{eq:vote}
    u_a := \sum\nolimits_{T\in\mathcal{H}(N-1,k)} \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T))=a].
\end{equation}
Then the ensemble policy $\smpolicy$ takes the action $\widetilde{a}$ which has the most votes, i.e.,
\begin{equation}
\label{eq:ensemble_pi_dist}
    \widetilde{a} = \smpolicy(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \; u_a
\end{equation}
% \fh{How about $\tilde{a} = \smpolicy\Big(o, \{\funabl(\mathbf{m}, T_d)\}_{d=1}^D\Big) := \mathrm{ argmax}_{a\in\mathcal{A}} \; u_a.$?}
\end{definition}
\textbf{Remarks.}
(1) The ensemble policy $\smpolicy$ takes the action suggested by the majority-vote of all size-$k$ message subsets. There are $\binom{N-1}{k}$ number of such size-$k$ subsets in total.
(2) In many practical multi-agent problems, $N$ is not very large, e.g., the number of drones in an area. Therefore, $\binom{N-1}{k}$ is relatively small and not expensive to compute. For example, when $N=10,k=2$, $\binom{N-1}{k}=36$.
% \fh{And we can defend against up to $C=?$ malicious messages.
% I added it to the discussion on ablation size k.
(3) In the case where $\binom{N-1}{k}$ is large, we also provide a variant of the algorithm which takes $D<\binom{N-1}{k}$ samples of message subsets whose certification guarantee is provided in Section~\ref{sec:algo_partial}.

At any step, let $o$ be the observation, $\goodmsg$ and $\advmsg$ be the benign message list before attack and the corrupted message list after attack, respectively.
% $\goodmsg$ be the benign messages (before attack), and $\advmsg$ be the messages after attack (with up to $C$ messages being corrupted). 
Note that $\goodmsg$ and $\advmsg$ both have $N-1$ messages while they differ by up to $C$ messages. 
With the above notation, we define a set of actions rendered by pure-benign message subsets in Definition~\ref{def:safeact_dist}. As the agent is likely to take these actions in a non-adversarial environment, they can be regarded as safe actions to take. 
\begin{definition}[Benign Action Set $\safeaction$]
\label{def:safeact_dist}
For any step, define $\safeaction \subseteq \mathcal{A}$ as a set of actions that $\ablpolicy$ may select under randomly sampled benign messages.
\begin{equation}
\label{eq:safeact_dist}
     \safeaction := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}
\end{equation}
\end{definition}


Next, we provide both action certificate and reward certificate for the above ensemble policy $\smpolicy$.

\textbf{Action Certificate}\quad
% $\safeactiondist \subseteq \mathcal{A}$ is a set of actions that $\ablpolicy$  may select at the current step under randomly sampled benign messages.
The following theorem suggests that the ensemble policy $\smpolicy$ always takes benign actions in $\safeaction$ under mild conditions, even when malicious information is present in the input.

% In this case, the following theorem suggests that the ensemble policy $\smpolicy$ is not influenced by the malicious messages under mild conditions.

\begin{theorem}[Action Certificate for Discrete Action Space]
\label{thm:main_dist}
% Assume that subset size $k$  and ensemble policy $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. 
Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees benign actions under $\advmsg$, i.e.,
\begin{equation}
    \widetilde{a} = \smpolicy(o, \advmsg) \in \safeaction,
    \label{eq:cert_dist}
\end{equation}
if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% where 
% \begin{equation}
%     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% \end{equation}
\end{theorem}
\textbf{Remarks.}
(1) Theorem~\ref{thm:main_dist} certifies that for every step of execution, $\smpolicy$ selects a benign action when the agent receives $\advmsg$ with up to $C$ malicious messages. 
% \fh{Is there a specific reason why we emphasize one step? Should the certification certify every step? Is it possible that the actions appears safe for this round, but not safe for the next round? Oh, maybe the concept of safe already guarantees long-term safety? I feel the emphasis on current-step may cause confusion. We either need to talk about this current-step guarantees long-term safety or we just talk about long-term safety without mentioning current-step?} 
(2) The condition $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ is easy to satisfy when $C \ll N$. This condition accounts for the worst-case scenario when the adversarial messages collaborate to vote for an unsafe action and outweigh benign messages in all base policies. 
But such a worst-case scenario is uncommon in practice, so our algorithm makes the agents robust without requiring this condition of $u_{\widetilde{a}}$, as verified in experiments. 
  
\textbf{Reward Certificate}\quad
Theorem~\ref{thm:main_dist} justifies that under sufficient majority votes $u_{\tilde{a}}$, the ensemble policy $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a benign action that is suggested by some benign message combinations even when the malicious messages are not identified.
Therefore, the ensemble policy $\smpolicy$'s action in every step falls into a benign action set, and thus its cumulative reward under adversarial communications is also guaranteed to be no lower than the worst natural reward the base policy $\ablpolicy$ can get under random benign message subsets. The detailed reward certification is shown in Corollary~\ref{cor:reward_dist} in Appendix~\ref{app:theory_dist}.

\textbf{Discussion on Ablation Size $\boldsymbol k$}\quad 
As an essential condition for the above certificates to hold, Equation~\eqref{eq:k_cond} implies that among all size-$k$ message subsets, there are more purely benign subsets than subsets that contain adversarial messages. This condition always has solutions for $k$ as $C<\frac{N-1}{2}$, and $k=1$ is always a feasible solution. In general, if $k$ is smaller, the ensemble policy is more robust. However, the base ablation policy with a smaller $k$ could gain lower reward as it throws away many messages. Therefore, there is a trade-off between robustness and accuracy, as is pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}.
In practice, if we know $C$ in advance, we can set $k$ to be the largest integer satisfying Equation~\eqref{eq:k_cond}. On the other hand, if $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Equation~\eqref{eq:k_cond}, which shows how many adversarial messages the policy can tolerate. 
For example, when $N=10$, \ours can tolerate up to $C=4$ with $k=1$, and up to $C=2$ with $k=2$. 
Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Equation~\eqref{eq:k_cond}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages, and when $C$ is small, we can use a larger $k$ such that the natural performance is not compromised much.
% 

\subsection{\ours in Continuous Action Space}
\label{sec:algo_cont}

In this section, we introduce the implementation of ensemble policy in \ours and the robustness guarantees in an $L$-dimensional continuous action space. 
Instead of majority voting that is used in a discrete action space, we now use the median statistics to make a robust decision. Define a median function $\funmed$ such that $\funmed(\mathbf{g})$ returns the median value of a list $\mathbf{g}$. If $\mathbf{g}$ is a list of $L$-dimensional vectors, then $\funmed(\mathbf{g})$ returns the element-wise median value, which is also an $L$-dimensional vector.

% \textbf{Additional Notations}\quad
% For any random variable $X$ and a real-valued function $f(X)$, define the median function $\funmed_{X}(f(X))$ as 
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
% \label{eq:med}
% \funmed_{X}(f(X)) := \inf \{ c\in\mathbb{R}: \mathbb{P}_X [ f(X) \geq c ] \geq 0.5 \}.
% \end{equation*}
% For a vector-valued function $F = [f_1(X), \cdots, f_l(X)]^\top$, the $\funmed$ function is extended as the element-wise median value, i.e.,
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation*}
% \label{eq:med_func}
% \funmed_{X}(F(X)) = [\funmed_{X}(f_1(X)), \cdots, \funmed_{X}(f_l(X))]^\top.
% \end{equation*}


In a continuous action space, the ensemble policy $\smpolicy$ takes the median of base actions resulting from all message samples.
% \textcolor{purple}{PH: is this in the right place?  We introduce $D$ later in the section 3.4. Or do we mean to say: ... $\smpolicy$ takes the median of actions resulting from all ablated message samples of size $k$? }
\begin{definition}[\textbf{Ensemble Policy for Continuous Action Space}]
\label{def:ensemble_cont}
For a trained ablation policy $\ablpolicy$, define the ensemble policy $\smpolicy$ as
\begin{equation}
\label{eq:ensemble_pi_cont}
    \tilde{\pi}(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T): T\in\mathcal{H}(N-1,k) \}.
\end{equation}
% \small
% %\vspace{-1.5em}
% \textcolor{red}{
% \begin{equation}
% \label{eq:ensemble_pi_cont}
%     \tilde{\pi}(o, \mathbf{m}, \{T_d\}_{d=1}^D) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% }
% \fh{
% \begin{equation}
%     \resizebox{0.88\columnwidth}{!}{$\smpolicy\Big(o, \{\funabl(\mathbf{m}, T_d)\}_{d=1}^D\Big) =\funmed \Big(\{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D\Big)\label{eq:ensemble_pi_cont}.$}
% \end{equation}
% }
\end{definition}

% \vspace{-1em}
\textbf{Action Certificate}\quad
As in the discrete action case, the continuous ensemble policy will output an action $\widetilde{a}$ that follow the consensus of benign messages. But in a continuous action space, it is hard to ensure that $\widetilde{a}$ is exactly in $\safeaction$. Instead, $\widetilde{a}$ is guaranteed to be within the range of $\safeaction$, as detailed in the following theorem.

\begin{theorem}[Action Certificate for Continuous Action Space]
\label{thm:main_cont}
Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees benign actions under $\advmsg$, i.e.,
\begin{equation}
    \smpolicy(o, \advmsg) \in \mathsf{Range}(\safeaction) := \{a: \forall 1\leq l \leq L, \exists \underline{a}, \overline{a} \in \safeaction \text{ s.t } \underline{a}_l \leq a_l \leq \overline{a} \}.
    \label{eq:cert_cont}
\end{equation}
% then any dimension $l$ of $\smpolicy$'s output satisfies
% \begin{equation*}
%     \inf_{\krv} [\hat{a}]_l  
%     \leq [\smpolicy(o, \advmsg, \{T_d\}_{d=1}^D)]_l 
%     \leq \sup_{\krv} [\hat{a}]_l.
% \end{equation*}
% where $\hat{a} := \ablpolicy(o, \mathsf{Ablate}(m, \krv))$.
\end{theorem}

$\mathsf{Range}(\safeactioncont)$ is a set of actions that are coordinate-wise bounded by base actions resulted from pure-benign m-samples. It is reasonable to assume that actions in $\mathsf{Range}(\safeactioncont)$ are relatively safe. For example, if the action denotes the price a seller sells its product in a market, and the communication messages are the transaction signals in an information pool, then $\mathsf{Range}(\safeactioncont)$ is a price range that is determined based on uncorrupted messages. Therefore, the seller will set a reasonable price without being influenced by a malicious message. 


\textbf{Reward Certificate}\quad
Theorem~\ref{thm:main_cont} shows how the ensemble policy outputs an action that is coordinate-wisely bounded by the range of benign actions. Under mild assumptions, it can also lead to a reward guarantee, as detailed in Appendix~\ref{app:theory_cont}.

\subsection{Extension of \ours: Ensemble with Partial Samples}
\label{sec:algo_partial}

So far we have discussed the proposed \ours algorithm and the constructed ensemble policy that aggregates all $\binom{N-1}{k}$ number of message subsets out of $N-1$ messages. 
However, if $N$ is large, sampling all $\binom{N-1}{k}$ combinations of message subsets could be expensive. In this case, a smaller number of message-subset combinations can be used. That is, given a sample size $0<D\leq\binom{N-1}{k}$, we randomly select $D$ samples $\{T_d\}_{d=1}^D$ from $\mathcal{H}(N-1,k)$ (without replacement), and then we aggregate the ablation policy's decision on $\{\funabl(\mathbf{m}, T_d)\}_{d=1}^D$. 
In this way, we define a sampled version of the ensemble policy, namely \textit{$D$-ensemble policy} $\smpolicy_D$, formulated as below.
% , whose detailed definition is provided in Appendix~\ref{app:theory_sample}.
% define the $D$-ensemble policy $\smpolicy_D$ as the sampled version of $\smpolicy$
\begin{equation}
\label{eq:ensemble_pi_dist_d}
    \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
\end{equation}
for a discrete action space, and
\begin{equation}
\label{eq:ensemble_pi_cont_d}
    \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
\end{equation}\normalsize
for a continuous action space. 



In this case, we can still provide a high-probability robustness guarantee. Theorem~\ref{thm:sample_cont} shows the theoretical result for a continuous action space, while the result for a discrete action space is slightly different and is provided in Appendix~\ref{app:theory_sample}.
% in Theorem~\ref{thm:sample_dist} and Theorem~\ref{thm:sample_cont}. 

\begin{theorem}[General Action Guarantee for Continuous Action Space]
\label{thm:sample_cont}
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$,  under Assumption~\ref{assum:num}, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_cont_d} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, relation~\eqref{eq:cert_cont} holds with probability at least
\begin{equation}
\label{eq:p_sample_cont}
    p_D=\frac{\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n_1-n_2}{D-j}}{\binom{n_1}{D}},
\end{equation}
where $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$ and $\tilde{D} = {\lfloor \frac{D}{2} \rfloor}+1$. 
\end{theorem}
Therefore, for an arbitrary $D$, a benign action will be selected with high probability. The larger $D$ is, the higher the probability is. 
In Theorem~\ref{thm:sample_cont}, when $D=\binom{N-1}{k}$,  the probability $p_D$ is 1 and the result matches Theorem~\ref{thm:main_cont}. 
Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.


\subsection{More Discussion on Applicability and Flexibility of \ours}

\ys{general for any RL policy or decision-making model}

\ys{how a policy is trained}



\ys{training and testing hyperparameters}



==> cmarl/5_exp.tex <==
\section{Empirical Study}
\label{sec:exp}

\textbf{Environment Setup: FoodCollector}\quad
We design and implement a 2D particle environment named FoodCollector, adapted from the WaterWorld environment in PettingZoo~\cite{terry2020pettingzoo}. 
There are 9 agents (colored dots surrounded by black lines) relying on sensors (black lines around agents) to observe the world. Each agent's goal is to find the food (colored large dots) of the same color as itself, and avoid collision with poisons (black dots).
The action space can be either (1) discrete, with 9 actions including 8 moving directions and 1 no-move action, or (2) continuous, where the action is an acceleration decision, denoted by a 2-dimensional real-valued vector.
Due to the limited sensory range, each agent can only see the objects around it, and thus communication is helpful. We use a pre-defined protocol where agents share their observed food with each other. Figure~\ref{fig:food}(right) verifies the advantage of communication in FoodCollector. More details of the environment and the communication settings are shown in Appendix~\ref{app:exp_env}.



\textbf{Evaluation}\quad
To evaluate the effectiveness of our defense strategy, we seek to evaluate the performance of the ensemble policy under no attack and under various values of $C$ (for simplicity, we refer to $C$ as the \textit{number of adversaries}). 
Different from previous work~\cite{blumenkamp2020emergence} where the adversarial agent disrupts all the other agents, we consider the case where the attacker deliberately misleads a selected victim, which could evaluate the robustness of the victim under the harshest attacks. 
We use the following two attack methods:
(1) \textbf{non-adaptive attack} that randomly generates a message. Note that this is already a strong attack since a randomly generated message could be arbitrary and far from the original benign message;
% random attacks \fh{random looks too weak, can we justify this is a good attack? Can we give a better name to it?} 
(2) \textbf{learned adaptive attack} that learns the strongest/worst adversarial communication with an RL algorithm to minimize the victim's reward (a white-box attacker which knows the victim's reward). The learned attack can strategically mislead the victim (e.g., to a poison).
As shown in prior works~\cite{zhang2020robust,zhang2021robust,sun2021strongest}, the theoretically optimal attack (which minimizes the victim's reward) can be formed as an RL problem and learned by RL algorithms. 
We can regard this attack as a worst-case attack for the victim agents.
% Therefore, we train an RL attacker policy that maps adversarial agent's observations to adversarial communications. 
More details are in Appendix~\ref{app:exp_imple}.

\textbf{Implementation and Baselines}\quad
We compare our \ours with two baselines: (1) \textbf{(Vanilla)} vanilla training which learns a policy based on all benign messages. (2) \textbf{(AT)} adversarial training as in~\cite{zhang2021robust}, which alternatively trains an adaptive RL attacker and an agent. 
As is common in related work~\cite{lowe2017multi,gupta2017cooperative}, we use parameter sharing and train a shared policy network for all agents.
Our \ours and baselines are all trained with PPO~\cite{schulman2017proximal}, and more implementation details are provided in Appendix~\ref{app:exp_imple}.

\begin{figure}[t]
\vspace{-0.5em}
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{figs/foodcollector.png}
        \vspace{-0.5cm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figs/comm_dist_small}}
        \vspace{-0.5cm}
    \end{subfigure}
\vspace{-1em}
\caption{\textbf{Left:} The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. 
\textbf{Right:} Reward of agents trained with communication v.s. without communication in a discrete action space. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly. The result in a continuous action space is similar, as presented in Appendix~\ref{app:exp_env}.}
\label{fig:food}
\vspace{-1.5em}
\end{figure}

% \paragraph{Random Attacks} xxx

% \paragraph{Heuristic Attacks} xxx

% \paragraph{Optimal Attacks} Suppose there is an attacker manipulating communication messages from a subset of agents $\mathcal{Y}=\{ y_1, \cdots, y_C \}$ to $x$ ($x \notin \mathcal{Y})$, i.e., the attacker can control the communication channels to the victim from up to $C$ agents. \fh{Note that $C$ should be considered as a known hyperparameter, and we will provide more insight later in the paper about how to set $C$ in practice.} 
% As pointed out by some prior works~\cite{zhang2020robust,sun2021strongest}, the \textit{optimal attack} \fh{to an RL policy} can be learned by solving an RL problem:
% % {\small{
% \setlength\abovedisplayskip{-2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:adv_obj}
% \tag{$Q_A$}
% \begin{aligned}
%     \min_{\nu_1,\cdots,\nu_C} & \; \advobj^x :=  \mathbb{E} [ \sum_{t=0}^\infty \gamma^t [R(s\step, a_1\step, \cdots, a_N\step)]_{x} ] \\
%     \text{where } & \; a_i\step = \pi_i(o_i\step, \mtoi\step), \forall i\in [N], t \geq 0 \\
%      & \; m_{y_j \to x}\step = \nu_{j}(o_{y_j}\step), \forall j\in [C], t \geq 0
% \end{aligned}
% \end{equation}
% % }}
% \fh{ I tried to move something, but may not be complete and logic needs to be straightened out.}


% The minimizer to Problem~\eqref{eq:adv_obj}, $\nu_1^*,\cdots,\nu_C^*$ , defines an optimal communication attacking strategy that is adaptive to victim $\pi_x$. 
% In other words, the attacker learns $C$ communication policies that collaboratively minimizes the reward of the victim agent $x$.



\textbf{Experiment Results}\quad
As shown in Figure~\ref{fig:res_all}, the rewards of Vanilla and AT drastically drop under attacks, especially adaptive attackers. %(A random agent can gain reward -80.)
We find that AT does not achieve better robustness than Vanilla, since malicious messages can appear at any channel, and it is hard for AT to learn a general defense strategy, as explained in Appendix~\ref{app:exp_imple}.
% becomes too conservative as it is trained to adapt to adversarial messages from multiple channels, i.e., AT does not trust any communication, as detailed in Appendix~\ref{app:exp_imple}.
% , and thus AT cannot utilize well the benign messages.
% does not outperform Vanilla under communication attacks, because there are many communication channels and it is hard for the agent to adapt to all communication attacks.
% Note that the lowest possible reward in this environment is about -100, so in the discrete action case, 2 adaptive adversarial messages can already reduce the reward of Vanilla and AT to the lowest level.
In contrast, we use $k=2$ for our \ours, which provides performance guarantees against up to $C=2$ adversaries. We can see that the reward of \ours under $C=1$ or $C=2$ is similar to its reward under no attack, matching our theoretical analysis. 
The high performance of \ours verifies that it can utilize benign communication well while being robust to adversarial communication.
In both discrete and continuous action spaces, \ours achieves a significantly better performance than Vanilla and AT under various numbers of adversaries, even under 3 adversaries where the theoretical guarantees no longer hold. Therefore, \textit{\ours makes agents robust under varying numbers of adversaries.} 

\input{fig_food_res}

\input{fig_food_k_dist} 

% \textbf{Hyper-parameter Tests}\quad 
% % \ours requires a hyper-parameter $k$  which controls how many messages the base ablation policy relies on to output a base action. The partial-sample variant of \ours introduced in Section~\ref{sec:algo_partial} requires another hyper-parameter $D$, the number of message subset samples the ensemble policy uses. 
% To evaluate the effects of two hyper-parameters $k$ (ablation size) and $D$ (sample size, only used for partial-sample \ours introduced in Section~\ref{sec:algo_partial}), we train \ours with different $k$'s and $D$'s and plot the results in Figure~\ref{fig:res_k_dist} for discrete-action FoodCollector, and Figure~\ref{fig:res_k_cont} for continuous-action FoodCollector (in Appendix~\ref{app:exp_res}).
% \\
\textbf{Hyper-parameter Test of Ablation Size $\boldsymbol k$}\quad
As discussed in Section~\ref{sec:algo_dist}, the value of $k$ is related to the trade-off between natural performance and robustness. To see how $k$ influences the agent's performance, we evaluate \ours's natural reward and \ours's reward under $2$ adaptive adversaries with different ablation sizes $k$. The result in discrete-action FoodCollector is shown in Figure~\ref{fig:res_k_dist}(left), while the continuous-action result is similar and is in Appendix~\ref{app:exp_res}. We can see that increasing the ablation size $k$ improves the natural performance of the agent since each agent could gather more information from others. However, raising the ablation size $k$ also increases the risk of making decisions based on communication messages sent from an adversary. Therefore, \textit{increasing ablation size $k$ trades off robustness for natural performance.} 

\textbf{Hyper-parameter Test of Sample Size $\boldsymbol D$}\quad
We further evaluate the partial-sample variant of \ours introduced in Section~\ref{sec:algo_partial} using $k=2$ under $2$ adaptive adversaries, with $D$ varying from 28 (the largest sample size) to 1 (the smallest sample size). Figure~\ref{fig:res_k_dist}(right) shows the result in a discrete action space, and the continuous-action result is in Appendix~\ref{app:exp_res}. As $D$ goes down, \ours obtains lower reward under attackers, but it is still significantly more robust than baseline methods, even when $D=1$ where the agent makes decisions based on only 1 random message subset.

% Note that when $C=2$, the maximum $k$ such that our certificates hold is 2, according to Inequality~\eqref{eq:k_cond}. Figure~\ref{fig:res_k_dist} shows that, when $k$ increases from $1$ to $2$, the robust performance barely drops, which verifies again the effectiveness of our theoretical guarantees. In practice, to decide the ablation size $k$, we suggest first to estimate the number of attackers that one would like to defend and then choose the maximum $k$ satisfying the condition in Eq~\eqref{eq:k_cond} such that Theorem \ref{thm:main_dist} or \ref{thm:main_cont} hold.


% \begin{figure}[t]
% % \vspace{-0.1cm}
%  \centering
%  \hspace{-1em}
%  \begin{subfigure}[t]{0.42\columnwidth}
%   \input{figs/FoodCollector_Attacker_Dist}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.45\columnwidth}
%   \input{figs/FoodCollector_Ablation_k_2adv_dist}
%  \vspace{-1.5em}
%  \subcaption{Discrete Action Space} 
  
%  %\vspace{0.2cm}
%  \centering
%  \hspace{-1em}
%  \begin{subfigure}[t]{0.42\columnwidth}
%   \input{figs/FoodCollector_Attacker_Cont}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.45\columnwidth}
%   \input{figs/FoodCollector_Ablation_k_2adv_cont}
%  \end{subfigure}
%  \vspace{-1.5em}
%  \subcaption{Continuous Action Space}
% % \vspace{-0.5em}
% \caption{\textbf{Left}: Average return under different number of attackers for our Randomized Ablation defensive method against Adversarial Training and Vanilla Training. \textbf{Right}: Tradeoff between clean and robust performance through ablation size $k$}
% \vspace{-0.5em}
% \label{fig:n_attacker}
% \end{figure}

% \begin{figure}[h]
% \vspace{-0.2cm}
%  \centering
%  \begin{subfigure}[t]{1\columnwidth}
%  \centering
% \input{figs/FoodCollector_Ablation_k_2adv_dist.tex}
% \vspace{-0.2cm}
% \subcaption{Discrete Action Space}
% \end{subfigure}
% %\hfill
% \begin{subfigure}[t]{1\columnwidth}
%  \centering
% \input{figs/FoodCollector_Ablation_k_2adv_cont.tex}
% \vspace{-0.2cm}
% \subcaption{Continuous Action Space}
% \end{subfigure}
% \vspace{-0.4cm}
% \caption*{Tradeoff between clean and robust performance through ablation size $k$}
% \vspace{-0.3cm}
% \label{fig:ablation_k}
% \end{figure}


% \textbf{Increasing ablation sample size $D$ results in higher certification probability, which leads to higher robust performance}

% In the previous experiments, we used the full-sample ablation, i.e. $D=\binom{N-1}{k}$. However, in practice when the number of agents is large, it becomes too computationally expensive to compute all $\binom{N-1}{K}$ ablation combinations. In this case, theorem \ref{thm:main_cont} and \ref{thm:main_dist} provide a robust guarantee for partial-sample ablation when uniformly sampling $D$ combinations. To investigate the relationship between the certification probability $p_D$ provided in theorem 
% \begin{figure}[h]
% \vspace{-0.2cm}
%  \centering
% \input{figs/FoodCollector_Ablation_k_sample.tex}
% \vspace{-0.4cm}
% \caption{Effects of ablation sample size $D$ on robust reward and certification probability in Theorem\ref{thm:main_dist}}
% \label{fig:ablation_k_sample}
% \end{figure}

% \textit{Detection of Adversaries is possible with randomized ablation in continuous action space.}


% \begin{figure}[h]
% \vspace{-0.1cm}
%  \centering
% \input{figs/FoodCollector_Ablation_k_2adv_dist.tex}
% \vspace{-0.3cm}
% \caption{Attacker identification based on action bias $\nu_j$. Adv1 and Adv2 stands for Adversary 1 and 2. B1 up to B6 stands for 6 other benign agents.}
% \vspace{-0.5cm}
% \label{fig:detect_adv}
% \end{figure}



%\textbf{Baselines.}\quad

%\ys{todo: try other attacks?}

%\ys{In each environment, results we expect to show are:

%1. 
%clean reward and attacked reward (under different numbers of attackers) %for (1) (baseline) vanilla training, (2) (baseline) alternate adversarial %training, (3) ablation with a good choice of k

%2. [optional]
%different values of k

%3. [optional]
%different values of sample size, results with trustworthy scores

% \begin{figure}[!h]
%  \centering
%  \begin{subfigure}[b]{0.45\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{figs/attacker_1.jpg}
%     \caption{Under 1 attacker.}
%      \label{sfig:ablation_1}
%  \end{subfigure}
%  \hfill
% \begin{subfigure}[b]{0.45\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{figs/attacker_2.jpg}
%      \caption{Under 2 attackers.}
%      \label{sfig:ablation_2}
%  \end{subfigure}
% \caption{Simple randomized ablation vs. vanilla training under attacks in a 9-agent FoodCollector.}
% \label{fig:ablation}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figs/sampling.png}
%     \caption{Sample-based advanced randomized ablation vs. vanilla training under 2 attackers in a 9-agent FoodCollector. Note that sample size 1 is equivalent to the simple ablation method, and sample size 28 is equivalent to the exhausted ablation. }
%     \label{fig:ablation}
% \end{figure} 

==> cmarl/5_exp_arxiv.tex <==
\section{Empirical Study}
\label{sec:exp}

\subsection{Defending against Adversarial Position Messages in A Particle Domain}
\label{sec:exp_particle}

\textbf{Environment Setup}\quad We design and implement a practical 2D particle environment named FoodCollector, adapted from the WaterWorld environment in PettingZoo~\cite{terry2020pettingzoo}. 
There are 9 agents (colored dots surrounded by black lines) relying on sensors (black lines around agents) to observe the world. Each agent's goal is to find the food (colored large dots) of the same color as itself, and avoid collision with poisons (black dots).
The action space can be either (1) discrete, with 9 actions including 8 moving directions and 1 no-move action, or (2) continuous, where the action is an acceleration decision, denoted by a 2-dimensional real-valued vector.
Due to the limited sensory range, each agent can only see the objects around it, and thus communication is helpful. We use a pre-defined protocol where agents share their observed food with each other. Figure~\ref{fig:food} verifies the advantage of communication in FoodCollector. More details of the FoodCollector environment and the communication settings are shown in Appendix~\ref{app:exp_env}.


\textbf{Evaluation}\quad
To evaluate the effectiveness of our defense strategy, we seek to evaluate the performance of the ensemble policy under no attack and under various values of $C$ (for simplicity, we refer to $C$ as the \textit{number of adversaries}). 
Different from previous work~\cite{blumenkamp2020emergence} where the adversarial agent disrupts all the other agents, we consider the case where the attacker deliberately misleads a selected victim, which could evaluate the robustness of the victim under the harshest attacks. 
We use the following two attack methods:
(1) \textbf{non-adaptive attack} that randomly generates a message. Note that this is already a strong attack since a randomly generated message could be arbitrary and far from the original benign message;
% random attacks \fh{random looks too weak, can we justify this is a good attack? Can we give a better name to it?} 
(2) \textbf{learned adaptive attack} that learns the strongest/worst adversarial communication with an RL algorithm to minimize the victim's reward (a white-box attacker which knows the victim's reward). The learned attack can strategically mislead the victim (e.g., to a poison).
As shown in prior works~\cite{zhang2020robust,zhang2021robust,sun2021strongest}, the theoretically optimal attack (which minimizes the victim's reward) can be formed as an RL problem and learned by RL algorithms. 
We can regard this attack as a worst-case attack for the victim agents.
% Therefore, we train an RL attacker policy that maps adversarial agent's observations to adversarial communications. 
More details are in Appendix~\ref{app:exp_imple}.

\textbf{Implementation and Baselines}\quad
We compare our \ours with two baselines: (1) \textbf{(Vanilla)} vanilla training which learns a policy based on all benign messages. (2) \textbf{(AT)} adversarial training as in~\cite{zhang2021robust}, which alternatively trains an adaptive RL attacker and an agent. 
As is common in related work~\cite{lowe2017multi,gupta2017cooperative}, we use parameter sharing and train a shared policy network for all agents.
Our \ours and baselines are all trained with PPO~\cite{schulman2017proximal}, and more implementation details are provided in Appendix~\ref{app:exp_imple}.

\begin{figure}[t]
\vspace{-0.5em}
    \centering
    \begin{subfigure}[t]{0.32\columnwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{figs/foodcollector.png}
        \vspace{-0.5cm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figs/comm_dist_small}}
        \vspace{-0.5cm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figs/comm_cont}}
        \vspace{-0.5cm}
    \end{subfigure}
% \vspace{-1em}
\caption{\textbf{Left:} The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. 
\textbf{Middle/Right:} Reward of agents trained with communication v.s. without communication in discrete/continuous action space. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly. 
%The result in a continuous action space is similar, as presented in Appendix~\ref{app:exp_env}.
}
\label{fig:food}
\vspace{-1.5em}
\end{figure}

% \paragraph{Random Attacks} xxx

% \paragraph{Heuristic Attacks} xxx

% \paragraph{Optimal Attacks} Suppose there is an attacker manipulating communication messages from a subset of agents $\mathcal{Y}=\{ y_1, \cdots, y_C \}$ to $x$ ($x \notin \mathcal{Y})$, i.e., the attacker can control the communication channels to the victim from up to $C$ agents. \fh{Note that $C$ should be considered as a known hyperparameter, and we will provide more insight later in the paper about how to set $C$ in practice.} 
% As pointed out by some prior works~\cite{zhang2020robust,sun2021strongest}, the \textit{optimal attack} \fh{to an RL policy} can be learned by solving an RL problem:
% % {\small{
% \setlength\abovedisplayskip{-2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:adv_obj}
% \tag{$Q_A$}
% \begin{aligned}
%     \min_{\nu_1,\cdots,\nu_C} & \; \advobj^x :=  \mathbb{E} [ \sum_{t=0}^\infty \gamma^t [R(s\step, a_1\step, \cdots, a_N\step)]_{x} ] \\
%     \text{where } & \; a_i\step = \pi_i(o_i\step, \mtoi\step), \forall i\in [N], t \geq 0 \\
%      & \; m_{y_j \to x}\step = \nu_{j}(o_{y_j}\step), \forall j\in [C], t \geq 0
% \end{aligned}
% \end{equation}
% % }}
% \fh{ I tried to move something, but may not be complete and logic needs to be straightened out.}


% The minimizer to Problem~\eqref{eq:adv_obj}, $\nu_1^*,\cdots,\nu_C^*$ , defines an optimal communication attacking strategy that is adaptive to victim $\pi_x$. 
% In other words, the attacker learns $C$ communication policies that collaboratively minimizes the reward of the victim agent $x$.



\textbf{Robust performance Under Attacks}\quad
As shown in Figure~\ref{fig:res_all}, the rewards of Vanilla and AT drastically drop under attacks, especially adaptive attackers. %(A random agent can gain reward -80.)
We find that AT does not achieve better robustness than Vanilla, since malicious messages can appear at any channel, and it is hard for AT to learn a general defense strategy, as explained in Appendix~\ref{app:exp_imple}.
% becomes too conservative as it is trained to adapt to adversarial messages from multiple channels, i.e., AT does not trust any communication, as detailed in Appendix~\ref{app:exp_imple}.
% , and thus AT cannot utilize well the benign messages.
% does not outperform Vanilla under communication attacks, because there are many communication channels and it is hard for the agent to adapt to all communication attacks.
% Note that the lowest possible reward in this environment is about -100, so in the discrete action case, 2 adaptive adversarial messages can already reduce the reward of Vanilla and AT to the lowest level.
In contrast, we use $k=2$ for our \ours, which provides performance guarantees against up to $C=2$ adversaries. We can see that the reward of \ours under $C=1$ or $C=2$ is similar to its reward under no attack, matching our theoretical analysis. 
The high performance of \ours verifies that it can utilize benign communication well while being robust to adversarial communication.
In both discrete and continuous action spaces, \ours achieves a significantly better performance than Vanilla and AT under various numbers of adversaries, even under 3 adversaries where the theoretical guarantees no longer hold. Therefore, \textit{\ours makes agents robust under varying numbers of adversaries.} 

\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist_naive}}
  \vspace{-1.5em}
  \caption{Disc. \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist}}
  \vspace{-1.5em}
  \caption{Disc. \& Adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Cont_naive}}
  \vspace{-1.5em}
  \caption{Cont. \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\textwidth}{!}{ \input{figs/FoodCollector_Attacker_Cont}}
  \vspace{-1.5em}
  \caption{Cont. \& Adaptive}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Reward comparison between our \ours and baselines in FoodCollector with discrete/continuous action space, under no attacker or non-adaptive/adaptive attacks under varying numbers of adversaries. Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_all}
\end{figure}





\subsection{Defending against Adversarial Demand Messages in A Market Domain}
\label{sec:exp_market}

\textbf{Environment Setup}\quad 
We design a practical environment called \textit{MarketEnv} which simulates the real-world inventory management problem, where $N=10$ heterogeneous seller agents carry inventory for $M=3$ products. A population of $B=300$ buyers request a product from a randomly selected seller agent according to a demand distribution. Sellers manage their inventory by restocking products through interacting with the buyers. The game is episodic with horizon set to $50$. At the beginning of each episode, a realization of the demand distribution $\mathbf{p}$ is randomly generated and the agents' inventory for each product is randomly initialized from $[0, \frac{B}{N}]$, where $\frac{B}{N}$ is the expected number of buyers per seller. 
Sellers are penalized for mismatch between their inventory and the demand for a product, and they aim to restock enough units of a product at each step to prevent insufficient inventory without accruing a surplus at the end of each step. Sellers communicate with each other by exchanging their own demand observations, so that they can estimate the true demand distribution more accurately and manage stock better. More details of the Market environment and the communication settings are shown in Appendix~\ref{app:market_env}.


\textbf{Evaluation and Implementation}\quad
As in the FoodCollector environment, we compare \ours with Vanilla and AT against learned adaptive attacks and non-adaptive attacks. To simulate various types of practical attacks, we design multiple non-adaptive attack formulations: (1) \permute that randomly permutes the order of the demand observation of $M$ products; (2) \swap that swaps the highest demand and the lowest demand, the second highest demand with the second lowest demand and so forth; (3) \flip that flips the demand values with respect to the average demand observation. The agents and the adaptive attackers are both learned with PPO, detailed in Appendix~\ref{app:market_imple}. 


\paragraph{Robust performance Under Attacks} \quad
In this section, we evaluate robustness of the proposed \ours defense strategy in MarketEnv and compare it against Vanilla Learning and Adversarial Training. Figure~\ref{fig:res_all_market} shows the natural and robust performance of \ours with $k=2$, which provides performance guarantees against up to $C=2$ adversarial messages. The performance is compared with AT when the agents policy is alternatively trained against $2$ adversaries. We observe that there is a considerable reduction in the Vanilla and AT rewards under attacks, especially for the strong adaptive attack and \swap. Similar to the FoodCollector, adversarial training is not robust to adversarial communications in the MarketEnv such that for two or more adversarial messages the performance is close to or much lower than the reward achieved with no communications. However, as expected for $k=2$, \ours is able to achieve rewards comparable to the no-attack case  under $C=1$ and $C=2$ adversaries even for strong adversarial attacks. Moreover, \ours outperforms the baselines for $C=3$ for which the theoretical guarantees no longer hold. Even though the gap between natural and robust performance under the weak \permute is less for all three strategies, \ours achieves the highest reward. In  MarketEnv, \ours is able to preserve the communication gains arising from informative messages shared among the agents while being robust against adversarial communications.

  
\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
  \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_adaptive}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_permute}}
  \vspace{-1.5em}
  \caption{\permute}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_flip}}
  \vspace{-1.5em}
  \caption{\swap}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
  \resizebox{\linewidth}{!}{ \input{figs/MarketEnv/MarketEnv_Attacker_Dist_swap}}
  \vspace{-1.5em}
  \caption{\flip}
 \end{subfigure}
%  \vspace{-0.5em}
\caption{\textbf{MarketEnv}: Reward comparison between our \ours and baselines with continuous action space, under no attacker and varying numbers of adversaries for (a) adaptive and (b), (c), (d) non-adaptive attacks. Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_all_market}
\end{figure}




\subsection{Defending against Adversarial Communication in Multi-agent Image Classification}
\label{sec:exp_mnist}

\textbf{Environment Setup}\quad 
Communicative multi-agent learning is also used in vision tasks. For example, \cite{mousavi2019multi} use MARL for image classification in the MNIST dataset. There are multiple agents aiming to classify an image within  a limited time horizon. At every step, each agent observes a patch of the image, and can take an action to move to an adjacent patch, based on an LSTM policy. In the meanwhile, agents are allowed to exchange information (encoded local beliefs) with other agents to update their own beliefs. Therefore, different from the hand-coded communication protocols used in FoodCollector and MarketEnv, agents in this MNIST classification task use learned communication.

\textbf{Evaluation and Implementation}\quad 
Our implementation is based on \cite{mnistgithub} that reproduces the results of~\cite{mousavi2019multi}.
We first test the robustness of the original LSTM policies proposed by \cite{mousavi2019multi} under communication attacks, i.e., $C$ out of $N-1$ communication messages (encodings) are corrupted. Then, we equip the LSTM policy with \ours by message ablation and ensemble, and verify its robustness against random attacks and learned adaptive attacks. More environment description and implementation details are provided in Appendix~\ref{app:mnist}.


\textbf{Robust performance Under Attacks}\quad
Figure~\ref{fig:res_mnist} demonstrates the robust performance of the MARL algorithm proposed by~\cite{mousavi2019multi} without or with our \ours defense. We set $N=9$ and $k=2$ for all experiments.
Under learned adaptive attackers, the original MARL classifier~\cite{mousavi2019multi}  without \ours suffers from significant performance drop in terms of both precision and recall, while \ours considerably improves the robustness of agents across different numbers of attackers. 
Under random attacks, we find that the MARL classifier~\cite{mousavi2019multi} is moderately robust when a few communication signals are randomly perturbed. However, when noise exists in many communication channels (e.g. $C=6$), the performance decreases a lot. In contrast, our \ours still achieves high performance when $C=6$ communication messages are corrupted.

\begin{figure}[h]
% \vspace{-0.5em}
\hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/MNIST_Adaptive_Attacker_Precision}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MNIST_Adaptive_Attacker_Recall}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/MNIST_Random_Attacker_Precision}}
  \vspace{-1.5em}
  \caption{Non-adaptive Attack}
 \end{subfigure}
\hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MNIST_Random_Attacker_Recall}}
  \vspace{-1.5em}
  \caption{Non-adaptive Attack}
 \end{subfigure}
\vspace{-0.5em}
\caption{Precision and recall of MARL classification on MNIST without or with \ours, under learned adaptive attacks and non-adaptive random attacks. }
% \vspace{-1.5em}
\label{fig:res_mnist}
\end{figure}


\subsection{Hyper-parameter Tests}
\label{sec:exp_hyper}

\textbf{Hyper-parameter Test of Ablation Size $\boldsymbol k$}\quad
As discussed in Section~\ref{sec:algo_dist}, the value of $k$ is related to the trade-off between natural performance and robustness. To see how $k$ influences the agent's performance, we evaluate \ours's natural reward and \ours's reward under the same number ($C=2$) of strong adaptive adversaries with different ablation sizes $k$. 
The results in FoodCollector and MarketEnv are shown in Figure~\ref{sfig:hyper_k_food} and Figure~\ref{sfig:hyper_k_market}, respectively.
We can see that increasing the ablation size $k$ improves the natural performance of the agent since each agent could gather more information from others. However, raising the ablation size $k$ also increases the risk of making decisions based on communication messages sent from an adversary. Therefore, \textit{increasing ablation size $k$ trades off robustness for natural performance.} 


\textbf{Hyper-parameter Test of Sample Size $\boldsymbol D$}\quad
We further evaluate the partial-sample variant of \ours introduced in Section~\ref{sec:algo_partial} using $k=2$ under $C=2$ adaptive adversaries, with $D$ varying from $N-1 \choose k$ (the largest sample size) to 1 (the smallest sample size). Figure~\ref{sfig:hyper_d_food} and Figure~\ref{sfig:hyper_d_market} demonstrate the performance of different $D$'s in FoodCollector and MarketEnv. As $D$ goes down, \ours obtains lower reward under attackers, but it is still significantly more robust than baseline methods, even when $D=1$ where the agent makes decisions based on only 1 random message subset.

\begin{figure}[htbp]
% \vspace{-0.5em}
\hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_cont}}
  \vspace{-1.5em}
  \caption{FoodCollector}
  \label{sfig:hyper_k_food}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}}
  \vspace{-1.5em}
  \caption{MarketEnv}
  \label{sfig:hyper_k_market}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_sample_cont}}
  \vspace{-1.5em}
  \caption{FoodCollector}
  \label{sfig:hyper_d_food}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_K_sampleD}}
  \vspace{-1.5em}
  \caption{MarketEnv}
  \label{sfig:hyper_d_market}
 \end{subfigure}
\vspace{-0.5em}
\caption{Hyper-parameter tests of ablation size $k$ and sample size $D$. 
We show how natural reward and attacked performance change with \textbf{(a)} various $k$ in continuous-action FoodCollector, \textbf{(b)} various $D$ in continuous-action FoodCollector, \textbf{(c)} various $k$ in MarketEnv, and \textbf{(d)} various $D$ in MarketEnv. (Dashed green lines refer to the performance of Vanilla agent under $C=2$ attacks.) The result of discrete-action FoodCollector is similar as shown in Figure~\ref{fig:res_k_dist} in Appendix~\ref{app:exp_res}.}
\vspace{-1.5em}
\label{fig:res_hyper}
\end{figure}



% \textbf{Hyper-parameter Tests}\quad 
% % \ours requires a hyper-parameter $k$  which controls how many messages the base ablation policy relies on to output a base action. The partial-sample variant of \ours introduced in Section~\ref{sec:algo_partial} requires another hyper-parameter $D$, the number of message subset samples the ensemble policy uses. 
% To evaluate the effects of two hyper-parameters $k$ (ablation size) and $D$ (sample size, only used for partial-sample \ours introduced in Section~\ref{sec:algo_partial}), we train \ours with different $k$'s and $D$'s and plot the results in Figure~\ref{fig:res_k_dist} for discrete-action FoodCollector, and Figure~\ref{fig:res_k_cont} for continuous-action FoodCollector (in Appendix~\ref{app:exp_res}).
% \\





% \paragraph{Hyper-parameter Test of Ablation Size $\boldsymbol k$} 
% Figure~\ref{fig:res_k_cont_market}(left)  shows how the agent's natural performance and robustness varies with the ablation size $k$. We compare \ours’s natural reward and \ours’s reward under $C=2$ adversarial communication messages for adaptive and non-adaptive attacks  with different values of $k$. Similar to the FoodCollector, As the ablation size $k$ increase, the agent is able to improve its natural performance by utilizing information communicated by more agents. However, the agent becomes more vulnerable to adversarial communications which can impacts its decision-making for managing its inventory. Therefore, ablation size $k$ trades off robustness for natural performance. Additionally, we observe that the non-adaptive \swap which constructs the  adversarial communications strategically to mislead the victim agent is quite effective in reducing the victims reward compared to the \permute which communicates adversarial messages without tactically modifying the adversary's observed demands.
 
% \paragraph{Hyper-parameter Test of Sample Size $\boldsymbol D$}
% In Figure~\ref{fig:res_k_cont_market}(right), we evaluate the robustness of the partial-sample variant of \ours presented in Section~\ref{sec:algo_partial} against $C=2$  adversaries for ablation size $k=2$, when $D$  varies from $36$ (the largest sample size) to $1$ (the smallest sample size). It is shown that with lower $D$, \ours achieves lower rewards under adversarial communications, but is considerably more robust compared to the baseline method. When the agent makes decisions based on a single random message with $D=1$, the agent's average robust reward is higher than the Vanilla reward.


% \begin{figure}[h]
%  \centering
%  \begin{subfigure}[t]{0.49\textwidth}
%  \centering
%   \resizebox{0.6\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.49\textwidth}
%  \centering
%   \resizebox{0.6\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_K_sampleD}}
%  \end{subfigure}
% %  \vspace{-2em}
% %  \subcaption{Continuous Action Space}
% \vspace{-0.5em}
% \caption{\textbf{MarketEnv} Hyper-parameter test in continuous-action MarketEnv. \textbf{Left:}  Natural and robust performance with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. Dashed green line refers to Vanilla under $C=2$ attacks.}
% \vspace{-0.5em}
% \label{fig:res_k_cont_market}
% \end{figure}

==> cmarl/6_discuss.tex <==
\vspace{-0.5em}
\section{Conclusion and Discussion}
\label{sec:discuss}
% \vspace{-0.5em}

This paper formulates communication attacks in MARL problems, and proposes \ours, a certifiable defense against multiple arbitrarily perturbed adversarial communication messages, based on randomized ablation and aggregation. The idea of \ours can also be extended to detect attackers, by measuring the difference between the action suggested by any specific communication message and the ensemble policy's action, as empirically verified in Appendix~\ref{app:exp_detect}. 
\ys{flexibility of different $k$'s in training and test.}

==> cmarl/a1_proof.tex <==
\section{Proofs of Main Theorems}
For the simplicity of the proof, we make the following definition.
\label{app:proof}
\begin{definition} (Safe Message Combination)
For a message combination $T\in \mathcal{H}(N-1, k)$, $\funabl(\textbf{m}, T)=[m_{j_1},...,m_{j_k}]$ is a \emph{safe message combination} iff for every $1\leq n\leq k$, $m_{j_n}$ is a benign communication message. Otherwise, it is  an \emph{unsafe message combination}. 

% \textcolor{purple}{PH: I think the terminology here may not be consistent with the main paper. 
% \begin{itemize}
%     \item $T$ is the index set of messages, but here we are referring to it as "combination message". Should we use $[m_{j_1}\dots, m_{j_k}]$?
%     \item  In section 2.2 [Formulation of Communication Attack] and Assumption 2.1, we talk about One attacker that can perturb $C$ of the communication messages (channels). However, here we are talking about $k$ benign/adversarial agents. Maybe we could say "iff $m_{j_n}$ is a benign communication message for every $1\leq n\leq k$"?
% \end{itemize}}
\end{definition}
For simplicity, we will refer to the indexes $T$ as a safe message combination iff $\funabl(\textbf{m}, T)$ is a safe  message combination. Note that the total  number of safe message combinations is $n_2=\binom{N-C-1}{k}$, and the total number of unsafe message combinations is $n_1-n_2=\binom{N-1}{k}-\binom{N-C-1}{k}$.

\subsection{Proofs in Discrete Action Space}
\begin{proof}[Proof of Theorem~\ref{thm:main_dist} and Theorem~\ref{thm:sample_dist}]
The majority voted action $\tilde{a}$ is a benign action, i.e., $\tilde{a}\in \safeactiondist$, if the ablation policy $\hat{\pi}$ renders action $\tilde{a}$ for
at least one safe message combination.  If $u_{\tilde{a}}>n_1-n_2$, since $n_1-n_2$ is exactly the total number of unsafe combinations, then it is guaranteed that there is at least one safe combination for which $\hat{\pi}$ renders $\tilde{a}$. Thus, $\tilde{a}\in \safeactiondist$.
%Here, the majority voted action $\tilde{a}\in \safeactiondist$ is equivalent to the condition that $\tilde{a}$ is chosen by at least one safe message combination. Therefore, if $u_{\tilde{a}}>n_1-n_2$, where $n_1-n_2$ is exactly the total number of unsafe combinations, then it is guaranteed that $\tilde{a}$ is chosen by at least one safe combination. Thus, $\tilde{a}\in \safeactiondist$ is a safe action.

However, if $u_{\tilde{a}}\leq n_1-n_2$, then in order for $\tilde{a}$ to be safe, among the $u_{\tilde{a}}$ message combinations resulting in $\tilde{a}$ there can be at most $u_{\tilde{a}}-1$ unsafe combinations.  % Therefore, the maximum number of votes coming from unsafe message combination is $u_{\tilde{a}}-1$. 
There are $ \sum_{j=0}^{u_{\tilde{a}}-1}\binom{n_1-n_2}{j}\binom{n_2}{D-j}$ such possibilities in terms of the sampling of $D$, and the total number of possibilities are $\binom{n_1}{D}$. Therefore, we get Equation \eqref{eq:p_sample_dist}.



The proof of Theorem~\ref{thm:main_dist} follows as a special case of Theorem~\ref{thm:sample_dist} when $D=\binom{N-1}{k}$. In this case, the only non-zero term left in the numerator of $p_D$ is $\binom{n_2}{j}\binom{n_1-n_2}{n_1-j}=\binom{n_2}{n_2}\binom{n_1-n_2}{n_1-n_2}=1$ ($j=n_2$), so $p_D=1$.

% Let $m_{:\to i}$ denote the message list communicated to agent $i$ by all other agents in the non-adversarial setting. In the adversarial setting, $K\in [n]$ is the set of malicious agents attacking agent $i$ ($K$ is not known to agent $i$), and $m_{:\to i}^\prime$ denotes the communicated message list in this setting. Then, 
% \begin{align}
% &\mathbb{P}(\hat{\pi}(o, m_{:\to i})=\hat{\pi}(o, m_{:\to i}^\prime))\\
% \geq& \mathbb{P}(\hat{\pi}(o, m_{:\to i})=\hat{\pi}(o, m_{:\to i}^\prime), \mathcal{T} \wedge K = \emptyset )\\
% =& \mathbb{P}(\hat{\pi}(o, m_{:\to i})=\hat{\pi}(o, m_{:\to i}^\prime)|\mathcal{T} \wedge K = \emptyset) \mathbb{P}(\mathcal{T} \wedge K = \emptyset)\\
% =& \mathbb{P}(\mathcal{T} \wedge K = \emptyset) 
% % \;\; (\text{Because}\; \hat{\pi}(o, m)=\hat{\pi}(o, m^\prime) \;\text{if}\;  \mathcal{T} \wedge K = \emptyset) 
% \\
% =& \frac{\binom{N-C}{k}}{\binom{N}{k}}
% \end{align}
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:reward_dist}]

Based on the definition of benign action set, $\smpolicy$ selects an action $\widetilde{a}$ if and only if there exists an index set $T$ such that the benign message combination $\funabl(\mathbf{m},T)$ makes the ablation policy $\ablpolicy$ select $\widetilde{a}$. Therefore, for any trajectory generated by $\smpolicy$ under attacks, there is a trajectory of $\ablpolicy$ with a list of indices sets $T_1,T_2,\cdots$ that renders the same cumulative reward under no attack.

\end{proof}


\subsection{Proofs in Continuous Action Space}

\begin{proof}[Proof of Theorem~\ref{thm:main_cont} and Theorem~\ref{thm:sample_cont}]
To understand the intuition of element-wise median operation in continuous action space, let us first start with an intuitive example: consider 5 arbitrary numbers $x_1$,...,$x_5$, if we already know 3 of them $x_1$,$x_2$,$x_3$, then it is certain that Min($x_1$,$x_2$,$x_3$)$\leq$Median($x_1$,...,$x_5$)$\leq$Max($x_1$,$x_2$,$x_3$). Applying this element-wise, when safe message combinations form the majority, the median action falls into the range of actions produced by safe messages. 

Concretely, in continuous action space,  $\tilde{a}\in \safeactioncont$ is equivalent to the condition that out of the $D$ sampled message combinations, safe message combinations make up the majority. There are $\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n1-n2}{D-j}$ such possibilities in terms of the sampling of $D$, where $\tilde{D}={\lfloor \frac{D}{2} \rfloor}+1$. Once again the total number of possibilities is $\binom{n_1}{D}$. Therefore, we get Equation \eqref{eq:p_sample_cont}.

The proof of Theorem~\ref{thm:main_cont} follows as a special case of Theorem~\ref{thm:sample_cont} when $D=\binom{N-1}{k}=n_1$. Same as above, in this case, the only non-zero term left in the numerator of $p_D$ is $\binom{n_2}{j}\binom{n_1-n_2}{n_1-j}=\binom{n_2}{n_2}\binom{n_1-n_2}{n_1-n_2}=1$ ($j=n_2$), so $p_D=1$.
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:reward_cont}]

Similar to the proof of Corollary~\ref{cor:reward_dist}, at any state $s$, the action $\widetilde{a}$ generated by $\smpolicy$ is always bounded by actions generated from $\ablpolicy$ with some indices set. Due to Assumption~\ref{assump:order}, there exists $a^\prime\sim\ablpolicy$ such that $R(s,a^\prime) \leq R(s,\widetilde{a})$. Therefore, the cumulative reward of $\smpolicy$ is lower bounded by the minimal cumulative reward of $\ablpolicy$ among all indices set lists.

\end{proof}

==> cmarl/a2_theory.tex <==
\section{Additional Theoretical Definitions and Analysis}
\label{app:theory}

\textbf{Relation between Communication Attack and $\boldsymbol \ell_0$ Observation Attack}\quad
The communication threat model described in Section~\ref{sec:setup_adv} is analogous to a constrained $\ell_0$ attack on policy inputs. When agent $i$ is attacked, the input space of its acting policy $\pi_i$ is $\tilde{\mathcal{O}}_i := \mathcal{O}_i \times \mathcal{M}^{N-1}$. Therefore, when $C$ communication messages are corrupted, the original observation $\tilde{o}_i$ gets perturbed to $\tilde{o}_i^\prime$. Let $d$ be the dimension of a communication message, then $\tilde{o}_i$ and $\tilde{o}_i^\prime$ differ by up to $dC$ dimensions, which is similar to an $\ell_0$ attack constrained in certain dimensions. 



\subsection{Additional Analysis of \ours in Discrete Action Space}
\label{app:theory_dist}

Theorem~\ref{thm:main_dist} justifies that under sufficient majority votes $u_{\tilde{a}}$, the ensemble policy $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a safe action that is suggested by some benign message combinations even when the malicious messages are not identified.
Therefore, with ensemble policy $\smpolicy$, the agent's cumulative reward under adversarial communications would be similar to the natural reward of $\ablpolicy$ under no attacks, as justified in the following corollary.
% The corollary below shows the relationship between the attacked reward of $\smpolicy$ and the natural reward of $\ablpolicy$. Note that $\ablpolicy$ is the policy learned during training time in a clean (non-adversarial) environment, and it is easy for us to evaluate its natural cumulative reward. $\smpolicy$ is 
% \fh{I feel the current description doesn't make it easy to  distinguish between $\ablpolicy$ and $\smpolicy$.}

\begin{corollary}[Reward Certificate for Discrete Action Space]
\label{cor:reward_dist}
With ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} under adversarial communication satisfying Assumption~\ref{assum:num} is no lower than the lowest cumulative reward that the ablation policy $\ablpolicy$ can obtain with randomly selected message subsets under no attacks, i.e.,
\begin{equation}
\begin{aligned}
    \advobj(\smpolicy) \geq \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
\end{aligned}
\end{equation}
where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under attacks, and $\natobj(\ablpolicy|T_1,T_2,\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ whose message is ablated by index set $T_t$ at step $t>0$.
\end{corollary}

% \begin{corollary}[Reward Certificate for Discrete Action Space]
% \label{cor:reward_dist}
% \fh{Under sample size $D=\binom{N-1}{k}$, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with a message subset size $k$ satisfying Equation~\eqref{eq:k_cond} obtains a total reward no worse than that obtained by the base ablation policy $\ablpolicy$ using benign messages:
% \begin{align}
%   & \advobj\Big(\smpolicy\big(o, \{\funabl(\advmsg, T_d)\}_{d=1}^D\big)\Big) \geq \nonumber \\
%   & \min_{T} \natobj\Big(\ablpolicy\big(o, \funabl(\goodmsg, T)\big)\Big) \label{eq:reward_dist}
% \end{align}
% if the majority votes $u_{\tilde{a}}$ satisfies $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step.
% }
% \textcolor{red}{Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If $D=\binom{N-1}{k}$, and the majority votes satisfy 
% $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step, 
% then the total reward of $\smpolicy$ satisfies
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:reward_dist}
%     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy),
% \end{equation}}
% Here $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the \textcolor{red}{sampled message indices}\fh{indices of the message subsets?} used by $\ablpolicy$ at all steps. \fh{What does this mean? My equation doesn't use $\tau$, rather I use $T$.}
% \end{corollary}
Note that $\min_{\tau} \natobj(\ablpolicy)$ can be estimated by executing $\ablpolicy$ during training time, so that the test-time performance of $\smpolicy$ is guaranteed to be no lower than this value, even if there are up to $C$ corrupted messages at every step.




\subsection{Additional Analysis of \ours in Continuous Action Space}
\label{app:theory_cont}

% \begin{definition}[Q Value of Ablation Policy $\ablpolicy$]
% \label{def:q_abl}
% Suppose that agent $i$ is executing policy $\ablpolicy$, and all other agents are also executing fixed policies denoted as $\pi_{-i}$. Then, the action value of $\ablpolicy$ can be defined as below.
% \begin{equation}
% \label{eq:q_abl}
%     \hat{Q}^{\ablpolicy}(s,a):=\mathbb{E}_{\krv\step \sim \mathcal{U}(N-1,k), P, \pi_{-i}}[\sum_{t=0}^\infty \gamma^t r\step | s_0=s, a_0=a, a_t\sim\ablpolicy(o\step, \funabl(\mtoi\step, \krv\step))],
% \end{equation}
% where $r\step$ is the reward obtained by $i$ at step $t$.
% \end{definition}


Theorem~\ref{thm:main_cont} shows how the ensemble policy outputs an action bounded by safe actions. However, to obtain a reward certificate, an extra assumption about the reward structure is needed.
% Now we further discuss how it can lead to a reward certificate.
% Let $\preccurlyeq$ define the element-wise less than or equal to relation between two vectors.
% The following assumption is essential for obtaining a reward certificate, which suggests that a coordinate-wisely bounded action also has lower bounded reward.
\begin{assumption}
\label{assump:order}
Let $R: \mathcal{S} \times \mathcal{A} \to \mathbb{R}$ be the reward function of the current agent. For any state $s\in\mathcal{S}$, assume $R(s,a) \geq \min_{\hat{a}\in\mathsf{\safeaction}} R(s,\hat{a})$.
\end{assumption}
% \begin{assumption}[Ordered Action]
% \label{assump:order}
% For any state $s\in\mathcal{S}$, and any actions 
% $a_1\preccurlyeq a_2 \preccurlyeq a_3$, we have either $R(s,a_2) \geq R(s,a_1)$, or $R(s,a_2) \geq R(s,a_3)$, where $R$ is the reward function for the current agent.
% \end{assumption}

Assumption~\ref{assump:order} suggests that there is no ``caveat'' in the safe action set. 
This assumption is mild and practical in many real-life scenarios where actions have concrete meanings (e.g. price, speed, etc). For example, if driving at 40 mph and driving at 50 mph are both safe, then driving at 45 mph is also safe. 
Note that without the assumption of reward structure, there may exist extreme cases where some actions in $\safeaction$ could lead to low reward, which makes the reward not certifiable. In practice, we can usually expect this assumption to hold when the safe action range generated by the ablation policy is relatively narrow, i.e., the benign communication messages achieve agreements.

With Assumption~\ref{assump:order}, the following reward certificate holds.

\begin{corollary}[Reward Certificate for Continuous Action Space]
\label{cor:reward_cont}
Under Assumption~\ref{assump:order}, with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} under adversarial communication satisfying Assumption~\ref{assum:num} is no lower than the lowest cumulative reward the ablation policy $\ablpolicy$ can obtain with randomly selected message subsets under no attacks, i.e.,
\begin{equation}
\begin{aligned}
    \advobj(\smpolicy) \geq \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
\end{aligned}
\end{equation}
where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under attacks, and $\natobj(\ablpolicy|T_1,T_2,\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ whose message is ablated by indices set $T_t$ at step $t>0$.
\end{corollary}


% \begin{corollary}[Reward Certificate for Continuous Action Space]
% \label{cor:reward_cont}
% Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If Assumption~\ref{assump:order} holds, and $D=\binom{N-1}{k}$, 
% then the total reward of $\smpolicy$ satisfies
% \begin{equation}
% \label{eq:reward_cont}
%     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy)
% \end{equation}
% where $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the sampled message indices used by $\ablpolicy$ at all steps.
% \end{corollary}



\subsection{Additional Definitions for \ours with Partial Samples}
\label{app:theory_sample}

% The $D$-ensemble policy $\pi_D$ is defined as
% \begin{equation}
% \label{eq:ensemble_pi_dist_d}
%     \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
% \end{equation}
% for a discrete action space, and
% \begin{equation}
% \label{eq:ensemble_pi_cont_d}
%     \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% for a continuous action space. 

The following theorem shows a general guarantee for $D$-ensemble policy in a discrete action space.

\begin{theorem}[General Action Guarantee for Discrete Action Space]
\label{thm:sample_dist}
Let $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$. 
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$, under Assumption~\ref{assum:num}, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_dist_d} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, relation~\eqref{eq:cert_dist} holds deterministically if $u_{\tilde{a}}>n_1-n_2$. Otherwise it holds with probability at least
%\vspace{-0.1cm}
\begin{equation}
\label{eq:p_sample_dist}
    p_D=\frac{\sum_{j=0}^{u_{\tilde{a}}-1}\binom{n_1-n_2}{j}\binom{n_2}{D-j}}{\binom{n_1}{D}}.
\end{equation}
\end{theorem}

==> cmarl/a3_exp.tex <==
\section{Additional Experiment Settings and Results in FoodCollector Environment}
\label{app:exp}

\subsection{Description of FoodCollector Environment}
\label{app:exp_env}

The FoodCollector environment is a 2D particle world shown by Figure~\ref{fig:food}(left). There are $N=9$ agents with different colors, and $N$ foods with colors corresponding to the $N$ agents. Agents are rewarded when eating foods with the same color. A big round obstacle is located in the center of the map, which the agent cannot go through. There are some poisons (shown as black dots) in the environment, and the agents get penalized whenever they touch the poison. Each agent has 6 sensors that detect the objects around it, including the poisons and the colored foods. 
The game is episodic, with horizon set to be 200. In the beginning of each episode, the agents, foods and poisons are randomly generated in the world. 
At every step, each agent will receives a negative reward $-0.5$ if it has not eaten all its food. Therefore, every agent should explore the environment and eat all food as fast as possible.
% Every time an agent eats a food, the food disappears, and the world re-generate a food with the same color in a random position. Therefore, an agent is supposed to explore the world and to eat as many foods as possible within limited number of steps.

Each of the 6 sensors can detect the following values when the corresponding element is within the sensor's range:\\
(1) (if detects a food) the distance to a food (real-valued); \\
(2) (if detects a food) the color of the food (one-hot); \\
(3) (if detects an obstacle) the distance to the obstacle (real-valued); \\
(4) (if detects the boundary) the distance to the boundary (real-valued); \\ (5) (if detects another agent) the distance to another agent (real-valued).\\
The observation of an agent includes an agent-identifier (one-hot encoding), its own location (2D coordinates), its own velocity, two flags of colliding with its food and colliding with poison, and the above sensory inputs. So, the observation space is a ($7N+30$)-dimensional vector space. 

The action space can be either \textit{discrete} or \textit{continuous}. For the discrete version, there are 9 actions including 8 moving directions (north, northwest, west, southwest, south, southeast, east, northeast) and 1 no-move action. For the continuous version, the action is an acceleration decision, denoted by a 2-dimensional real-valued vector, with each coordinate taking values in $[-0.01,0.01]$. 

\begin{figure}[h]
% \vspace{-1em}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/foodcollector.png}
    % \vspace{-0.5em}
    % \caption{The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. }
    % \label{fig:food}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{figs/comm_dist}
        % \vspace{-0.1cm}
        \caption{Discrete action space}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{figs/comm_cont}
        % \vspace{-0.1cm}
        \caption{Continuous action space}
    \end{subfigure}
% \vspace{-0.5em}
\caption{Reward of agents trained with communication v.s. without communication. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.}
\label{fig:food_comm}
% \vspace{-0.4cm}
\end{figure}

Due to the limited sensory range, every agent can only see the objects around it and thus only partially observe the world. Therefore, communication among agents can help them find their foods much faster. Since our focus is to defend against adversarially perturbed communications, we first define a valid and beneficial communication protocol, where an agent sends a message to a receiver once it observes a food with the receiver's color. For example, if a red agent encounters a blue food, it can then send a message to the blue agent so that the blue agent knows where to find its food. 
% The communication follows the protocol below. Once agent $i$ detects the location of some food or poison from its sensors, it will update the communication channel to every other agent with the latest sensor observation containing its position and its sensory data, which contains the relative location of the food and/or poison. 
To remember the up-to-date communication, every agent maintains a list of most recent $N-1$ messages sent from other $N-1$ agents.
A message contains the sender's current location and the relative distance to the food (recorded by the 6 sensors). Therefore, a message is a $8$-dimensional vector, and each agent's communication list has $8(N-1)$ dimensions in total.

During training with communication, we concatenate the observation and the communication list of the agent to an MLP-based policy, compared to the non-communicative case where the policy only takes in local observations.
As verified in Figure~\ref{fig:food_comm}, communication does help the agent to obtain a much higher reward in both discrete action and continuous action cases, which suggests that the agents tend to rely heavily on the communication messages for finding their food. 
% \fh{Since we will consider the communication protocol as part of the environment, shall we describe the protocol concretely here in this foodcollector experiment?}




\subsection{Implementation Details}
\label{app:exp_imple}

\textbf{Implementation of Trainer}\quad
In our experiments, we use the Proximal Policy Optimization (PPO) \cite{schulman2017proximal}  algorithm to train all  agents as well as the  attackers. Specifically, we adapt from the elegant OpenAI Spinning Up \cite{SpinningUp2018} Implementation for PPO training algorithm. On top of the Spinning Up PPO implementation, we also keep track of the running average and standard deviation of the observation and normalize the observation.

For the policy network, we use a multi-layer perceptron (MLP) with two hidden layers of size 64. Because the action space of our environment is bounded between -0.01 and 0.01, we parameterize the policy as a Beta distribution, which has been proposed in previous works to better solve reinforcement learning problems with bounded actions  \cite{pmlr-v70-chou17a}. In particular, we parameterize the shape parameteres of the Beta distribution as $\alpha=\log(1+e^{\alpha_{\theta}(s)})+1$ and $\beta=\log(1+e^{\beta_{\theta}(s)})+1$ (1 is added to make sure that $\alpha, \beta\geq 1$). $\pi(a|s)=f(\frac{a-h}{2h};\alpha, \beta)$, where $h=0.01$, and $f(x;\alpha, \beta)=\frac{\Gamma(\alpha+\beta)}{\Gamma(\alpha)\Gamma(\beta)}x^{\alpha-1}(1-x)^{\beta-1}$ is the density function of the Beta Distribution.
For the value network, we also use an MLP with two hidden layers of size 64. 

In terms of other hyperparameters used in the experiments, we use a learning rate of 0.0003 for the policy network, and a learning rate of 0.001 is used for the value network. We use the Adam optimizer with $\beta_1=0.99$ and  $\beta_2 = 0.999$. For every training epoch, the PPO agent interacts with the environment for 4000 steps, and it is trained for 500 epochs in our experiments.

% \textcolor{purple}{PH: before describing the  type of attackers, should we mention what an attacker is training. For example, we say below that " The action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1." Perhaps we can state it here to make it more clear the attacker is learning a communication policy and not taking over the actions of agents?}


\textbf{Attacker}\quad
An attacker maps its own observation to the malicious communication messages that it will send to the victim agent. Thus, the action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1. 
\vspace{-0.5cm}
\begin{itemize}
\item \emph{Non-adaptive Attacker}\quad
We implement a fast and naive attacking method for the adversary. At every dimension, the naive attacker randomly picks 1 or -1 as its action, and then sends the perturbed message which consists entirely of 1 or -1 to the victim agent. 
\vspace{-0.2cm}
\item \emph{Adaptive RL Attacker}\quad
We use the PPO algorithm to train the attacker, where we set the reward of the attacker to be the negative reward of the victim. The attacker uses a Gaussian policy, where the action is clipped to be in the valid communication range. The network architecture and all other hyperparameter settings follow the exact same from the clean agent training.
\end{itemize}
\vspace{-0.2cm}

\textbf{Implementation of Baselines}\quad
\vspace{-0.2cm}
\begin{itemize}
\item \emph{Vanilla Learning}\quad
For Vanilla method, we train a shared policy network to map observations and communication to actions. Note that the messages are symmetric (of the same format), we shuffle the messages before feeding them into the policy network, to reduce the bias caused by agent order. We find that shuffling the messages helps the agent converge much faster (50\% fewer total steps).
\vspace{-0.2cm}
\item \emph{Adversarial Training (AT)}\quad
For adversarial training, we alternate between the training of attacker and the training of the victim agent. Both the victim and attackers are trained by PPO. For every 200 training epochs, we switch the training, where we either fix the trained victim and train the attacker for the victim or fix the trained attacker and train the victim under attack. We continue this process for 10 iterations. Similar to Vanilla, the victim also shuffles the communication messages to obtain higher reward and converge faster.
\end{itemize}
\vspace{-0.2cm}


\emph{Adversarial Training does not improve agent's robust performance.}
As we observed in Figure \ref{fig:res_all}, adversarial training does not improve the robustness of the agent in both discrete and continuous action space, although AT achieves good robustness against observation attacks in a single-agent environment~\cite{zhang2021robust}. 
We hypothesize that it is due to (1) the large number of total agents, and (2) the uncertainty of adversarial message channels. 
To be more specific, during the training of AT, we alternately train the agent and the attacker, and the attacker can change the channels it controls among iterations. As a result, the agent might not be able to distinguish adversarial messages and benign messages. 
% We hypothesize that it is due to the communication shuffling of the agent. In fact, this is also similar to another practical scenario where at different time steps, the attacker might hijack different agents. As a consequence, in both scenarios, malicious messages could randomly appear in any part of the agent's input vector. 
Therefore, simply training the agent and attacker together cannot make the agent learn how to detect the malicious messages and ignore them. 


\subsection{Additional Experiment Results}
\label{app:exp_res}

In addition to Figure \ref{fig:res_k_dist}, we also provide the plot for Hyper-parameter test in continuous-action FoodCollector in Figure \ref{fig:res_k_cont}. 
\input{fig_food_k_cont}






==> cmarl/a4_hyper.tex <==
\section{Additional Discussion on the Choice of Ablation Size $k$}
\label{app:hyper}

Our \ours defensive mechanism proposed in Section~\ref{sec:algo_overview} requires an extra hyperparameter: the ablation size $k$. (The sample size $D$ is only for the partial-sample variant introduced in Section~\ref{sec:algo_more}, not needed in the original form of \ours.) In this section, we discuss the selection of $k$ in practice. We start by discussing the relationship between $k$ and the required theoretical conditions.

% Decreasing the ablation size $k$ trades off natural performance under no attack for robust performance under attack. 
% Choosing a smaller $k$ could make the agents more robust, but could also potentially hurt their natural performance since the agents would have access to less information shared by others. Based on the previous experimental results, it is crucial to set $k$ such that Condition~\ref{cond:k} and Condition~\ref{cond:cons} are satisfied so that agents could have performance certificates and thus remain robust under attack. Next, we analyze the relationship between $k$ and the required conditions.

\textbf{I. (For Continuous Action Space) Condition~\ref{cond:k} and $\boldsymbol{k}$}

We first decompose Equation~\eqref{eq:k_cond} as below.
\begin{align}
    \binom{N-1-C}{k} &> \frac{1}{2} \binom{N-1}{k} \\
    \frac{(N-1-C)!}{(N-1-C-k)!k!} &> \frac{(N-1)!}{2(N-1-k)!k!} \\
    1 &> \frac{(N-1)\cdots(N-C)}{2(N-k-1)\cdots(N-k-C)}
\end{align}
Therefore, Equation~\eqref{eq:k_cond} is equivalent to
\begin{equation}
\label{eq:k_1}
    (N-k-1)\cdots(N-k-C) > \frac{1}{2} (N-1)\cdots(N-C)
\end{equation}

When $k=1$, the above inequality becomes
\begin{align}
    (N-2)\cdots(N-C)(N-C-1) &> \frac{1}{2}(N-1)(N-2)\cdots(N-C) \\
    (N-C-1) &> \frac{1}{2}(N-1) \\
    \frac{1}{2}(N-1) &> C,
\end{align}
which holds under Assumption~\ref{assum:num}. Therefore, \textbf{$\boldsymbol{k=1}$ is always a feasible solution for Condition~\ref{cond:k}.}

Then, when $C$ is fixed and $k$ goes up from 1, the LHS of Equation~\eqref{eq:k_1} goes down while the RHS does not change. Therefore, for a given number of agents ($N$) and a fixed number of adversaries ($C$), there exists an integer $k_0$ such that any $k \leq k_0$ satisfies Condition~\ref{cond:k}. In practice, if we have an estimate of the number of adversarial messages that we would like to defend against, then we could choose the maximum $k$ satisfying Equation \eqref{eq:k_cond}.
% Figure~\ref{sfig:C&K} shows how the largest feasible $k$ decreases as $C$ goes up.

On the other hand, when $k$ is fixed, there exists a $C_0$ such that any $C \leq C_0$ can let Equation~\eqref{eq:k_1} hold. Therefore, if $C$ is unknown, for any selection of $k$, Equation~\eqref{eq:k_1} can justify the maximum number of adversaries for the current selection.
% If not, based on the total number of agents, we could say that \ours could certifiably defend up to maximum $C$ attackers. 

From Equation~\eqref{eq:k_1}, we can see the interdependence between three parameters: total number of agents $N$, number of adversaries $C$, and the ablation size $k$. In Figure \ref{fig:ablation_cnk} we visualize their relationship by fixing one variable at a time. From these figures, we can see an obvious trade-off between $C$ and $k$ --- if there are more adversaries, $k$ has to be set smaller. But when $C$ is small, e.g. $C=1$, $k$ can be relatively large, so the agent does not need to compromise much natural performance to achieve robustness. 
% Importantly, when $C$ is much smaller than $N$, e.g. $C=1, N=30$, $k$ can be set relatively large, e.g. 15. Therefore, the natural performance is not compromised too much to achieve robustness. \textcolor{purple}{PH: not a big deal, but $K$ in the figures (title and legend) is upper case rather than lowercase $k$ used in the paper YS: fixed!}

\begin{figure*}[h]
% \vspace{-0.1cm}
 \centering
    \begin{subfigure}[t]{0.31\textwidth}
    \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_C_K}}
     \vspace{-0.5cm}
      \subcaption{$C$ vs. $k$}
      \label{sfig:C&K}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.30\textwidth}
     \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_N_C}}
     \label{sfig:N&C}
     \vspace{-0.5cm}
      \subcaption{$N$ vs. $C$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.30\textwidth}
     \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_N_K}}
     \label{sfig:N&K}
     \vspace{-0.5cm}
     \subcaption{$N$ vs. $k$}
    \end{subfigure}
% \vspace{-0.3cm}
\caption{Relationship between the total number of agents $N$, number of attackers $C$, and ablation size $k$. \textbf{(a)}: Maximum certifiable ablation size $k$ under different number of attackers. \textbf{(b)}: Maximum defensible number of attackers $C$ with different total number of agents $N$. \textbf{(c)}: Maximum certifiable ablation size $k$ with different total number of agents $N$.}
\label{fig:ablation_cnk}
% \vspace{-0.1cm}
\end{figure*}


\textbf{II. (For Discrete Action Space) Condition~\ref{cond:cons} and $\boldsymbol{k}$}

Different from Condition~\ref{cond:k} which is independent of the environment, Condition~\ref{cond:cons} required in a discrete action space is related to the environment and the communication quality. Intuitively, Condition~\ref{cond:cons} can be satisfied if the benign messages can reach some ``consensus'', i.e., there are enough purely benign \ksamples voting for the same action. This can be achieved when the environment is relatively deterministic (e.g., there is a certainly optimal direction to go). Fortunately, Condition~\ref{cond:cons} can be checked during training time, and we can train the \ablname and the communication policy to increase $u_{\max}$ as much as possible. 

On the other hand, Condition~\ref{cond:cons} is also related to the selection of ablation size $k$. The ratio of contaminated votes is $\frac{\binom{N-1}{k}-\binom{N-1-C}{k}}{\binom{N-1}{k}}$, and it is easy to show that this rate increases as $k$ when $k \leq N-C-1$. Therefore, when $k$ is smaller, it is relatively easier to satisfy Condition~\ref{cond:cons} as the adversarial messages can take over a smaller proportion of the total number of votes.


\textbf{Selecting $\boldsymbol{k}$ to Balance between Natural Performance and Robustness}

The above analysis shows that a smaller $k$ makes the agent more robust, while the natural performance may be sacrificed as the \ablname makes decisions based on less benign information. Such a trade-off between natural performance and robustness is common in the literature of adversarial learning~\cite{tsipras2018robustness,zhang2019theoretically}. \\
In practice, we suggest setting $k$ to be the largest integer satisfying Equation~\eqref{eq:k_cond}. If higher robustness is needed, then $k$ can be further decreased. If robustness is not the major concern while higher natural performance is required, one can increase $k$. Note that if $k=N-1$, \ours degenerates to the original vanilla policy without defense.

\textbf{What If Conditions Are Not Satisfied?}
Even if Condition~\ref{cond:k} and Condition~\ref{cond:cons} are not satisfied, the agent can still be robust under attacks as verified in our experiments (\ours with $k=2$ still achieves relatively robust performance under $C=3$ which exceeds the theoretically largest number of certifiable adversaries). Because these conditions are needed for the certificates which consider the theoretically worst-case attacks. However, in practice, an attacker has restricted power and knowledge (e.g., it does not know the victim policy/reward, and does not know the environment dynamics as prior), and is likely to be even weaker than the learned adaptive white-box attacker we use in experiments. As a result, even if a larger $k$ may break the conditions, it can still improve the empirical robustness of an agent in practice.

\textbf{Extension: Adaptive Defense with Different $k$'s}\quad
Moreover, to allow higher flexibility, one can train multiple \ablnames with different selections of $k$'s during training. Then, an adaptive strategy can be used in test time. For example, if $u_{\max}$ is too small, we can use a larger $k$ with the corresponding trained \ablname.


\textbf{Extension: Gaining both Natural Performance and Robustness by Attack Detection}\quad
From the analysis of the relation between $N$, $C$ and $k$, we can see that when the number of adversaries is large, the corresponding ablation size $k$ is supposed to be smaller. This is reasonable because a more conservative defense is needed against a stronger attacker. But if we can identify some adversarial messages and rule them out before message ablation and ensemble, we can still defend with guarantees using a relatively large $k$. For example, if we have identified $c$ adversarial messages, then we only need to deal with the remaining $C-c$ adversarial messages out of $N-1-c$ messages. By Equation~\eqref{eq:k_cond}, a larger $k$ can be used compared to defending $C$ adversarial messages out of $N-1$ messages. We also provide an adversary detection algorithm in Appendix~\ref{app:exp_detect} using a similar idea of \ours.

==> cmarl/a5_detect.tex <==
\section{Discussion: Detecting Malicious Messages with Ablation}
\label{app:exp_detect}

% Theorem~\ref{thm:main_dist} and Theorem~\ref{thm:main_cont} provide strong theoretical guarantees for the proposed \ours defense. For the theorems to hold, one has to choose a $k$ to satisfy Equation \eqref{eq:k_cond}. As shown in Figure~\ref{fig:ablation_cnk}, 
As discussed in Appendix~\ref{app:hyper}, to defend against a larger $C$, one has to choose a relatively small $k$ for certifiable performance. However, Figure \ref{fig:res_hyper} suggests that a small $k$ also sacrifices the natural performance of the agent to obtain higher robustness. This is known as the trade-off between robustness and accuracy~\cite{tsipras2018robustness,zhang2019theoretically}. Can we achieve better robustness while not sacrificing much natural performance, or obtain higher natural reward while not losing robustness?

We point out that with our proposed \ours defense, it is possible to choose a larger $k$ than what is required by Condition~\ref{cond:k} without sacrificing robust performance by identifying the malicious messages beforehand. 
The idea is to detect the adversarial messages and to rule out them before message ablation and ensemble, during the test time.

We hypothesize that given a well-trained victim policy, malicious messages tend to mislead the victim agent to take an action that is "far away" from a "good" action that the victim is supposed to take. 
To verify this hypothesis, we first train a \ablname $\ablpolicy_i$ with $k=1$ for agent $i$. Then for every communication message that another agent $j$ sends, we compute the action $a_j$ that the victim policy $\ablpolicy_i$ chooses based on all message subsets containing message $m_{j\to i}$, i.e. $a_j = \ablpolicy(\tau_i, m_{j\to i})$ (note that $k=1$ so $\ablpolicy$ only takes in one message at a time). We then define the \emph{action bias} as $\beta_j=\|a_j-\funmed\{a_k\}_{k=1}^{N}\|_1$. Based on our hypothesis, an agent which has been hacked by attackers should induce a significantly larger action bias since they are trying to mislead the victim to take a completely different action. Here, we execute the policy of two hacked agents together with six other good agents for twenty episodes and calculate the average action bias for each agent.
As shown in in Figure \ref{fig:detect_adv}, the agents hacked by attackers indeed induce a larger action bias compared to other benign agents, which suggests the effectiveness of identifying the malicious messages by action bias. 


% Note that although there is no theoretical guarantee for identifying the adversarial communication messages, 
After filtering out $c$ messages, one could compute the required $k$ by Equation~\eqref{eq:k_cond} based on $C-c$ malicious messages and $N-1-c$ total messages, which can be larger than the largest $k$ induced by $C$ malicious messages out of $N-1$ total messages. For example, if $N=30$, $C=3$, then the largest $k$ satisfying Equation~\eqref{eq:k_cond} is 5, but when 1 adversarial message is filtered out, the largest $k$ that can defend against the remaining 2 adversarial messages is 8. Although the adversary identification is not theoretically guaranteed to be accurate, Figure \ref{fig:detect_adv} demonstrates the effectiveness of the adversarial message detection, which, combined with \ours with larger $k$'s, has the potential to achieve high natural performance and strong robustness in practice.
% one could still apply Theorem \ref{thm:main_cont} with $C-A$ malicious messages and $N-A$ good messages in total.

\begin{figure}[h]
% \vspace{-0.1cm}
 \centering
\input{figs/Attacker Identification.tex}
% \vspace{-0.3cm}
\caption{Attacker identification based on action bias $\nu_j$. Adv1 and Adv2 stands for two agents hacked by the attacker. B1 up to B6 stands for six other benign agents.}
% \vspace{-0.5cm}
\label{fig:detect_adv}
\end{figure}

==> cmarl/a6_market.tex <==
\section{Additional Experiment Settings and Results in Market Environment}
\label{app:market}

% \textcolor{red}{we need to mention in the main text that we have additional experiments on MarketEnv in the Appendix} 

\subsection{Description of Market Environment}
\label{app:market_env}
The \textit{MarketEnv} environment is an inventory management setup, where $N=10$ heterogeneous seller agents carry inventory for $M=3$ products. A population of $B=300$ buyers request a product from a randomly selected seller agent according to a demand distribution $\mathbf{p}=[p_1,\dots,p_M]$. We denote the demand realization for seller $i$ with $\mathbf{d_i}=[d_{i,1},\dots,d_{i,M}]$. Sellers manage their inventory by restocking products through interacting with the buyers. The game is episodic with horizon set to $50$. At the beginning of each episode, a realization of the demand distribution $\mathbf{p}$ is randomly generated and the agents' inventory for each product is randomly initialized from $[0, \frac{B}{N}]$, where $\frac{B}{N}$ is the expected number of buyers per seller. %\ys{describe the initial inventory in every episode?} 
Sellers are penalized for mismatch between their inventory and the demand for a product, and they aim to restock enough units of a product at each step to prevent insufficient inventory without accruing a surplus at the end of each step.  %\ys{defining the reward function by math?}
\begin{itemize}
    \item State observation: A seller agent's observation includes its inventory for each product, and the products that were requested by buyers during the previous step. The observation space is a $2M$-dimensional vector.
    
    \item Agent action: Sellers manage their inventory by restocking new units of each product or discarding part of the leftover inventory at the beginning of each step. Hence, agents take both positive and negative actions denoted by an $M$-dimensional vector, and the action space can be either discrete or continuous. In our experiments, we use continuous actions assuming that products are divisible and sellers can restock and hold fractions of a product unit.
    
    \item Agent reward function: During each step, agent $i$'s reward is defined as $r_i = - || \max( \mathbf{I}_i+\mathbf{a}_i, 0) - \mathbf{d}_i||_2$, where $\mathbf{I}_i$ denotes the agents initial inventory vector, and $\mathbf{a}_i$ denotes the inventory restock vector from action policy $\pi_i$.  
    
    
    \item Agent communication: Sellers learn the demand distribution and optimize their inventory by interacting with their own customers (i.e., portion of buyers that request a product from that seller). Sellers would benefit from sharing their observed demands with each other, so that they could estimate the demand distribution more accurately for managing inventory. At the end of each step, a seller communicates an $M$-dimensional vector reporting its observed demands to all other agents. In the case of adversarial communications, this message may differ from the agents' truly observed demands.
    
    During training with communication, messages received from all other agents are concatenated to the agent's observation, which is used to train an MLP-based policy, compared to the non-communicative case where the policy is trained using only local observations. As observed from Figure \ref{fig:marketenv_comm}, communication helps agents obtain  higher rewards since they are able to manage their inventory based on the overall demands observed across the population of buyers rather than their local observation. Results are reported by averaging rewards corresponding to $5$ experiments run with different training seeds.
\end{itemize}
 
\begin{figure}[h]
\vspace{-0.1cm}
 \centering
\resizebox{.4\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_comm_dist}}
\vspace{-0.1cm}
\caption{\textbf{MarketEnv}: Reward of agents trained with communication v.s. without communication. %Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.
} 
\label{fig:marketenv_comm}
\end{figure}
 
 



\subsection{Implementation Details}
\label{app:market_imple}
\textbf{Implementation of Trainer}\quad 
As in the FoodCollector experiments, we use the PPO algorithm to train all agent action policy as well as adversarial agent communication policies. We use the same MLP-based policy and value networks as the FoodCollector but parameterize the policy as a Gaussian distribution. The PPO agent interacts with the environment for $50$ steps, and it is trained for $10000$ episodes. The learning rate is set to be 0.0003 for the policy network, and 0.001 for the value network.
% All other hyper-parameters are set similar to the FoodCollector experiments.


\textbf{Attacker}\quad 
The attacker uses its observations to communicate malicious messages to  victim sellers, and its action space is the communication space of a benign agent.  We consider the following non-adaptive and adaptive attackers:
\begin{itemize}
    \item \textit{Non-adaptive Attacker}: The attacker's goal is to harm the victim agent by misreporting its observed demands so that the victim seller under-estimates or over-estimates the restocking of products. In our experiments, we evaluate the effectiveness of defense strategies against the following attack strategies:
    \begin{itemize}
     \item{\permute}: The communication message is a random permutation of the true demand vector observed by the attacker.
    \item {\swap}: In order to construct a communication vector as different as possible from its observed demand, the attacker reports the most requested products as the least request ones and vice versa. Therefore, the highest demand among the products is interchanged with the lowest demand, the second highest demand is interchanged with the second lowest demand and so forth.
    \item{\flip:} Adversary $i$ modifies its observed demand $\mathbf{d}_i$ by mirroring it with respect to $\eta=\frac{1}{M}\sum_{j=1}^M d_{ij}$, such that products demanded less than $\eta$ are reported as being requested more, and conversely, highly demanded products are reported as less popular.
    \end{itemize}
   
    
    \item \textit{Adaptive Attacker}: The attacker communication policy is trained using the PPO algorithm, and its reward is set as the negative reward of the victim agent. The attacker uses a Gaussian policy with a softmax activation in the output layer to learn a adversarial probability distribution across products, which is then scaled by the total observed demands $\sum_{j=1}^M d_{ij}$ to construct the communication message.

\end{itemize} 


 

\textbf{Implementation of Baselines}\quad 
\begin{itemize}
    \item \textit{Vanilla Learning}: In the vanilla training method with no defense mechanism against adversarial  communication, we train a shared policy network using agents' local observations and their received communication messages.
     \item \textit{Adversarial Training (AT)}: We alternate between training the agent action policy and the victim communication policy, both using PPO. For the first iteration we train the policies for $10000$ episodes, and then use $1000$ episodes for $5$ additional training alteration iterations for both the action policy and the adversarial communication policy. For more efficient adversarial training, we first shuffle the received communication messages before feeding them into the policy network. Consequently, the trained policy  treats communications received from different agents in a similar manner, and we are able to only train the policy with a fixed set of adversarial agents rather than training the network on all possible combinations of adversarial agents. We do not shuffle the  communication messages being input to the policy trained with vanilla learning as we did not observe improved convergence, as in the FoodCollector environment. %\ys{maybe mention the communication permuting here? and explain why permutation is not used for vanilla (performance no better than vanilla). }

\end{itemize}


 


\subsection{Experiment Results in Market Environment}
\label{app:market_res}

\paragraph{Robust performance Under Attacks} \quad
In this section, we evaluate robustness of the proposed \ours defense strategy in MarketEnv and compare it against Vanilla Learning and Adversarial Training. Figure~\ref{fig:res_all_market} shows the natural and robust performance of \ours with $k=2$, which provides performance guarantees against up to $C=2$ adversarial messages. The performance is compared with AT when the agents policy is alternatively trained against $2$ adversaries. We observe that there is a considerable reduction in the Vanilla and AT rewards under attacks, especially for the strong adaptive attack and \swap. Similar to the FoodCollector, adversarial training is not robust to adversarial communications in the MarketEnv such that for two or more adversarial messages the performance is close to or much lower than the reward achieved with no communications. However, as expected for $k=2$, \ours is able to achieve rewards comparable to the no-attack case  under $C=1$ and $C=2$ adversaries even for strong adversarial attacks. Moreover, \ours outperforms the baselines for $C=3$ for which the theoretical guarantees no longer hold. Even though the gap between natural and robust performance under the weak \permute is less for all three strategies, \ours achieves the highest reward. In  MarketEnv, \ours is able to preserve the communication gains arising from informative messages shared among the agents while being robust against adversarial communications.

  
 
\input{fig_market_res}

\paragraph{Hyper-parameter Test of Ablation Size $\boldsymbol k$} 
Figure~\ref{fig:res_k_cont_market}(left)  shows how the agent's natural performance and robustness varies with the ablation size $k$. We compare \ours’s natural reward and \ours’s reward under $C=2$ adversarial communication messages for adaptive and non-adaptive attacks  with different values of $k$. Similar to the FoodCollector, As the ablation size $k$ increase, the agent is able to improve its natural performance by utilizing information communicated by more agents. However, the agent becomes more vulnerable to adversarial communications which can impacts its decision-making for managing its inventory. Therefore, ablation size $k$ trades off robustness for natural performance. Additionally, we observe that the non-adaptive \swap which constructs the  adversarial communications strategically to mislead the victim agent is quite effective in reducing the victims reward compared to the \permute which communicates adversarial messages without tactically modifying the adversary's observed demands.
 
\paragraph{Hyper-parameter Test of Sample Size $\boldsymbol D$}
In Figure~\ref{fig:res_k_cont_market}(right), we evaluate the robustness of the partial-sample variant of \ours presented in Section~\ref{sec:algo_partial} against $C=2$  adversaries for ablation size $k=2$, when $D$  varies from $36$ (the largest sample size) to $1$ (the smallest sample size). It is shown that with lower $D$, \ours achieves lower rewards under adversarial communications, but is considerably more robust compared to the baseline method. When the agent makes decisions based on a single random message with $D=1$, the agent's average robust reward is higher than the Vanilla reward.

\input{fig_market_k_dist} 



 

==> cmarl/a7_exp_arxiv.tex <==


\section{Additional Implementation Details and Results in FoodCollector}
\label{app:exp}

\subsection{Description of FoodCollector Environment}
\label{app:exp_env}

The FoodCollector environment is a 2D particle world shown by Figure~\ref{fig:food}(left). There are $N=9$ agents with different colors, and $N$ foods with colors corresponding to the $N$ agents. Agents are rewarded when eating foods with the same color. A big round obstacle is located in the center of the map, which the agent cannot go through. There are some poisons (shown as black dots) in the environment, and the agents get penalized whenever they touch the poison. Each agent has 6 sensors that detect the objects around it, including the poisons and the colored foods. 
The game is episodic, with horizon set to be 200. In the beginning of each episode, the agents, foods and poisons are randomly generated in the world. 
At every step, each agent will receives a negative reward $-0.5$ if it has not eaten all its food. Therefore, every agent should explore the environment and eat all food as fast as possible.
% Every time an agent eats a food, the food disappears, and the world re-generate a food with the same color in a random position. Therefore, an agent is supposed to explore the world and to eat as many foods as possible within limited number of steps.

Each of the 6 sensors can detect the following values when the corresponding element is within the sensor's range:\\
(1) (if detects a food) the distance to a food (real-valued); \\
(2) (if detects a food) the color of the food (one-hot); \\
(3) (if detects an obstacle) the distance to the obstacle (real-valued); \\
(4) (if detects the boundary) the distance to the boundary (real-valued); \\ (5) (if detects another agent) the distance to another agent (real-valued).\\
The observation of an agent includes an agent-identifier (one-hot encoding), its own location (2D coordinates), its own velocity, two flags of colliding with its food and colliding with poison, and the above sensory inputs. So, the observation space is a ($7N+30$)-dimensional vector space. 

The action space can be either \textit{discrete} or \textit{continuous}. For the discrete version, there are 9 actions including 8 moving directions (north, northwest, west, southwest, south, southeast, east, northeast) and 1 no-move action. For the continuous version, the action is an acceleration decision, denoted by a 2-dimensional real-valued vector, with each coordinate taking values in $[-0.01,0.01]$. 

% \begin{figure}[h]
% % \vspace{-1em}
%     \centering
%     % \includegraphics[width=0.5\columnwidth]{figs/foodcollector.png}
%     % \vspace{-0.5em}
%     % \caption{The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. }
%     % \label{fig:food}
%     \centering
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \input{figs/comm_dist}
%         % \vspace{-0.1cm}
%         \caption{Discrete action space}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \input{figs/comm_cont}
%         % \vspace{-0.1cm}
%         \caption{Continuous action space}
%     \end{subfigure}
% % \vspace{-0.5em}
% \caption{Reward of agents trained with communication v.s. without communication. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.}
% \label{fig:food_comm}
% % \vspace{-0.4cm}
% \end{figure}

Due to the limited sensory range, every agent can only see the objects around it and thus only partially observe the world. Therefore, communication among agents can help them find their foods much faster. Since our focus is to defend against adversarially perturbed communications, we first define a valid and beneficial communication protocol, where an agent sends a message to a receiver once it observes a food with the receiver's color. For example, if a red agent encounters a blue food, it can then send a message to the blue agent so that the blue agent knows where to find its food. 
% The communication follows the protocol below. Once agent $i$ detects the location of some food or poison from its sensors, it will update the communication channel to every other agent with the latest sensor observation containing its position and its sensory data, which contains the relative location of the food and/or poison. 
To remember the up-to-date communication, every agent maintains a list of most recent $N-1$ messages sent from other $N-1$ agents.
A message contains the sender's current location and the relative distance to the food (recorded by the 6 sensors). Therefore, a message is a $8$-dimensional vector, and each agent's communication list has $8(N-1)$ dimensions in total.

During training with communication, we concatenate the observation and the communication list of the agent to an MLP-based policy, compared to the non-communicative case where the policy only takes in local observations.
As verified in Figure~\ref{fig:food}, communication does help the agent to obtain a much higher reward in both discrete action and continuous action cases, which suggests that the agents tend to rely heavily on the communication messages for finding their food. 
% \fh{Since we will consider the communication protocol as part of the environment, shall we describe the protocol concretely here in this foodcollector experiment?}




\subsection{Implementation Details}
\label{app:exp_imple}

\textbf{Implementation of Trainer}\quad
In our experiments, we use the Proximal Policy Optimization (PPO) \cite{schulman2017proximal}  algorithm to train all  agents as well as the  attackers. Specifically, we adapt from the elegant OpenAI Spinning Up \cite{SpinningUp2018} Implementation for PPO training algorithm. On top of the Spinning Up PPO implementation, we also keep track of the running average and standard deviation of the observation and normalize the observation.

For the policy network, we use a multi-layer perceptron (MLP) with two hidden layers of size 64. Because the action space of our environment is bounded between -0.01 and 0.01, we parameterize the policy as a Beta distribution, which has been proposed in previous works to better solve reinforcement learning problems with bounded actions  \cite{pmlr-v70-chou17a}. In particular, we parameterize the shape parameteres of the Beta distribution as $\alpha=\log(1+e^{\alpha_{\theta}(s)})+1$ and $\beta=\log(1+e^{\beta_{\theta}(s)})+1$ (1 is added to make sure that $\alpha, \beta\geq 1$). $\pi(a|s)=f(\frac{a-h}{2h};\alpha, \beta)$, where $h=0.01$, and $f(x;\alpha, \beta)=\frac{\Gamma(\alpha+\beta)}{\Gamma(\alpha)\Gamma(\beta)}x^{\alpha-1}(1-x)^{\beta-1}$ is the density function of the Beta Distribution.
For the value network, we also use an MLP with two hidden layers of size 64. 

In terms of other hyperparameters used in the experiments, we use a learning rate of 0.0003 for the policy network, and a learning rate of 0.001 is used for the value network. We use the Adam optimizer with $\beta_1=0.99$ and  $\beta_2 = 0.999$. For every training epoch, the PPO agent interacts with the environment for 4000 steps, and it is trained for 500 epochs in our experiments.

% \textcolor{purple}{PH: before describing the  type of attackers, should we mention what an attacker is training. For example, we say below that " The action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1." Perhaps we can state it here to make it more clear the attacker is learning a communication policy and not taking over the actions of agents?}


\textbf{Attacker}\quad
An attacker maps its own observation to the malicious communication messages that it will send to the victim agent. Thus, the action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1. 
% \vspace{-0.2cm}
\begin{itemize}
\item \emph{Non-adaptive Attacker}\quad
We implement a fast and naive attacking method for the adversary. At every dimension, the naive attacker randomly picks 1 or -1 as its action, and then sends the perturbed message which consists entirely of 1 or -1 to the victim agent. 
% \vspace{-0.2cm}
\item \emph{Adaptive RL Attacker}\quad
We use the PPO algorithm to train the attacker, where we set the reward of the attacker to be the negative reward of the victim. The attacker uses a Gaussian policy, where the action is clipped to be in the valid communication range. The network architecture and all other hyperparameter settings follow the exact same from the clean agent training.
\end{itemize}
\vspace{-0.2cm}

\textbf{Implementation of Baselines}\quad
% \vspace{-0.2cm}
\begin{itemize}
\item \emph{Vanilla Learning}\quad
For Vanilla method, we train a shared policy network to map observations and communication to actions. Note that the messages are symmetric (of the same format), we shuffle the messages before feeding them into the policy network, to reduce the bias caused by agent order. We find that shuffling the messages helps the agent converge much faster (50\% fewer total steps).
% \vspace{-0.2cm}
\item \emph{Adversarial Training (AT)}\quad
For adversarial training, we alternate between the training of attacker and the training of the victim agent. Both the victim and attackers are trained by PPO. For every 200 training epochs, we switch the training, where we either fix the trained victim and train the attacker for the victim or fix the trained attacker and train the victim under attack. We continue this process for 10 iterations. Similar to Vanilla, the victim also shuffles the communication messages to obtain higher reward and converge faster.
\end{itemize}
\vspace{-0.2cm}


\emph{Adversarial Training does not improve agent's robust performance.}
As we observed in Figure \ref{fig:res_all}, adversarial training does not improve the robustness of the agent in both discrete and continuous action space, although AT achieves good robustness against observation attacks in a single-agent environment~\cite{zhang2021robust}. 
We hypothesize that it is due to (1) the large number of total agents, and (2) the uncertainty of adversarial message channels. 
To be more specific, during the training of AT, we alternately train the agent and the attacker, and the attacker can change the channels it controls among iterations. As a result, the agent might not be able to distinguish adversarial messages and benign messages. 
% We hypothesize that it is due to the communication shuffling of the agent. In fact, this is also similar to another practical scenario where at different time steps, the attacker might hijack different agents. As a consequence, in both scenarios, malicious messages could randomly appear in any part of the agent's input vector. 
Therefore, simply training the agent and attacker together cannot make the agent learn how to detect the malicious messages and ignore them. 


\subsection{Additional Experiment Results}
\label{app:exp_res}

In addition to Figure \ref{fig:res_hyper}, we also provide the plot for Hyper-parameter test in discrete-action FoodCollector in Figure \ref{fig:res_k_dist}. 
\input{fig_food_k_dist}




\section{Additional Implementation Details and Results in MarketEnv}
\label{app:market}

% \textcolor{red}{we need to mention in the main text that we have additional experiments on MarketEnv in the Appendix} 

\subsection{Description of Market Environment}
\label{app:market_env}
The \textit{MarketEnv} environment is an inventory management setup, where $N=10$ heterogeneous seller agents carry inventory for $M=3$ products. A population of $B=300$ buyers request a product from a randomly selected seller agent according to a demand distribution $\mathbf{p}=[p_1,\dots,p_M]$. We denote the demand realization for seller $i$ with $\mathbf{d_i}=[d_{i,1},\dots,d_{i,M}]$. Sellers manage their inventory by restocking products through interacting with the buyers. The game is episodic with horizon set to $50$. At the beginning of each episode, a realization of the demand distribution $\mathbf{p}$ is randomly generated and the agents' inventory for each product is randomly initialized from $[0, \frac{B}{N}]$, where $\frac{B}{N}$ is the expected number of buyers per seller. %\ys{describe the initial inventory in every episode?} 
Sellers are penalized for mismatch between their inventory and the demand for a product, and they aim to restock enough units of a product at each step to prevent insufficient inventory without accruing a surplus at the end of each step.  %\ys{defining the reward function by math?}
\begin{itemize}
    \item State observation: A seller agent's observation includes its inventory for each product, and the products that were requested by buyers during the previous step. The observation space is a $2M$-dimensional vector.
    
    \item Agent action: Sellers manage their inventory by restocking new units of each product or discarding part of the leftover inventory at the beginning of each step. Hence, agents take both positive and negative actions denoted by an $M$-dimensional vector, and the action space can be either discrete or continuous. In our experiments, we use continuous actions assuming that products are divisible and sellers can restock and hold fractions of a product unit.
    
    \item Agent reward function: During each step, agent $i$'s reward is defined as $r_i = - || \max( \mathbf{I}_i+\mathbf{a}_i, 0) - \mathbf{d}_i||_2$, where $\mathbf{I}_i$ denotes the agents initial inventory vector, and $\mathbf{a}_i$ denotes the inventory restock vector from action policy $\pi_i$.  
    
    
    \item Agent communication: Sellers learn the demand distribution and optimize their inventory by interacting with their own customers (i.e., portion of buyers that request a product from that seller). Sellers would benefit from sharing their observed demands with each other, so that they could estimate the demand distribution more accurately for managing inventory. At the end of each step, a seller communicates an $M$-dimensional vector reporting its observed demands to all other agents. In the case of adversarial communications, this message may differ from the agents' truly observed demands.
    
    During training with communication, messages received from all other agents are concatenated to the agent's observation, which is used to train an MLP-based policy, compared to the non-communicative case where the policy is trained using only local observations. As observed from Figure \ref{fig:marketenv_comm}, communication helps agents obtain  higher rewards since they are able to manage their inventory based on the overall demands observed across the population of buyers rather than their local observation. Results are reported by averaging rewards corresponding to $5$ experiments run with different training seeds.
\end{itemize}
 
\begin{figure}[h]
\vspace{-0.1cm}
 \centering
\resizebox{.4\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_comm_dist}}
\vspace{-0.1cm}
\caption{\textbf{MarketEnv}: Reward of agents trained with communication v.s. without communication. %Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.
} 
\label{fig:marketenv_comm}
\end{figure}
 
 



\subsection{Implementation Details}
\label{app:market_imple}
\textbf{Implementation of Trainer}\quad 
As in the FoodCollector experiments, we use the PPO algorithm to train all agent action policy as well as adversarial agent communication policies. We use the same MLP-based policy and value networks as the FoodCollector but parameterize the policy as a Gaussian distribution. The PPO agent interacts with the environment for $50$ steps, and it is trained for $10000$ episodes. The learning rate is set to be 0.0003 for the policy network, and 0.001 for the value network.
% All other hyper-parameters are set similar to the FoodCollector experiments.


\textbf{Attacker}\quad 
The attacker uses its observations to communicate malicious messages to  victim sellers, and its action space is the communication space of a benign agent.  We consider the following non-adaptive and adaptive attackers:
\begin{itemize}
    \item \textit{Non-adaptive Attacker}: The attacker's goal is to harm the victim agent by misreporting its observed demands so that the victim seller under-estimates or over-estimates the restocking of products. In our experiments, we evaluate the effectiveness of defense strategies against the following attack strategies:
    \begin{itemize}
     \item{\permute}: The communication message is a random permutation of the true demand vector observed by the attacker.
    \item {\swap}: In order to construct a communication vector as different as possible from its observed demand, the attacker reports the most requested products as the least request ones and vice versa. Therefore, the highest demand among the products is interchanged with the lowest demand, the second highest demand is interchanged with the second lowest demand and so forth.
    \item{\flip:} Adversary $i$ modifies its observed demand $\mathbf{d}_i$ by mirroring it with respect to $\eta=\frac{1}{M}\sum_{j=1}^M d_{ij}$, such that products demanded less than $\eta$ are reported as being requested more, and conversely, highly demanded products are reported as less popular.
    \end{itemize}
   
    
    \item \textit{Adaptive Attacker}: The attacker communication policy is trained using the PPO algorithm, and its reward is set as the negative reward of the victim agent. The attacker uses a Gaussian policy with a softmax activation in the output layer to learn a adversarial probability distribution across products, which is then scaled by the total observed demands $\sum_{j=1}^M d_{ij}$ to construct the communication message.

\end{itemize} 


 

\textbf{Implementation of Baselines}\quad 
\begin{itemize}
    \item \textit{Vanilla Learning}: In the vanilla training method with no defense mechanism against adversarial  communication, we train a shared policy network using agents' local observations and their received communication messages.
     \item \textit{Adversarial Training (AT)}: We alternate between training the agent action policy and the victim communication policy, both using PPO. For the first iteration we train the policies for $10000$ episodes, and then use $1000$ episodes for $5$ additional training alteration iterations for both the action policy and the adversarial communication policy. For more efficient adversarial training, we first shuffle the received communication messages before feeding them into the policy network. Consequently, the trained policy  treats communications received from different agents in a similar manner, and we are able to only train the policy with a fixed set of adversarial agents rather than training the network on all possible combinations of adversarial agents. We do not shuffle the  communication messages being input to the policy trained with vanilla learning as we did not observe improved convergence, as in the FoodCollector environment. %\ys{maybe mention the communication permuting here? and explain why permutation is not used for vanilla (performance no better than vanilla). }

\end{itemize}


 


% \subsection{Experiment Results in Market Environment}
% \label{app:market_res}

% \paragraph{Robust performance Under Attacks} \quad
% In this section, we evaluate robustness of the proposed \ours defense strategy in MarketEnv and compare it against Vanilla Learning and Adversarial Training. Figure~\ref{fig:res_all_market} shows the natural and robust performance of \ours with $k=2$, which provides performance guarantees against up to $C=2$ adversarial messages. The performance is compared with AT when the agents policy is alternatively trained against $2$ adversaries. We observe that there is a considerable reduction in the Vanilla and AT rewards under attacks, especially for the strong adaptive attack and \swap. Similar to the FoodCollector, adversarial training is not robust to adversarial communications in the MarketEnv such that for two or more adversarial messages the performance is close to or much lower than the reward achieved with no communications. However, as expected for $k=2$, \ours is able to achieve rewards comparable to the no-attack case  under $C=1$ and $C=2$ adversaries even for strong adversarial attacks. Moreover, \ours outperforms the baselines for $C=3$ for which the theoretical guarantees no longer hold. Even though the gap between natural and robust performance under the weak \permute is less for all three strategies, \ours achieves the highest reward. In  MarketEnv, \ours is able to preserve the communication gains arising from informative messages shared among the agents while being robust against adversarial communications.

  
 
% \input{fig_market_res}

% \paragraph{Hyper-parameter Test of Ablation Size $\boldsymbol k$} 
% Figure~\ref{fig:res_k_cont_market}(left)  shows how the agent's natural performance and robustness varies with the ablation size $k$. We compare \ours’s natural reward and \ours’s reward under $C=2$ adversarial communication messages for adaptive and non-adaptive attacks  with different values of $k$. Similar to the FoodCollector, As the ablation size $k$ increase, the agent is able to improve its natural performance by utilizing information communicated by more agents. However, the agent becomes more vulnerable to adversarial communications which can impacts its decision-making for managing its inventory. Therefore, ablation size $k$ trades off robustness for natural performance. Additionally, we observe that the non-adaptive \swap which constructs the  adversarial communications strategically to mislead the victim agent is quite effective in reducing the victims reward compared to the \permute which communicates adversarial messages without tactically modifying the adversary's observed demands.
 
% \paragraph{Hyper-parameter Test of Sample Size $\boldsymbol D$}
% In Figure~\ref{fig:res_k_cont_market}(right), we evaluate the robustness of the partial-sample variant of \ours presented in Section~\ref{sec:algo_partial} against $C=2$  adversaries for ablation size $k=2$, when $D$  varies from $36$ (the largest sample size) to $1$ (the smallest sample size). It is shown that with lower $D$, \ours achieves lower rewards under adversarial communications, but is considerably more robust compared to the baseline method. When the agent makes decisions based on a single random message with $D=1$, the agent's average robust reward is higher than the Vanilla reward.

% \input{fig_market_k_dist} 


\section{Additional Implementation Details of MARL-MNIST Environment}
\label{app:mnist}

\subsection{Description of MARL-MNIST Environment}

We use the environment setup proposed by~\cite{mousavi2019multi}, where agents collaboratively classify an unknown image by their observations and inter-agent communication. 
More specifically, we use $N=9$ agents in the MNIST dataset of handwritten digits~\cite{lecun1998gradient}.  The dataset consists
of 60,000 training images and 10,000 testing images, where
each image has $28 \times 28$ pixels. 
There are $h=5$ steps in an episode. In the beginning, all agents start from a pre-determined spatial configuration. At every step, each agent observes a local $5 \time 5$ patch, performing some local data processing, and communicating the result with neighboring agents (we use a fully connected communication graph). 
With given observation and communication, each agent outputs an action in $\{Up, Down, Left, Right\}$. By each movement, the agent is translated in the desired direction by $5$ pixels. In the end of an episode, agents make predictions, and all of them are rewarded by $- prediction_loss$. 


\subsection{Implementation Details}

We use the same network architecture and hyperparameter setting as~\cite{mousavi2019multi}, which are implemented in~\cite{mnistgithub}. 

\textbf{Network Architecture}\quad
Concretely, at every step, the input of every agent contains 3 components: (1) an encoded observation with two convolutional layers followed by vectorization and a fully connected layer; (2) the average of all communication messages from other agents; (3) a position encoding computed by feeding the current position into a single linear layer.
These 3 components are concatenated and passed to two independent LSTM modules, one is for an acting policy, another is for a message generator. 
In the end of an episode, every agent uses its final cell state to generate a prediction using a 2-layer MLP. Then we take the average of the output logits of all agents, and use a softmax function to obtain the final probabilistic label prediction. The reward is the opposite number of the L2 difference between the prediction and the one-hot encoding of true image label.

\textbf{Hyperparameters}\quad
In our experiments, we follow the default hyperparameter setting in~\cite{mnistgithub}. We use $N=9$ agents. The size of LSTM belief state is 128. The hidden layers have size 160. The message size is set to be 32. The state encoding has size 8. We use an Adam optimizer with learning rate 1e-3. We train the agents in the MNIST dataset for 40 epochs.

\textbf{Attackers}\quad
Since the communication messages are learned by neural networks, we perturb the $C$ messages received by each agent. To make sure that the messages are not obviously detectable, we clip every dimension of the perturbed message into the range of $[-3,3]$. The non-adaptive attacker randomly generates a new message. The adaptive attacker learns a new message generator based on its own belief state, which is trained with learning rate 1e-3 for 50 epochs.


\section{Additional Discussion on the Choice of Ablation Size $\boldsymbol k$}
\label{app:hyper}

In our proposed \ours defensive mechanism, the most crucial hyperparameter is the ablation size $k$. 
% Decreasing the ablation size $k$ trades off natural performance under no attack for robust performance under attack. 
Choosing a smaller $k$ could make the agents more robust, but could also potentially hurt their natural performance since the agents would have access to less information shared by others. Based on the previous experimental results, it is crucial to set $k$ such that condition $\eqref{eq:k_cond}$ is satisfied so that the agent could have performance certificate and thus remains robust under attack. 


In practice, if we have an estimate of the number of attackers that we would like to defend against, then we could choose the maximum $k$ satisfying Equation \eqref{eq:k_cond}. If not, based on the total number of agents, we could say that \ours could certifiably defend up to maximum $C$ attackers. So there is an interdependence between three parameters: total number of agents $N$, number of attackers $C$, and the ablation size $k$. In Figure \ref{fig:ablation_cnk} we visualize their relationship by fixing one variable at a time. From these figures, we can see an obvious trade-off between $C$ and $k$ --- if there are more attackers, $k$ has to be set smaller. But when $C$ is small, e.g. $C=1$, $k$ can be relatively large, so the agent does not need to compromise much natural performance to achieve robustness. 
% Importantly, when $C$ is much smaller than $N$, e.g. $C=1, N=30$, $k$ can be set relatively large, e.g. 15. Therefore, the natural performance is not compromised too much to achieve robustness. \textcolor{purple}{PH: not a big deal, but $K$ in the figures (title and legend) is upper case rather than lowercase $k$ used in the paper YS: fixed!}

\begin{figure*}[h]
\vspace{-0.1cm}
 \centering
    \begin{subfigure}[t]{0.31\textwidth}
    \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_C&K}}
     \label{sfig:C&K}
     \vspace{-0.5cm}
      \subcaption{$C$ vs. $k$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_N&C}}
     \label{sfig:N&C}
     \vspace{-0.5cm}
      \subcaption{$N$ vs. $C$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \resizebox{\textwidth}{!}{\input{figs/Ablation_N&K}}
     \label{sfig:N&K}
     \vspace{-0.5cm}
     \subcaption{$N$ vs. $k$}
    \end{subfigure}
% \vspace{-0.3cm}
\caption{Relationship between the total number of agents $N$, number of attackers $C$, and ablation size $k$. \textbf{(a)}: Maximum certifiable ablation size $k$ under different number of attackers. \textbf{(b)}: Maximum defensible number of attackers $C$ with different total number of agents $N$. \textbf{(c)}: Maximum certifiable ablation size $k$ with different total number of agents $N$.}
\label{fig:ablation_cnk}
\vspace{-0.1cm}
\end{figure*}
\label{app:exp}


 \section{Discussion: Detecting Malicious Messages with Ablation}
\label{app:exp_detect}

Theorem~\ref{thm:main_dist} and Theorem~\ref{thm:main_cont} provide strong theoretical guarantees for the proposed \ours defense. For the theorems to hold, one has to choose a $k$ to satisfy Equation \eqref{eq:k_cond}. As shown in Figure~\ref{fig:ablation_cnk}, to defend against a larger $C$, one has to choose a relatively small $k$ for certifiable performance. However, Figure \ref{sfig:hyper_k_food}, Figure \ref{sfig:hyper_k_market} and Figure~\ref{fig:res_k_dist} suggest that a small $k$ also sacrifices the natural performance of the agent to obtain higher robustness. This is known as the trade-off between robustness and accuracy~\cite{tsipras2018robustness,zhang2019theoretically}. Can we achieve better robustness while not sacrificing much natural performance, or obtain higher natural reward while not losing robustness?

We point out that with our proposed \ours defense, it is possible to choose a larger $k$ than required by condition~\ref{eq:k_cond} without sacrificing robust performance by identifying the malicious messages beforehand. We hypothesize that given a well-trained victim policy, malicious messages should mislead the victim agent to take an action that is "far away" from a "good" action that the victim is supposed to take.

To verify this hypothesis, we first train the agent $i$ with a randomized ablation policy of $k=1$. Then for every communication message that another agent $j$ sends, we compute the action $a_j$ that the victim policy $\pi_i$ chooses based on all message subsets containing message $m_{j\to i}$, i.e. $a_j = \ablpolicy(o, m_{j\to i})$ (note that $k=1$ so $\ablpolicy$ only takes in one message at a time). We then define the \emph{action bias} as $\nu_j=\|a_j-\funmed\{a_k\}_{k=1}^{N}\|_1$. Based on our hypothesis, an agent which has been hacked by attackers should induce a significantly larger action bias since they are trying to mislead the victim to take a completely different action. Here, we execute the policy of two hacked agents together with six other good agents for twenty episodes and calculate the average action bias for each agent.
As shown in in Figure \ref{fig:detect_adv}, the agents hacked by attackers indeed induce a larger action bias compared to other benign agents, which suggests the effectiveness of identifying the malicious messages by action bias. 

% Note that although there is no theoretical guarantee for identifying the adversarial communication messages, 
After filtering out $A$ messages, one could compute the required $k$ by Equation~\ref{eq:k_cond} based on $C-A$ malicious messages and $N-A$ total messages, which can be larger than the largest $k$ induced by $C$ malicious messages out of $N$ total messages. For example, if $N=30$, $C=3$, then the largest $k$ satisfying Equation~\ref{eq:k_cond} is 5, but when 1 adversarial message is filtered out, the largest $k$ that can defend against the remaining 2 adversarial messages is 8. Although the adversary identification is not theoretically guaranteed to be accurate, Figure \ref{fig:detect_adv} demonstrates the effectiveness of the adversarial message detection, which, combined with \ours with larger $k$'s, has the potential to achieve high natural performance and strong robustness in practice.
% one could still apply Theorem \ref{thm:main_cont} with $C-A$ malicious messages and $N-A$ good messages in total.
\begin{figure}[h]
\vspace{-0.1cm}
 \centering
\input{figs/Attacker Identification.tex}
\vspace{-0.3cm}
\caption{Attacker identification based on action bias $\nu_j$. Adv1 and Adv2 stands for two agents hacked by the attacker. B1 up to B6 stands for six other benign agents.}
\vspace{-0.5cm}
\label{fig:detect_adv}
\end{figure}

==> cmarl/algo_test.tex <==
% \begin{figure}[t]
% % \vspace{-0.5em}
% \vspace{-2em}
% \centering
% \begin{algorithm}[H]
%   \caption{Testing Phase of \ours}
%   \label{alg:test}
% \begin{algorithmic}[1]
%     \STATE {\bfseries Input:} trained ablation policy $\ablpolicy_i, \forall i \in [N]$, \\ 
%     \quad\quad ablation size $k$ satisfying Inequality~\eqref{eq:k_cond}, \\
%     \quad\quad sample size $0<D\leq\binom{N-1}{k}$
%   \REPEAT
%       \FOR{$i=1$ {\bfseries to} $N$}
%             \STATE Observe $o_i$, receive a list of messages $\mtoi$ with at most $C$ malicious messages
%             \STATE Randomly select $D$ samples $\{T_d\}_{d=1}^D$ from $\mathcal{H}(N-1,k)$ (without replacement)
%             \STATE Take $a\leftarrow$ {\small{$\smpolicy_i (o_i, \{\funabl(\mtoi, T_d)\}_{d=1}^D)$}},
%             % $a_i \leftarrow \smpolicy_i (o_i, \mtoi, \{T_d\}_{d=1}^D)$, 
%             where $\smpolicy$ is the ensemble policy defined by Equation~\eqref{eq:ensemble_pi_dist} for discrete $\mathcal{A}_i$, and Equation~\eqref{eq:ensemble_pi_cont} for continuous $\mathcal{A}_i$
%       \ENDFOR
%   \UNTIL{end of test}
% \end{algorithmic}
% \end{algorithm}
% \vspace{-2em}
% \end{figure}

\begin{figure}[h]
% \vspace{-0.5em}
\vspace{-2em}
\centering
\begin{algorithm}[H]
   \caption{Defending Phase of \ours}
   \label{alg:test}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} ablation size $k$; trained \ablname $\ablpolicy_i, \forall i \in [N]$, \\ 
    % \quad\quad 
    % satisfying Equation~\eqref{eq:k_cond}
   \REPEAT
       \FOR{$i=1$ {\bfseries to} $N$}
            \STATE Receive a list of messages $\mtoi$ with at most $C$ malicious messages, get local observation $o_i$ and update interaction history $\his_i$
            \STATE Take $\widetilde{a}_i \leftarrow \smpolicy_i (\his_i, \mtoi)$, 
            % {\small{$\smpolicy_i (o_i, \{\funabl(\mtoi, T_d)\}_{d=1}^D)$}},
            where $\smpolicy_i$ is the \ensname defined with $\ablpolicy$ by Equation~\eqref{eq:ensemble_pi_dist} for discrete $\mathcal{A}_i$, and Equation~\eqref{eq:ensemble_pi_cont} for continuous $\mathcal{A}_i$
       \ENDFOR
   \UNTIL{end of test}
\end{algorithmic}
\end{algorithm}
% \vspace{-2.5em}
\end{figure}

==> cmarl/algo_train.tex <==
\begin{figure}[h]
\vspace{-1em}
\centering
\begin{algorithm}[H]
\caption{Training Phase of \ours}
\label{alg:train}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} ablation size $k$
   \STATE Initialize $\ablpolicy_i$ for every agent $i \in [N]$.
   \REPEAT
       \FOR{$i=1$ {\bfseries to} $N$}
            \STATE Receive a list of messages $\mtoi$, get local observation $o_i$ and update interaction history $\his_i$
            \STATE Randomly sample $\msgki\sim \mathrm{Uniform}(\allmsgki)$
            \STATE Take action based on $\his_i$ and the \ksample $\msgki$, i.e.,
            $a_i \leftarrow \ablpolicy_i (\his_i, \msgki)$ 
            % \fh{$a_i \leftarrow \ablpolicy_i (o_i, \funabl(\mtoi, T))$?}
            \STATE Update the replay buffer and policy $\ablpolicy_i$
       \ENDFOR
   \UNTIL{end of training}
   \STATE {\bfseries Output:} \ablname $\ablpolicy_i, \forall i \in [N]$
\end{algorithmic}
\end{algorithm}
\vspace{-1em}
\end{figure}

==> cmarl/arxiv/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% \draft{We study the attacks and defenses in communicative multi-agent reinforcement learning.
% Our contributions:
% 1. formulate the adversarial problem in CMARL.
% 2. propose a certifiable defense algorithm
% 3. empirical study in a simulated game and a market environment.
% }
% Recent years have witnessed significant advances in reinforcement learning (RL), especially deep reinforcement learning (DRL). Although vanilla RL considers the interaction between a single agent and the environment, many real-world applications have multiple agents involved, such as autonomous driving~\cite{shalev2016safe}, robotics~\cite{dudek1996taxonomy}, etc. 
% \ys{start from decision making?}
% With the rapid improvement of deep reinforcement learning (DRL) techniques, neural network-based 
Neural network-based multi-agent reinforcement learning (MARL) has achieved significant advances in many real-world applications, such as autonomous driving~\cite{shalev2016safe,sallab2017deep}. In a multi-agent system, especially in a cooperative game, communication usually plays an important role. By feeding communication messages as additional inputs to the policy network, each agent can obtain more information about the environment and other agents, and thus can learn a better policy~\cite{foerster2016learning,hausknecht2016cooperation,sukhbaatar2016learning}. 
% Many recent works~\cite{foerster2016learning,hausknecht2016cooperation,sukhbaatar2016learning} have shown that feeding communication messages to RL networks can result in better decision makers.

However, neural networks are shown to be vulnerable to adversarial attacks~\cite{chakraborty2018adversarial}, i.e.,
% , especially network-based RL policies~\cite{huang2017adversarial} \fh{network-based RL policies are not a special case of neural networks. So the logic here is a bit unsmooth.}, 
a well-trained network may output a wrong answer if the input to the network is slightly perturbed~\cite{goodfellow2014explaining}.
% if the inputs to the network are slightly but deliberately perturbed, the network, although well-trained on clean datasets \fh{rather than datasets, shall we say unattacked environment or safe environment, since RL is not necessarily trained on a ``dataset''?}, may output a wrong answer. 
As a result, although a policy can obtain a high reward by taking in the messages sent by other agents, it may also get drastically misled by inaccurate information or even adversarial communication from malicious attackers. 
For example, when several drones execute pre-trained policies and exchange information via wireless communication, it is possible that messages get noisy in a hostile environment, or even some malicious attacker eavesdrops on their communication and intentionally perturbs some messages to a victim agent via cyber attacks. 
Moreover, even if the communication channel is protected by advanced encryption algorithms, an attacker may also hack some agents and alter the messages before they are sent out (e.g. hacking IoT devices that usually lack sufficient protection~\cite{naik2017cyber}). Figure~\ref{fig:diagram} shows an example of communication attacks, where the agents are trained with benign communication, but attackers may perturb the communication during the test time. The attacker may lure a well-trained agent to a dangerous location through malicious message propagation and cause fatal damage. 
Although our paper focuses on adversarial perturbations of the communication messages, it also includes unintentional perturbations, such as misinformation due to malfunctioning sensors or communication failures; these natural perturbations are no worse than adversarial attacks.

\begin{figure*}[!t]
% \vspace{-3em}
    \centering
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth,natwidth=462,natheight=305]{figs/marl.jpg}
         \vspace{-0.5em}
         \caption{Training time}
         \label{sfig:train}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth,natwidth=483,natheight=308]{figs/marl_adv.jpg}
         \vspace{-0.5em}
         \caption{Test time (in deployment)}
         \label{sfig:test}
     \end{subfigure}
     \vspace{-0.5em}
    \caption{An example of test-time communication attacks in a communicative MARL system.  (a) During training, agents are trained collaboratively in a safe environment, such as a simulated environment. (b) In deployment, agents execute pre-trained policies in the real world, where malicious attackers may modify the benign ({\color{darkpastelgreen}{green}}) messages into adversarial ({\color{red}{red}}) signals to mislead some victim agent(s). 
    % \myst{In this figure, arrows denote communication channels among agents, {\color{darkpastelgreen}{green}} messages stand for benign communication, and {\color{red}{red}} messages stand for adversarial communication.}
    % \myst{Agents can be heterogeneous as depicted by various icons.}
    }
    \label{fig:diagram}
% \vspace{-2em}
\end{figure*}

Although adversarial attacks and defenses have been extensively studied in supervised learning~\cite{madry2018towards,cohen2019certified,zhang2019theoretically} and reinforcement learning~\cite{zhang2020robust,zhang2021robust,oikarinen2020robust}, there has been little discussion on the robustness issue against adversarial communication in MARL problems. 
Therefore, to safely improve decision-making with communication in high-stakes multi-agent scenarios, it is crucial to robustify MARL policies against adversarial communication.  
% \textcolor{red}{Defending against the adversarial communication while still utilizing the benign communication}\fh{needs rewording. Maybe: Achieving high performance in a multi-agent cooperative game through inter-agent communication while remain robust to adversarial communication attacks} 
Achieving high performance in a multi-agent cooperative game through inter-agent communication while being robust to adversarial communication is a challenging problem due to the following reasons. 
\textbf{Challenge I}: 
% \myst{The attacker may construct malicious messages in various ways, so that they are hard to be distinguished from benign messages.} 
% \myst{For example, the malicious messages shown in Figure}~\ref{sfig:test} \myst{are in the same form as the benign messages and also make semantic sense.}
Sometimes communication attacks are stealthier as misleading
messages  (which share the form of benign messages and are semantically meaningful in Figure~\ref{sfig:test}) can be hard to recognize, while attacking by abnormal actions~\cite{gleave2020adversarial} can be easier for humans to notice.
\textbf{Challenge II}: A strong attacker can even be \textit{adaptive} to the victim agent and significantly reduce the victim's total reward. For instance, for a victim agent who moves according to the average of GPS coordinates sent by others, the attacker may learn to send extreme coordinates to influence the average.
% the attacker may learn an RL policy to send sequential misleading messages. \fh{This point is not very clear.}
\textbf{Challenge III}: There can be more than one attacker (or an attacker can perturb more than one message at one step), such that they can collaborate to mislead a victim agent.

Tu et al.~\cite{tu2021adversarial} apply adversarial training~\cite{madry2018towards} to improve model robustness against communication perturbations. But they focus on perturbations with small $\ell_p$ distances, which do not cover many attack scenarios as discussed in Section~\ref{sec:setup_adv}.
Some recent works~\cite{blumenkamp2020emergence,xue2021mis,mitchell2020gaussian} take the first step to investigate adversarial communications in MARL and propose several defending methods, such as a learned message filter~\cite{xue2021mis}. However, these empirical defenses do not fully address the aforementioned challenges, and are not guaranteed to be robust, especially under adaptive attacks. 
% \textcolor{purple}{PH: all communication attacks, any communication attack? YS: should be all, thanks} 
%\textcolor{purple}{PH: Is it clear what we mean by adaptive attacks? In challenge 2 we are kind of defining it. Would it make sense to make the \textit{adaptive} italic in challenge 2 to stand out? YS: Sure! Good point}
% Levine et al.~\cite{Levine_Feizi_2020} use randomized ablation to defend against sparse attacks in image classification, where a fraction of pixels may be corrupted. However, their high-probability guarantee is not suitable for sequential decision-making problems, as the guaranteed probability decreases along propagation over time. Moreover, their algorithm does not work when the policy takes continuous actions. 

In this paper, we address all aforementioned challenges by proposing {a certifiable defense, named \textbf{\oursfull (\ours)}, that can guarantee the performance of agents when a fraction of communication messages are perturbed}. 
The main idea of \ours is to make decisions based on multiple different subsets of communication messages (i.e., ablated messages). Specifically, for a list of messages coming from different agents, we train a \emph{\ablname} that takes in a subset of messages and outputs a \emph{base action}. Then, we construct an \emph{\ensname} by aggregating multiple base actions coming from multiple ablated message subsets. 
% The main idea of \ours is to construct an \emph{ensemble policy} which makes decisions based on multiple different subsets of communication messages (i.e., ablated messages). 
% Specifically, for a list of messages coming from different agents, we train a \emph{base ablation policy} that takes in a subset of messages and outputs a \emph{base action}. 
For a discrete action space, the ensemble policy takes the majority of the multiple base actions obtained, while for a continuous action space, the ensemble policy takes the median of these base actions. \ours is a generic framework that works for any agent that observes multiple messages from different sources, as long as the agent receives more benign communication messages than adversarial ones. We also show in Section~\ref{sec:algo_more} that \ours can be used in many other decision-making scenarios beyond defending against communication attacks. 
A similar randomized ablation idea is used by Levine et al.~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification. However, they provide high-probability guarantee for a single-step decision, which is not suitable for sequential decision-making problems, as the guaranteed probability decreases when it propagates over timesteps. Moreover, their algorithm does not work when the model has a continuous output space. 
In contrast, \ours has robustness guarantees for both the immediate action and the long-term reward, and for both discrete and continuous actions. 
% A similar randomized ablation idea is used by Levine et al.~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification. However, their high-probability guarantee is not suitable for RL \fh{sequential decision-making} problems, as the probability decreases along propagation over time. Moreover, their algorithm does not work for a continuous action space. In contrast, \ours has robustness guarantees for the long-term reward, and works on both discrete and continuous action spaces. 

% \ys{compare to Levine et al. high probability reduces along propagation of time / may not lead to reliable multi-step robustness due to the long horizon.}
% Therefore, \ours can be extended to defend against 
% \ys{flexibility, as discussed later}

Our contributions can be summarized as below:\\
\textbf{(1)} We formulate the problem of adversarial attacks and defenses in communicative MARL (CMARL). \\
% \fhc{Do we still use CMARL? If not, it is fine. If so, explain it.}.\\
\textbf{(2)} We propose a novel defense method, \ours, 
% \SF{perhaps introduce ``ablation" terminology in the previous paragraph so readers become familiar with it at this point}
% based on randomized ablation on communication messages. \ours 
that is certifiably robust against arbitrary perturbations of up to $C<\frac{N-1}{2}$ communications, where $N$ is the number of agents. \\
% both in discrete action space and in continuous action space. \fh{I feel the contribution is not that we include both discrete or continuous action space, but rather, we can achieve very strong results in the discrete space, as well as good results in the continuous space. I feel the current wording sounds a bit off the path.}\\
\textbf{(3)} Experiment in several multi-agent environments shows that \ours obtains significantly higher reward than baseline methods under both non-adaptive and adaptive attackers. 
% The agent trained with \ours achieves similar 
% \SF{add a bit more details here; what environments; discrete or cont; what gains do we achieve?}. 
% \fh{maybe some numbers in terms of performance improvement etc}



==> cmarl/arxiv/2_relate.tex <==
% \vspace{-0.5em}
\section{Related Work}
\label{sec:relate}


\textbf{Adversarial Robustness of RL Agents}\quad
% As RL techniques have been applied to more and more applications, the robustness of agents under environment noise or adversarial attacks becomes an emerging research topic. 
Section~\ref{sec:setup_adv} introduces several adversarial attacks on single-agent and multi-agent problems.
To improve the robustness of agents, adversarial training (i.e., introducing adversarial agents to the system during training~\cite{pinto2017robust,phan2021resilient,zhang2021robust,sun2021strongest}) and network regularization~\cite{zhang2020robust,shen2020deep,oikarinen2020robust} are empirically shown to be effective under $\ell_p$ attacks, although such robustness is not theoretically guaranteed. 
Certifying the robustness of a network is an important research problem~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness}.
% There is an important line of work studying guaranteed robustness of neural networks~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness} when the input data is perturbed within an $\ell_p$ norm ball. 
In an effort to certify RL agents' robustness, some approaches~\cite{lutjens2020certified,zhang2020robust,oikarinen2020robust,fischer2019online} apply network certification tools to bound the Q networks and improve the worst-case value of the policy. Kumar et al.~\cite{kumar2021policy} and Wu et al.~\cite{wu2021crop} follow the idea of randomized smoothing~\cite{cohen2019certified} and smooth out the policy by adding Gaussian noise to the input.



\textbf{Communication in MARL}\quad
Communication is crucial in solving collaborative MARL problems. There are many existing studies learning communication protocols across multiple agents. Foerster et al. \cite{foerster2016learning} are the first to learn differentiable communication protocols that is end-to-end trainable across agents. Another work by Sukhbaatar et al. \cite{sukhbaatar2016learning} proposes an efficient permutation-invariant centralized learning algorithm which learns a large feed-forward neural network to map inputs of all agents to their actions. 
It is also important to communicate selectively, since some communication may be less informative or unnecessarily expensive. To tackle this challenge, Das et al. \cite{das2020tarmac} propose an attention mechanism for agents to adaptively select which other agents to send messages to. Liu et al. \cite{liu2020who2com} introduce a handshaking procedure so that the agents communicate only when needed. Our work assumes a pre-trained communication protocol and does not consider the problem of learning communication mechanisms.

\textbf{Adversarial Attacks and Defenses in CMARL}\quad
Recently, the problem of adversarial communication in MARL has attracted increasing attention.  
Blumenkamp et al.~\cite{blumenkamp2020emergence} show that in a cooperative game, communication policies of some self-interest agents can hurt other agents' performance. 
% To accommodate multiple agent objectives, they propose \change{Aggregation}\fh{aggregated? is aggregation GNN a terminology? I've not heard of it.} Graph Neural Networks to model and learn an inter-agent communication policy. 
To achieve robust communication, Mitchell et al.~\cite{mitchell2020gaussian} adopt a Gaussian Process-based probabilistic model to compute the posterior probabilities that whether each partner is truthful. 
Tu et al.~\cite{tu2021adversarial} investigate the vulnerability of multi-agent autonomous systems against communication attacks, with a focus on vision tasks.
% \change{multiple aspects} \fh{?}.
Xue et al.~\cite{xue2021mis} propose an algorithm to defend against one adversarial communication message by an anomaly detector and a message reconstructor, which are trained with groundtruth labels and messages.

To the best of our knowledge, our \ours is the first certifiable defense in MARL against communication attacks. Moreover, we consider a strong threat model where up to half of the communication messages can be arbitrarily corrupted, capturing many realistic types of attacks.



==> cmarl/arxiv/4_algo_long.tex <==
\section{Provably Robust Defense for CMARL}
\label{sec:algo}

In this section, we present our defense algorithm, \textit{\oursfull (\ours)}, against test-time communication attacks in CMARL. 
% \ours has two phases: the training phase where a base policy is trained for each agent we aim to robustify, and the defending phase where the base policy is used to make
% relatively safe
% decisions via message ablation and ensemble.  
We first introduce the algorithm design in Section~\ref{sec:algo_overview}, then present the theoretical analysis in Section~\ref{sec:algo_theory}.
Section~\ref{sec:algo_more} discusses several extensions of \ours.


\subsection{\oursfull (\ours)}
\label{sec:algo_overview}

% \SF{In the intro, we call the method ensemble policy; we should use the same terminology. I like AME} >> Sure, I added AME to the intro.
% As characterized in Section~\ref{sec:setup}, in a CMARL game, every agent makes decisions based on not only its own observations, but also all received messages. If an agent trusts the communication from all other agents, it may fail when some communication is maliciously corrupted.
% On the other hand, if an agent does not trust communication, it can not benefit from the useful information shared by other benign agents.
% Therefore, there is a trade-off between natural performance (i.e., reward under no attack) and robustness (i.e., reward under attacks).
% Our goal is to learn and execute a robust policy for any agent in the environment, so that the agent can perform well in both a non-adversarial environment and an adversarial environment.


% \textbf{Main Idea}\quad
% Intuitively, if an agent $i$ overly relies on the information given by agent $j$, then a strong adaptive attacker can easily mislead $i$ by perturbing the messages from $j$. On the other hand, if an agent does not trust communication, it can not benefit from the useful information shared by other benign agents.
% Therefore, there is a trade-off between natural performance (i.e., reward under no attack) and robustness (i.e., reward under attacks). 
% 
Our goal is to learn and execute a robust policy for any agent in the environment, so that the agent can perform well in both a non-adversarial environment and an adversarial environment. 
To ease the illustration, we focus on robustifying an arbitrary agent $i\in\agents$, and the same defense is applicable to all other agents.
We omit the agent subscript ${}_i$, and denote the agent's observation space, action space, and interaction history space as $\mathcal{O}$, $\mathcal{A}$, and $\hisspace$, respectively. 
% We aim to train a robust acting policy for the agent as $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$, where $\hisspace$ is the space of the interaction histories.

Let $\msg \in \mathcal{M}^{N-1}$ denote a set of $N-1$ messages received by the agent. Then, we can build an ablated message subset of $\msg$ with $k$ randomly selected messages, as defined below.

\begin{definition}[$\boldsymbol{k}$-Ablation Message Sample (k-Sample)]
For a message set $\msg \in \mathcal{M}^{N-1}$ and any integer $1 \leq k \leq N-1$, define a $k$-ablation message sample (or \ksample for short), $\msgk \in \mathcal{M}^k$, as a set of $k$ randomly sampled messages from $\msg$. Let $\allmsgk$ be the collection of all unique \ksamples of $\msg$, and thus $|\allmsgk|=\binom{N-1}{k}$.
\end{definition}


% \textbf{Notations}\quad
% % \textbf{(1) Agent and policy.} To ease the illustration, we focus on robustifying an arbitrary agent $i\in\agents$, and the same defense is applicable to all other agents.
% % We omit the agent subscript ${}_i$, and denote the agent's observation space and action space as $\mathcal{O}$ and $\mathcal{A}$. We aim to train a robust acting policy for the agent as $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$, where $\hisspace$ is the space of the interaction histories.  \\
% \textbf{(1) Ablated $k$ message samples (k-samples) $\boldsymbol{\msgk}$.} 
% Let $\msg \in \mathcal{M}^{N-1}$ denote a set of messages received by the agent with cardinality $N-1$. For any $1 \leq k \leq N-1$, define a $k$ message sample (or k-sample for short) $\msgk \in \mathcal{M}^k$ as a set of $k$ messages randomly sampled from $\msg$. \\
% \textbf{(2) All k-sample Combinations $\boldsymbol{\allmsgk}$.} 
% Among all $N-1$ messages in $\msg$, there are $\binom{N-1}{k}$ unique k-samples. Let $\allmsgk$ be the collection of all unique k-samples of $\msg$.

% Moreover, the benign messages sent from other agents usually contain redundant/overlapping information.
% \myst{, as the goal of communication is to provide the agent additional information and to help the agent make better decisions. }
Motivated by the fact that the benign messages sent from other agents usually contain overlapping information that may suggest similar decisions, the \textbf{main idea} of our defense is to make decisions based on the \emph{consensus} of the benign messages. 
To be more specific, we train a base policy that makes decisions with one \ksample at each step. During test time when communication messages can be perturbed, the agent collects multiple \ksamples at every step, and applies the trained base policy to each \ksample to get multiple resulting base actions. Then, the agent selects the action that reflects the majority opinion. By carefully designed ablation and ensemble strategies, we can ensure that the majority of these base actions is dominated by benign messages.
% , even if there exist $C$ adversarial messages.

% By a careful design of , the agent is guaranteed to make a ``good'' decision if it takes a collection of wisdom from the ensemble of all resulting actions, since the majority of these resulting actions are guaranteed to be dominated by benign messages.
% For a message set $\msg$, our proposed \ours 

% where a base policy is trained in a clean environment to act according under a random \ksample, and the testing/defending phase where the communications may be perturbed, uses the trained base policy by aggregating multiple \ksamples.



% % and the set has $N-1$ elements, each is a message received. 
% Our defense makes decisions based on multiple random subsets of this message set, called \emph{randomly-ablated message samples} (or \textit{m-samples} for short).
% Under a carefully designed ablation mechanism, benign m-samples can outweigh malicious ones.
% To be more specific, we train a \emph{base policy} that makes decisions with one 
% % \myst{randomly selected subset of the message set} 
% m-sample at each step. 
% Note that agents are trained without any attacks, such that the base policy learns to behave under purely-benign m-samples.
% Then, during test-time where communication messages can be perturbed, the agent generates multiple m-samples at every step.
% % One can design an ablation strategy which guarantees that a majority number of these m-samples contain no malicious messages.
% Then the agent applies the trained base policy to  
% % \myst{randomly ablated messages, and aggregate the base-policy actions by sampling multiple message combinations, so that the agent can make safe decisions with theoretical guarantees.}
% each of these m-samples, getting multiple resulting actions where the majority of them are generated based on benign messages only. 
% % The majority of these resulting actions are based on benign messages only and thus safe. 
% Therefore, the agent is guaranteed to make a ``good'' decision if it takes a collection of wisdom from the ensemble of all resulting actions, since the majority of these resulting actions are guaranteed to be dominated by benign messages.
% \myst{guided by} benign \myst{messages}.


% A similar randomized ablation defense is used to defend against $\ell_0$ attacks in image classification~\cite{Levine_Feizi_2020}. 
% But our defensive mechanism is fundamentally different from the image classification defense~\cite{Levine_Feizi_2020} which provides a high-probability guarantee for discrete image label outputs, as our defense achieves both action and long-term reward certification (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output, which is non-trivial.


With the above intuition, we propose \oursfull (\ours), a generic defense framework that can be fused with any policy learning algorithm. 
% We first introduce some important notations for the algorithm.
% shown in Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test}, respectively, in Appendix~\ref{app:algo}. 
\ours has two phases: the training phase where agents are trained in a clean environment, and a testing/defending phase where communications may be perturbed. 
The training and defending strategies of \ours are illustrated below, and the pseudocode is shown by Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test}.% in Appendix~\ref{app:algo}.

\input{algo_train}
\input{algo_test}

\textbf{Training Phase with \ablnamecap $\boldsymbol\ablpolicy$ (Algorithm~\ref{alg:train})}\quad
During training time, the agent learns a \textit{\ablname} $\ablpolicy: \hisspace \times \mathcal{M}^k \to \mathcal{A}$ which maps its own interaction history $\his$ and a random \ksample $\msgk\sim \mathrm{Uniform}(\allmsgk)$ to an action, where $\mathrm{Uniform}(\allmsgk)$ is the uniform distribution over all \ksamples from the message set $\msg$ it receives.
% i.e., $a\step \sim \ablpolicy(\his\step,\msgk\step)$.
% $a\sim\ablpolicy(\his, \mathsf{Ablate}(\msg, T))$, where $T\in\mathcal{H}(N-1,k)$.
Here $k$ is a user-specified hyperparameter selected to satisfy certain conditions, as discussed in Section~\ref{sec:algo_theory}. 
The training objective is to maximize the cumulative reward of $\ablpolicy$ based on randomly sampled \ksamples in a non-adversarial environment. Any policy optimization algorithm can be used for training.
% Since all messages lie in the same message space $\mathcal{M}$, each agent only needs to learn a single ablation policy.
% which achieves as high reward as possible based on randomly sampled $k$ messages. 

% \fhc{Section 4.2 doesn't explain this specific hyperparameter.}
% Equation~\eqref{eq:k_cond} plays an important role in our robustness guarantees shown in Section~\ref{sec:algo_theory}.
% % Note that attacks do not exist during training.
% In every step, an agent randomly samples $k$ out of $N-1$ benign communication messages, and uses its current acting policy $\ablpolicy$ to take an action based on its observation history and the selected $k$ messages.
% react to its current observation and the selected $k$ messages (Line 7 in Algorithm~\ref{alg:train}). 
% Therefore, we optimize and make decisions via $\ablpolicy(\his, \mathsf{Ablate}(\msg, T))$, where $\mathsf{Ablate}(\msg, T)$ denotes the selected $k$ messages sent from other agents to agent $i$. 



\textbf{Defending Phase with \ensnamecap $\boldsymbol\smpolicy$ (Algorithm~\ref{alg:test})}\quad
Once we obtain a reasonable \ablname $\ablpolicy$, we can execute it with ablation and aggregation during test time to defend against adversarial communication. 
The main idea is to collect all possible \ksamples from $\allmsgk$, and select an action suggested by the majority of those \ksamples. 
Specifically, we construct a \textit{\ensname} $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$ that outputs an action by aggregating the base actions produced by $\ablpolicy$ on multiple \ksamples (Line 5 in Algorithm~\ref{alg:test}). 
The construction of the \ensname depends on whether the agent's action space $\mathcal{A}$ is discrete or continuous, which is given below by Definition~\ref{def:ensemble_dist} and Definition~\ref{def:ensemble_cont}, respectively. 
% For notation simplicity, the definitions only focus on one agent (although our defense works for multiple agents) and omit the subscript $i$. We further use $\mathbf{m}$ to denote the message list $\mtoi$ received by the current agent at the current step. 
% The \ensname $\smpolicy_i$ depends on whether the action space $\mathcal{A}_i$ is discrete or continuous, 
% which will be detailed in Section~\ref{sec:algo_dist} and Section~\ref{sec:algo_cont}, with corresponding theoretical guarantees on actions and rewards.
% \textcolor{purple}{PH: would it help mentioning $\smpolicy_i: \mathcal{O}_i \times \mathcal{M}^{N-1} \to \mathcal{A}_i$?}

% \fhc{Shall we put the test algorithm back?}

\begin{definition}[\ensnamecap for Discrete Action Space]
\label{def:ensemble_dist}
For a \ablname $\ablpolicy$ with observation history $\his$ and received message set $\msg$, define the \ensname $\smpolicy$ as
\begin{equation}
\label{eq:ensemble_pi_dist}
    \smpolicy(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)=a].
\end{equation}
\end{definition}

% \begin{definition}[\textbf{\ensnamecap for Discrete Actions}]
% \label{def:ensemble_dist}
% For a \ablname $\ablpolicy$ with observation history $\his$, define $u_a$ as the number of times/votes such that the \ablname $\ablpolicy$ renders action $a$ when taking each of \ksamples in $\allmsgk$, i.e.,
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:vote}
%     u_a := \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)].
%     % u_a := \sum\nolimits_{T\in\mathcal{H}(N-1,k)} \mathbbm{1}[\ablpolicy(\his, \funabl(\mathbf{m}, T))=a].
% \end{equation}
% Then the \ensname $\smpolicy$ takes the action with the most votes, i.e.,
% \begin{equation}
% \label{eq:ensemble_pi_dist}
%     \smpolicy(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \; u_a
% \end{equation}
% % \fh{How about $\tilde{a} = \smpolicy\Big(o, \{\funabl(\mathbf{m}, T_d)\}_{d=1}^D\Big) := \mathrm{ argmax}_{a\in\mathcal{A}} \; u_a.$?}
% \end{definition}

\begin{definition}[\ensnamecap for Continuous Action Space]
\label{def:ensemble_cont}
For a \ablname $\ablpolicy$ with observation history $\his$ and received message set $\msg$, define the \ensname $\smpolicy$ as
\begin{equation}
\label{eq:ensemble_pi_cont}
    \tilde{\pi}(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \msgk): \msgk\in\allmsgk \},
    % \tilde{\pi}(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \funabl(\mathbf{m}, T): T\in\mathcal{H}(N-1,k) \},
\end{equation}
where $\funmed$ is a function that returns the element-wise median value of a set of vectors.
\end{definition}

% Recall that there are up to $C$ malicious messages out of $N-1$ total messages, and at least $N-1-C$ benign messages. 
Therefore, the \ensname $\smpolicy$ takes the action suggested by the consensus of all \ksamples (majority vote in a discrete action space, and median action for a continuous action space). We will show in the next section that, with some mild conditions, 
% the performance of $\smpolicy$ under adversarial communications is certifiable. 
$\smpolicy$ under adversarial communications works similarly as the \ablname $\ablpolicy$ under all-benign communications.
% , with mild assumptions \fhc{note}.

\textbf{Computation Complexity of \ours}\quad
Different from many model-ensemble methods~\cite{kurutach2018modelensemble,harutyunyan2014shaping} that learn multiple network models, \emph{we learn a single policy $\ablpolicy$ during training, and use a single policy $\smpolicy$ during testing.}
Therefore, the training process does not require extra computations compared to the original policy learning method.
In the defending phase, we aggregate decisions from $\binom{N-1}{k}$ \ksamples, which require $\binom{N-1}{k}$ forward passes through $\ablpolicy$. 
Note that $\binom{N-1}{k}$ is generally small, because the number of agents in practical multi-agent problems is usually small (e.g., the number of drones in an area). 
For example, when $N=10,k=2$, $\binom{N-1}{k}=36$.
In the case where $\binom{N-1}{k}$ is large, we provide a variant of the algorithm in Section~\ref{sec:algo_more}, which takes $D$ \ksamples for $D\leq\binom{N-1}{k}$.
Then the certificate of \ours becomes a high-probability guarantee, depending on the value of $D$.
% The defense objective is to make a \textit{\myst{safe} \fh{benign} decision} that is robust to malicious massages. 


% Note that the ensemble policy $\smpolicy$ takes the action suggested by the consensus of all size-$k$ message subsets (majority vote in a discrete action space, and median action for a continuous action space). 
% There are $\binom{N-1}{k}$ number of such size-$k$ subsets in total. In many practical multi-agent problems, $N$ is not very large, e.g., the number of drones in an area. Therefore, $\binom{N-1}{k}$ is relatively small and not expensive to compute. For example, when $N=10,k=2$, $\binom{N-1}{k}=36$.
% In the case where $\binom{N-1}{k}$ is large, we also provide a variant of the algorithm which takes $D<\binom{N-1}{k}$ samples of message subsets whose certification guarantee is provided in Section~\ref{sec:algo_more}.

\subsection{Robustness Certificates of \ours}
\label{sec:algo_theory}


% Our defense lets an agent make decisions based on multiple size-$k$ random subsets of all messages in $\mathbf{m}$. 
In this section, we provide theoretical guarantees for the robustness of \ours.
During test time, at any step, let $\his$ be the interaction history, $\goodmsg$ be the unperturbed benign message set, and $\advmsg$ be the perturbed message set. 
% $\goodmsg$ be the benign messages (before attack), and $\advmsg$ be the messages after attack (with up to $C$ messages being corrupted). 
Note that $\goodmsg$ and $\advmsg$ both have $N-1$ messages while they differ by up to $C$ messages. 
With the above notation, we define a set of actions rendered by purely benign \ksamples in Definition~\ref{def:safeact_dist}. As the agent using a well-trained \ablname is likely to take these actions in a non-adversarial environment, they can be regarded as ``good'' actions to take. 

\begin{definition}[Benign Action Set $\safeaction$]
\label{def:safeact_dist}
For the execution of the \ablname $\ablpolicy$ at any step, define $\safeaction \subseteq \mathcal{A}$ as a set of actions that $\ablpolicy$ may select under benign \ksamples.
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
\label{eq:safeact_dist}
    \safeaction := \cup_{\goodmsgk\in\goodallmsgk} \left\{\ablpolicy(\his, \goodmsgk) \right\}.
    %  \safeaction := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
\end{equation}
\end{definition}

\subsubsection{Certificates for Discrete Action Space}
\label{sec:algo_theory_dist}

We first characterize the action and reward certificate of \ours in a discrete action space, the \ablname takes the action with the most votes from all \ksamples as suggested by Equation~\eqref{eq:ensemble_pi_dist}. To ensure that this action stands for the consensus of benign messages, the following condition is needed.

\begin{condition}[Confident Consensus]
\label{cond:cons}
The highest number of votes among all actions $u_{\max}:=\max_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)=a]$ satisfies
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{0pt}
\begin{equation}
    \label{eq:u_cond}
    u_{\max} > {\small{\binom{N-1}{k} - \binom{N-1-C}{k}}} =: u_{\mathrm{adv}},
\end{equation}
where $u_{\mathrm{adv}}$ is the number of votes that adversarial messages may affect (number of \ksamples that contain at least one adversarial message). 
\end{condition}

\textbf{Remarks}.
(1) This condition ensures the consensus has more votes than the votes that adversarial messages are involved in. Therefore, when $\smpolicy$ takes an action, there must exist some purely-benign \ksamples voting for this action. 
(2) This condition is easy to satisfy when $C \ll N$ as $\binom{N-1}{k} \approx \binom{N-1-C}{k}$. 
(3) This condition can be easily checked at every step of execution. 

Condition~\ref{cond:cons} considers the worst-case scenario when the adversarial messages collaborate to vote for a malicious action and outweigh benign messages in all \ksamples. 
However, such a worst-case attack is uncommon in practice as attackers are usually not omniscient. Therefore, Condition~\ref{cond:cons} is sufficient but not necessary for the robustness of $\smpolicy$ during execution. 
In real-world problems, our algorithm achieves strong robustness without requiring this condition, as verified in experiments. 


% We now provide both action and reward certificates for the ensemble policy $\smpolicy$ in the discrete-action case. The analysis for a continuous action space is provided in Appendix~\ref{app:theory_cont}.

\textbf{Action Certificate for Discrete Action Space}\quad
The following theorem suggests that the ensemble policy $\smpolicy$ always takes benign actions under the above conditions no matter whether attacks exist.
\begin{theorem}[Action Certificate for Discrete Action Space]
\label{thm:main_dist}
When Condition~\ref{cond:cons} holds, the ensemble policy $\smpolicy$ in Definition~\ref{def:ensemble_dist} produces benign actions under $\advmsg$, i.e.,
\begin{equation}
    \widetilde{a} = \smpolicy(\his, \advmsg) \in \safeaction.
    \label{eq:cert_dist}
\end{equation}
% if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% where 
% \begin{equation}
%     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% \end{equation}
\end{theorem}
\vspace{-0.5em}

Under Condition~\ref{cond:cons} which are easy to check, Theorem~\ref{thm:main_dist} certifies that $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a benign action that is suggested by some benign message combinations, even when the malicious messages are not identified. 
Then, we can further derive a reward certificate as introduced below. 
% Note that a high-probability robustness guarantee~\cite{Levine_Feizi_2020} does not 

  
\textbf{Reward Certificate for Discrete Action Space}\quad
When Condition~\ref{cond:cons} holds, the \ensname $\smpolicy$'s action in every step falls into a benign action set, and thus \emph{its cumulative reward under adversarial communications is also guaranteed to be no lower than the worst natural reward the base policy $\ablpolicy$ can get under random benign message subsets.} Therefore, adversarial communication under Assumption~\ref{assum:num} cannot drop the reward of any agent trained with \ours. The formal reward certificate is shown in Corollary~\ref{cor:reward_dist} in Appendix~\ref{app:theory_dist}. 


\subsubsection{Certificates in Continuous Action Space}
\label{sec:algo_theory_cont}

The conditions and theoretical results in a continuous action space is slightly different from the discrete case introduced above. We first introduce a condition for certificates to hold.

\begin{condition}[Dominating Benign Sample]
\label{cond:k}
The ablation size $k$ of \ours satisfies
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
    \label{eq:k_cond}
    \binom{N-1-C}{k} > \frac{1}{2} \binom{N-1}{k}.
\end{equation}
\end{condition}
\vspace{-0.5em}

\textbf{Remarks.}
(1) For the message set $\advmsg$ that has up to $C$ adversarial messages, Equation~\eqref{eq:k_cond} implies that among all \ksamples from $\advmsg$, there are more purely benign \ksamples than \ksamples that contain adversarial messages. 
(2) Under Assumption~\ref{assum:num}, this condition \textit{always has solutions }for $k$ as $C<\frac{N-1}{2}$, and $k=1$ is always a feasible solution. 
% (3) In practice, the value of $k$ is related to the trade-off between natural performance and robustness, as discussed in details in Section~\ref{sec:exp}.
% Condition~\ref{cond:k} is important for the 

\textbf{Action Certificate for Continuous Action Space}\quad
As in the discrete action case, the continuous ensemble policy will output an action $\widetilde{a}$ that follows the consensus of benign messages. But in a continuous action space, it is hard to ensure that $\widetilde{a}$ is exactly in $\safeaction$. Instead, $\widetilde{a}$ is guaranteed to be within the range of $\safeaction$, as detailed in the following theorem.

\begin{theorem}[Action Certificate for Continuous Action Space]
\label{thm:main_cont}
Under Condition~\ref{cond:k}, the action $\widetilde{a} = \smpolicy(\his, \advmsg)$ generated by the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} satisfies
\begin{equation}
    \widetilde{a} \in \mathsf{Range}(\safeaction) := \{a: \forall 1\leq l \leq L, \exists \underline{a}, \overline{a} \in \safeaction \text{ s.t } \underline{a}_l \leq a_l \leq \overline{a}_l \}.
    \label{eq:cert_cont}
\end{equation}
\end{theorem}

In other words, if the \ensname takes an action $\widetilde{a}$, then at each dimension $l$, there must exist $a_1$ and $a_2$ suggested by some purely benign \ksamples such that the $l$-th dimension of $\widetilde{a}$ is lower and upper bounded by the $l$-th dimension of $a_1$ and $a_2$, respectively. In many practical problems, it is reasonable to assume that actions in $\mathsf{Range}(\safeaction)$ are relatively safe, especially when benign actions in $\safeaction$ are concentrated. For example, if the action denotes the driving speed, and benign message combinations have suggested driving at 40 mph or driving at 50 mph, then driving at 45 mph is also safe. Appendix~\ref{app:theory_cont} provides more examples to explain $\mathsf{Range}(\safeaction)$ in practice.

\textbf{Reward Certificate for Continuous Action Space}\quad
We prove that under Condition~\ref{cond:k}, the reward of the \ensname under communication attacks is lower bounded by the natural reward of \ablname subtracting a environment-dependent constant. Intuitively, the gap between the natural performance and the  worst-case performance under attacks is smaller when the environment dynamics are relatively smooth and the benign \ksamples achieve good consensus. Formal theoretical results and analysis is in Appendix~\ref{app:theory_cont}.

% Section~\ref{sec:exp} shows ablation experiments of $k$.

% % As pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}, there exists a \textit{trade-off between robustness and accuracy}. 
% Intuitively, the more an agent trusts communications from others, the more it may benefit from additional information, but it is more exposed to the risk of being attacked. Therefore, there exists a \textit{trade-off between robustness and accuracy}~\cite{tsipras2018robustness,zhang2019theoretically}. 
% We find that the ablation size $k$ directly controls such a trade-off: when $k$ is small, the \ensname is more robust since there are much more purely-benign \ksamples than adversarial \ksamples. However, the trained \ablname may not obtain a high reward with $k$ messages.
% % In general, if $k$ is smaller, the ensemble policy is more robust. However, the base ablation policy with a smaller $k$ could gain lower reward as it throws away many messages. Therefore, there is a \textit{trade-off between robustness and accuracy}, as is pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}. 
% Therefore, we can adjust $k$ based on our practical needs.
% If we know $C$ (or an upper bound of $C$), we can set $k$ to be the largest integer satisfying Condition~\ref{cond:k} such that the natural performance is not compromised much. 
% If $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Condition~\ref{cond:k}.
% % which shows how many adversarial messages the policy can tolerate. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Condition~\ref{cond:k}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
% Experiments in Section~\ref{sec:exp} verifies our claim by an ablation study of $k$.

% and when $C$ is small, we can use a larger $k$ such that the natural performance is not compromised much. 

\textbf{How to Select Ablation Size $k$: Trade-off between Performance and Robustness}\quad
The ablation size $k$ is an important hyperparameter for the guarantees to hold. For a fixed $C$, both Condition~\ref{cond:cons} and Condition~\ref{cond:k} prefer a relatively small $k$ as detailed in Appendix~\ref{app:hyper}. That is, a smaller $k$ can improve the robustness in general. Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
% Condition~\ref{cond:cons} is easier to be satisfied for a smaller $k$, because $u_{\mathrm{adv}}$ increases as $k$ (verified in Appendix~\ref{app:hyper}). 
However, we also point out that a smaller $k$ restricts the power of information sharing, as the \ablname can access fewer messages in one step. Therefore, the value of $k$ is related to the \emph{trade-off between robustness and natural performance}~\cite{tsipras2018robustness,zhang2019theoretically}. 
In experiments, we use \textit{the largest $k$ satisfying Equation~\eqref{eq:k_cond}}. 
In practice, one can also train several \ablnames with different $k$'s during training, and later adaptively select a \ablname to construct a \ensname during execution (decrease $k$ if higher robustness is needed). 


\vspace{-0.5em}
\subsection{Extensions of \ours}
\label{sec:algo_more}

% In this section, we discuss the effects of hyperparameter $k$, the broader applications of \ours, and an extensions of \ours for scaling up to a large number of agents.

% \textbf{Discussion on Ablation Size $\boldsymbol k$}\quad 
% As an essential condition for the certificates in Section~\ref{sec:algo_theory} to hold, Equation~\eqref{eq:k_cond} implies that among all size-$k$ message subsets, there are more purely benign subsets than subsets that contain adversarial messages. This condition \textit{always has solutions }for $k$ as $C<\frac{N-1}{2}$, and $k=1$ is always a feasible solution. In general, if $k$ is smaller, the ensemble policy is more robust. However, the base ablation policy with a smaller $k$ could gain lower reward as it throws away many messages. Therefore, there is a \textit{trade-off between robustness and accuracy}, as is pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}.
% In practice, if we know $C$ in advance, we can set $k$ to be the largest integer satisfying Equation~\eqref{eq:k_cond}. On the other hand, if $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Equation~\eqref{eq:k_cond}, which shows how many adversarial messages the policy can tolerate. 
% % For example, when $N=10$, \ours can tolerate up to $C=4$ with $k=1$, and up to $C=2$ with $k=2$. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Equation~\eqref{eq:k_cond}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages, and when $C$ is small, we can use a larger $k$ such that the natural performance is not compromised much. 




\textbf{Scaling Up: Ensemble with Partial Samples}\quad
So far we have discussed the proposed \ours defense and the constructed ensemble policy that aggregates all $\binom{N-1}{k}$ number of \ksamples out of $N-1$ messages. 
However, if $N$ is large, sampling all $\binom{N-1}{k}$ combinations of message subsets could be expensive. In this case, a smaller number of \ksamples can be used. That is, given a sample size $0<D\leq\binom{N-1}{k}$, we randomly select $D$ number of \ksamples from $\allmsgk$ (without replacement), and then we aggregate the \ablname's decisions on selected \ksamples. 
In this way, we define a partial-sample version of the ensemble policy, namely \textit{$D$-ensemble policy} $\smpolicy_D$, whose formal definition is provided in Appendix~\ref{app:theory_sample}. In this case, the robustness guarantee holds with high probability that increases as $D$ gets larger, as detailed in Theorem~\ref{thm:sample_cont} in Appendix~\ref{app:theory_sample}. 
Decreasing the hyperparameter $D$ trades some robustness guarantee for higher computational efficiency.
In our experiments, we empirically show that \ours usually works well even for a small $D$ (e.g. $D=1$).


\textbf{More Applications of \ours}\quad
The central idea of \ours is to make decisions based on the consensus instead of each individual.
Therefore, \ours can be combined with any decision-making model to work with possibly-untrustworthy information sources, not only restricted to communication attacks in CMARL. 
For example, when one collects data from multiple sources (e.g., different websites, multiple questionnaires, etc.) and some sources may contain malicious information, \ours can be used to make decisions based on the collected statistics without being significantly misled by false data.
Moreover, the idea of \ours can also be extended to detect attackers, by measuring the difference between the action suggested by any specific communication message and the ensemble policy's action, as detailed and empirically verified in Appendix~\ref{app:exp_detect}. 












% formulated as below.
% , whose detailed definition is provided in Appendix~\ref{app:theory_sample}.
% define the $D$-ensemble policy $\smpolicy_D$ as the sampled version of $\smpolicy$
% \begin{equation}
% \label{eq:ensemble_pi_dist_d}
%     \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
% \end{equation}
% for a discrete action space, and
% \begin{equation}
% \label{eq:ensemble_pi_cont_d}
%     \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% for a continuous action space. 


% \subsection{Extension of \ours: Ensemble with Partial Samples}
% \label{sec:algo_partial}

% So far we have discussed the proposed \ours algorithm and the constructed ensemble policy that aggregates all $\binom{N-1}{k}$ number of message subsets out of $N-1$ messages. 
% However, if $N$ is large, sampling all $\binom{N-1}{k}$ combinations of message subsets could be expensive. In this case, a smaller number of message-subset combinations can be used. That is, given a sample size $0<D\leq\binom{N-1}{k}$, we randomly select $D$ samples $\{T_d\}_{d=1}^D$ from $\mathcal{H}(N-1,k)$ (without replacement), and then we aggregate the ablation policy's decision on $\{\funabl(\mathbf{m}, T_d)\}_{d=1}^D$. 
% In this way, we define a sampled version of the ensemble policy, namely \textit{$D$-ensemble policy} $\smpolicy_D$, formulated as below.
% % , whose detailed definition is provided in Appendix~\ref{app:theory_sample}.
% % define the $D$-ensemble policy $\smpolicy_D$ as the sampled version of $\smpolicy$
% \begin{equation}
% \label{eq:ensemble_pi_dist_d}
%     \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
% \end{equation}
% for a discrete action space, and
% \begin{equation}
% \label{eq:ensemble_pi_cont_d}
%     \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% for a continuous action space. 



% In this case, we can still provide a high-probability robustness guarantee. Theorem~\ref{thm:sample_cont} shows the theoretical result for a continuous action space, while the result for a discrete action space is slightly different and is provided in Appendix~\ref{app:theory_sample}.
% % in Theorem~\ref{thm:sample_dist} and Theorem~\ref{thm:sample_cont}. 

% \begin{theorem}[General Action Guarantee for Continuous Action Space]
% \label{thm:sample_cont}
% Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$,  under Assumption~\ref{assum:num}, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_cont_d} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, relation~\eqref{eq:cert_cont} holds with probability at least
% \begin{equation}
% \label{eq:p_sample_cont}
%     p_D=\frac{\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n_1-n_2}{D-j}}{\binom{n_1}{D}},
% \end{equation}
% where $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$ and $\tilde{D} = {\lfloor \frac{D}{2} \rfloor}+1$. 
% \end{theorem}
% Therefore, for an arbitrary $D$, a benign action will be selected with high probability. The larger $D$ is, the higher the probability is. 
% In Theorem~\ref{thm:sample_cont}, when $D=\binom{N-1}{k}$,  the probability $p_D$ is 1 and the result matches Theorem~\ref{thm:main_cont}. 
% Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.


% \subsection{More Discussion on Applicability and Flexibility of \ours}

% \ys{general for any RL policy or decision-making model}

% \ys{how a policy is trained}



% \ys{training and testing hyperparameters}



==> cmarl/arxiv/6_discuss.tex <==
% \vspace{-0.5em}
\section{Conclusion}
\label{sec:discuss}
% \vspace{-0.5em}

This paper formulates communication attacks in MARL problems, and proposes a defense framework \ours, which is certifiably robust against multiple arbitrarily perturbed adversarial communication messages, based on randomized ablation and aggregation of messages. 
We show in theory and by experiments that \ours maintains its performance under various communication perturbations.
Even when theoretical conditions do not hold, \ours is still moderately robust and significantly outperforms other defenses baselines.
\ours is a generic defense that can be applied to any policy learning workflow, and can easily scale up to many real-world tasks. 
% Environments verify the effectiveness of \ours in different tasks. 
In Appendix~\ref{app:hyper}, we provide detailed analysis on hyperparameter selection and its relation to the trade-off between natural performance and robustness. 
The idea of \ours can also be extended to attack detection as discussed in Appendix~\ref{app:exp_detect}.
% \ys{flexibility of different $k$'s in training and test.}

==> cmarl/arxiv/a2_theory.tex <==
\section{Additional Theoretical Definitions and Analysis}
\label{app:theory}

\textbf{Relation between Communication Attack and $\boldsymbol \ell_0$ Observation Attack}\quad
The communication threat model described in Section~\ref{sec:setup_adv} is analogous to a constrained $\ell_0$ attack on policy inputs. When agent $i$ is attacked, the input space of its acting policy $\pi_i$ is $\mathcal{X}_i := \hisspace_i \times \mathcal{M}^{N-1}$. Therefore, when $C$ communication messages are corrupted, the original input $x_i$ gets perturbed to $\tilde{x}_i$. Let $d$ be the dimension of a communication message, then $x_i$ and $\tilde{x}_i$ differ by up to $dC$ dimensions, which is similar to an $\ell_0$ attack constrained in certain dimensions. 



\subsection{Additional Analysis of \ours in Discrete Action Space}
\label{app:theory_dist}

\textbf{Reward Certificate}\quad
Theorem~\ref{thm:main_dist} justifies that under sufficient majority votes, the \ensname $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a benign action that is suggested by some benign message combinations, even when the malicious messages are not identified.
It is important to note that, when the \ensname $\smpolicy$ selects an action $\widetilde{a}$, there must exist at least one purely benign \ksample that let the \ablname $\ablpolicy$ produce $\widetilde{a}$. Therefore, as long as $\ablpolicy$ can obtain high reward with randomly selected benign \ksamples, $\smpolicy$ can also obtain high reward with ablated adversarial communication due to its design.


Specifically, we consider a specific agent with \ablname $\ablpolicy$ and \ensname $\smpolicy$ (suppose other agents are executing fixed policies). 
Let $\nu:\mathcal{M}^{N-1}\to\mathcal{M}^{N-1}$ be an attack algorithm that perturbs at most $C$ messages in a message set. 
Let $\zeta \sim Z(P,\ablpolicy)$ be a trajectory of policy $\ablpolicy$ under no attack, i.e., $\zeta=(o^{(0)},\msg^{(0)},a^{(0)},r^{(0)},o^{(1)},\msg^{(1)},a^{(0)},r^{(0)},\cdots)$. (Recall that a \ablname $\ablpolicy$ takes in a random size-$k$ subset of $\msg\step$ and outputs action $a\step$.)
When there exists attack with $\nu$, let $\zeta_\nu \sim Z(P,\smpolicy;\nu)$ be a trajectory of policy $\smpolicy$ under communication attacks, i.e., $\zeta_\nu=(o^{(0)},\nu(\msg^{(0)}),a^{(0)},r^{(0)},o^{(1)},\nu(\msg^{(1)}),a^{(0)},r^{(0)},\cdots)$. 
For any trajectory $\zeta$, let $r(\zeta)$ be the discounted cumulative reward of this trajectory.

% Let $\zeta=(o^{(0)},\msg^{(0)},a^{(0)},r^{(0)},o^{(1)},\msg^{(1)},a^{(0)},r^{(0)},\cdots)$ denote a trajectory. If \ablname is used, we have 
% $a\step = \ablpolicy(\his\step, \msgk)$ where $\msgk\sim\mathrm{Uniform}(\mathcal{H}_{k}(\msg\step))$. If \ensname is used, we have $a\step = \smpolicy(\his\step, \msg\step)$. 
% Let $\natobj(\zeta)$ denote the natural cumulative reward of a policy under no attack.
% Let $\advobj(\zeta)$ denote the cumulative reward of a policy under attacks, where at every step $t$, up to $C$ messages in the message set $\msg\step$ can be perturbed arbitrarily.

With the above notations, we propose the following reward certificate.
% let $\goodmsg\step$ and $\advmsg\step$ be the original benign message list and the perturbed message list the agent receives at step $t$, respectively. We use 
% \begin{equation}
%     \natobj(\pi) := J(\pi|\goodmsg^{(1)}, \goodmsg^{(2)},\cdots)
% \end{equation}
% to denote the expected cumulative reward of policy $\pi$ when it receives benign messages $\goodmsg^{(1)}, \goodmsg^{(2)},\cdots$, and use
% \begin{equation}
%     \advobj(\pi) := J(\pi|\advmsg^{(1)}, \advmsg^{(2)},\cdots)
% \end{equation}
% to denote the expected cumulative reward of policy $\pi$ when it receives perturbed messages $\advmsg^{(1)}, \advmsg^{(2)},\cdots$. Then, the following corollary presents the reward certificate of the \ensname when the agent's action space is discrete.

\begin{corollary}[Reward Certificate for Discrete Action Space]
\label{cor:reward_dist}
When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold at every step of execution, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} under adversarial communication is no lower than the lowest cumulative reward that the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
\begin{equation}
\begin{aligned}
    \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta),
    %  \min_{\advmsg^{(1)}, \advmsg^{(2)},\cdots} \advobj(\smpolicy) \geq \min_{[\goodmsg^{(1)}]_k,[\goodmsg^{(2)}]_k,\cdots} \natobj(\ablpolicy),
    % \advobj(\smpolicy) \geq \min_{\msgk^{(1)},\msgk^{(2)},\cdots} \natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)
    % \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
\end{aligned}
\end{equation}
for any attacker $\nu$ satisfying Assumption~\ref{assum:num} ($C<\frac{N-1}{2}$).
% where $[\goodmsg\step]_k\sim\mathrm{Uniform}(\mathcal{H}_{k}(\goodmsg\step))$.
% where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under arbitrary attacks to up to $C$ communication messages, and $\natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ when the random \ksample in the first step is $\msgk^{(1)}$, the random \ksample in the second step is $\msgk^{(2)}$, etc.
\end{corollary}

\textbf{Remarks.} 
(1) The certificate holds for any attack algorithm $\nu$ with $C<\frac{N-1}{2}$. 
(2) The \ablname $\ablpolicy$ has extra randomness from the sampling of \ksamples. That is, at every step, $\ablpolicy$ takes a uniformly randomly selected \ksample from $\allmsgk$. Therefore, the $\min_\zeta$ in the RHS considers the worst-case message sampling in the clean environment without attacks. Since $\smpolicy$ always takes actions selected by some purely-benign message combinations, the trajectory generated by $\smpolicy$ can also be produced by the \ablname.
(3) Note that the RHS ($\min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta)$) can be approximately estimated by executing $\ablpolicy$ during training time, so that the test-time performance of $\smpolicy$ is guaranteed to be no lower than this value, even if there are up to $C$ corrupted messages at every step.

% \begin{corollary}[Reward Certificate for Discrete Action Space]
% \label{cor:reward_dist}
% \fh{Under sample size $D=\binom{N-1}{k}$, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with a message subset size $k$ satisfying Equation~\eqref{eq:k_cond} obtains a total reward no worse than that obtained by the base ablation policy $\ablpolicy$ using benign messages:
% \begin{align}
%   & \advobj\Big(\smpolicy\big(o, \{\funabl(\advmsg, T_d)\}_{d=1}^D\big)\Big) \geq \nonumber \\
%   & \min_{T} \natobj\Big(\ablpolicy\big(o, \funabl(\goodmsg, T)\big)\Big) \label{eq:reward_dist}
% \end{align}
% if the majority votes $u_{\tilde{a}}$ satisfies $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step.
% }
% \textcolor{red}{Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If $D=\binom{N-1}{k}$, and the majority votes satisfy 
% $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step, 
% then the total reward of $\smpolicy$ satisfies
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:reward_dist}
%     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy),
% \end{equation}}
% Here $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the \textcolor{red}{sampled message indices}\fh{indices of the message subsets?} used by $\ablpolicy$ at all steps. \fh{What does this mean? My equation doesn't use $\tau$, rather I use $T$.}
% \end{corollary}


Appendix~\ref{app:proof} provides detailed proofs for the above theoretical results.


\subsection{Additional Analysis of \ours in Continuous Action Space}
\label{app:theory_cont}



% \textbf{Action Certificate}\quad
% As in the discrete action case, the continuous ensemble policy will output an action $\widetilde{a}$ that follows the consensus of benign messages. But in a continuous action space, it is hard to ensure that $\widetilde{a}$ is exactly in $\safeaction$. Instead, $\widetilde{a}$ is guaranteed to be within the range of $\safeaction$, as detailed in the following theorem.

% \begin{theorem}[Action Certificate for Continuous Action Space]
% \label{thm:main_cont}
% Under Condition~\ref{cond:k}, the action $\widetilde{a} = \smpolicy(\his, \advmsg)$ generated by the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} satisfies
% \begin{equation}
%     \widetilde{a} \in \mathsf{Range}(\safeaction) := \{a: \forall 1\leq l \leq L, \exists \underline{a}, \overline{a} \in \safeaction \text{ s.t } \underline{a}_l \leq a_l \leq \overline{a}_l \}.
%     \label{eq:cert_cont}
% \end{equation}
% % then any dimension $l$ of $\smpolicy$'s output satisfies
% % \begin{equation*}
% %     \inf_{\krv} [\hat{a}]_l  
% %     \leq [\smpolicy(o, \advmsg, \{T_d\}_{d=1}^D)]_l 
% %     \leq \sup_{\krv} [\hat{a}]_l.
% % \end{equation*}
% % where $\hat{a} := \ablpolicy(o, \mathsf{Ablate}(m, \krv))$.
% \end{theorem}

% In other words, if the \ensname takes an action $\widetilde{a}$, then at each dimension $l$, there must exist $a_1$ and $a_2$ suggested by some purely benign \ksamples such that the $l$-th dimension of $\widetilde{a}$ is lower and upper bounded by the $l$-th dimension of $a_1$ and $a_2$, respectively. 
Note that Theorem~\ref{thm:main_cont} certifies that the selected action is in a set of actions that are close to benign actions $\mathsf{Range}(\safeaction)$, but does not make any assumption on this set. Next we interpret this result in details.

\textbf{How to Understand $\mathsf{Range}(\safeaction)$?}\quad
Theoretically, $\mathsf{Range}(\safeaction)$ is a set of actions that are coordinate-wise bounded by base actions resulted from purely benign \ksamples. In many practical problems, it is reasonable to assume that actions in $\mathsf{Range}(\safeaction)$ are relatively safe, especially when benign actions in $\safeaction$ are concentrated. The following examples illustrate some scenarios where actions in $\mathsf{Range}(\safeaction)$ are relatively good.

\begin{enumerate}
    \item If the action denotes the price a seller sells its product in a market, and the communication messages are the transaction signals in an information pool, then $\mathsf{Range}(\safeaction)$ is a price range that is determined based on purely benign messages. Therefore, the seller will set a reasonable price without being influenced by a malicious message. 
    \item If the action denotes the driving speed, and benign message combinations have suggested driving at 40 mph or driving at 50 mph, then driving at 45 mph is also safe. 
    \item If the action is a vector denoting movements of all joints of a robot (as in many MuJoCo tasks), and two slightly different joint movements are suggested by two benign message combinations, then an action that does not exceed the range of the two benign movements at every joint is likely to be safe as well.
\end{enumerate}  

The above examples show by intuition why the \ensname can be regarded as a relatively robust policy. 
However, in extreme cases where there exists ``caveat'' in $\mathsf{Range}(\safeaction)$, taking an action in this set may also be unsafe. To quantify the influence of $\mathsf{Range}(\safeaction)$ on the long-term reward, we next analyze the cumulative reward of the \ensname in the continuous-action case.



\textbf{How Does $\mathsf{Range}(\safeaction)$ Lead to A Reward Certificate?}\quad
Different from the discrete-action case, the \ensname $\smpolicy$ in a continuous action space may take actions not in $\safeaction$ such that it generates trajectories not seen by the \ablname $\ablpolicy$. However, since the action of $\smpolicy$ is guaranteed to stay in $\mathsf{Range}(\safeaction)$, we can bound the difference between the value of $\smpolicy$ and the value of $\ablpolicy$, and how large the different is depends on some properties of $\mathsf{Range}(\safeaction)$.

Concretely, Let $R$ and $P$ be the reward function and transition probability function of the current agent when the other agents execute fixed policies. So $R(s,a)$ is the immediate reward of taking action $a$ at state $s$, and $P(s^\prime|s,a)$ is the probability of transitioning to state $s^\prime$ from $s$ by taking action $a$. (Note that $s$ is the underlying state which may not be observed by the agent.)
% Let $R_{\max}$ denote the supremum of the absolute value of $R$, i.e., $R_{\max}:=\sup_{s,a} |R(s,a)|$. 

\begin{definition}[Dynamics Discrepancy of $\ablpolicy$]
\label{def:disc}
A \ablname $\ablpolicy$ is called $\epsilon_R$,$\epsilon_P$-discrepant if $\epsilon_R$, $\epsilon_P$ are the smallest values such that for any $s\in\mathcal{S}$ and the corresponding \safename set $\safeaction$, we have $\forall a_1, a_2 \in \mathsf{Range}(\safeaction)$, 
\begin{align}
    & |R(s,a_1) - R(s,a_2)| \leq \epsilon_R, \\
    & \int | P(s^\prime| s, a_1) - P(s^\prime| s, a_2) | \mathrm{d}s^\prime \leq \epsilon_P. \label{eq:p_disc}
\end{align}
% Given a \ablname $\ablpolicy$, $\mathsf{Range}(\safeaction)$
% let $f_{\ablpolicy}$ be a mapping from state $s\in\mathcal{S}$ to the corresponding benign action range induced by $\ablpolicy$ at state $s$, i.e., $f_{\ablpolicy}(s)$ is 
\end{definition}

\textbf{Remarks.}
(1) Equation~\eqref{eq:p_disc} is equivalent to that the total variance distance between $P(\cdot| s, a_1)$ and $P(\cdot| s, a_2)$ is less than or equal to $\epsilon_P/2$.
(2) For any environment with bounded reward, $\epsilon_R$ and $\epsilon_P$ always exist. 
% (3) $\epsilon_R$ and $\epsilon_P$ are related to the \ablname, the communication quality, and the environment properties. When the reward function and transition function are smooth, and when the benign communications can reach some ``consensus'' of actions by propagating through $\ablpolicy$, $\epsilon_R$ and $\epsilon_P$ will be relatively small.



Definition~\ref{def:disc} characterizes how different the local dynamics of actions in $\mathsf{Range}(\safeaction)$ are, over all possible states. If $\mathsf{Range}(\safeaction)$ is small and the environment is relatively smooth, then taking different actions within this range will not result in very different future rewards. The theorem below shows a reward certificate for the \ensname $\smpolicy$.

% When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold at every step of execution, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} under adversarial communication is no lower than the lowest cumulative reward that the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
% \begin{equation}
% \begin{aligned}
%     \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta),
% \end{aligned}
% \end{equation}
% for any attacker $\nu$ satisfying Assumption~\ref{assum:num} ($C<\frac{N-1}{2}$).

\begin{theorem}[Reward Certificate for Continuous Action Space]
\label{thm:reward_cont}
Let $V^{\ablpolicy}(s)$ be the clean value (discounted cumulative reward) of $\ablpolicy$ starting from state $s$ under no attack; let $\tilde{V}^{\smpolicy}_\nu(s)$ be the value of $\smpolicy$ starting from state $s$ under attack algorithm $\nu$, where $\nu$ satisfies Assumption~\ref{assum:num}; let $k$ be an ablation size satisfying Condition~\ref{cond:k}.
If $\ablpolicy$ is $\epsilon_R$,$\epsilon_P$-discrepant, then for any state $s\in\mathcal{S}$, we have
\begin{equation}
    % \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta) - \frac{1}{1-\gamma}\epsilon_R - \frac{\gamma R_{\max}}{(1-\gamma)^2} \epsilon_P.
    \min_{\nu} \tilde{V}^{\smpolicy}_\nu(s) \geq V^{\ablpolicy}(s) - \frac{\epsilon_R+\gamma V_{\max}\epsilon_P}{1-\gamma},
\end{equation}
where $V_{\max} := \sup_{s,\pi}  |V^\pi(s)|$. 
% the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} is no lower than the lowest cumulative reward the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
% \begin{equation}
%     \min_{\advmsg^{(1)}, \advmsg^{(2)},\cdots} \advobj(\smpolicy) \geq \min_{[\goodmsg^{(1)}]_k,[\goodmsg^{(2)}]_k,\cdots} \natobj(\ablpolicy),
% \end{equation}
% where $[\goodmsg\step]_k\sim\mathrm{Uniform}(\mathcal{H}_{k}(\goodmsg\step))$.
\end{theorem}

\textbf{Remarks.}
(1) The certificate holds for any attack algorithm $\nu$ with $C<\frac{N-1}{2}$. 
(2) If $\epsilon_R$ and $\epsilon_P$ are small, then the performance of \ensname $\smpolicy$ under attacks is similar to the performance of the \ablname $\ablpolicy$ under no attack. 

It is important to note that $\epsilon_R$ and $\epsilon_P$ are intrinsic properties of $\ablpolicy$, independent of the attacker. Therefore, one can approximately measure $\epsilon_R$ and $\epsilon_P$ during training. 
Similar to Condition~\ref{cond:cons} required for a discrete action space, the gap between the attacked reward of $\smpolicy$ and the natural reward of $\ablpolicy$ depends on how well the benign messages are reaching a consensus. (Smaller $\epsilon_R$ and $\epsilon_P$ imply that the actions in $\safeaction$ are relatively concentrated and the environment dynamics are relatively smooth.)

Moreover, one can optimize $\ablpolicy$ during training such that $\epsilon_R$ and $\epsilon_P$ are as small as possible, to further improve the robustness guarantee of $\smpolicy$. This can be a future extension of this work.


Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.







\subsection{Extension of \ours with Partial Samples}
\label{app:theory_sample}

As motivated in Section~\ref{sec:algo_more}, our \ours can be extended to a partial-sample version, where the ensemble policy is constructed by $D$ instead of $\binom{N-1}{k}$ samples. Let $\allmsgkd$ be a subset of $\allmsgk$ that contains $D$ random \ksamples from $\allmsgk$. Then the $D$-ensemble policy $\pi_D$ is defined as
\begin{equation}
\label{eq:ensemble_pi_dist_d}
    \smpolicy_D(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum_{\msgk\in\allmsgkd} \mathbbm{1}[\ablpolicy(o, \msgk)=a],
\end{equation}
for a discrete action space, and
\begin{equation}
\label{eq:ensemble_pi_cont_d}
    \tilde{\pi}_D(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \msgk) \}_{\msgk\in\allmsgkd}.
\end{equation}\normalsize
for a continuous action space. 

In the partial-sample version of \ours, we can still provide high-probability robustness guarantees. 



For notation simplicity, let $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$. 
Define the majority vote as 
\begin{equation}
\label{eq:vote}
    u_{\max}:=\max_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgkd} \mathbbm{1}[\ablpolicy(\his, \msgk)=a].
\end{equation}
The following theorem shows a general guarantee for $D$-ensemble policy in a discrete action space. 

\begin{theorem}[General Action Guarantee for Discrete Action Space]
\label{thm:sample_dist}
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_dist_d},
Relation~\eqref{eq:cert_dist} holds deterministically if the majority vote $u_{\max}>n_1-n_2$. 
Otherwise it holds with probability at least
%\vspace{-0.1cm}
\begin{equation}
\label{eq:p_sample_dist}
    p_D=\frac{\sum_{j=0}^{u_{\max}-1}\binom{n_1-n_2}{j}\binom{n_2}{D-j}}{\binom{n_1}{D}}.
\end{equation}
\end{theorem}
Note that Theorem~\ref{thm:main_dist} is a special case of Theorem~\ref{thm:sample_dist}, since it assumes $u_{\max}>n_1-n_2$. 


Theorem~\ref{thm:sample_cont} below further shows the theoretical result for a continuous action space.

\begin{theorem}[General Action Guarantee for Continuous Action Space]
\label{thm:sample_cont}
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_cont_d} with an ablation size $k$ satisfying Condition~\ref{cond:k}, Relation~\eqref{eq:cert_cont} holds with probability at least
\begin{equation}
\label{eq:p_sample_cont}
    p_D=\frac{\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n_1-n_2}{D-j}}{\binom{n_1}{D}},
\end{equation}
where $\tilde{D} = {\lfloor \frac{D}{2} \rfloor}+1$. 
\end{theorem}

The larger $D$ is, the higher the probability $p_D$ is, the more likely that the \ensname selects an action in $\safeactioncont$.
In Theorem~\ref{thm:sample_cont}, when $D=\binom{N-1}{k}$,  the probability $p_D$ is 1 and the result matches Theorem~\ref{thm:main_cont}. 


Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.

==> cmarl/backup_algo.tex <==
%%% Old version of algorithm theory


\textbf{Action Certificate}\quad
First, we define a set of actions rendered by random combinations of benign messages. As the agent is likely to take these actions in a non-adversarial environment, they can be regarded as safe actions to take.
\begin{definition}[Discrete Safe Action Set $\safeactiondist$]
\label{def:fsafeact_dist}
For any step, define $\safeactiondist \subseteq \mathcal{A}$ as a set of actions that $\ablpolicy$ may select under randomly sampled benign messages.
\begin{equation}
\label{eq:safeact_dist}
     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}
\end{equation}
\end{definition}
% $\safeactiondist \subseteq \mathcal{A}$ is a set of actions that $\ablpolicy$  may select at the current step under randomly sampled benign messages.
The following theorem suggests that the ensemble policy $\smpolicy$ always takes safe actions in $\safeactiondist$ under mild conditions, even when malicious information is present in the input.


% In this case, the following theorem suggests that the ensemble policy $\smpolicy$ is not influenced by the malicious messages under mild conditions.

\begin{theorem}[Action Certificate for Discrete Action Space]
\label{thm:main_dist}
% Assume that subset size $k$  and ensemble policy $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. 
Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees safe actions under $\advmsg$, i.e.,
\begin{equation}
    \widetilde{a} = \smpolicy(o, \advmsg) \in \safeactiondist,
    \label{eq:cert_dist}
\end{equation}
if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% where 
% \begin{equation}
%     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% \end{equation}
\end{theorem}
\textbf{Remarks.}
(1) Theorem~\ref{thm:main_dist} certifies that for every step of execution, $\smpolicy$ selects a safe action when the agent receives $\advmsg$ with up to $C$ malicious messages. 
% \fh{Is there a specific reason why we emphasize one step? Should the certification certify every step? Is it possible that the actions appears safe for this round, but not safe for the next round? Oh, maybe the concept of safe already guarantees long-term safety? I feel the emphasis on current-step may cause confusion. We either need to talk about this current-step guarantees long-term safety or we just talk about long-term safety without mentioning current-step?} 
(2) \change{The condition $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ is for the worst-case consideration, which ensures robustness even if the adversarial messages collaborate to vote for an unsafe action and outweigh benign messages in all base policies. 
But in practice, our algorithm works well without requiring such a condition as verified in experiments. }
% \textcolor{red}{select some bad action} \fh{they don't have the freedom to choose actions, maybe change to something like:craft sophisticated malicious messages}
% Also, this condition is mild since $C$ is usually much smaller than $N$.


% \change{
% \textbf{Action Certificate}
% The following theorem suggests that the ensemble policy $\smpolicy$ always takes ``safe'' actions resulting from pure benign messages under mild conditions, even when malicious information is present in the input.
% \begin{theorem}[Action Certificate for Discrete Action Space]
% \label{thm:main_dist}
% Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees safe actions under $\advmsg$, i.e.,
% \begin{equation}
%     \widetilde{a} = \smpolicy(o, \advmsg) \in \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\} =: \safeactiondist,
%     \label{eq:cert_dist}
% \end{equation}
% if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% % where 
% % \begin{equation}
% %     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% % \end{equation}
% \end{theorem}
% \textbf{Remarks.}
% (1) $\safeactiondist$ is a set of actions rendered by random combinations of benign messages. As the agent is likely to take these actions in a non-adversarial environment, they can be regarded as ``safe'' actions to take.
% (2) Theorem~\ref{thm:main_dist} certifies that for every step of execution, $\smpolicy$ selects a safe action when the agent receives $\advmsg$ with up to $C$ malicious messages. 
% (3) The condition $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ is for the worst-case consideration, which ensures robustness even if the adversarial messages collaborate to vote for an unsafe action and outweigh benign messages in all base policies. 
% But in practice, our algorithm works well without requiring such a condition as verified in experiments. }



%%% Continuous action

\textbf{Action Certificate}\quad
As in the discrete action case, we first define the safe action set in the continuous action case $\safeactioncont$ as the set of actions that do not exceed the ``safe action range'' resulting from all combinations of $k$ benign messages.
% \ys{explain the safe action set with more intuition}
\begin{definition}[Continuous Safe Action Set $\safeactioncont$]
\label{def:safeact_cont}
For every $a\in \mathcal{A}\subseteq \mathbb{R}^L$, $a\in \safeactioncont$ iff for every coordinate $1\leq l\leq L$,
\vspace{-1.5em}

\small
\begin{equation}
\label{eq:safeact_cont}
\begin{aligned}
    \min\nolimits_{T\in\mathcal{H}(N-1,k)} [\ablpolicy(o, \funabl(\goodmsg, T))]_l
    \leq a_l 
    \leq 
    \max\nolimits_{T\in\mathcal{H}(N-1,k)} [\ablpolicy(o, \funabl(\goodmsg, T))]_l
\end{aligned}
\end{equation}\normalsize
\end{definition}
\vspace{-0.5em}

% We first define the safe action set in continuous-action case $\safeactioncont$ as the set of actions that does not exceed ``safe action range'' resulted by all possible combinations of benign messages. That is, in the current step, an action $a$ is in $\safeactioncont$ iff each coordinate $l \in L$ satisfy
% \begin{equation}
% \begin{aligned}
%     \inf_{T\in\mathcal{H}(N-1,k)} [\ablpolicy(o, \funabl(\goodmsg, T))]_l
%     \leq a_l \\ 
%     \leq 
%     \sup_{T\in\mathcal{H}(N-1,k)} [\ablpolicy(o, \funabl(\goodmsg, T))]_l
% \end{aligned}
% \end{equation}

$\safeactioncont \subseteq \mathcal{A}$ is a set of actions inside the range of $\ablpolicy$ under randomly sampled benign messages in the current step. 
It is reasonable to assume that actions in $\safeactioncont$ are relatively safe. For example, if the action denotes the price a seller sells its product in a market, and the communication messages are the transaction signals in an information pool, then $\safeactioncont$ is a price range  that is determined based on uncorrupted messages. Therefore, the seller will set a reasonable price without being influenced by a malicious message. 
With this definition, the following action certificate holds.
\begin{theorem}[Action Certificate for Continuous Action Space]
\label{thm:main_cont}
Under Assumption~\ref{assum:num}, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond} guarantees safe actions under $\advmsg$, i.e.,
\begin{equation}
    \smpolicy(o, \advmsg) \in \safeactioncont 
    \label{eq:cert_cont}
    % \textcolor{purple}{PH: \advmsg or  \mathbf{m}?}
\end{equation}
% then any dimension $l$ of $\smpolicy$'s output satisfies
% \begin{equation*}
%     \inf_{\krv} [\hat{a}]_l  
%     \leq [\smpolicy(o, \advmsg, \{T_d\}_{d=1}^D)]_l 
%     \leq \sup_{\krv} [\hat{a}]_l.
% \end{equation*}
% where $\hat{a} := \ablpolicy(o, \mathsf{Ablate}(m, \krv))$.
\end{theorem}

==> cmarl/fig_food_k_cont.tex <==
\begin{figure}[h]
 \centering
 \begin{subfigure}[t]{0.49\textwidth}
 \centering
  \input{figs/FoodCollector_Ablation_k_2adv_cont}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\textwidth}
 \centering
  \input{figs/FoodCollector_Ablation_k_sample_cont}
 \end{subfigure}
%  \vspace{-2em}
%  \subcaption{Continuous Action Space}
\vspace{-0.8em}
\caption{Hyper-parameter test in continuous-action FoodCollector. \textbf{Left:}  Natural and robust performance with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. Dashed green line refers to Vanilla under $C=2$ attacks.}
\vspace{-0.5em}
\label{fig:res_k_cont}
\end{figure}


==> cmarl/fig_food_k_dist.tex <==
\begin{figure}[h]
\vspace{-0.5em}
\hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.49\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_dist}}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_sample_dist}}
 \end{subfigure}
%  \vspace{-1em}
%  \subcaption{Continuous Action Space}
% \vspace{-1em}
\caption{Hyper-parameter test in discrete-action FoodCollector. \textbf{Left:}  Natural and robust performance with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. Dashed green line refers to Vanilla under $C=2$ attacks.}
\vspace{-1.5em}
\label{fig:res_k_dist}
\end{figure}


==> cmarl/fig_food_res.tex <==
\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.49\columnwidth}
  \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist_naive}}
  \vspace{-1.5em}
  \caption{Discrete \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist}}
  \vspace{-1.5em}
  \caption{Discrete \& Adaptive}
 \end{subfigure}
 \\
 %\hfill
 \begin{subfigure}[t]{0.49\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Cont_naive}}
  \vspace{-1.5em}
  \caption{Continuous \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\columnwidth}
  \resizebox{\textwidth}{!}{ \input{figs/FoodCollector_Attacker_Cont}}
  \vspace{-1.5em}
  \caption{Continuous \& Adaptive}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Reward comparison between our \ours and baselines in FoodCollector with discrete/continuous action space, under no attacker or non-adaptive/adaptive attacks under varying numbers of adversaries. Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_all}
\end{figure}





==> cmarl/fig_market_k_dist.tex <==

\begin{figure}[h]
 \centering
 \begin{subfigure}[t]{0.49\textwidth}
 \centering
  \input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\textwidth}
 \centering
  \input{figs/MarketEnv/MarketEnv_Ablation_K_sampleD}
 \end{subfigure}
%  \vspace{-2em}
%  \subcaption{Continuous Action Space}
\vspace{-0.8em}
\caption{\textbf{MarketEnv} Hyper-parameter test in continuous-action MarketEnv. \textbf{Left:}  Natural and robust performance with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. Dashed green line refers to Vanilla under $C=2$ attacks.}
\vspace{-0.5em}
\label{fig:res_k_cont_market}
\end{figure}




 

==> cmarl/fig_market_res.tex <==
\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.35\textwidth}%{0.49\columnwidth}
  \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_adaptive}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.35\textwidth}%{0.49\columnwidth}
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_permute}}
  \vspace{-1.5em}
  \caption{Non-adaptive (\permute)}
 \end{subfigure}
 \\
 %\hfill
 \begin{subfigure}[t]{0.35\textwidth}%{0.49\columnwidth}
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_flip}}
  \vspace{-1.5em}
  \caption{Non-adaptive (\swap)}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.35\textwidth}%{0.49\columnwidth}
  \resizebox{\linewidth}{!}{ \input{figs/MarketEnv/MarketEnv_Attacker_Dist_swap}}
  \vspace{-1.5em}
  \caption{Non-adaptive (\flip)}
 \end{subfigure}
 \vspace{-0.5em}
\caption{\textbf{MarketEnv}: Reward comparison between our \ours and baselines with continuous action space, under no attacker and varying numbers of adversaries for (a) adaptive and (b), (c) non-adaptive attacks. Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_all_market}
\end{figure}





==> cmarl/figs/QMIX_AME.tex <==
\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.3\columnwidth}
  \resizebox{\textwidth}{!}{\input{figs/QMIX_non_adaptive}}
  \vspace{-1.5em}
  \caption{Discrete \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.3\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/QMIX_adaptive}}
  \vspace{-1.5em}
  \caption{Discrete \& Adaptive}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Reward comparison between original QMIX and QMIX combined with our \ours in FoodCollector with discrete action space, under no attacker or non-adaptive/adaptive attacks under varying numbers of adversaries. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_qmix}
\end{figure}

==> cmarl/figs/dist_n.tex <==
% This file was created with tikzplotlib v0.9.12.
\definecolor{color0}{rgb}{0.917647058823529,0.917647058823529,0.949019607843137}
\definecolor{color1}{rgb}{0.56078431372549,0.737254901960784,0.56078431372549}
\definecolor{color2}{rgb}{1,0.388235294117647,0.27843137254902}
 
\draw[draw=black,fill=color1] (axis cs:-0.1,0) rectangle (axis cs:0.1,86.55);
\draw[draw=black,fill=color1] (axis cs:0.9,0) rectangle (axis cs:1.1,31.58);
\draw[draw=black,fill=color1] (axis cs:1.9,0) rectangle (axis cs:2.1,14.73);
\draw[draw=black,fill=color1] (axis cs:2.9,0) rectangle (axis cs:3.1,12.56);
\draw[draw=black,fill=color2] (axis cs:0.1,0) rectangle (axis cs:0.3,74.19);
\draw[draw=black,fill=color2] (axis cs:1.1,0) rectangle (axis cs:1.3,73.72);
\draw[draw=black,fill=color2] (axis cs:2.1,0) rectangle (axis cs:2.3,71.91);
\draw[draw=black,fill=color2] (axis cs:3.1,0) rectangle (axis cs:3.3,43.27);
\addplot [semithick, green!50!black, mark=*, mark size=3, mark options={solid}]
table {%
0 86.55
1 31.58
2 14.73
3 12.56
};
\addlegendentry{vanilla training}
\addplot [semithick, red, mark=square*, mark size=3, mark options={solid}]
table {%
0.2 74.19
1.2 73.72
2.2 71.91
3.2 43.27
};
\addlegendentry{randomized ablation $(k=2)$}


==> cmarl/figs/mnist/MNIST_Adaptive_Attacker_Precision.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkseagreen}{RGB}{143,188,143}
\definecolor{deepskyblue}{RGB}{0,191,255}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{tomato}{RGB}{255,99,71}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.3, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
% tick pos=both,
ytick pos = left,
xtick pos = lower,
x grid style={darkgray176},
xmin=-0.48, xmax=3.48,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={No Attacker,C=1,C=2,C=3},
y grid style={darkgray176},
ylabel={Precision},
ymin=0.7, ymax=1.03,
ytick style={color=black}
]
\draw[draw=black,fill=darkseagreen] (axis cs:-0.3,0) rectangle (axis cs:-0.1,0.9428);
\draw[draw=black,fill=darkseagreen] (axis cs:0.7,0) rectangle (axis cs:0.9,0.9182);
\draw[draw=black,fill=darkseagreen] (axis cs:1.7,0) rectangle (axis cs:1.9,0.8568);
\draw[draw=black,fill=darkseagreen] (axis cs:2.7,0) rectangle (axis cs:2.9,0.7796);
\draw[draw=black,fill=deepskyblue] (axis cs:-0.1,0) rectangle (axis cs:0.1,0.935);
\draw[draw=black,fill=deepskyblue] (axis cs:0.9,0) rectangle (axis cs:1.1,0.9);
\draw[draw=black,fill=deepskyblue] (axis cs:1.9,0) rectangle (axis cs:2.1,0.822);
\draw[draw=black,fill=deepskyblue] (axis cs:2.9,0) rectangle (axis cs:3.1,0.744);
\draw[draw=black,fill=tomato] (axis cs:0.1,0) rectangle (axis cs:0.3,0.9324);
\draw[draw=black,fill=tomato] (axis cs:1.1,0) rectangle (axis cs:1.3,0.9278);
\draw[draw=black,fill=tomato] (axis cs:2.1,0) rectangle (axis cs:2.3,0.9222);
\draw[draw=black,fill=tomato] (axis cs:3.1,0) rectangle (axis cs:3.3,0.9046);
\path [draw=black, semithick]
(axis cs:-0.2,0.937925576957219)
--(axis cs:-0.2,0.947674423042782);

\path [draw=black, semithick]
(axis cs:0.8,0.899096073701985)
--(axis cs:0.8,0.937303926298015);

\path [draw=black, semithick]
(axis cs:1.8,0.825800645168004)
--(axis cs:1.8,0.887799354831996);

\path [draw=black, semithick]
(axis cs:2.8,0.741329384640432)
--(axis cs:2.8,0.817870615359568);

\path [draw=black, semithick]
(axis cs:0,0.927624364434166)
--(axis cs:0,0.942375635565834);

\path [draw=black, semithick]
(axis cs:1,0.893675444679663)
--(axis cs:1,0.906324555320337);

\path [draw=black, semithick]
(axis cs:2,0.782301133517442)
--(axis cs:2,0.861698866482558);

\path [draw=black, semithick]
(axis cs:3,0.733801960972814)
--(axis cs:3,0.754198039027186);

\path [draw=black, semithick]
(axis cs:0.2,0.924460226703488)
--(axis cs:0.2,0.940339773296512);

\path [draw=black, semithick]
(axis cs:1.2,0.916338760974485)
--(axis cs:1.2,0.939261239025516);

\path [draw=black, semithick]
(axis cs:2.2,0.910226696362323)
--(axis cs:2.2,0.934173303637676);

\path [draw=black, semithick]
(axis cs:3.2,0.896077089698935)
--(axis cs:3.2,0.913122910301065);

\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
-0.2 0.937925576957219
0.8 0.899096073701985
1.8 0.825800645168004
2.8 0.741329384640432
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
-0.2 0.947674423042782
0.8 0.937303926298015
1.8 0.887799354831996
2.8 0.817870615359568
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0 0.927624364434166
1 0.893675444679663
2 0.782301133517442
3 0.733801960972814
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0 0.942375635565834
1 0.906324555320337
2 0.861698866482558
3 0.754198039027186
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0.2 0.924460226703488
1.2 0.916338760974485
2.2 0.910226696362323
3.2 0.896077089698935
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0.2 0.940339773296512
1.2 0.939261239025516
2.2 0.934173303637676
3.2 0.913122910301065
};
\addplot [semithick, green01270, mark=*, mark size=3, mark options={solid}]
table {%
-0.2 0.9428
0.8 0.9182
1.8 0.8568
2.8 0.7796
};
\addlegendentry{Vanilla}
\addplot [semithick, blue, mark=x, mark size=3, mark options={solid}]
table {%
0 0.935
1 0.9
2 0.822
3 0.744
};
\addlegendentry{AT}
\addplot [semithick, red, mark=square*, mark size=3, mark options={solid}]
table {%
0.2 0.9324
1.2 0.9278
2.2 0.9222
3.2 0.9046
};
\addlegendentry{AME (ours)}
\end{axis}

\end{tikzpicture}


==> cmarl/figs/mnist/MNIST_Adaptive_Attacker_Recall.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkseagreen}{RGB}{143,188,143}
\definecolor{deepskyblue}{RGB}{0,191,255}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{tomato}{RGB}{255,99,71}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.3, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=both,
x grid style={darkgray176},
xmin=-0.48, xmax=3.48,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={No Attacker,C=1,C=2,C=3},
y grid style={darkgray176},
ylabel={Recall},
ymin=0.4, ymax=1.15,
ytick style={color=black}
]
\draw[draw=black,fill=darkseagreen] (axis cs:-0.3,0) rectangle (axis cs:-0.1,0.9436);
\draw[draw=black,fill=darkseagreen] (axis cs:0.7,0) rectangle (axis cs:0.9,0.916);
\draw[draw=black,fill=darkseagreen] (axis cs:1.7,0) rectangle (axis cs:1.9,0.836);
\draw[draw=black,fill=darkseagreen] (axis cs:2.7,0) rectangle (axis cs:2.9,0.594);
\draw[draw=black,fill=deepskyblue] (axis cs:-0.1,0) rectangle (axis cs:0.1,0.9354);
\draw[draw=black,fill=deepskyblue] (axis cs:0.9,0) rectangle (axis cs:1.1,0.898);
\draw[draw=black,fill=deepskyblue] (axis cs:1.9,0) rectangle (axis cs:2.1,0.766);
\draw[draw=black,fill=deepskyblue] (axis cs:2.9,0) rectangle (axis cs:3.1,0.47);
\draw[draw=black,fill=tomato] (axis cs:0.1,0) rectangle (axis cs:0.3,0.9306);
\draw[draw=black,fill=tomato] (axis cs:1.1,0) rectangle (axis cs:1.3,0.928);
\draw[draw=black,fill=tomato] (axis cs:2.1,0) rectangle (axis cs:2.3,0.9242);
\draw[draw=black,fill=tomato] (axis cs:3.1,0) rectangle (axis cs:3.3,0.9028);
\path [draw=black, semithick]
(axis cs:-0.2,0.938064658998761)
--(axis cs:-0.2,0.949135341001239);

\path [draw=black, semithick]
(axis cs:0.8,0.893550055679356)
--(axis cs:0.8,0.938449944320644);

\path [draw=black, semithick]
(axis cs:1.8,0.791909184629903)
--(axis cs:1.8,0.880090815370097);

\path [draw=black, semithick]
(axis cs:2.8,0.470452438308156)
--(axis cs:2.8,0.717547561691844);

\path [draw=black, semithick]
(axis cs:0,0.928035218944191)
--(axis cs:0,0.942764781055809);

\path [draw=black, semithick]
(axis cs:1,0.890516685226452)
--(axis cs:1,0.905483314773548);

\path [draw=black, semithick]
(axis cs:2,0.684366673472166)
--(axis cs:2,0.847633326527834);

\path [draw=black, semithick]
(axis cs:3,0.351509494051211)
--(axis cs:3,0.588490505948789);

\path [draw=black, semithick]
(axis cs:0.2,0.920933563221125)
--(axis cs:0.2,0.940266436778876);

\path [draw=black, semithick]
(axis cs:1.2,0.91633809621031)
--(axis cs:1.2,0.939661903789691);

\path [draw=black, semithick]
(axis cs:2.2,0.913685248457524)
--(axis cs:2.2,0.934714751542476);

\path [draw=black, semithick]
(axis cs:3.2,0.892247275233382)
--(axis cs:3.2,0.913352724766618);

\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
-0.2 0.938064658998761
0.8 0.893550055679356
1.8 0.791909184629903
2.8 0.470452438308156
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
-0.2 0.949135341001239
0.8 0.938449944320644
1.8 0.880090815370097
2.8 0.717547561691844
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0 0.928035218944191
1 0.890516685226452
2 0.684366673472166
3 0.351509494051211
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0 0.942764781055809
1 0.905483314773548
2 0.847633326527834
3 0.588490505948789
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0.2 0.920933563221125
1.2 0.91633809621031
2.2 0.913685248457524
3.2 0.892247275233382
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0.2 0.940266436778876
1.2 0.939661903789691
2.2 0.934714751542476
3.2 0.913352724766618
};
\addplot [semithick, green01270, mark=*, mark size=3, mark options={solid}]
table {%
-0.2 0.9436
0.8 0.916
1.8 0.836
2.8 0.594
};
\addlegendentry{Vanilla}
\addplot [semithick, blue, mark=x, mark size=3, mark options={solid}]
table {%
0 0.9354
1 0.898
2 0.766
3 0.47
};
\addlegendentry{AT}
\addplot [semithick, red, mark=square*, mark size=3, mark options={solid}]
table {%
0.2 0.9306
1.2 0.928
2.2 0.9242
3.2 0.9028
};
\addlegendentry{AME (ours)}
\end{axis}

\end{tikzpicture}


==> cmarl/figs/mnist/MNIST_Random_Attacker_Precision.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkseagreen}{RGB}{143,188,143}
\definecolor{deepskyblue}{RGB}{0,191,255}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{tomato}{RGB}{255,99,71}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.3, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=both,
x grid style={darkgray176},
xmin=-0.48, xmax=3.48,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={No Attacker,C=2,C=4,C=6},
y grid style={darkgray176},
ylabel={Precision},
ymin=0.75, ymax=1.02,
ytick style={color=black}
]
\draw[draw=black,fill=darkseagreen] (axis cs:-0.3,0) rectangle (axis cs:-0.1,0.9428);
\draw[draw=black,fill=darkseagreen] (axis cs:0.7,0) rectangle (axis cs:0.9,0.944);
\draw[draw=black,fill=darkseagreen] (axis cs:1.7,0) rectangle (axis cs:1.9,0.914);
\draw[draw=black,fill=darkseagreen] (axis cs:2.7,0) rectangle (axis cs:2.9,0.834);
\draw[draw=black,fill=deepskyblue] (axis cs:-0.1,0) rectangle (axis cs:0.1,0.935);
\draw[draw=black,fill=deepskyblue] (axis cs:0.9,0) rectangle (axis cs:1.1,0.932);
\draw[draw=black,fill=deepskyblue] (axis cs:1.9,0) rectangle (axis cs:2.1,0.894);
\draw[draw=black,fill=deepskyblue] (axis cs:2.9,0) rectangle (axis cs:3.1,0.82);
\draw[draw=black,fill=tomato] (axis cs:0.1,0) rectangle (axis cs:0.3,0.9324);
\draw[draw=black,fill=tomato] (axis cs:1.1,0) rectangle (axis cs:1.3,0.93);
\draw[draw=black,fill=tomato] (axis cs:2.1,0) rectangle (axis cs:2.3,0.922);
\draw[draw=black,fill=tomato] (axis cs:3.1,0) rectangle (axis cs:3.3,0.9);
\path [draw=black, semithick]
(axis cs:-0.2,0.937925576957219)
--(axis cs:-0.2,0.947674423042782);

\path [draw=black, semithick]
(axis cs:0.8,0.939101020514434)
--(axis cs:0.8,0.948898979485566);

\path [draw=black, semithick]
(axis cs:1.8,0.899033370452904)
--(axis cs:1.8,0.928966629547096);

\path [draw=black, semithick]
(axis cs:2.8,0.786)
--(axis cs:2.8,0.882);

\path [draw=black, semithick]
(axis cs:0,0.927624364434166)
--(axis cs:0,0.942375635565834);

\path [draw=black, semithick]
(axis cs:1,0.924516685226452)
--(axis cs:1,0.939483314773548);

\path [draw=black, semithick]
(axis cs:2,0.886)
--(axis cs:2,0.902);

\path [draw=black, semithick]
(axis cs:3,0.797196491498017)
--(axis cs:3,0.842803508501983);

\path [draw=black, semithick]
(axis cs:0.2,0.924460226703488)
--(axis cs:0.2,0.940339773296512);

\path [draw=black, semithick]
(axis cs:1.2,0.921055728090001)
--(axis cs:1.2,0.938944271909999);

\path [draw=black, semithick]
(axis cs:2.2,0.904795349465915)
--(axis cs:2.2,0.939204650534085);

\path [draw=black, semithick]
(axis cs:3.2,0.891055728090001)
--(axis cs:3.2,0.908944271909999);

\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
-0.2 0.937925576957219
0.8 0.939101020514434
1.8 0.899033370452904
2.8 0.786
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
-0.2 0.947674423042782
0.8 0.948898979485566
1.8 0.928966629547096
2.8 0.882
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0 0.927624364434166
1 0.924516685226452
2 0.886
3 0.797196491498017
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0 0.942375635565834
1 0.939483314773548
2 0.902
3 0.842803508501983
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0.2 0.924460226703488
1.2 0.921055728090001
2.2 0.904795349465915
3.2 0.891055728090001
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0.2 0.940339773296512
1.2 0.938944271909999
2.2 0.939204650534085
3.2 0.908944271909999
};
\addplot [semithick, green01270, mark=*, mark size=3, mark options={solid}]
table {%
-0.2 0.9428
0.8 0.944
1.8 0.914
2.8 0.834
};
\addlegendentry{Vanilla}
\addplot [semithick, blue, mark=x, mark size=3, mark options={solid}]
table {%
0 0.935
1 0.932
2 0.894
3 0.82
};
\addlegendentry{AT}
\addplot [semithick, red, mark=square*, mark size=3, mark options={solid}]
table {%
0.2 0.9324
1.2 0.93
2.2 0.922
3.2 0.9
};
\addlegendentry{AME (ours)}
\end{axis}

\end{tikzpicture}


==> cmarl/figs/mnist/MNIST_Random_Attacker_Recall.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkseagreen}{RGB}{143,188,143}
\definecolor{deepskyblue}{RGB}{0,191,255}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{tomato}{RGB}{255,99,71}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.3, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=both,
x grid style={darkgray176},
xmin=-0.48, xmax=3.48,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={No Attacker,C=2,C=4,C=6},
y grid style={darkgray176},
ylabel={Recall},
ymin=0.75, ymax=1.02,
ytick style={color=black}
]
\draw[draw=black,fill=darkseagreen] (axis cs:-0.3,0) rectangle (axis cs:-0.1,0.9436);
\draw[draw=black,fill=darkseagreen] (axis cs:0.7,0) rectangle (axis cs:0.9,0.944);
\draw[draw=black,fill=darkseagreen] (axis cs:1.7,0) rectangle (axis cs:1.9,0.914);
\draw[draw=black,fill=darkseagreen] (axis cs:2.7,0) rectangle (axis cs:2.9,0.794);
\draw[draw=black,fill=deepskyblue] (axis cs:-0.1,0) rectangle (axis cs:0.1,0.9354);
\draw[draw=black,fill=deepskyblue] (axis cs:0.9,0) rectangle (axis cs:1.1,0.932);
\draw[draw=black,fill=deepskyblue] (axis cs:1.9,0) rectangle (axis cs:2.1,0.894);
\draw[draw=black,fill=deepskyblue] (axis cs:2.9,0) rectangle (axis cs:3.1,0.81);
\draw[draw=black,fill=tomato] (axis cs:0.1,0) rectangle (axis cs:0.3,0.9306);
\draw[draw=black,fill=tomato] (axis cs:1.1,0) rectangle (axis cs:1.3,0.932);
\draw[draw=black,fill=tomato] (axis cs:2.1,0) rectangle (axis cs:2.3,0.918);
\draw[draw=black,fill=tomato] (axis cs:3.1,0) rectangle (axis cs:3.3,0.894);
\path [draw=black, semithick]
(axis cs:-0.2,0.938064658998761)
--(axis cs:-0.2,0.949135341001239);

\path [draw=black, semithick]
(axis cs:0.8,0.939101020514434)
--(axis cs:0.8,0.948898979485566);

\path [draw=black, semithick]
(axis cs:1.8,0.899033370452904)
--(axis cs:1.8,0.928966629547096);

\path [draw=black, semithick]
(axis cs:2.8,0.715107668306736)
--(axis cs:2.8,0.872892331693264);

\path [draw=black, semithick]
(axis cs:0,0.928035218944191)
--(axis cs:0,0.942764781055809);

\path [draw=black, semithick]
(axis cs:1,0.924516685226452)
--(axis cs:1,0.939483314773548);

\path [draw=black, semithick]
(axis cs:2,0.882)
--(axis cs:2,0.906);

\path [draw=black, semithick]
(axis cs:3,0.78243190249582)
--(axis cs:3,0.83756809750418);

\path [draw=black, semithick]
(axis cs:0.2,0.920933563221125)
--(axis cs:0.2,0.940266436778876);

\path [draw=black, semithick]
(axis cs:1.2,0.924516685226452)
--(axis cs:1.2,0.939483314773548);

\path [draw=black, semithick]
(axis cs:2.2,0.897603921945629)
--(axis cs:2.2,0.938396078054371);

\path [draw=black, semithick]
(axis cs:3.2,0.882)
--(axis cs:3.2,0.906);

\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
-0.2 0.938064658998761
0.8 0.939101020514434
1.8 0.899033370452904
2.8 0.715107668306736
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
-0.2 0.949135341001239
0.8 0.948898979485566
1.8 0.928966629547096
2.8 0.872892331693264
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0 0.928035218944191
1 0.924516685226452
2 0.882
3 0.78243190249582
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0 0.942764781055809
1 0.939483314773548
2 0.906
3 0.83756809750418
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0.2 0.920933563221125
1.2 0.924516685226452
2.2 0.897603921945629
3.2 0.882
};
\addplot [semithick, black, mark=-, mark size=6, mark options={solid}, only marks, forget plot]
table {%
0.2 0.940266436778876
1.2 0.939483314773548
2.2 0.938396078054371
3.2 0.906
};
\addplot [semithick, green01270, mark=*, mark size=3, mark options={solid}]
table {%
-0.2 0.9436
0.8 0.944
1.8 0.914
2.8 0.794
};
\addlegendentry{Vanilla}
\addplot [semithick, blue, mark=x, mark size=3, mark options={solid}]
table {%
0 0.9354
1 0.932
2 0.894
3 0.81
};
\addlegendentry{AT}
\addplot [semithick, red, mark=square*, mark size=3, mark options={solid}]
table {%
0.2 0.9306
1.2 0.932
2.2 0.918
3.2 0.894
};
\addlegendentry{AME (ours)}
\end{axis}

\end{tikzpicture}


==> cmarl/include/supp_macros.tex <==
% Comments
\newcommand{\ys}[1]{{\color{blue}{YS:#1}}}
\newcommand{\rj}[1]{{\color{purple}{RJ:#1}}}
\newcommand{\draft}[1]{{\color{gray}{DRAFT:#1}}}
\newcommand{\fh}[1]{{\color{orange}{{#1}}}}
\newcommand{\fhc}[1]{{\color{orange}{\scriptsize{[FH:#1]}}}}
\newcommand{\change}[1]{{\color{red}{#1}}}
\newcommand{\SF}[1]{{\color{red}{SF:#1}}}

%%% functions
\newcommand{\natobj}{J_{\mathrm{nat}}}
\newcommand{\advobj}{J_{\mathrm{att}}}
\newcommand{\funabl}{\mathsf{Ablate}}
\newcommand{\funmed}{\mathsf{Median}}
\newcommand{\commfunc}{\xi}

%%% spaces
\newcommand{\agents}{\mathcal{D}}
\newcommand{\his}{\tau}
\newcommand{\hisspace}{\Gamma}

%%% others
\newcommand{\step}{^{(t)}}
\newcommand{\krv}{\mathcal{T}}
\newcommand{\robaction}{\widetilde{a}}

\newcommand{\ablpolicy}{\hat{\pi}}
\newcommand{\smpolicy}{\widetilde{\pi}}

\newcommand{\safeaction}{\mathcal{A}_{\mathrm{benign}}}
\newcommand{\safeactiondist}{\mathcal{A}_{\mathrm{benign}}^{\mathrm{d}}}
\newcommand{\safeactioncont}{\mathsf{Range}(\safeaction)}


%%% messages
\newcommand{\mtoi}{\mathbf{m}_{: \to i}}
\newcommand{\msg}{\mathbf{m}}
\newcommand{\msgk}{[\mathbf{m}]_k}
\newcommand{\allmsgk}{\mathcal{H}_{k}(\msg)}
\newcommand{\allmsgkd}{\mathcal{H}_{k,D}(\msg)}
\newcommand{\msgki}{[\mtoi]_k}
\newcommand{\allmsgki}{\mathcal{H}_{k}(\mtoi)}
\newcommand{\ablmi}{\hat{\mathbf{m}}^k_{i}}
\newcommand{\goodmsg}{\mathbf{m}_{\mathrm{benign}}}
\newcommand{\advmsg}{\mathbf{m}_{\mathrm{adv}}}
\newcommand{\goodmsgk}{[\mathbf{m}_{\mathrm{benign}}]_k}
\newcommand{\advmsgk}{[\mathbf{m}_{\mathrm{adv}}]_k}
\newcommand{\goodallmsgk}{\mathcal{H}_{k}(\goodmsg)}
\newcommand{\advallmsgk}{\mathcal{H}_{k}(\advmsg)}




%%% names
\newcommand{\oursfull}{{Ablated Message Ensemble}\xspace}
\newcommand{\ours}{{AME}\xspace}
\newcommand{\ablname}{{message-ablation policy}\xspace}
\newcommand{\ablnames}{{message-ablation policies}\xspace}
\newcommand{\ensname}{{message-ensemble policy}\xspace}
\newcommand{\ablnamecap}{{Message-Ablation Policy}\xspace}
\newcommand{\ensnamecap}{{Message-Ensemble Policy}\xspace}
\newcommand{\safename}{{benign action}\xspace}
\newcommand{\ksample}{{k-sample}\xspace}
\newcommand{\ksamples}{{k-samples}\xspace}


\newcommand{\permute}{{Perm-Attack}\xspace}
\newcommand{\swap}{{Swap-Attack}\xspace}
\newcommand{\flip}{{Flip-Attack}\xspace}

\newcommand{\marketenv}{{InventoryManager}\xspace}
\newcommand{\mnistenv}{{MARL-MNIST}\xspace}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}

\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}

\newcommand{\myst}[1]{\textcolor{red}{\st{#1}}}

==> cmarl/include/supp_packages.tex <==
% \usepackage{hyperref}
\usepackage{url}
% \usepackage{natbib}
\usepackage{graphicx}
% \usepackage{amsfonts}
% \usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{bbm}
\usepackage{xcolor}
% \usepackage{algorithm}
\usepackage{scalerel}
% \usepackage[noend]{algpseudocode}
\setlength\parindent{0pt}

% \usepackage{natbib}
\usepackage[outdir=./]{epstopdf}
\usepackage{graphicx,float,pgfplots,wrapfig,sidecap,lipsum}

\usepackage{colortbl}
\usepackage{tablefootnote}
%\usepackage{subfig}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{subcaption}
\usepackage{subfloat}
% \usepackage{hyperref,psfrag} % not allowed by AAAI
\usepackage{tikz}
\usetikzlibrary{fit}
\usetikzlibrary{calc,shapes}
\usetikzlibrary{decorations.pathmorphing} % noisy shapes
\usetikzlibrary{fit}					% fitting shapes to coordinates
\usetikzlibrary{backgrounds}	% drawing the background after the foreground
\usetikzlibrary{pgfplots.groupplots}

\usepackage[utf8]{inputenc}
\usepackage{pgfplots}
\DeclareUnicodeCharacter{2212}{−}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}

\usepackage{xspace}
\usepackage{soul}

==> cmarl/neurips/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% \draft{We study the attacks and defenses in communicative multi-agent reinforcement learning.
% Our contributions:
% 1. formulate the adversarial problem in CMARL.
% 2. propose a certifiable defense algorithm
% 3. empirical study in a simulated game and a market environment.
% }
% Recent years have witnessed significant advances in reinforcement learning (RL), especially deep reinforcement learning (DRL). Although vanilla RL considers the interaction between a single agent and the environment, many real-world applications have multiple agents involved, such as autonomous driving~\cite{shalev2016safe}, robotics~\cite{dudek1996taxonomy}, etc. 
% \ys{start from decision making?}
% With the rapid improvement of deep reinforcement learning (DRL) techniques, neural network-based 
Neural network-based multi-agent reinforcement learning (MARL) has achieved significant advances in many real-world applications, such as autonomous driving~\cite{shalev2016safe,sallab2017deep}. In a multi-agent system, especially in a cooperative game, communication usually plays an important role. By feeding communication messages as additional inputs to the policy network, each agent can obtain more information about the environment and other agents, and thus can learn a better policy~\cite{foerster2016learning,hausknecht2016cooperation,sukhbaatar2016learning}. 
% Many recent works~\cite{foerster2016learning,hausknecht2016cooperation,sukhbaatar2016learning} have shown that feeding communication messages to RL networks can result in better decision makers.

However, neural networks are shown to be vulnerable to adversarial attacks~\cite{chakraborty2018adversarial}, i.e.,
% , especially network-based RL policies~\cite{huang2017adversarial} \fh{network-based RL policies are not a special case of neural networks. So the logic here is a bit unsmooth.}, 
a well-trained network may output a wrong answer if the input to the network is slightly perturbed~\cite{goodfellow2014explaining}.
% if the inputs to the network are slightly but deliberately perturbed, the network, although well-trained on clean datasets \fh{rather than datasets, shall we say unattacked environment or safe environment, since RL is not necessarily trained on a ``dataset''?}, may output a wrong answer. 
As a result, although a policy can obtain a high reward by taking in the messages sent by other agents, it may also get drastically misled by inaccurate information or even adversarial communication from malicious attackers. 
For example, when several drones execute pre-trained policies and exchange information via wireless communication, it is possible that messages get noisy in a hostile environment, or even some malicious attacker eavesdrops on their communication and intentionally perturbs some messages to a victim agent via cyber attacks. 
Moreover, even if the communication channel is protected by advanced encryption algorithms, an attacker may also hack some agents and alter the messages before they are sent out (e.g. hacking IoT devices that usually lack sufficient protection~\cite{naik2017cyber}). Figure~\ref{fig:diagram} shows an example of communication attacks, where the agents are trained with benign communication, but attackers may perturb the communication during the test time. The attacker may lure a well-trained agent to a dangerous location through malicious message propagation and cause fatal damage. 
Although our paper focuses on adversarial perturbations of the communication messages, it also includes unintentional perturbations, such as misinformation due to malfunctioning sensors or communication failures; these natural perturbations are no worse than adversarial attacks.

\begin{figure*}[!t]
\vspace{-3em}
    \centering
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{figs/marl.pdf}
         \vspace{-0.5em}
         \caption{Training time}
         \label{sfig:train}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{figs/marl_adv.pdf}
         \vspace{-0.5em}
         \caption{Test time (in deployment)}
         \label{sfig:test}
     \end{subfigure}
     \vspace{-0.5em}
    \caption{An example of test-time communication attacks in a communicative MARL system.  (a) During training, agents are trained collaboratively in a safe environment, such as a simulated environment. (b) In deployment, agents execute pre-trained policies in the real world, where malicious attackers may modify the benign ({\color{darkpastelgreen}{green}}) messages into adversarial ({\color{red}{red}}) signals to mislead some victim agent(s). 
    % \myst{In this figure, arrows denote communication channels among agents, {\color{darkpastelgreen}{green}} messages stand for benign communication, and {\color{red}{red}} messages stand for adversarial communication.}
    % \myst{Agents can be heterogeneous as depicted by various icons.}
    }
    \label{fig:diagram}
\vspace{-2em}
\end{figure*}

Although adversarial attacks and defenses have been extensively studied in supervised learning~\cite{madry2018towards,cohen2019certified,zhang2019theoretically} and reinforcement learning~\cite{zhang2020robust,zhang2021robust,oikarinen2020robust}, there has been little discussion on the robustness issue against adversarial communication in MARL problems. 
Therefore, to safely improve decision-making with communication in high-stakes multi-agent scenarios, it is crucial to robustify MARL policies against adversarial communication.  
% \textcolor{red}{Defending against the adversarial communication while still utilizing the benign communication}\fh{needs rewording. Maybe: Achieving high performance in a multi-agent cooperative game through inter-agent communication while remain robust to adversarial communication attacks} 
Achieving high performance in a multi-agent cooperative game through inter-agent communication while being robust to adversarial communication is a challenging problem due to the following reasons. 
\textbf{Challenge I}: 
% \myst{The attacker may construct malicious messages in various ways, so that they are hard to be distinguished from benign messages.} 
% \myst{For example, the malicious messages shown in Figure}~\ref{sfig:test} \myst{are in the same form as the benign messages and also make semantic sense.}
Sometimes communication attacks are stealthier as misleading
messages  (which share the form of benign messages and are semantically meaningful in Figure~\ref{sfig:test}) can be hard to recognize, while attacking by abnormal actions~\cite{gleave2020adversarial} can be easier for humans to notice.
\textbf{Challenge II}: A strong attacker can even be \textit{adaptive} to the victim agent and significantly reduce the victim's total reward. For instance, for a victim agent who moves according to the average of GPS coordinates sent by others, the attacker may learn to send extreme coordinates to influence the average.
% the attacker may learn an RL policy to send sequential misleading messages. \fh{This point is not very clear.}
\textbf{Challenge III}: There can be more than one attacker (or an attacker can perturb more than one message at one step), such that they can collaborate to mislead a victim agent.

Tu et al.~\cite{tu2021adversarial} apply adversarial training~\cite{madry2018towards} to improve model robustness against communication perturbations. But they focus on perturbations with small $\ell_p$ distances, which do not cover many attack scenarios as discussed in Section~\ref{sec:setup_adv}.
Some recent works~\cite{blumenkamp2020emergence,xue2021mis,mitchell2020gaussian} take the first step to investigate adversarial communications in MARL and propose several defending methods, such as a learned message filter~\cite{xue2021mis}. However, these empirical defenses do not fully address the aforementioned challenges, and are not guaranteed to be robust, especially under adaptive attacks. 
% \textcolor{purple}{PH: all communication attacks, any communication attack? YS: should be all, thanks} 
%\textcolor{purple}{PH: Is it clear what we mean by adaptive attacks? In challenge 2 we are kind of defining it. Would it make sense to make the \textit{adaptive} italic in challenge 2 to stand out? YS: Sure! Good point}
% Levine et al.~\cite{Levine_Feizi_2020} use randomized ablation to defend against sparse attacks in image classification, where a fraction of pixels may be corrupted. However, their high-probability guarantee is not suitable for sequential decision-making problems, as the guaranteed probability decreases along propagation over time. Moreover, their algorithm does not work when the policy takes continuous actions. 

In this paper, we address all aforementioned challenges by proposing {a certifiable defense, named \textbf{\oursfull (\ours)}, that can guarantee the performance of agents when a fraction of communication messages are perturbed}. 
The main idea of \ours is to make decisions based on multiple different subsets of communication messages (i.e., ablated messages). Specifically, for a list of messages coming from different agents, we train a \emph{\ablname} that takes in a subset of messages and outputs a \emph{base action}. Then, we construct an \emph{\ensname} by aggregating multiple base actions coming from multiple ablated message subsets. 
% The main idea of \ours is to construct an \emph{ensemble policy} which makes decisions based on multiple different subsets of communication messages (i.e., ablated messages). 
% Specifically, for a list of messages coming from different agents, we train a \emph{base ablation policy} that takes in a subset of messages and outputs a \emph{base action}. 
For a discrete action space, the ensemble policy takes the majority of the multiple base actions obtained, while for a continuous action space, the ensemble policy takes the median of these base actions. \ours is a generic framework that works for any agent that observes multiple messages from different sources, as long as the agent receives more benign communication messages than adversarial ones. We also show in Section~\ref{sec:algo_more} that \ours can be used in many other decision-making scenarios beyond defending against communication attacks. 
A similar randomized ablation idea is used by Levine et al.~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification. However, they provide high-probability guarantee for a single-step decision, which is not suitable for sequential decision-making problems, as the guaranteed probability decreases when it propagates over timesteps. Moreover, their algorithm does not work when the model has a continuous output space. 
In contrast, \ours has robustness guarantees for both the immediate action and the long-term reward, and for both discrete and continuous actions. 
% A similar randomized ablation idea is used by Levine et al.~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification. However, their high-probability guarantee is not suitable for RL \fh{sequential decision-making} problems, as the probability decreases along propagation over time. Moreover, their algorithm does not work for a continuous action space. In contrast, \ours has robustness guarantees for the long-term reward, and works on both discrete and continuous action spaces. 

% \ys{compare to Levine et al. high probability reduces along propagation of time / may not lead to reliable multi-step robustness due to the long horizon.}
% Therefore, \ours can be extended to defend against 
% \ys{flexibility, as discussed later}

Our contributions can be summarized as below:\\
\textbf{(1)} We formulate the problem of adversarial attacks and defenses in communicative MARL (CMARL). \\
% \fhc{Do we still use CMARL? If not, it is fine. If so, explain it.}.\\
\textbf{(2)} We propose a novel defense method, \ours, 
% \SF{perhaps introduce ``ablation" terminology in the previous paragraph so readers become familiar with it at this point}
% based on randomized ablation on communication messages. \ours 
that is certifiably robust against arbitrary perturbations of up to $C<\frac{N-1}{2}$ communications, where $N$ is the number of agents. \\
% both in discrete action space and in continuous action space. \fh{I feel the contribution is not that we include both discrete or continuous action space, but rather, we can achieve very strong results in the discrete space, as well as good results in the continuous space. I feel the current wording sounds a bit off the path.}\\
\textbf{(3)} Experiment in several multi-agent environments shows that \ours obtains significantly higher reward than baseline methods under both non-adaptive and adaptive attackers. 
% The agent trained with \ours achieves similar 
% \SF{add a bit more details here; what environments; discrete or cont; what gains do we achieve?}. 
% \fh{maybe some numbers in terms of performance improvement etc}



==> cmarl/neurips/2_relate.tex <==
\vspace{-0.5em}
\section{Related Work}
\label{sec:relate}


\textbf{Adversarial Robustness of RL Agents}\quad
% As RL techniques have been applied to more and more applications, the robustness of agents under environment noise or adversarial attacks becomes an emerging research topic. 
Section~\ref{sec:setup_adv} introduces several adversarial attacks on single-agent and multi-agent problems.
To improve the robustness of agents, adversarial training (i.e., introducing adversarial agents to the system during training~\cite{pinto2017robust,phan2021resilient,zhang2021robust,sun2021strongest}) and network regularization~\cite{zhang2020robust,shen2020deep,oikarinen2020robust} are empirically shown to be effective under $\ell_p$ attacks, although such robustness is not theoretically guaranteed. 
Certifying the robustness of a network is an important research problem~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness}.
% There is an important line of work studying guaranteed robustness of neural networks~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness} when the input data is perturbed within an $\ell_p$ norm ball. 
In an effort to certify RL agents' robustness, some approaches~\cite{lutjens2020certified,zhang2020robust,oikarinen2020robust,fischer2019online} apply network certification tools to bound the Q networks and improve the worst-case value of the policy. Kumar et al.~\cite{kumar2021policy} and Wu et al.~\cite{wu2021crop} follow the idea of randomized smoothing~\cite{cohen2019certified} and smooth out the policy by adding Gaussian noise to the input.




\textbf{Adversarial Attacks and Defenses in CMARL}\quad
Appendix~\ref{app:related} discusses some related works on learning effective communication among agents~\cite{foerster2016learning,sukhbaatar2016learning,das2020tarmac}. 
Recently, the problem of adversarial communication in MARL has attracted increasing attention.  
Blumenkamp et al.~\cite{blumenkamp2020emergence} show that in a cooperative game, communication policies of some self-interest agents can hurt other agents' performance. 
% To accommodate multiple agent objectives, they propose \change{Aggregation}\fh{aggregated? is aggregation GNN a terminology? I've not heard of it.} Graph Neural Networks to model and learn an inter-agent communication policy. 
To achieve robust communication, Mitchell et al.~\cite{mitchell2020gaussian} adopt a Gaussian Process-based probabilistic model to compute the posterior probabilities that whether each partner is truthful. 
Tu et al.~\cite{tu2021adversarial} investigate the vulnerability of multi-agent autonomous systems against communication attacks, with a focus on vision tasks.
% \change{multiple aspects} \fh{?}.
Xue et al.~\cite{xue2021mis} propose an algorithm to defend against one adversarial communication message by an anomaly detector and a message reconstructor, which are trained with groundtruth labels and messages.

To the best of our knowledge, our \ours is the first certifiable defense in MARL against communication attacks. Moreover, we consider a strong threat model where up to half of the communication messages can be arbitrarily corrupted, capturing many realistic types of attacks.

% In comparison, we focus on a different and strong threat model where a fraction of communication messages are arbitrarily corrupted, capturing many realistic types of attacks. Our proposed defense has certifiable performance and achieves strong robustness in experiments.

% A similar randomized ablation defense is used to defend against $\ell_0$ attacks in image classification~\cite{Levine_Feizi_2020}.
% But our defensive mechanism is fundamentally different from the image classification defense~\cite{Levine_Feizi_2020} which provides a high-probability guarantee for discrete image label outputs, as our defense achieves both action and long-term reward certification (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output, which is non-trivial.

% Levine et al.~\cite{Levine_Feizi_2020} propose a similar defense based on randomized ablation against $\ell_0$ attacks in image classification.
% But our defense and theoretical results are fundamentally different and non-trivial extensions of this work~\cite{Levine_Feizi_2020}.
% Levine et al.~\cite{Levine_Feizi_2020} provide a high-probability guarantee for discrete image label outputs, while our defense achieves both action and reward certificates (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output.


% formulates adversarial attacks in a general \fh{are previous works not generic? Why?}communicative MARL (CMARL) setting, and 
% \fh{Is \cite{xue2021mis} attack agnostic? The current description doesn't answer this question.}.


% This threat model can cover many realistic attacking scenarios that the $\ell_p$ model does not solve.

% This paper \myst{is also closely related to} \fh{bears some similarities with}~\cite{gleave2020adversarial}, which studies the effects of adversarial actions in an MARL problem. In contrast, our work aims to defend against communication attacks that can be more stealthy in practice.
% Randomized ablation is proposed by~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification problems, in which the classifier is trained by randomly ablating pixels of images. 
% We are the first to extend the idea of randomized ablation to MARL and to achieve action and reward certificates against communication attacks.
% Note that the number of pixels in an image and the number of agents in an MARL problem are in different scales. Also, a classifier outputs discrete labels, while a policy may have discrete or continuous output space. Therefore, our problem setup, methodology and theoretical results are significantly different from~\cite{Levine_Feizi_2020} and are novel.

% \textbf{parameter sharing} Sharing parameters are a common way to take advantage of centralized training \cite{lowe2017multi,foerster2016learning} by learning a single shared critic network for multiple agents. \cite{gupta2017cooperative} uses single-agent RL methods to learn policies in cooperative environments.

==> cmarl/neurips/3_setup_new.tex <==
% \section{Problem Formulation}
% \label{sec:setup}
% \section{\myst{Preliminaries: }Communicative Muti-agent Reinforcement Learning \fh{(CMARL)}}
\section{Communicative Muti-agent Reinforcement Learning (CMARL)}
\label{sec:setup_cmarl}
\textbf{Dec-POMDP Model}\quad
We consider a Decentralised Partially Observable Markov Decision Process (Dec-POMDP)~\cite{oliehoek2012decentralized,oliehoek2015concise,das2020tarmac} which is a multi-agent generalization of the single-agent POMDP models. 
A Dec-POMDP can be modeled as a tuple $\langle \mathcal{D}, \mathcal{S}, \mathcal{A}_{\agents}, \mathcal{O}_{\agents}, O, P, R, \gamma, \rho_0 \rangle$. 
$\mathcal{D}=\{1,\cdots,N\}$ is the set of $N$ agents.
$\mathcal{S}$ is the underlying state space. $\mathcal{A}_{\agents}=\times_{i\in\mathcal{D}}\mathcal{A}_i$ is the \emph{joint} action space. $\mathcal{O}_{\agents}=\times_{i\in\mathcal{D}}\mathcal{O}_i$ is the \emph{joint} observation space, with $O$ being the observation emission function.
$P: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \Delta(\mathcal{S}) $ is the state transition function\footnote{$\Delta(\mathcal{X})$ denotes the space of probability distributions over space $\mathcal{X}$.}.
$R: \mathcal{S}\times\mathcal{A}_1\times\cdots\mathcal{A}_N \to \mathbb{R}$ is the shared reward function.
$\gamma$ is the shared discount factor, and $\rho_0$ is the initial state distribution. 
% \fhc{Shall we mention the Cooperative game?}\ys{we can discuss it in the communication paragraph}

\textbf{Communication Policy $\commfunc$ in Dec-POMDP}\quad
Due to the partial observability, communication among agents is crucial for them to obtain high rewards. Consider a shared message space $\mathcal{M}$, where a message $m\in\mathcal{M}$ can be a scalar or a vector, e.g., signal of GPS coordinates. 
The communication policy of agent $i\in\mathcal{D}$, denoted as $\commfunc_i$, generates messages based on the agent's observation or interaction history. 
At every step $t$, agent $i$ sends a communication message $m_{i \to j}\step$ to agent $j$ for all $j\neq i$. 
(For notational simplicity, we will later omit ${}\step$ when there is no ambiguity.)
% Here $m_{i \to j}\step$ denotes a message sent from agent $i$ to $j$ in step $t$. 
% We use $\mtoi$ to denote the list of messages received by agent $i$, i.e., $\mtoi:=\{m_{j \to i} | 1\leq j \leq N, j\neq i \}$. 
We assume that agents are fully connected for communication, although our algorithm directly applies to partially connected communication graphs. That is, at each step, every agent sends $N-1$ messages (one for each agent other than itself), and receives $N-1$ messages from others. \\
This paper studies a general defense under any given communication protocol, so we do not make any assumption on how the communication policy $\commfunc$ is obtained (e.g., from a pre-defined communication protocol, or a learning algorithm~\cite{foerster2016learning,das2020tarmac}). 
% \myst{Moreover, although we focus on cooperative agents, our defense applies to any agent that relies on communications, even if it is not fully cooperative with others.}
% from the encoded observation~\cite{mousavi2019multi,tu2021adversarial}, or from a learning algorithm~\cite{foerster2016learning,das2020tarmac}). 

\textbf{Acting Policy $\pi$ with Communication}\quad
The goal of each agent $i\in\agents$ is to maximize the discounted cumulative reward $\sum_{t=0}^\infty \gamma^t r\step$ by learning an acting policy $\pi_i$. 
When there exists communication, the policy input contains both its own interaction history, denoted by $\his_i\in\hisspace_i$, and the communication messages $\mtoi:=\{m_{j \to i} | 1\leq j \leq N, j\neq i \}$. 
% That is, $\pi_i(a|\tau_i, \mtoi)$ is the probability of agent $i$ taking action $a$ when observing $\tau_i$ and receiving messages $\mtoi$, where $\tau_i$ 
Similar to the communication policy $\commfunc$, we do not make any assumption on how the acting policy $\pi$ is formulated, as our defense mechanism introduced later can be plugged into any policy learning procedure.


% Communication messages from other agents are important for the acting policy to gain high rewards~\cite{foerster2016learning,liu2018energy}. However, as will be discussed in Section~\ref{sec:setup_adv} below, communication can be a double-edge sword --- it expedites learning by information sharing but may make agents vulnerable to adversarial attacks.


\section{Problem Formulation: Communication Attacks in Deployment of CMARL}
\label{sec:setup_adv}

Communication is important for agents to obtain high rewards, but it can be a double-edged sword --- it benefits decision making but may make agents vulnerable to perturbations of messages.
Communication attacks in MARL has recently attracted increasing attention~\cite{blumenkamp2020emergence,tu2021adversarial,xue2021mis} with different focuses, as summarized in Section~\ref{sec:relate}. 
In this paper, we consider a practical and strong threat model where malicious attackers can arbitrarily perturb a subset of communication messages during test time.

\textbf{Formulation of Communication Attack: The Threat Model}\quad 
During test time, agents execute well-trained policies $\pi_1,\cdots, \pi_N$. 
As shown in Figure~\ref{sfig:test}, the attacker may perturb communication messages to mislead a specific victim agent. Without loss of generality, suppose $i\in\agents$ is the victim agent receiving $N-1$ communication messages from other agents. We consider the sparse attack setup where up to $C$ messages can be arbitrarily perturbed at every step, among all $N-1$ messages. 
Here $C$ is a reflection of the attacker's attacking power.
% , which is usually limited in practice (i.e., $C$ is not too large).
% Once the attacker has control over a communication channel (e.g. channel from $j$ to $i$), it is able to arbitrarily change the corresponding messages (e.g. $m_{j \to i}$ can be arbitrarily perturbed). 
The victim agent has no knowledge of which messages are adversarial. 
% , and the attacker may attack at different $C$ channels at each step. 
We make the following mild assumption for the attacking power.
\begin{assumption} [Attacking Power]
\label{assum:num}
An attacker can arbitrarily manipulate fewer than a half of the communication messages, i.e.,
$C<\frac{N-1}{2}$.
% $C<\lfloor\frac{N}{2}\rfloor$. 
% \textcolor{purple}{PH: less than half of the communication channels?}
\end{assumption}
This is a realistic assumption, as it takes the attacker's resources to hack or control each communication channel. It is less likely that an attacker can change the majority of communications among agents without being detected. Moreover, communications can be corrupted due to hardware failures, which usually affect a limited fraction of communications.
Note that this is a strong threat model as the $C$ attacked messages can be arbitrarily perturbed based on the attacker's attacking algorithm.
% For example, communication can happen between various types of hardware, including well-protected advanced computers and (probably) underprotect IoT devices.

\textbf{Comparison with $\ell_p$ Threat Models}\quad 
Many existing works on adversarial attack and defense~\cite{goodfellow2014explaining,huang2017adversarial,zhang2020robust,tu2021adversarial} assume that the perturbation is small in $\ell_p$ norm. However, many realistic and stealthy attacks can not be covered by the $\ell_p$ threat model. For example, the attacker may replace a word in a sentence as in Figure~\ref{sfig:test}, add a patch to an image, or shift the signal by some bits. In these cases, the $\ell_p$ distance between the clean value and the perturbed value is large, such that $\ell_p$ defenses do not work.
In contrast, these attacks are covered by our threat model which allows arbitrary perturbations to $C$ messages. Therefore, our setting can work for broader applications. 
% This type of limited attacking power assumption is common in adversarial learning, i.e.,  attack with bounded radius in $\ell_p$ norm. 


\textbf{Comparison between Communication Attacks and Other Attacks in MARL}\quad
Adversarial attacks and defenses in RL systems have recently attracted more and more attention, and are considered in many different scenarios. 
The majority of related work focuses on \textit{directly attacking a victim} by perturbing its observations~\cite{huang2017adversarial,gleave2020adversarial,oikarinen2020robust,sun2021strongest} or actions~\cite{tessler2019action,pinto2017robust}. 
However, an attacker may not have direct access to the specific victim's observation or action. 
In this case, \textit{indirect attacks via other agents} can be an alternative. For example, Gleave et al.~\cite{gleave2020adversarial} propose to attack the victim by changing the other agent's actions. Therefore, even if the victim agent has well-protected sensors, the attacker can still influence it by manipulating other under-protected agents. But the intermediary agent whose actions are altered will obtain sub-optimal reward, which makes the attack noticeable and less stealthy. 
In contrast, if an attacker alters the communication messages sent from the other agents (e.g., by man-in-the-middle attacks~\cite{mallik2019man}), the behaviors of other agents are not changed, and thus it is relatively hard to find who has sent adversarial messages and which messages are not trustworthy. \\
It is also worth pointing out that, since an acting policy $\pi$ takes in both its own observation and the communication messages, communication can be regarded as a subset of policy inputs. Therefore, the communication attack is related to traditional adversarial defenses of deep neural policies against $\ell_0$ perturbations to the input~\cite{Levine_Feizi_2020}, as detailed in Appendix~\ref{app:theory}.
% But different from most literature that consider $\ell_\infty$ or $\ell_2$ perturbations on the entire input vector, we focus on the case where a fraction of inputs can be totally corrupted, analogous to an $\ell_0$ attack (sparse attack) model as detailed in Appendix~\ref{app:theory}.


\textbf{Goal: A General and Certifiable Defense}\quad
As formulated above, the attacker can perturb up to $C$ communication messages sent to any agent at every step. 
However, we do not make any assumption on what attack algorithm the attacker uses, i.e., how a message is perturbed. 
In practice, an attacker may randomly change the communication signal, or learn a function to perturb the communication based on the current situation. 
The attacker can either be white-box or black-box, based on whether it knows the victim agent's policy, as extensively studied in the field of adversarial supervised learning~\cite{chakraborty2018adversarial}. 
To achieve generic robustness under a wide range of practical scenarios, it is highly desirable for a defense to be agnostic to attack algorithms and work for arbitrary (including strongest/worst) perturbations. This is achieved by our defense which will be introduced in Section~\ref{sec:algo}. 


==> cmarl/neurips/4_algo_short.tex <==
\section{Provably Robust Defense for CMARL}
\label{sec:algo}

In this section, we present our defense algorithm, \textit{\oursfull (\ours)}, against test-time communication attacks in CMARL. 
% \ours has two phases: the training phase where a base policy is trained for each agent we aim to robustify, and the defending phase where the base policy is used to make
% relatively safe
% decisions via message ablation and ensemble.  
We first introduce the algorithm design in Section~\ref{sec:algo_overview}, then present the theoretical analysis in Section~\ref{sec:algo_theory}.
Section~\ref{sec:algo_more} discusses several extensions of \ours.


\subsection{\oursfull (\ours)}
\label{sec:algo_overview}

% \SF{In the intro, we call the method ensemble policy; we should use the same terminology. I like AME} >> Sure, I added AME to the intro.
% As characterized in Section~\ref{sec:setup}, in a CMARL game, every agent makes decisions based on not only its own observations, but also all received messages. If an agent trusts the communication from all other agents, it may fail when some communication is maliciously corrupted.
% On the other hand, if an agent does not trust communication, it can not benefit from the useful information shared by other benign agents.
% Therefore, there is a trade-off between natural performance (i.e., reward under no attack) and robustness (i.e., reward under attacks).
% Our goal is to learn and execute a robust policy for any agent in the environment, so that the agent can perform well in both a non-adversarial environment and an adversarial environment.


% \textbf{Main Idea}\quad
% Intuitively, if an agent $i$ overly relies on the information given by agent $j$, then a strong adaptive attacker can easily mislead $i$ by perturbing the messages from $j$. On the other hand, if an agent does not trust communication, it can not benefit from the useful information shared by other benign agents.
% Therefore, there is a trade-off between natural performance (i.e., reward under no attack) and robustness (i.e., reward under attacks). 
% 
Our goal is to learn and execute a robust policy for any agent in the environment, so that the agent can perform well in both a non-adversarial environment and an adversarial environment. 
To ease the illustration, we focus on robustifying an arbitrary agent $i\in\agents$, and the same defense is applicable to all other agents.
We omit the agent subscript ${}_i$, and denote the agent's observation space, action space, and interaction history space as $\mathcal{O}$, $\mathcal{A}$, and $\hisspace$, respectively. 
% We aim to train a robust acting policy for the agent as $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$, where $\hisspace$ is the space of the interaction histories.

Let $\msg \in \mathcal{M}^{N-1}$ denote a set of $N-1$ messages received by the agent. Then, we can build an ablated message subset of $\msg$ with $k$ randomly selected messages, as defined below.

\begin{definition}[$\boldsymbol{k}$-Ablation Message Sample (k-Sample)]
For a message set $\msg \in \mathcal{M}^{N-1}$ and any integer $1 \leq k \leq N-1$, define a $k$-ablation message sample (or \ksample for short), $\msgk \in \mathcal{M}^k$, as a set of $k$ randomly sampled messages from $\msg$. Let $\allmsgk$ be the collection of all unique \ksamples of $\msg$, and thus $|\allmsgk|=\binom{N-1}{k}$.
\end{definition}


% \textbf{Notations}\quad
% % \textbf{(1) Agent and policy.} To ease the illustration, we focus on robustifying an arbitrary agent $i\in\agents$, and the same defense is applicable to all other agents.
% % We omit the agent subscript ${}_i$, and denote the agent's observation space and action space as $\mathcal{O}$ and $\mathcal{A}$. We aim to train a robust acting policy for the agent as $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$, where $\hisspace$ is the space of the interaction histories.  \\
% \textbf{(1) Ablated $k$ message samples (k-samples) $\boldsymbol{\msgk}$.} 
% Let $\msg \in \mathcal{M}^{N-1}$ denote a set of messages received by the agent with cardinality $N-1$. For any $1 \leq k \leq N-1$, define a $k$ message sample (or k-sample for short) $\msgk \in \mathcal{M}^k$ as a set of $k$ messages randomly sampled from $\msg$. \\
% \textbf{(2) All k-sample Combinations $\boldsymbol{\allmsgk}$.} 
% Among all $N-1$ messages in $\msg$, there are $\binom{N-1}{k}$ unique k-samples. Let $\allmsgk$ be the collection of all unique k-samples of $\msg$.

% Moreover, the benign messages sent from other agents usually contain redundant/overlapping information.
% \myst{, as the goal of communication is to provide the agent additional information and to help the agent make better decisions. }
Motivated by the fact that the benign messages sent from other agents usually contain overlapping information that may suggest similar decisions, the \textbf{main idea} of our defense is to make decisions based on the \emph{consensus} of the benign messages. 
To be more specific, we train a base policy that makes decisions with one \ksample at each step. During test time when communication messages can be perturbed, the agent collects multiple \ksamples at every step, and applies the trained base policy to each \ksample to get multiple resulting base actions. Then, the agent selects the action that reflects the majority opinion. By carefully designed ablation and ensemble strategies, we can ensure that the majority of these base actions is dominated by benign messages.
% , even if there exist $C$ adversarial messages.

% By a careful design of , the agent is guaranteed to make a ``good'' decision if it takes a collection of wisdom from the ensemble of all resulting actions, since the majority of these resulting actions are guaranteed to be dominated by benign messages.
% For a message set $\msg$, our proposed \ours 

% where a base policy is trained in a clean environment to act according under a random \ksample, and the testing/defending phase where the communications may be perturbed, uses the trained base policy by aggregating multiple \ksamples.



% % and the set has $N-1$ elements, each is a message received. 
% Our defense makes decisions based on multiple random subsets of this message set, called \emph{randomly-ablated message samples} (or \textit{m-samples} for short).
% Under a carefully designed ablation mechanism, benign m-samples can outweigh malicious ones.
% To be more specific, we train a \emph{base policy} that makes decisions with one 
% % \myst{randomly selected subset of the message set} 
% m-sample at each step. 
% Note that agents are trained without any attacks, such that the base policy learns to behave under purely-benign m-samples.
% Then, during test-time where communication messages can be perturbed, the agent generates multiple m-samples at every step.
% % One can design an ablation strategy which guarantees that a majority number of these m-samples contain no malicious messages.
% Then the agent applies the trained base policy to  
% % \myst{randomly ablated messages, and aggregate the base-policy actions by sampling multiple message combinations, so that the agent can make safe decisions with theoretical guarantees.}
% each of these m-samples, getting multiple resulting actions where the majority of them are generated based on benign messages only. 
% % The majority of these resulting actions are based on benign messages only and thus safe. 
% Therefore, the agent is guaranteed to make a ``good'' decision if it takes a collection of wisdom from the ensemble of all resulting actions, since the majority of these resulting actions are guaranteed to be dominated by benign messages.
% \myst{guided by} benign \myst{messages}.


% A similar randomized ablation defense is used to defend against $\ell_0$ attacks in image classification~\cite{Levine_Feizi_2020}. 
% But our defensive mechanism is fundamentally different from the image classification defense~\cite{Levine_Feizi_2020} which provides a high-probability guarantee for discrete image label outputs, as our defense achieves both action and long-term reward certification (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output, which is non-trivial.


With the above intuition, we propose \oursfull (\ours), a generic defense framework that can be fused with any policy learning algorithm. 
% We first introduce some important notations for the algorithm.
% shown in Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test}, respectively, in Appendix~\ref{app:algo}. 
\ours has two phases: the training phase where agents are trained in a clean environment, and a testing/defending phase where communications may be perturbed. 
The training and defending strategies of \ours are illustrated below, and the pseudocode is shown by Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test} in Appendix~\ref{app:algo}.

\textbf{Training Phase with \ablnamecap $\boldsymbol\ablpolicy$ (Algorithm~\ref{alg:train})}\quad
During training time, the agent learns a \textit{\ablname} $\ablpolicy: \hisspace \times \mathcal{M}^k \to \mathcal{A}$ which maps its own interaction history $\his$ and a random \ksample $\msgk\sim \mathrm{Uniform}(\allmsgk)$ to an action, where $\mathrm{Uniform}(\allmsgk)$ is the uniform distribution over all \ksamples from the message set $\msg$ it receives.
% i.e., $a\step \sim \ablpolicy(\his\step,\msgk\step)$.
% $a\sim\ablpolicy(\his, \mathsf{Ablate}(\msg, T))$, where $T\in\mathcal{H}(N-1,k)$.
Here $k$ is a user-specified hyperparameter selected to satisfy certain conditions, as discussed in Section~\ref{sec:algo_theory}. 
The training objective is to maximize the cumulative reward of $\ablpolicy$ based on randomly sampled \ksamples in a non-adversarial environment. Any policy optimization algorithm can be used for training.
% Since all messages lie in the same message space $\mathcal{M}$, each agent only needs to learn a single ablation policy.
% which achieves as high reward as possible based on randomly sampled $k$ messages. 

% \fhc{Section 4.2 doesn't explain this specific hyperparameter.}
% Equation~\eqref{eq:k_cond} plays an important role in our robustness guarantees shown in Section~\ref{sec:algo_theory}.
% % Note that attacks do not exist during training.
% In every step, an agent randomly samples $k$ out of $N-1$ benign communication messages, and uses its current acting policy $\ablpolicy$ to take an action based on its observation history and the selected $k$ messages.
% react to its current observation and the selected $k$ messages (Line 7 in Algorithm~\ref{alg:train}). 
% Therefore, we optimize and make decisions via $\ablpolicy(\his, \mathsf{Ablate}(\msg, T))$, where $\mathsf{Ablate}(\msg, T)$ denotes the selected $k$ messages sent from other agents to agent $i$. 



\textbf{Defending Phase with \ensnamecap $\boldsymbol\smpolicy$ (Algorithm~\ref{alg:test})}\quad
Once we obtain a reasonable \ablname $\ablpolicy$, we can execute it with ablation and aggregation during test time to defend against adversarial communication. 
The main idea is to collect all possible \ksamples from $\allmsgk$, and select an action suggested by the majority of those \ksamples. 
Specifically, we construct a \textit{\ensname} $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$ that outputs an action by aggregating the base actions produced by $\ablpolicy$ on multiple \ksamples (Line 5 in Algorithm~\ref{alg:test}). 
The construction of the \ensname depends on whether the agent's action space $\mathcal{A}$ is discrete or continuous, which is given below by Definition~\ref{def:ensemble_dist} and Definition~\ref{def:ensemble_cont}, respectively. 
% For notation simplicity, the definitions only focus on one agent (although our defense works for multiple agents) and omit the subscript $i$. We further use $\mathbf{m}$ to denote the message list $\mtoi$ received by the current agent at the current step. 
% The \ensname $\smpolicy_i$ depends on whether the action space $\mathcal{A}_i$ is discrete or continuous, 
% which will be detailed in Section~\ref{sec:algo_dist} and Section~\ref{sec:algo_cont}, with corresponding theoretical guarantees on actions and rewards.
% \textcolor{purple}{PH: would it help mentioning $\smpolicy_i: \mathcal{O}_i \times \mathcal{M}^{N-1} \to \mathcal{A}_i$?}

% \fhc{Shall we put the test algorithm back?}

\begin{definition}[\ensnamecap for Discrete Action Space]
\label{def:ensemble_dist}
For a \ablname $\ablpolicy$ with observation history $\his$ and received message set $\msg$, define the \ensname $\smpolicy$ as
\begin{equation}
\label{eq:ensemble_pi_dist}
    \smpolicy(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)=a].
\end{equation}
\end{definition}

% \begin{definition}[\textbf{\ensnamecap for Discrete Actions}]
% \label{def:ensemble_dist}
% For a \ablname $\ablpolicy$ with observation history $\his$, define $u_a$ as the number of times/votes such that the \ablname $\ablpolicy$ renders action $a$ when taking each of \ksamples in $\allmsgk$, i.e.,
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:vote}
%     u_a := \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)].
%     % u_a := \sum\nolimits_{T\in\mathcal{H}(N-1,k)} \mathbbm{1}[\ablpolicy(\his, \funabl(\mathbf{m}, T))=a].
% \end{equation}
% Then the \ensname $\smpolicy$ takes the action with the most votes, i.e.,
% \begin{equation}
% \label{eq:ensemble_pi_dist}
%     \smpolicy(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \; u_a
% \end{equation}
% % \fh{How about $\tilde{a} = \smpolicy\Big(o, \{\funabl(\mathbf{m}, T_d)\}_{d=1}^D\Big) := \mathrm{ argmax}_{a\in\mathcal{A}} \; u_a.$?}
% \end{definition}

\begin{definition}[\ensnamecap for Continuous Action Space]
\label{def:ensemble_cont}
For a \ablname $\ablpolicy$ with observation history $\his$ and received message set $\msg$, define the \ensname $\smpolicy$ as
\begin{equation}
\label{eq:ensemble_pi_cont}
    \tilde{\pi}(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \msgk): \msgk\in\allmsgk \},
    % \tilde{\pi}(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \funabl(\mathbf{m}, T): T\in\mathcal{H}(N-1,k) \},
\end{equation}
where $\funmed$ is a function that returns the element-wise median value of a set of vectors.
\end{definition}

% Recall that there are up to $C$ malicious messages out of $N-1$ total messages, and at least $N-1-C$ benign messages. 
Therefore, the \ensname $\smpolicy$ takes the action suggested by the consensus of all \ksamples (majority vote in a discrete action space, and median action for a continuous action space). We will show in the next section that, with some mild conditions, 
% the performance of $\smpolicy$ under adversarial communications is certifiable. 
$\smpolicy$ under adversarial communications works similarly as the \ablname $\ablpolicy$ under all-benign communications.
% , with mild assumptions \fhc{note}.

\textbf{Computation Complexity of \ours}\quad
Different from many model-ensemble methods~\cite{kurutach2018modelensemble,harutyunyan2014shaping} that learn multiple network models, \emph{we learn a single policy $\ablpolicy$ during training, and use a single policy $\smpolicy$ during testing.}
Therefore, the training process does not require extra computations compared to the original policy learning method.
In the defending phase, we aggregate decisions from $\binom{N-1}{k}$ \ksamples, which require $\binom{N-1}{k}$ forward passes through $\ablpolicy$. 
Note that $\binom{N-1}{k}$ is generally small, because the number of agents in practical multi-agent problems is usually small (e.g., the number of drones in an area). 
For example, when $N=10,k=2$, $\binom{N-1}{k}=36$.
In the case where $\binom{N-1}{k}$ is large, we provide a variant of the algorithm in Section~\ref{sec:algo_more}, which takes $D$ \ksamples for $D\leq\binom{N-1}{k}$.
Then the certificate of \ours becomes a high-probability guarantee, depending on the value of $D$.
% The defense objective is to make a \textit{\myst{safe} \fh{benign} decision} that is robust to malicious massages. 


% Note that the ensemble policy $\smpolicy$ takes the action suggested by the consensus of all size-$k$ message subsets (majority vote in a discrete action space, and median action for a continuous action space). 
% There are $\binom{N-1}{k}$ number of such size-$k$ subsets in total. In many practical multi-agent problems, $N$ is not very large, e.g., the number of drones in an area. Therefore, $\binom{N-1}{k}$ is relatively small and not expensive to compute. For example, when $N=10,k=2$, $\binom{N-1}{k}=36$.
% In the case where $\binom{N-1}{k}$ is large, we also provide a variant of the algorithm which takes $D<\binom{N-1}{k}$ samples of message subsets whose certification guarantee is provided in Section~\ref{sec:algo_more}.

\subsection{Robustness Certificates of \ours}
\label{sec:algo_theory}


% Our defense lets an agent make decisions based on multiple size-$k$ random subsets of all messages in $\mathbf{m}$. 
In this section, we provide theoretical guarantees for the robustness of \ours.
During test time, at any step, let $\his$ be the interaction history, $\goodmsg$ be the unperturbed benign message set, and $\advmsg$ be the perturbed message set. 
% $\goodmsg$ be the benign messages (before attack), and $\advmsg$ be the messages after attack (with up to $C$ messages being corrupted). 
Note that $\goodmsg$ and $\advmsg$ both have $N-1$ messages while they differ by up to $C$ messages. 
With the above notation, we define a set of actions rendered by purely benign \ksamples in Definition~\ref{def:safeact_dist}. As the agent using a well-trained \ablname is likely to take these actions in a non-adversarial environment, they can be regarded as ``good'' actions to take. 

\begin{definition}[Benign Action Set $\safeaction$]
\label{def:safeact_dist}
For the execution of the \ablname $\ablpolicy$ at any step, define $\safeaction \subseteq \mathcal{A}$ as a set of actions that $\ablpolicy$ may select under benign \ksamples.
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
\label{eq:safeact_dist}
    \safeaction := \cup_{\goodmsgk\in\goodallmsgk} \left\{\ablpolicy(\his, \goodmsgk) \right\}.
    %  \safeaction := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
\end{equation}
\end{definition}

% Since there are at most $C$ adversarial messages among the $N-1$ messages in $\advmsg$, we know that there are at least $\binom{N-1-C}{k}$ purely benign \ksamples in $\advallmsgk$. 
% For notation simplicity, let $n_1=\binom{N-1}{k}$ and $n_2=\binom{N-1-C}{k}$. That is, $n_1$ is the total number of \ksamples, while $n_2$ is the number of purely benign \ksamples. 
% In this section, we analyze the robustness guarantees of the proposed defense \ours. 
Next, we characterize a condition for the ablation size $k$, the extra hyperparameter introduced by \ours, which is important for our theoretical certificates to hold.
\begin{condition}[Dominating Benign Sample]
\label{cond:k}
The ablation size $k$ of \ours satisfies
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
    \label{eq:k_cond}
    \binom{N-1-C}{k} > \frac{1}{2} \binom{N-1}{k}.
\end{equation}
\end{condition}
\vspace{-0.5em}

\textbf{Remarks.}
(1) For the message set $\advmsg$ that has up to $C$ adversarial messages, Equation~\eqref{eq:k_cond} implies that among all \ksamples from $\advmsg$, there are more purely benign \ksamples than \ksamples that contain adversarial messages. 
(2) Under Assumption~\ref{assum:num}, this condition \textit{always has solutions }for $k$ as $C<\frac{N-1}{2}$, and $k=1$ is always a feasible solution. 
% (3) In practice, the value of $k$ is related to the trade-off between natural performance and robustness, as discussed in details in Section~\ref{sec:exp}.
% Condition~\ref{cond:k} is important for the 

In addition, for a discrete action space, the \ablname takes the action with the most votes from all \ksamples as suggested by Equation~\eqref{eq:ensemble_pi_dist}. To ensure that this action stands for the consensus of benign messages, the following condition is needed.

\begin{condition}[Confident Consensus (for discrete-action only)]
\label{cond:cons}
The highest number of votes among all actions $u_{\max}:=\max_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)=a]$ satisfies
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{0pt}
\begin{equation}
    \label{eq:u_cond}
    u_{\max} > {\small{\binom{N-1}{k} - \binom{N-1-C}{k}}} =: u_{\mathrm{adv}},
\end{equation}
where $u_{\mathrm{adv}}$ is the number of votes that adversarial messages may affect (number of \ksamples that contain at least one adversarial message). 
\end{condition}

\textbf{Remarks}.
(1) This condition ensures the consensus has more votes than the votes that adversarial messages are involved in. Therefore, when $\smpolicy$ takes an action, there must exist some purely-benign \ksamples voting for this action. 
(2) This condition is easy to satisfy when $C \ll N$ as $\binom{N-1}{k} \approx \binom{N-1-C}{k}$. 
(3) This condition can be easily checked at every step of execution. 

Condition~\ref{cond:cons} considers the worst-case scenario when the adversarial messages collaborate to vote for a malicious action and outweigh benign messages in all \ksamples. 
However, such a worst-case attack is uncommon in practice as attackers are usually not omniscient. Therefore, Condition~\ref{cond:cons} is sufficient but not necessary for the robustness of $\smpolicy$ during execution. 
In real-world problems, our algorithm achieves strong robustness without requiring this condition, as verified in experiments. 


We now provide both action and reward certificates for the ensemble policy $\smpolicy$ in the discrete-action case. The analysis for a continuous action space is provided in Appendix~\ref{app:theory_cont}.

\textbf{Action Certificate for Discrete Action Space}\quad
The following theorem suggests that the ensemble policy $\smpolicy$ always takes benign actions under the above conditions no matter whether attacks exist.
\begin{theorem}[Action Certificate for Discrete Action Space]
\label{thm:main_dist}
When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold, the ensemble policy $\smpolicy$ in Definition~\ref{def:ensemble_dist} produces benign actions under $\advmsg$, i.e.,
\begin{equation}
    \widetilde{a} = \smpolicy(\his, \advmsg) \in \safeaction.
    \label{eq:cert_dist}
\end{equation}
% if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% where 
% \begin{equation}
%     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% \end{equation}
\end{theorem}
\vspace{-0.5em}

Under Condition~\ref{cond:k} and Condition~\ref{cond:cons} which are easy to check, Theorem~\ref{thm:main_dist} certifies that $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a benign action that is suggested by some benign message combinations, even when the malicious messages are not identified. 
Then, we can further derive a reward certificate as introduced below. 
% Note that a high-probability robustness guarantee~\cite{Levine_Feizi_2020} does not 

  
\textbf{Reward Certificate for Discrete Action Space}\quad
When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold, the \ensname $\smpolicy$'s action in every step falls into a benign action set, and thus \emph{its cumulative reward under adversarial communications is also guaranteed to be no lower than the worst natural reward the base policy $\ablpolicy$ can get under random benign message subsets.} Therefore, adversarial communication under Assumption~\ref{assum:num} cannot drop the reward of any agent trained with \ours. The formal reward certificate is shown in Corollary~\ref{cor:reward_dist} in Appendix~\ref{app:theory_dist}. 


\textbf{How to Select Ablation Size $k$: Trade-off between Performance and Robustness}\quad
The ablation size $k$ is an important hyperparameter for the guarantees to hold. For a fixed $C$, both Condition~\ref{cond:k} and Condition~\ref{cond:cons} prefer a relatively small $k$ as detailed in Appendix~\ref{app:hyper}. That is, a smaller $k$ can improve the robustness in general. Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
% Condition~\ref{cond:cons} is easier to be satisfied for a smaller $k$, because $u_{\mathrm{adv}}$ increases as $k$ (verified in Appendix~\ref{app:hyper}). 
However, we also point out that a smaller $k$ restricts the power of information sharing, as the \ablname can access fewer messages in one step. Therefore, the value of $k$ is related to the \emph{trade-off between robustness and natural performance}~\cite{tsipras2018robustness,zhang2019theoretically}. 
In experiments, we use \textit{the largest $k$ satisfying Equation~\eqref{eq:k_cond}}. 
In practice, one can also train several \ablnames with different $k$'s during training, and later adaptively select a \ablname to construct a \ensname during execution (decrease $k$ if higher robustness is needed). 
% Section~\ref{sec:exp} shows ablation experiments of $k$.

% % As pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}, there exists a \textit{trade-off between robustness and accuracy}. 
% Intuitively, the more an agent trusts communications from others, the more it may benefit from additional information, but it is more exposed to the risk of being attacked. Therefore, there exists a \textit{trade-off between robustness and accuracy}~\cite{tsipras2018robustness,zhang2019theoretically}. 
% We find that the ablation size $k$ directly controls such a trade-off: when $k$ is small, the \ensname is more robust since there are much more purely-benign \ksamples than adversarial \ksamples. However, the trained \ablname may not obtain a high reward with $k$ messages.
% % In general, if $k$ is smaller, the ensemble policy is more robust. However, the base ablation policy with a smaller $k$ could gain lower reward as it throws away many messages. Therefore, there is a \textit{trade-off between robustness and accuracy}, as is pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}. 
% Therefore, we can adjust $k$ based on our practical needs.
% If we know $C$ (or an upper bound of $C$), we can set $k$ to be the largest integer satisfying Condition~\ref{cond:k} such that the natural performance is not compromised much. 
% If $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Condition~\ref{cond:k}.
% % which shows how many adversarial messages the policy can tolerate. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Condition~\ref{cond:k}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
% Experiments in Section~\ref{sec:exp} verifies our claim by an ablation study of $k$.

% and when $C$ is small, we can use a larger $k$ such that the natural performance is not compromised much. 


\vspace{-0.5em}
\subsection{Extensions of \ours}
\label{sec:algo_more}

% In this section, we discuss the effects of hyperparameter $k$, the broader applications of \ours, and an extensions of \ours for scaling up to a large number of agents.

% \textbf{Discussion on Ablation Size $\boldsymbol k$}\quad 
% As an essential condition for the certificates in Section~\ref{sec:algo_theory} to hold, Equation~\eqref{eq:k_cond} implies that among all size-$k$ message subsets, there are more purely benign subsets than subsets that contain adversarial messages. This condition \textit{always has solutions }for $k$ as $C<\frac{N-1}{2}$, and $k=1$ is always a feasible solution. In general, if $k$ is smaller, the ensemble policy is more robust. However, the base ablation policy with a smaller $k$ could gain lower reward as it throws away many messages. Therefore, there is a \textit{trade-off between robustness and accuracy}, as is pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}.
% In practice, if we know $C$ in advance, we can set $k$ to be the largest integer satisfying Equation~\eqref{eq:k_cond}. On the other hand, if $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Equation~\eqref{eq:k_cond}, which shows how many adversarial messages the policy can tolerate. 
% % For example, when $N=10$, \ours can tolerate up to $C=4$ with $k=1$, and up to $C=2$ with $k=2$. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Equation~\eqref{eq:k_cond}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages, and when $C$ is small, we can use a larger $k$ such that the natural performance is not compromised much. 



\textbf{Scaling Up: Ensemble with Partial Samples}\quad
So far we have discussed the proposed \ours defense and the constructed ensemble policy that aggregates all $\binom{N-1}{k}$ number of \ksamples out of $N-1$ messages. 
However, if $N$ is large, sampling all $\binom{N-1}{k}$ combinations of message subsets could be expensive. In this case, a smaller number of \ksamples can be used. That is, given a sample size $0<D\leq\binom{N-1}{k}$, we randomly select $D$ number of \ksamples from $\allmsgk$ (without replacement), and then we aggregate the \ablname's decisions on selected \ksamples. 
In this way, we define a partial-sample version of the ensemble policy, namely \textit{$D$-ensemble policy} $\smpolicy_D$, whose formal definition is provided in Appendix~\ref{app:theory_sample}. In this case, the robustness guarantee holds with high probability that increases as $D$ gets larger, as detailed in Theorem~\ref{thm:sample_cont} in Appendix~\ref{app:theory_sample}. 
Decreasing the hyperparameter $D$ trades some robustness guarantee for higher computational efficiency.
In our experiments, we empirically show that \ours usually works well even for a small $D$ (e.g. $D=1$).


\textbf{More Applications of \ours}\quad
The central idea of \ours is to make decisions based on the consensus instead of each individual.
Therefore, \ours can be combined with any decision-making model to work with possibly-untrustworthy information sources, not only restricted to communication attacks in CMARL. 
For example, when one collects data from multiple sources (e.g., different websites, multiple questionnaires, etc.) and some sources may contain malicious information, \ours can be used to make decisions based on the collected statistics without being significantly misled by false data.
Moreover, the idea of \ours can also be extended to detect attackers, by measuring the difference between the action suggested by any specific communication message and the ensemble policy's action, as detailed and empirically verified in Appendix~\ref{app:exp_detect}. 












% formulated as below.
% , whose detailed definition is provided in Appendix~\ref{app:theory_sample}.
% define the $D$-ensemble policy $\smpolicy_D$ as the sampled version of $\smpolicy$
% \begin{equation}
% \label{eq:ensemble_pi_dist_d}
%     \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
% \end{equation}
% for a discrete action space, and
% \begin{equation}
% \label{eq:ensemble_pi_cont_d}
%     \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% for a continuous action space. 


% \subsection{Extension of \ours: Ensemble with Partial Samples}
% \label{sec:algo_partial}

% So far we have discussed the proposed \ours algorithm and the constructed ensemble policy that aggregates all $\binom{N-1}{k}$ number of message subsets out of $N-1$ messages. 
% However, if $N$ is large, sampling all $\binom{N-1}{k}$ combinations of message subsets could be expensive. In this case, a smaller number of message-subset combinations can be used. That is, given a sample size $0<D\leq\binom{N-1}{k}$, we randomly select $D$ samples $\{T_d\}_{d=1}^D$ from $\mathcal{H}(N-1,k)$ (without replacement), and then we aggregate the ablation policy's decision on $\{\funabl(\mathbf{m}, T_d)\}_{d=1}^D$. 
% In this way, we define a sampled version of the ensemble policy, namely \textit{$D$-ensemble policy} $\smpolicy_D$, formulated as below.
% % , whose detailed definition is provided in Appendix~\ref{app:theory_sample}.
% % define the $D$-ensemble policy $\smpolicy_D$ as the sampled version of $\smpolicy$
% \begin{equation}
% \label{eq:ensemble_pi_dist_d}
%     \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
% \end{equation}
% for a discrete action space, and
% \begin{equation}
% \label{eq:ensemble_pi_cont_d}
%     \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% for a continuous action space. 



% In this case, we can still provide a high-probability robustness guarantee. Theorem~\ref{thm:sample_cont} shows the theoretical result for a continuous action space, while the result for a discrete action space is slightly different and is provided in Appendix~\ref{app:theory_sample}.
% % in Theorem~\ref{thm:sample_dist} and Theorem~\ref{thm:sample_cont}. 

% \begin{theorem}[General Action Guarantee for Continuous Action Space]
% \label{thm:sample_cont}
% Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$,  under Assumption~\ref{assum:num}, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_cont_d} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, relation~\eqref{eq:cert_cont} holds with probability at least
% \begin{equation}
% \label{eq:p_sample_cont}
%     p_D=\frac{\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n_1-n_2}{D-j}}{\binom{n_1}{D}},
% \end{equation}
% where $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$ and $\tilde{D} = {\lfloor \frac{D}{2} \rfloor}+1$. 
% \end{theorem}
% Therefore, for an arbitrary $D$, a benign action will be selected with high probability. The larger $D$ is, the higher the probability is. 
% In Theorem~\ref{thm:sample_cont}, when $D=\binom{N-1}{k}$,  the probability $p_D$ is 1 and the result matches Theorem~\ref{thm:main_cont}. 
% Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.


% \subsection{More Discussion on Applicability and Flexibility of \ours}

% \ys{general for any RL policy or decision-making model}

% \ys{how a policy is trained}



% \ys{training and testing hyperparameters}



==> cmarl/neurips/5_exp.tex <==
\vspace{-0.5em}
\section{Empirical Study}
\label{sec:exp}

\input{\texhome/figs_all}

In this section, we verify the robustness of our \ours in multiple different CMARL environments against various communication attack algorithms. % and evaluate the hyperparameters by ablation study.
Then, we conduct hyperparameter tests for the ablation size $k$ and the sample size $D$ (for the variant of \ours introduced in Section~\ref{sec:algo_more}).




\textbf{Environments}\quad 
To evaluate the effectiveness of \ours, we consider the following environments.\\
$\bullet$ \textit{FoodCollector}: a 2D particle environment adapted from the WaterWorld task in PettingZoo~\cite{terry2020pettingzoo}. In our experiment, there are $N=9$ agents with different colors searching for foods with the same colors. Agents use their limited-range sensors to observe the surrounding objects, while communicating with each other to share their observations. The action space can be either discrete (9 moving directions and 1 no-move action), or continuous (2-dimensional vector denoting acceleration). Agents are penalized for having leftover foods at every step, so they seek to find all foods as fast as possible. \\
$\bullet$ \textit{\marketenv}: simulating a real-world inventory management problem. 
$N=10$ cooperative distributor agents carry inventory for 3 products. There are 300 buyers sharing an underlying demand distribution.
At every step, each buyer requests products from a randomly selected distributor. 
% At every step, each distributor observes random demand requests from a population of buyers, according to an underlying demand distribution. 
Then, each distributor agent observes random demand requests, takes restocking actions (continuous) to adjust its own inventory, and communicates with others by sending its demand observations.
% there are $300$ buyers requesting each product from a randomly selected distributor according to a demand distribution. 
Distributors are penalized for mismatches between their inventory and the demands. \\
% Distributors can take restocking actions (continuous) to adjust their inventory at every step, and communicate with each other by exchanging their own demand observations. \\
% \fh{$\bullet$ \textit{MNIST}:} \fh{An MARL classification task in MNIST from \cite{mousavi2019multi} is also used to verify the performance of \ours for image observations.}\\
% an MARL classification task in the MNIST dataset, which is proposed by Mousavi et al.~\cite{mousavi2019multi}
% $\bullet$ \textit{MNIST-Classification}: an MARL classification framework in the MNIST dataset, proposed by Mousavi et al.~\cite{mousavi2019multi}. $N=9$ agents aim to classify an image within a limited time horizon. At every step, each agent observes a patch of the image, and can take an action to move to an adjacent patch. In the meanwhile, agents are allowed to exchange information (encoded local beliefs) with other agents to update their own beliefs. \\
The detailed description of each environment is in Appendix~\ref{app:exp_env}, where we empirically show that agents benefit a lot from communication in these environments.
Since our focus is to defend against adversarial communication over any communication policy, we let the benign agents communicate via fixed protocols detailed in Appendix~\ref{app:exp_env}. But our method also works for learned communications, as verified by additional experiments on an \textit{MARL image classification task} in Appendix~\ref{app:exp_mnist}.
% Therefore, different from the hand-coded communication protocols used in FoodCollector and MarketEnv, agents in this MNIST classification task use learned communication.




\textbf{Implementation and Baselines}\quad
As discussed in Section~\ref{sec:algo}, our \ours is designed to defend against communication attacks, and can be fused with any policy learning algorithm. 
In FoodCollector and \marketenv, we use PPO~\cite{schulman2017proximal} with parameter sharing~\cite{terry2020parameter} as the base policy learning algorithm as it achieves relatively high natural performance. But our \ours can be applied to other MARL algorithms, such as QMIX~\cite{rashid2018qmix} that is evaluated in Appendix~\ref{app:exp_results}.
% But other more advanced MARL algorithms can be used  
% (see Appendix~\ref{app:exp_results} for results of QMIX~\cite{rashid2018qmix}).
With the same policy learning method, we compare our \ours with two defense baselines: 
(1) \textbf{(Vanilla)}: vanilla training without defense, which learns a policy based on all benign messages. 
(2) \textbf{(AT)} adversarial training as in~\cite{zhang2021robust}, which alternately trains an adaptive RL attacker and an agent. 
% As is common in related work~\cite{lowe2017multi,gupta2017cooperative}, we use parameter sharing and train a shared policy network for all agents.
% Due to the symmetricity of the agents, we train \ours and baselines using PPO~\cite{schulman2017proximal} with parameter sharing~\cite{terry2020parameter}. 
% For MNIST-Classification, our implementation is based on \cite{mnistgithub} that reproduces the results of~\cite{mousavi2019multi}. 
During training and defending, we set the ablation size \ours as $k=2$, the largest solution to Equation~\eqref{eq:k_cond} for $C=2$ when $N=9$ (FoodCollector) or $N=10$ (\marketenv). For AT, we train the agent against $C=2$ learned adversaries. 
More implementation details are provided in Appendix~\ref{app:exp_imple}.

\textbf{Evaluation Metrics}\quad
To evaluate the effectiveness of our defense strategy, we test the performance of the trained policies under no attack and under various values of $C$ (for simplicity, we refer to $C$ as the \textit{number of adversaries}). 
Different from previous work~\cite{blumenkamp2020emergence} where the adversarial agent disrupts all the other agents, we consider the case where the attacker deliberately misleads a selected victim, which could evaluate the robustness of the victim under the harshest attacks. We report the victim's local reward under the following two types of attack methods: 
(1) \textit{Non-adaptive attack} that perturbs messages based on heuristics. In FoodCollector, we consider randomly generated messages within the valid range of communication messages. Note that this is already a strong attack since a randomly generated message could be arbitrary and far from the original benign message. For \marketenv where messages have clear physical meanings (demand of buyers), we consider 3 realistic attacks: \permute, \swap, \flip, which permute, swap or flip the demand observations, respectively, as detailed in Appendix~\ref{app:exp_imple:market}. 
(2) \textit{Learned adaptive attack} that learns the strongest/worst adversarial communication with an RL algorithm to minimize the victim's reward (a white-box attacker which knows the victim's reward). The learned attack can strategically mislead the victim.
As shown in prior works~\cite{zhang2020robust,zhang2021robust,sun2021strongest}, the theoretically optimal attack (which minimizes the victim's reward) can be formed as an RL problem and learned by RL algorithms. 
Therefore, we can regard this attack as a worst-case attack for the victim agents.
% Therefore, we train an RL attacker policy that maps adversarial agent's observations to adversarial communications. 
More details are in Appendix~\ref{app:exp_imple}.





\textbf{Experiment Results}\quad
The results are shown in Figure~\ref{fig:res_all}. 
We can see that the rewards of Vanilla and AT drastically drop under attacks. Under strong adaptive attackers, Vanilla and AT sometimes perform worse than a non-communicative agent shown by dashed red lines, which suggests that communication can be a double-edged sword. Although AT is usually effective for $\ell_p$ attacks~\cite{zhang2021robust}, we find that AT does not achieve better robustness than Vanilla, since it can not adapt to arbitrary perturbations to several messages.
% because the strong attacker we consider can arbitrarily perturb a subset of messages. 
(More analysis of AT is in Appendix~\ref{app:exp_imple}.)
In contrast, \textit{\ours can utilize benign communication well while being robust to adversarial communication. }
We use $k=2$ for our \ours, which in theory provides performance guarantees against up to $C=2$ adversaries for $N=9$ and $N=10$. 
We can see that the reward of \ours under $C=1$ or $C=2$ is similar to its reward under no attack, matching our theoretical analysis. 
Even under 3 adversaries where the theoretical guarantees no longer hold, \ours still obtains superior performance compared to Vanilla and AT.
Therefore, \textit{\ours makes agents robust under varying numbers of adversaries.} 
% Moreover, we find that AT does not achieve better robustness than Vanilla, although AT is usually effective for $\ell_p$ attacks~\cite{zhang2021robust}. One possible reason is that the message perturbation is relatively large, such that it is hard for AT to adapt to adversaries, as explained in Appendix~\ref{app:exp_imple}.

\begin{wrapfigure}{r}{0.3\textwidth}
\vspace{-1.5em}
\hspace{-1em}
 \centering
 \resizebox{0.26\columnwidth}{!}{\input{figs/mnist/MNIST_Adaptive_Attacker_Precision}}
 \vspace{-0.5em}
\caption{\textbf{(MARL-MNIST)}: Precision of MARL classification on MNIST without or with \ours, under learned adaptive attacks.}
\vspace{-1.5em}
\label{fig:res_mnist_sample}
\end{wrapfigure}

\textbf{Additional Results in MARL Image Classification}\quad
In addition to the above two environments, we also evaluate our proposed \ours defense in an MARL classification task in the MNIST dataset~\cite{lecun1998gradient}, which is proposed by Mousavi et al.~\cite{mousavi2019multi}. In this classification problem, every agent observes a local patch of an image and takes actions to move to adjacent patches. Agents are allowed to communicate their encoded local beliefs which are \textit{learned} by LSTM networks~\cite{hochreiter1997long}. Figure~\ref{fig:res_mnist_sample} shows the classification precision of \ours and baselines under adaptive attacks. We can see that the attacks significantly mislead Vanilla and AT, while \ours stays robust.
% Results show that the original policies are vulnerable to adversarial attacks ($17.3\%$ reward drop under strong adaptive attacks), and applying \ours to the policies significantly improves their robustness (less than $3\%$ reward drop under strong adaptive attacks). 
More details and results of this task are provided in Appendix~\ref{app:exp_mnist}.

% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-1em}
% \centering
%     \begin{subfigure}[t]{0.24\columnwidth}
%         \centering
%         \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_cont}}
%         \vspace{-1.5em}
%         \caption{\small{FoodCollector (Cont.)}}
%         % \label{sfig:maxq}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\columnwidth}
%         \centering
%         \resizebox{\textwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}}
%         \vspace{-1.5em}
%         \caption{\small{MarketEnv}}
%         % \label{sfig:maxq}
%     \end{subfigure}
%     \vspace{-0.5em}
%     \caption{\small{Hyperparameter test of ablation size $k$ in (a) continuous-action FoodCollector and (b) MarketEnv.}}
%     \label{fig:hyper_k}
% \vspace{-1em}
% \end{wrapfigure}


\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2em}
% \hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_dist}}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_sample_dist}}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Natural and robust performance of \ours with various values of \textbf{(left)} ablation size $k$ and \textbf{(right)} sample size $D$, in discrete-action FoodCollector under $C=2$. 
% \textbf{Left:}   with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. 
% Dashed green line refers to the robust performance of Vanilla under $C=2$ attacks.
}
\vspace{-1em}
\label{fig:res_k_dist}
\end{wrapfigure}



% \textbf{Ablation Size $k$: Balancing between Performance and Robustness}\quad
% As pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}, there exists a \textit{trade-off between robustness and accuracy}. 
% In a CMARL problem, the more an agent trusts communications from others, the more it may benefit from additional information, but it is exposed to the risk of being attacked. 
% We find that the ablation size $k$ directly controls such a trade-off: when $k$ is small, the \ensname is more robust since there are much more purely-benign messages than adversarial messages. However, the trained \ablname may not obtain a high reward with $k$ messages.
% Therefore, we can adjust $k$ based on our practical needs.
% If we know $C$ (or an upper bound of $C$), we can set $k$ to be the largest integer satisfying Condition~\ref{cond:k} such that the natural performance is not compromised much. 
% If $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Condition~\ref{cond:k}.
% % which shows how many adversarial messages the policy can tolerate. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Condition~\ref{cond:k}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
\textbf{Hyperparameter Tests for Ablation Size $\boldsymbol k$}\quad
% As discussed in Section~\ref{sec:algo_theory}, the ablation size $k$ controls the trade-off between natural performance and robustness. 
To see the empirical influence of $k$ on \ours, we evaluate \ours's natural reward and reward under $C=2$ attacks with different ablation sizes $k$. 
The result in discrete-action FoodCollector is shown in Figure~\ref{fig:res_k_dist}(left), while results in other environments are similar and are put in Appendix~\ref{app:exp_results}.
We observe that a larger $k$ leads to higher natural performance since each agent could gather more information from others. However, raising $k$ also increases the risk of making decisions based on communication messages sent from an adversary. 
Therefore, \textit{increasing ablation size $k$ trades off robustness for natural performance}, matching the analysis in Section~\ref{sec:algo_theory}.
Moreover, as the largest solution to Equation~\eqref{eq:k_cond} in Condition~\ref{cond:k}, ablation size $k=2$ achieves a good balance between performance and robustness. Even when $k>2$ which breaks Condition~\ref{cond:k}, \ours is still more robust than baselines.
% there exist a ``sweet spot'' (e.g., $k=2$), where the performance and robustness are well-balanced.

\textbf{Hyper-parameter Test for Sample Size $\boldsymbol D$}\quad
We further evaluate the partial-sample variant of \ours introduced in Section~\ref{sec:algo_more} using $k=2$ under $C=2$ adversaries, with $D$ varying from $N-1 \choose k$ (the largest sample size) to 1 (the smallest sample size). Figure~\ref{fig:res_k_dist}(right) demonstrate the performance of different $D$'s in discrete-action FoodCollector, and Appendix~\ref{app:exp_results} shows other results. 
As $D$ goes down, \ours obtains lower reward under attackers, but it is still significantly more robust than baseline methods. For example, \ours in FoodCollector obtains much higher reward than Vanilla under attacks even when $D=1$ (using only 1 random \ksample in the \ensname). 
% which is both computationally efficient and robust.






==> cmarl/neurips/5_exp_temp.tex <==
\vspace{-0.5em}
\section{Empirical Study}
\label{sec:exp}

\input{\texhome/figs_all}

In this section, we verify the robustness of our \ours in multiple different CMARL environments against various communication attack algorithms. % and evaluate the hyperparameters by ablation study.
Then, we conduct hyperparameter tests for the ablation size $k$ and the sample size $D$ (introduced in Section~\ref{sec:algo_more}).




\textbf{Environments}\quad 
To evaluate the effectiveness of \ours, we consider the following environments.\\
$\bullet$ \textit{FoodCollector}: a 2D particle environment adapted from the WaterWorld task in PettingZoo~\cite{terry2020pettingzoo}. In our experiment, there are $N=9$ agents with different colors searching for foods with the same colors. Agents use their limited-range sensors to observe the surrounding objects, while communicating with each other to share their observations. The action space can be either discrete (9 moving directions and 1 no-move action), or continuous (2-dimensional vector denoting acceleration). Agents are penalized for having leftover foods at every step, so they seek to find all foods as soon as possible. \\
$\bullet$ \textit{\marketenv}: a simulator of the real-world inventory management problem. There are $N=10$ cooperative distributors carrying inventory for $3$ products. Every of $300$ buyers requests each product from a randomly selected distributor agent according to a demand distribution. The distributor agents are penalized for mismatches between their inventory and the demand for each product. Distributors can take restocking actions (continuous) to adjust their inventory at every step, and communicate with each other by exchanging their own demand observations. \\
$\bullet$ \textit{MARL-MNIST}: an MARL image classification task proposed by Mousavi et al.~\cite{mousavi2019multi} in the MNIST dataset. $N=9$ agents aim to classify an image within a limited time horizon. At every step, each agent observes a patch of the image, and can take an action to move to an adjacent patch. Agents use learned communication policies to share their encoded local beliefs with each other.
% an MARL classification task in the MNIST dataset, which is proposed by Mousavi et al.~\cite{mousavi2019multi}
% $\bullet$ \textit{MNIST-Classification}: an MARL classification framework in the MNIST dataset, proposed by Mousavi et al.~\cite{mousavi2019multi}. $N=9$ agents aim to classify an image within a limited time horizon. At every step, each agent observes a patch of the image, and can take an action to move to an adjacent patch. In the meanwhile, agents are allowed to exchange information (encoded local beliefs) with other agents to update their own beliefs. \\
% Since our focus is to defend against adversarial communication over any communication policy, we let the benign agents communicate via fixed protocols detailed in Appendix~\ref{app:exp_env}. But our method also works for learned communications, as verified by additional experiments in Appendix~\ref{app:exp_mnist}. 
The detailed description of each environment is in Appendix~\ref{app:exp_env}, where we empirically show that agents benefit a lot from benign communications in these environments.
% Therefore, different from the hand-coded communication protocols used in FoodCollector and MarketEnv, agents in this MNIST classification task use learned communication.




\textbf{Implementation and Baselines}\quad
As discussed in Section~\ref{sec:algo}, our \ours is designed to defend against communication attacks, and can be fused with any policy learning algorithm. 
In FoodCollector and \marketenv, we use PPO~\cite{schulman2017proximal} with parameter sharing~\cite{terry2020parameter} as the base policy learning algorithm as it achieves relatively high natural performance. But other more advanced MARL algorithms can be used  
(see Appendix~\ref{app:exp_results} for results of QMIX~\cite{rashid2018qmix}). 
In \mnistenv, we use the LSTM policy architecture proposed by Mousavi et al~\cite{mousavi2019multi} following the existing implementation~\cite{mnistgithub}.
With the same policy learning method, we compare our \ours with two defense baselines: 
(1) \textbf{(Vanilla)}: vanilla training without defense, which learns a policy based on all benign messages. 
(2) \textbf{(AT)} adversarial training as in~\cite{zhang2021robust}, which alternatively trains an adaptive RL attacker and an agent. 
% As is common in related work~\cite{lowe2017multi,gupta2017cooperative}, we use parameter sharing and train a shared policy network for all agents.
% Due to the symmetricity of the agents, we train \ours and baselines using PPO~\cite{schulman2017proximal} with parameter sharing~\cite{terry2020parameter}. 
% For MNIST-Classification, our implementation is based on \cite{mnistgithub} that reproduces the results of~\cite{mousavi2019multi}. 
During training and defending, we set the ablation size \ours as $k=2$, as suggested by Equation~\eqref{eq:k_cond} for both $N=9$ (FoodCollector) and $N=10$ (\marketenv). For AT, we train the agent against $C=2$ learned adversaries. 
More implementation details are provided in Appendix~\ref{app:exp_imple}.

\textbf{Evaluation Metrics}\quad
To evaluate the effectiveness of our defense strategy, we test the performance of the trained policies under no attack and under various values of $C$ (for simplicity, we refer to $C$ as the \textit{number of adversaries}). 
Different from previous work~\cite{blumenkamp2020emergence} where the adversarial agent disrupts all the other agents, we consider the case where the attacker deliberately misleads a selected victim, which could evaluate the robustness of the victim under the harshest attacks. We report the victim's local reward under the following two types of attack methods: 
(1) \textit{Non-adaptive attack} that perturbs messages based on heuristics. In FoodCollector, we consider randomly generated messages within the valid range of communication messages. Note that this is already a strong attack since a randomly generated message could be arbitrary and far from the original benign message. For \marketenv where messages have clear physical meanings (demand of buyers), we consider 3 realistic attacks: \permute, \swap, \flip, which permute, swap or flip the demand observations, respectively, as detailed in Appendix~\ref{app:exp_imple:market}. 
(2) \textit{Learned adaptive attack} that learns the strongest/worst adversarial communication with an RL algorithm to minimize the victim's reward (a white-box attacker which knows the victim's reward). The learned attack can strategically mislead the victim.
As shown in prior works~\cite{zhang2020robust,zhang2021robust,sun2021strongest}, the theoretically optimal attack (which minimizes the victim's reward) can be formed as an RL problem and learned by RL algorithms. 
Therefore, we can regard this attack as a worst-case attack for the victim agents.
% Therefore, we train an RL attacker policy that maps adversarial agent's observations to adversarial communications. 
More details are in Appendix~\ref{app:exp_imple}.





\textbf{Experiment Results}\quad
The results are shown in Figure~\ref{fig:res_all}. 
We can see that the rewards of Vanilla and AT drastically drop under attacks. Under strong adaptive attackers, Vanilla and AT sometimes perform worse than a non-communicative agent shown by dashed red lines, which suggests that communication can be a double-edged sword. Although AT is usually effective for $\ell_p$ attacks~\cite{zhang2021robust}, we find that AT does not achieve better robustness than Vanilla, since it can not adapt to arbitrary perturbations to several messages.
% because the strong attacker we consider can arbitrarily perturb a subset of messages. 
(More analysis of AT is in Appendix~\ref{app:exp_imple}.)
In contrast, \textit{\ours can utilize benign communication well while being robust to adversarial communication. }
We use $k=2$ for our \ours, which in theory provides performance guarantees against up to $C=2$ adversaries for $N=9$ and $N=10$. 
We can see that the reward of \ours under $C=1$ or $C=2$ is similar to its reward under no attack, matching our theoretical analysis. 
Even under 3 adversaries where the theoretical guarantees no longer hold, \ours still obtains superior performance compared to Vanilla and AT.
Therefore, \textit{\ours makes agents robust under varying numbers of adversaries.} 
% Moreover, we find that AT does not achieve better robustness than Vanilla, although AT is usually effective for $\ell_p$ attacks~\cite{zhang2021robust}. One possible reason is that the message perturbation is relatively large, such that it is hard for AT to adapt to adversaries, as explained in Appendix~\ref{app:exp_imple}.

\begin{wrapfigure}{r}{0.3\textwidth}
\vspace{-1.5em}
\hspace{-1em}
 \centering
 \resizebox{0.28\columnwidth}{!}{\input{figs/mnist/MNIST_Adaptive_Attacker_Precision}}
 \vspace{-0.5em}
\caption{\textbf{(MARL-MNIST)}: Precision of MARL classification on MNIST without or with \ours, under learned adaptive attacks.}
\vspace{-1em}
\label{fig:res_mnist_sample}
\end{wrapfigure}

\textbf{Additional Results in MARL Image Classification}\quad
In addition to the above two environments, we also evaluate our proposed \ours defense in an MARL classification task in the MNIST dataset, which is proposed by Mousavi et al.~\cite{mousavi2019multi}. In this classification problem, every agent observes a local patch of an image and takes actions to move to adjacent patches. Agents are allowed to communicate with their encoded local beliefs which are \textit{learned} by LSTM networks~\cite{hochreiter1997long}. Figure~\ref{fig:res_mnist_sample} shows the classification precision of \ours and baselines under adaptive attacks. We can see that the attacks significantly mislead Vanilla and AT, while \ours stays robust.
% Results show that the original policies are vulnerable to adversarial attacks ($17.3\%$ reward drop under strong adaptive attacks), and applying \ours to the policies significantly improves their robustness (less than $3\%$ reward drop under strong adaptive attacks). 
More details and results of this task are provided in Appendix~\ref{app:exp_mnist}.

% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-1em}
% \centering
%     \begin{subfigure}[t]{0.24\columnwidth}
%         \centering
%         \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_cont}}
%         \vspace{-1.5em}
%         \caption{\small{FoodCollector (Cont.)}}
%         % \label{sfig:maxq}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\columnwidth}
%         \centering
%         \resizebox{\textwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}}
%         \vspace{-1.5em}
%         \caption{\small{MarketEnv}}
%         % \label{sfig:maxq}
%     \end{subfigure}
%     \vspace{-0.5em}
%     \caption{\small{Hyperparameter test of ablation size $k$ in (a) continuous-action FoodCollector and (b) MarketEnv.}}
%     \label{fig:hyper_k}
% \vspace{-1em}
% \end{wrapfigure}


\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2em}
% \hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_dist}}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_sample_dist}}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Natural and robust performance of \ours with various values of \textbf{(left)} ablation size $k$ and \textbf{(right)} sample size $D$ in discrete-action FoodCollector under $C=2$. 
% \textbf{Left:}   with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. 
% Dashed green line refers to the robust performance of Vanilla under $C=2$ attacks.
}
\vspace{-1em}
\label{fig:res_k_dist}
\end{wrapfigure}



% \textbf{Ablation Size $k$: Balancing between Performance and Robustness}\quad
% As pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}, there exists a \textit{trade-off between robustness and accuracy}. 
% In a CMARL problem, the more an agent trusts communications from others, the more it may benefit from additional information, but it is exposed to the risk of being attacked. 
% We find that the ablation size $k$ directly controls such a trade-off: when $k$ is small, the \ensname is more robust since there are much more purely-benign messages than adversarial messages. However, the trained \ablname may not obtain a high reward with $k$ messages.
% Therefore, we can adjust $k$ based on our practical needs.
% If we know $C$ (or an upper bound of $C$), we can set $k$ to be the largest integer satisfying Condition~\ref{cond:k} such that the natural performance is not compromised much. 
% If $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Condition~\ref{cond:k}.
% % which shows how many adversarial messages the policy can tolerate. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Condition~\ref{cond:k}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
\textbf{Hyperparameter Tests of Ablation Size $\boldsymbol k$}\quad
As discussed in Section~\ref{sec:algo_theory}, the ablation size $k$ controls the trade-off between natural performance and robustness. 
To see the empirical influence of $k$, we evaluate \ours's natural reward and reward under $C=2$ attacks with different ablation sizes $k$. 
The results in discrete-action FoodCollector is shown in Figure~\ref{fig:res_k_dist}(left), while results in other environments are similar and are put in Appendix~\ref{app:exp_results}.
We observe that a larger $k$ leads to higher natural performance since each agent could gather more information from others. However, raising $k$ also increases the risk of making decisions based on communication messages sent from an adversary. Therefore, \textit{increasing ablation size $k$ trades off robustness for natural performance.} On the other hand, $k=2$ as the largest solution to Equation~\eqref{eq:k_cond}, achieves a good balance between performance and robustness.
% there exist a ``sweet spot'' (e.g., $k=2$), where the performance and robustness are well-balanced.

\textbf{Hyper-parameter Test of Sample Size $\boldsymbol D$}\quad
We further evaluate the partial-sample variant of \ours introduced in Section~\ref{sec:algo_more} using $k=2$ under $C=2$ adversaries, with $D$ varying from $N-1 \choose k$ (the largest sample size) to 1 (the smallest sample size). Figure~\ref{fig:res_k_dist}(right) demonstrate the performance of different $D$'s in discrete-action FoodCollector, and Appendix~\ref{app:exp_results} shows other results. 
As $D$ goes down, \ours obtains lower reward under attackers, but it is still significantly more robust than baseline methods. For example, \ours in FoodCollector obtains much higher reward than Vanilla under attacks even when $D=1$ (using only 1 random \ksample). 
% which is both computationally efficient and robust.






==> cmarl/neurips/6_discuss.tex <==
\vspace{-0.5em}
\section{Conclusion}
\label{sec:discuss}
\vspace{-0.5em}

This paper formulates communication attacks in MARL problems, and proposes a defense framework \ours, which is certifiably robust against multiple arbitrarily perturbed adversarial communication messages, based on randomized ablation and aggregation of messages. 
\ours can easily scale up and extend to many real-world tasks. 
Environments verify the effectiveness of \ours in different tasks.
% \ys{flexibility of different $k$'s in training and test.}

==> cmarl/neurips/a1_related.tex <==
\section{Additional Related Work}
\label{app:related}

% \textbf{Adversarial Robustness of RL Agents}\quad
% As RL techniques have been applied to more and more applications, the robustness of agents under environment noise or adversarial attacks becomes an emerging research topic. 
% For a single-agent problem, there are many recent works on adversarial state perturbation~\cite{huang2017adversarial,zhang2020robust} and action perturbation~\cite{tan2020robustifying,tessler2019action}. In a multi-agent system, the interplay among agents introduces more uncertainty to the environment. \cite{gleave2020adversarial} point out that a well-trained agent can be completely misled by adversarial behaviors of another agent. Although adversarial training (i.e., introducing adversarial agents to the system during training~\cite{pinto2017robust,phan2021resilient}) can empirically improve agents' robustness, such robustness is not guaranteed to hold under all possible attackers.


% \textbf{Certifiable Defense}\quad
% There is an important line of work studying guaranteed robustness of neural networks~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness} while the input data is perturbed within an $\ell_p$ norm ball. In an effort to certify RL agents' robustness, \cite{lutjens2020certified} and \cite{oikarinen2020robust} utilize convex relaxation of Q networks to improve the worst-case performance of agents. \cite{kumar2021policy} and \cite{wu2021crop} follow the idea of randomized smoothing~\cite{cohen2019certified} and smooth out the policy by adding Gaussian noise to the input.
% To the best of our knowledge, our \ours is the first certifiable defense in MARL against communication attacks. Moreover, we consider a strong threat model where up to half of communication messages can be arbitrarily corrupted. 
% % \ys{flexibility}

\textbf{Communication in MARL}\quad
Communication is crucial in solving collaborative MARL problems. There are many existing studies learning communication protocols across multiple agents. Foerster et al. \cite{foerster2016learning} are the first to learn differentiable communication protocols that is end-to-end trainable across agents. Another work by Sukhbaatar et al. \cite{sukhbaatar2016learning} proposes an efficient permutation-invariant centralized learning algorithm which learns a large feed-forward neural network to map inputs of all agents to their actions. 
It is also important to communicate selectively, since some communication may be less informative or unnecessarily expensive. To tackle this challenge, Das et al. \cite{das2020tarmac} propose an attention mechanism for agents to adaptively select which other agents to send messages to. Liu et al. \cite{liu2020who2com} introduce a handshaking procedure so that the agents communicate only when needed. Our work assumes a pre-trained communication protocol and does not consider the problem of learning communication mechanisms.

==> cmarl/neurips/a2_theory.tex <==
\section{Additional Theoretical Definitions and Analysis}
\label{app:theory}

\textbf{Relation between Communication Attack and $\boldsymbol \ell_0$ Observation Attack}\quad
The communication threat model described in Section~\ref{sec:setup_adv} is analogous to a constrained $\ell_0$ attack on policy inputs. When agent $i$ is attacked, the input space of its acting policy $\pi_i$ is $\mathcal{X}_i := \hisspace_i \times \mathcal{M}^{N-1}$. Therefore, when $C$ communication messages are corrupted, the original input $x_i$ gets perturbed to $\tilde{x}_i$. Let $d$ be the dimension of a communication message, then $x_i$ and $\tilde{x}_i$ differ by up to $dC$ dimensions, which is similar to an $\ell_0$ attack constrained in certain dimensions. 



\subsection{Additional Analysis of \ours in Discrete Action Space}
\label{app:theory_dist}

\textbf{Reward Certificate}\quad
Theorem~\ref{thm:main_dist} justifies that under sufficient majority votes, the \ensname $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a benign action that is suggested by some benign message combinations, even when the malicious messages are not identified.
It is important to note that, when the \ensname $\smpolicy$ selects an action $\widetilde{a}$, there must exist at least one purely benign \ksample that let the \ablname $\ablpolicy$ produce $\widetilde{a}$. Therefore, as long as $\ablpolicy$ can obtain high reward with randomly selected benign \ksamples, $\smpolicy$ can also obtain high reward with ablated adversarial communication due to its design.

% Specifically, with ensemble policy $\smpolicy$, the agent's cumulative reward under adversarial communications would be similar to the natural reward of $\ablpolicy$ under no attacks, as justified in the following corollary.
% The corollary below shows the relationship between the attacked reward of $\smpolicy$ and the natural reward of $\ablpolicy$. Note that $\ablpolicy$ is the policy learned during training time in a clean (non-adversarial) environment, and it is easy for us to evaluate its natural cumulative reward. $\smpolicy$ is 
% \fh{I feel the current description doesn't make it easy to  distinguish between $\ablpolicy$ and $\smpolicy$.}
Specifically, we consider a specific agent with \ablname $\ablpolicy$ and \ensname $\smpolicy$ (suppose other agents are executing fixed policies). 
Let $\nu:\mathcal{M}^{N-1}\to\mathcal{M}^{N-1}$ be an attack algorithm that perturbs at most $C$ messages in a message set. 
Let $\zeta \sim Z(P,\ablpolicy)$ be a trajectory of policy $\ablpolicy$ under no attack, i.e., $\zeta=(o^{(0)},\msg^{(0)},a^{(0)},r^{(0)},o^{(1)},\msg^{(1)},a^{(0)},r^{(0)},\cdots)$. (Recall that a \ablname $\ablpolicy$ takes in a random size-$k$ subset of $\msg\step$ and outputs action $a\step$.)
When there exists attack with $\nu$, let $\zeta_\nu \sim Z(P,\smpolicy;\nu)$ be a trajectory of policy $\smpolicy$ under communication attacks, i.e., $\zeta_\nu=(o^{(0)},\nu(\msg^{(0)}),a^{(0)},r^{(0)},o^{(1)},\nu(\msg^{(1)}),a^{(0)},r^{(0)},\cdots)$. 
For any trajectory $\zeta$, let $r(\zeta)$ be the discounted cumulative reward of this trajectory.

% Let $\zeta=(o^{(0)},\msg^{(0)},a^{(0)},r^{(0)},o^{(1)},\msg^{(1)},a^{(0)},r^{(0)},\cdots)$ denote a trajectory. If \ablname is used, we have 
% $a\step = \ablpolicy(\his\step, \msgk)$ where $\msgk\sim\mathrm{Uniform}(\mathcal{H}_{k}(\msg\step))$. If \ensname is used, we have $a\step = \smpolicy(\his\step, \msg\step)$. 
% Let $\natobj(\zeta)$ denote the natural cumulative reward of a policy under no attack.
% Let $\advobj(\zeta)$ denote the cumulative reward of a policy under attacks, where at every step $t$, up to $C$ messages in the message set $\msg\step$ can be perturbed arbitrarily.

With the above notations, we propose the following reward certificate.
% let $\goodmsg\step$ and $\advmsg\step$ be the original benign message list and the perturbed message list the agent receives at step $t$, respectively. We use 
% \begin{equation}
%     \natobj(\pi) := J(\pi|\goodmsg^{(1)}, \goodmsg^{(2)},\cdots)
% \end{equation}
% to denote the expected cumulative reward of policy $\pi$ when it receives benign messages $\goodmsg^{(1)}, \goodmsg^{(2)},\cdots$, and use
% \begin{equation}
%     \advobj(\pi) := J(\pi|\advmsg^{(1)}, \advmsg^{(2)},\cdots)
% \end{equation}
% to denote the expected cumulative reward of policy $\pi$ when it receives perturbed messages $\advmsg^{(1)}, \advmsg^{(2)},\cdots$. Then, the following corollary presents the reward certificate of the \ensname when the agent's action space is discrete.

\begin{corollary}[Reward Certificate for Discrete Action Space]
\label{cor:reward_dist}
When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold at every step of execution, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} under adversarial communication is no lower than the lowest cumulative reward that the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
\begin{equation}
\begin{aligned}
    \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta),
    %  \min_{\advmsg^{(1)}, \advmsg^{(2)},\cdots} \advobj(\smpolicy) \geq \min_{[\goodmsg^{(1)}]_k,[\goodmsg^{(2)}]_k,\cdots} \natobj(\ablpolicy),
    % \advobj(\smpolicy) \geq \min_{\msgk^{(1)},\msgk^{(2)},\cdots} \natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)
    % \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
\end{aligned}
\end{equation}
for any attacker $\nu$ satisfying Assumption~\ref{assum:num} ($C<\frac{N-1}{2}$).
% where $[\goodmsg\step]_k\sim\mathrm{Uniform}(\mathcal{H}_{k}(\goodmsg\step))$.
% where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under arbitrary attacks to up to $C$ communication messages, and $\natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ when the random \ksample in the first step is $\msgk^{(1)}$, the random \ksample in the second step is $\msgk^{(2)}$, etc.
\end{corollary}

\textbf{Remarks.} 
(1) The certificate holds for any attack algorithm $\nu$ with $C<\frac{N-1}{2}$. 
(2) The \ablname $\ablpolicy$ has extra randomness from the sampling of \ksamples. That is, at every step, $\ablpolicy$ takes a uniformly randomly selected \ksample from $\allmsgk$. Therefore, the $\min_\zeta$ in the RHS considers the worst-case message sampling in the clean environment without attacks. Since $\smpolicy$ always takes actions selected by some purely-benign message combinations, the trajectory generated by $\smpolicy$ can also be produced by the \ablname.
(3) Note that the RHS ($\min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta)$) can be approximately estimated by executing $\ablpolicy$ during training time, so that the test-time performance of $\smpolicy$ is guaranteed to be no lower than this value, even if there are up to $C$ corrupted messages at every step.

% \begin{corollary}[Reward Certificate for Discrete Action Space]
% \label{cor:reward_dist}
% \fh{Under sample size $D=\binom{N-1}{k}$, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with a message subset size $k$ satisfying Equation~\eqref{eq:k_cond} obtains a total reward no worse than that obtained by the base ablation policy $\ablpolicy$ using benign messages:
% \begin{align}
%   & \advobj\Big(\smpolicy\big(o, \{\funabl(\advmsg, T_d)\}_{d=1}^D\big)\Big) \geq \nonumber \\
%   & \min_{T} \natobj\Big(\ablpolicy\big(o, \funabl(\goodmsg, T)\big)\Big) \label{eq:reward_dist}
% \end{align}
% if the majority votes $u_{\tilde{a}}$ satisfies $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step.
% }
% \textcolor{red}{Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If $D=\binom{N-1}{k}$, and the majority votes satisfy 
% $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step, 
% then the total reward of $\smpolicy$ satisfies
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:reward_dist}
%     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy),
% \end{equation}}
% Here $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the \textcolor{red}{sampled message indices}\fh{indices of the message subsets?} used by $\ablpolicy$ at all steps. \fh{What does this mean? My equation doesn't use $\tau$, rather I use $T$.}
% \end{corollary}


Appendix~\ref{app:proof} provides detailed proofs for the above theoretical results.


\subsection{Additional Analysis of \ours in Continuous Action Space}
\label{app:theory_cont}

\input{\texhome/theory_cont}



\subsection{Extension of \ours with Partial Samples}
\label{app:theory_sample}

As motivated in Section~\ref{sec:algo_more}, our \ours can be extended to a partial-sample version, where the ensemble policy is constructed by $D$ instead of $\binom{N-1}{k}$ samples. Let $\allmsgkd$ be a subset of $\allmsgk$ that contains $D$ random \ksamples from $\allmsgk$. Then the $D$-ensemble policy $\pi_D$ is defined as
\begin{equation}
\label{eq:ensemble_pi_dist_d}
    \smpolicy_D(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum_{\msgk\in\allmsgkd} \mathbbm{1}[\ablpolicy(o, \msgk)=a],
\end{equation}
for a discrete action space, and
\begin{equation}
\label{eq:ensemble_pi_cont_d}
    \tilde{\pi}_D(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \msgk) \}_{\msgk\in\allmsgkd}.
\end{equation}\normalsize
for a continuous action space. 

In the partial-sample version of \ours, we can still provide high-probability robustness guarantees. 



For notation simplicity, let $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$. 
Define the majority vote as 
\begin{equation}
\label{eq:vote}
    u_{\max}:=\max_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgkd} \mathbbm{1}[\ablpolicy(\his, \msgk)=a].
\end{equation}
The following theorem shows a general guarantee for $D$-ensemble policy in a discrete action space. 

\begin{theorem}[General Action Guarantee for Discrete Action Space]
\label{thm:sample_dist}
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_dist_d} with an ablation size $k$ satisfying Condition~\ref{cond:k},
Relation~\eqref{eq:cert_dist} holds deterministically if the majority vote $u_{\max}>n_1-n_2$. 
Otherwise it holds with probability at least
%\vspace{-0.1cm}
\begin{equation}
\label{eq:p_sample_dist}
    p_D=\frac{\sum_{j=0}^{u_{\max}-1}\binom{n_1-n_2}{j}\binom{n_2}{D-j}}{\binom{n_1}{D}}.
\end{equation}
\end{theorem}
Note that Theorem~\ref{thm:main_dist} is a special case of Theorem~\ref{thm:sample_dist}, since it assumes $u_{\max}>n_1-n_2$. 


Theorem~\ref{thm:sample_cont} below further shows the theoretical result for a continuous action space.

\begin{theorem}[General Action Guarantee for Continuous Action Space]
\label{thm:sample_cont}
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_cont_d} with an ablation size $k$ satisfying Condition~\ref{cond:k}, Relation~\eqref{eq:cert_cont} holds with probability at least
\begin{equation}
\label{eq:p_sample_cont}
    p_D=\frac{\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n_1-n_2}{D-j}}{\binom{n_1}{D}},
\end{equation}
where $\tilde{D} = {\lfloor \frac{D}{2} \rfloor}+1$. 
\end{theorem}

The larger $D$ is, the higher the probability $p_D$ is, the more likely that the \ensname selects an action in $\safeactioncont$.
In Theorem~\ref{thm:sample_cont}, when $D=\binom{N-1}{k}$,  the probability $p_D$ is 1 and the result matches Theorem~\ref{thm:main_cont}. 


Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.

==> cmarl/neurips/a3_proof.tex <==
\section{Technical Proofs}
\label{app:proof}



For the simplicity of the proof, we make the following definition.

\begin{definition} (Purely Benign \ksample and contaminated \ksample)
A \ksample $\msgk\in\allmsgk$ is purely benign if every message in $\msgk$ comes from a benign agent and is unperturbed. 
A \ksample $\msgk\in\allmsgk$ is contaminated if there exists some message in $\msgk$ that is perturbed.
% For a message combination $T\in \mathcal{H}(N-1, k)$, $\funabl(\textbf{m}, T)=[m_{j_1},...,m_{j_k}]$ is a \emph{safe message combination} iff for every $1\leq n\leq k$, $m_{j_n}$ is a benign communication message. Otherwise, it is  an \emph{unsafe message combination}. 
% \textcolor{purple}{PH: I think the terminology here may not be consistent with the main paper. 
% \begin{itemize}
%     \item $T$ is the index set of messages, but here we are referring to it as "combination message". Should we use $[m_{j_1}\dots, m_{j_k}]$?
%     \item  In section 2.2 [Formulation of Communication Attack] and Assumption 2.1, we talk about One attacker that can perturb $C$ of the communication messages (channels). However, here we are talking about $k$ benign/adversarial agents. Maybe we could say "iff $m_{j_n}$ is a benign communication message for every $1\leq n\leq k$"?
% \end{itemize}}
\end{definition}


% For simplicity, we will refer to the indexes $T$ as a safe message combination iff $\funabl(\textbf{m}, T)$ is a safe  message combination.
For notation simplicity, let $n_1:=|\allmsgk|=\binom{N-1}{k}$ be the total number of \ksamples from a message set $\msg$.
Note that the total number of purely benign \ksamples is $n_2:=\binom{N-C-1}{k}$, and the total number of contaminated \ksamples is $n_1-n_2=\binom{N-1}{k}-\binom{N-C-1}{k}$.

\subsection{Proofs in Discrete Action Space}

\textbf{Action Certificates}\quad
We first prove the action certificates in the discrete action. 
Note that Theorem~\ref{thm:main_dist} is a special case of Theorem~\ref{thm:sample_dist} ($u_{\max}>n_1-n_2$ and $D=\binom{N-1}{k}$), so we first prove the general version Theorem~\ref{thm:sample_dist} and then Theorem~\ref{thm:main_dist} holds as a result.
% , and the action certificate Theorem~\ref{thm:main_dist} is a special case of Theorem~\ref{thm:sample_dist} when $D=\binom{N-1}{k}$. Therefore, We first prove Theorem~\ref{thm:sample_dist}.

\begin{proof}[Proof of Theorem~\ref{thm:sample_dist} and Theorem~\ref{thm:main_dist}]

% We first prove Theorem~\ref{thm:sample_dist}, and then Theorem~\ref{thm:main_dist} holds as a special case of Theorem~\ref{thm:sample_dist}.

The majority voted action $\tilde{a}$ is a benign action, i.e., $\tilde{a}\in \safeaction$, if the ablation policy $\hat{\pi}$ renders action $\tilde{a}$ for
at least one purely benign \ksample.  
% Let $u_{\tilde{a}}$ denote the number of votes obtained by $\tilde{a}$, which equals $u_{\max}$.
If $u_{\max}>n_1-n_2$, since $n_1-n_2$ is exactly the total number of contaminated \ksamples, then it is guaranteed that there is at least one purely benign \ksample for which $\hat{\pi}$ renders $\tilde{a}$. Thus, $\tilde{a}\in \safeaction$, and Theorem~\ref{thm:main_dist} holds.
%Here, the majority voted action $\tilde{a}\in \safeactiondist$ is equivalent to the condition that $\tilde{a}$ is chosen by at least one safe message combination. Therefore, if $u_{\tilde{a}}>n_1-n_2$, where $n_1-n_2$ is exactly the total number of unsafe combinations, then it is guaranteed that $\tilde{a}$ is chosen by at least one safe combination. Thus, $\tilde{a}\in \safeactiondist$ is a safe action.

On the other hand, if $u_{\max}\leq n_1-n_2$, then in order for $\tilde{a}$ to be in $\safeaction$, among the $u_{\max}$ \ksamples resulting in $\tilde{a}$ there can be at most $u_{\max}-1$ contaminated \ksamples.  % Therefore, the maximum number of votes coming from unsafe message combination is $u_{\tilde{a}}-1$. 
There are $ \sum_{j=0}^{u_{\max}-1}\binom{n_1-n_2}{j}\binom{n_2}{D-j}$ such combinations in terms of the sampling of $D$, and the total number of combinations are $\binom{n_1}{D}$. Therefore, we get Equation \eqref{eq:p_sample_dist}.

\end{proof}

% \begin{proof}[Proof of Theorem~\ref{thm:main_dist}]

% The proof of Theorem~\ref{thm:main_dist} follows as a special case of Theorem~\ref{thm:sample_dist} when $D=\binom{N-1}{k}$. In this case, the only non-zero term left in the numerator of $p_D$ is $\binom{n_2}{j}\binom{n_1-n_2}{n_1-j}=\binom{n_2}{n_2}\binom{n_1-n_2}{n_1-n_2}=1$ ($j=n_2$), so $p_D=1$.

% \end{proof}

\textbf{Reward Certificate.}\quad
Next, following Theorem~\ref{thm:main_dist}, we proceed to prove the reward certificate.

\begin{proof}[Proof of Corollary~\ref{cor:reward_dist}]

Based on the definition of benign action set $\safeaction$, $\smpolicy$ selects an action $\widetilde{a}$ if and only if there exists a purely benign \ksample $\msgk\in\allmsgk$ such that the \ablname $\ablpolicy$ selects $\widetilde{a}=\ablpolicy(\tau, \msgk)$. 
Therefore, for any trajectory generated by $\smpolicy$ under attacks, there is a trajectory of $\ablpolicy$ with a list of \ksamples $\msgk^{(1)},\msgk^{(2)},\cdots$ that renders the same cumulative reward under no attack.

% Based on the definition of benign action set, $\smpolicy$ selects an action $\widetilde{a}$ if and only if there exists an index set $T$ such that the benign message combination $\funabl(\mathbf{m},T)$ makes the ablation policy $\ablpolicy$ select $\widetilde{a}$. Therefore, for any trajectory generated by $\smpolicy$ under attacks, there is a trajectory of $\ablpolicy$ with a list of indices sets $T_1,T_2,\cdots$ that renders the same cumulative reward under no attack.
\end{proof}


\subsection{Proofs in Continuous Action Space}

\textbf{Action Certificate.}\quad
Similar to the discrete-action case, we first prove Theorem~\ref{thm:sample_cont}, and then prove Theorem~\ref{thm:main_cont} as a special case of Theorem~\ref{thm:sample_cont}.

\begin{proof}[Proof of Theorem~\ref{thm:sample_cont}]

% We first prove Theorem~\ref{thm:sample_cont}, and then Theorem~\ref{thm:main_cont} holds as a special case of Theorem~\ref{thm:sample_cont}.

To understand the intuition of element-wise median operation in continuous action space, let us first start with an intuitive example: 
consider 5 arbitrary numbers $x_1$, ..., $x_5$, if we already know 3 of them $x_1$, $x_2$, $x_3$, then it is certain that 
$\min(x_1, x_2, x_3) \leq \funmed(x_1, \cdots, x_5) \leq \max(x_1, x_2, x_3)$.
Therefore, when purely benign \ksamples form the majority (Condition~\ref{cond:k}), the element-wise median action falls into the range of actions produced by safe messages. 

To be more general, in a continuous action space,  $\tilde{a}\in \safeactioncont$ is equivalent to the condition that out of the $D$ sampled \ksamples,  purely benign \ksamples make up the majority. There are $\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n1-n2}{D-j}$ such combinations in terms of the sampling of $D$, where $\tilde{D}={\lfloor \frac{D}{2} \rfloor}+1$. Once again the total number of combinations is $\binom{n_1}{D}$. Therefore, we get Equation \eqref{eq:p_sample_cont}.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:main_cont}]
The proof of Theorem~\ref{thm:main_cont} follows as a special case of Theorem~\ref{thm:sample_cont} when $D=\binom{N-1}{k}=n_1$. In this case, the only non-zero term left in the numerator of $p_D$ is $\binom{n_2}{j}\binom{n_1-n_2}{n_1-j}=\binom{n_2}{n_2}\binom{n_1-n_2}{n_1-n_2}=1$ (we need $n_2\geq j$ and $n_1-n_2 \geq n_1-j$ to keep the numerator from vanishing, which implies $j=n_2$, which is no lower than $\tilde{D}$ since $n_2>n_1/2$ due to Condition~\ref{cond:k}). Hence we have $p_D=1$. 
\end{proof}

\textbf{Reward Certificate.}\quad
Next, we derive the reward guarantee for the continuous-action case.

\begin{proof}[Proof of Theorem~\ref{thm:reward_cont}]

% Similar to the proof of Corollary~\ref{cor:reward_dist}, at any state $s$, the action $\widetilde{a}$ generated by $\smpolicy$ is always bounded by actions generated from $\ablpolicy$ with some indices set. Due to Assumption~\ref{assump:order}, there exists $a^\prime\sim\ablpolicy$ such that $R(s,a^\prime) \leq R(s,\widetilde{a})$. Therefore, the cumulative reward of $\smpolicy$ is lower bounded by the minimal cumulative reward of $\ablpolicy$ among all indices set lists.

We let $\mathbb{P}(a|s;\pi)$ be the probability of the \ablname $\ablpolicy$ taking action $a$ at state $s$, where $\pi$ can be either the \ablname $\ablpolicy$ or the \ensname $\smpolicy$. Note that this is a conditional probability function, and the policy does not necessarily observe $s$.

% note that the randomness comes from the observation emission function $O$ and the message uniform sampling process of $\ablpolicy$. Similarly, let $\smpolicy(a|s)$ be the probability of the \ensname $\smpolicy$ taking action $a$ at state $s$; note that the randomness comes from the observation emission function $O$ and the message uniform sampling process of $\ablpolicy$.

% According to Theorem~\ref{thm:main_cont}, at the same state $s\in\mathcal{S}$, the \ablname $\ablpolicy$ and the \ensname $\smpolicy$ both take actions within $\safeactioncont$. Based on Definition~\ref{def:disc}, we know that 

Without loss of generality, let $\nu^*$ be the optimal attacking algorithm that minimizes $\tilde{V}^{\smpolicy}_\nu$. 
Let $\mathcal{A}_s$ denote the range of \safename at state $s$ induced by the current \ablname $\ablpolicy$.
Then we have

\begin{equation}
    \begin{aligned}
    & \sup_{s\in\mathcal{S}} \left| V^{\ablpolicy}(s) - \tilde{V}^{\smpolicy}_{\nu^*}(s) \right| \\
    &= \sup_{s\in\mathcal{S}} \left| \mathbb{E}_{a\sim\mathbb{P}(a|s;\ablpolicy)} \left[R(s,a) + \gamma \int P(s^\prime|s,a) V^{\ablpolicy}(s^\prime) \mathrm{d}s^\prime \right] - \mathbb{E}_{a\sim\mathbb{P}(a|s;\smpolicy)} \left[R(s,a) + \gamma \int P(s^\prime|s,a) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime \right]   \right| \\
    &\leq \sup_{s\in\mathcal{S}} \sup_{a_1,a_2 \in \mathcal{A}_s} \left| R(s,a_1) + \gamma \int P(s^\prime|s,a_1) V^{\ablpolicy}(s^\prime) \mathrm{d}s^\prime - R(s,a_2) - \gamma \int P(s^\prime|s,a_2) \tilde{V}^{\smpolicy}_{\nu^*}(s)(s^\prime) \mathrm{d}s^\prime \right| \\
    &\leq \sup_{s\in\mathcal{S}} \sup_{a_1,a_2 \in \mathcal{A}_s} \left| R(s,a_1) - R(s,a_2) \right| + \sup_{a_1,a_2 \in \mathcal{A}_s} \left| \gamma \int P(s^\prime|s,a_1) V^{\ablpolicy}(s^\prime) \mathrm{d}s^\prime - \gamma \int P(s^\prime|s,a_2) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime \right| \\
    &\leq \epsilon_R + \gamma \sup_{s\in\mathcal{S}} \sup_{a_1,a_2 \in \mathcal{A}_s} \left| \int P(s^\prime|s,a_1) V^{\ablpolicy}(s^\prime) \mathrm{d}s^\prime - \int P(s^\prime|s,a_2) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime \right| \\
    &\leq \epsilon_R + \gamma \sup_{s\in\mathcal{S}} \sup_{a_1,a_2 \in \mathcal{A}_s} \left| \int P(s^\prime|s,a_1) V^{\ablpolicy}(s^\prime) \mathrm{d}s^\prime - \int P(s^\prime|s,a_1) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime \right| \\
    & \hspace{3em} + \gamma \sup_{s\in\mathcal{S}} \sup_{a_1,a_2 \in \mathcal{A}_s}\left|\int P(s^\prime|s,a_1) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime - \int P(s^\prime|s,a_2) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime \right| \\
    &\leq \epsilon_R + \gamma \sup_{s\in\mathcal{S}}\left| V^{\ablpolicy}(s) - \tilde{V}^{\smpolicy}_{\nu^*}(s) \right| + \gamma \left|\int P(s^\prime|s,a_1) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime - \int P(s^\prime|s,a_2) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime \right| \\
    &\leq \epsilon_R + \gamma \sup_{s\in\mathcal{S}}\left| V^{\ablpolicy}(s) - \tilde{V}^{\smpolicy}_{\nu^*}(s) \right| + \gamma V_{\max} \epsilon_P.
\end{aligned}
\end{equation}

By solving for the recurrence relation over $\sup_{s\in\mathcal{S}}\left| V^{\ablpolicy}(s) - \tilde{V}^{\smpolicy}_{\nu^*}(s) \right|$, we obtain
\begin{equation}
    \sup_{s\in\mathcal{S}}\left| V^{\ablpolicy}(s) - \tilde{V}^{\smpolicy}_{\nu^*}(s) \right| \leq \frac{\epsilon_R+\gamma V_{\max} \epsilon_P}{1-\gamma}.
\end{equation}
which leads to the desired relation in Theorem~\ref{thm:reward_cont}.

% For the second term, we can further decompose it into

% \begin{equation}
%     \begin{aligned}
%         \left| \int P(s^\prime|s,a_1) \tilde{V}^{\smpolicy}_{\nu^*}(s^\prime) \mathrm{d}s^\prime - \int P(s^\prime|s,a_2) V^{\ablpolicy}(s^\prime) \mathrm{d}s^\prime \right|
%     \end{aligned}
% \end{equation}


\end{proof}

==> cmarl/neurips/a4_exp.tex <==

\section{Experiment Details and Additional Results in FoodCollector and \marketenv}
\label{app:exp}


\subsection{More Environment Description}
\label{app:exp_env}

\subsubsection{FoodCollector}
\label{app:exp_env:food}



The FoodCollector environment is a 2D particle world shown by Figure~\ref{fig:food}(left). There are $N=9$ agents with different colors, and $N$ foods with colors corresponding to the $N$ agents. Agents are rewarded when eating foods with the same color. A big round obstacle is located in the center of the map, which the agent cannot go through. There are some poisons (shown as black dots) in the environment, and the agents get penalized whenever they touch the poison. Each agent has 6 sensors that detect the objects around it, including the poisons and the colored foods. 
The game is episodic, with horizon set to be 200. In the beginning of each episode, the agents, foods and poisons are randomly generated in the world. 
% Every time an agent eats a food, the food disappears, and the world re-generate a food with the same color in a random position. Therefore, an agent is supposed to explore the world and to eat as many foods as possible within limited number of steps.

\begin{figure}[htbp]
\vspace{-1em}
    \centering
    \includegraphics[width=0.4\columnwidth]{figs/foodcollector.png}
    \vspace{-0.5em}
    \caption{The FoodCollector Environment. For figure readability, we only show 3 agents colored as red/green/blue. In our experiments, there are 9 agents. }
    \label{fig:food}
\vspace{-1em}
\end{figure}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{figs/comm_dist}}
        % \vspace{-0.1cm}
        \caption{Discrete action space}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{figs/comm_cont}}
        % \vspace{-0.1cm}
        \caption{Continuous action space}
    \end{subfigure}
% \vspace{-0.5em}
\caption{\textbf{FoodCollector}: Reward of agents trained by PPO with communication v.s. without communication. Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.}
\label{fig:food_comm}
% \vspace{-0.4cm}
\end{figure}

\textbf{State Observation}\quad
Each of the 6 sensors can detect the following values when the corresponding element is within the sensor's range (the corresponding dimensions are 0's if nothing is detected):\\
(1) (if detects a food) the distance to a food (real-valued); \\
(2) (if detects a food) the color of the food (one-hot); \\
(3) (if detects an obstacle) the distance to the obstacle (real-valued); \\
(4) (if detects the boundary) the distance to the boundary (real-valued); \\ (5) (if detects another agent) the distance to another agent (real-valued).\\
The observation of an agent includes an agent-identifier (one-hot encoding), its own location (2D coordinates), its own velocity, two flags of colliding with its food and colliding with poison, and the above sensory inputs. Therefore, the observation space is a ($7N+30$)-dimensional vector space. 

\textbf{Agent Action}\quad
The action space can be either \textit{discrete} or \textit{continuous}. For the discrete version, there are 9 actions including 8 moving directions (north, northwest, west, southwest, south, southeast, east, northeast) and 1 no-move action. For the continuous version, the action is an acceleration decision, denoted by a 2-dimensional real-valued vector, with each coordinate taking values in $[-0.01,0.01]$. 

\textbf{Reward Function}\quad
At every step, each agent will receives a negative reward $-0.5$ if it has not eaten all its food. In addition, it receives extra $-1$ reward if it collides with a poison. 
Therefore, every agent is expected to explore the environment and eat all food as fast as possible. The team reward is calculated by the average of all agents' local rewards. Note that the agents' actions do not affect each other, because they have different target foods to collect. \emph{Agents collaborate only via communication introduced below.}

\textbf{Communication Protocol}\quad
Due to the limited sensory range, every agent can only see the objects around it and thus only partially observes the world. Therefore, communication among agents can help them find their foods much faster. Since our focus is to defend against adversarially perturbed communications, we first define a valid and beneficial communication protocol, where an agent sends a message to a receiver once it observes a food with the receiver's color. For example, if a red agent encounters a blue food, it can then send a message to the blue agent so that the blue agent knows where to find its food. 
% The communication follows the protocol below. Once agent $i$ detects the location of some food or poison from its sensors, it will update the communication channel to every other agent with the latest sensor observation containing its position and its sensory data, which contains the relative location of the food and/or poison. 
To remember the up-to-date communication, every agent maintains a list of most recent $N-1$ messages sent from other $N-1$ agents.
A message contains the sender's current location and the relative distance to the food (recorded by the 6 sensors), which are bounded between -1 and 1. Therefore, a message is a $8$-dimensional vector, and each agent's communication list has $8(N-1)$ dimensions in total.

\textbf{Communication Gain}\quad
During training with communication, we concatenate the observation and the communication list of the agent to an MLP-based policy, compared to the non-communicative case where the policy only takes in local observations. More implementation details are in Appendix~\ref{app:exp_imple:food}.
As verified in Figure~\ref{fig:food_comm}, communication does help the agent to obtain a much higher reward in both discrete action and continuous action cases, which suggests that the agents tend to rely heavily on the communication messages for finding their food. 



% \begin{wrapfigure}{r}{0.27\textwidth}
% \vspace{-1em}
% \centering
%     \includegraphics[width=0.25\columnwidth]{figs/foodcollector.png}
%     \caption{\small{The FoodCollector Environment with 3 agents.}}
%     \label{fig:food}
% \vspace{-1em}
% \end{wrapfigure}


\subsubsection{\marketenv}
\label{app:exp_env:market}

The \textit{\marketenv} environment is an inventory management setup, where $N=10$ cooperative heterogeneous distributors carry inventory for $M=3$ products. A population of $B=300$ buyers request a product from a randomly selected distributor agent according to a demand distribution $\mathbf{p}=[p_1,\dots,p_M]$. We denote the demand realization for distributor $i$ with $\mathbf{d_i}=[d_{i,1},\dots,d_{i,M}]$. Distributor agents manage their inventory by restocking products through interacting with the buyers. The game is episodic with horizon set to $50$. At the beginning of each episode, a realization of the demand distribution $\mathbf{p}$ is randomly generated and the distributors' inventory for each product is randomly initialized from $[0, \frac{B}{N}]$, where $\frac{B}{N}$ is the expected number of buyers per distributor. %\ys{describe the initial inventory in every episode?} 
The distributor agents are penalized for mismatch between their inventory and the demand for a product, and they aim to restock enough units of a product at each step to prevent insufficient inventory without accruing a surplus at the end of each step.  %\ys{defining the reward function by math?}


% \begin{itemize}
    % \item State observation: 
    \textbf{State Observation}\quad
    A distributor agent's observation includes its inventory for each product, and the products that were requested by buyers during the previous step. The observation space is a $2M$-dimensional vector.
    
    % \item Agent action: 
    \textbf{Agent Action}\quad
    Distributors manage their inventory by restocking new units of each product or discarding part of the leftover inventory at the beginning of each step. Hence, agents take both positive and negative actions denoted by an $M$-dimensional vector, and the action space can be either discrete or continuous. In our experiments, we use continuous actions assuming that products are divisible and distributors can restock and hold fractions of a product unit.
    
    % \item Agent reward function: 
    \textbf{Reward Function}\quad
    During each step, agent $i$'s reward is defined as $r_i = - || \max( \mathbf{I}_i+\mathbf{a}_i, 0) - \mathbf{d}_i||_2$, where $\mathbf{I}_i$ denotes the agents initial inventory vector, and $\mathbf{a}_i$ denotes the inventory restock vector from action policy $\pi_i$. Note that the agents' actions do not affect each other. \emph{Agents collaborate only via communication introduced below.}
    
    
    % \item Agent communication: 
    \textbf{Communication Protocol}\quad
    Distributors learn the demand distribution and optimize their inventory by interacting with their own customers (i.e., portion of buyers that request a product from that distributor). Distributors would benefit from sharing their observed demands with each other, so that they could estimate the demand distribution more accurately for managing inventory. At the end of each step, a distributor communicates an $M$-dimensional vector reporting its observed demands to all other agents. In the case of adversarial communications, this message may differ from the agents' truly observed demands.
    
    \textbf{Communication Gain}\quad
    During training with communication, messages received from all other agents are concatenated to the agent's observation, which is used to train an MLP-based policy, compared to the non-communicative case where the policy is trained using only local observations. As observed from Figure \ref{fig:marketenv_comm}, communication helps agents obtain  higher rewards since they are able to manage their inventory based on the overall demands observed across the population of buyers rather than their local observation. Results are reported by averaging rewards corresponding to $5$ experiments run with different training seeds.
% \end{itemize}
 
\begin{figure}[h]
\vspace{-0.1cm}
 \centering
\resizebox{.4\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_comm_dist}}
\vspace{-0.1cm}
\caption{\textbf{\marketenv}: Reward of agents trained with communication v.s. without communication. %Black dashed line stands for the mean performance of the agent when selecting actions uniformly randomly.
} 
\label{fig:marketenv_comm}
\end{figure}
 


% \subsubsection{MNIST-Classification}
% \label{app:exp_env:mnist}



\subsection{Implementation Details}
\label{app:exp_imple}


\subsubsection{FoodCollector}
\label{app:exp_imple:food}

\textbf{Implementation of Trainer}\quad
In our experiments, we use the Proximal Policy Optimization (PPO) \cite{schulman2017proximal} algorithm to train all agents (with parameter sharing among agents) as well as the  attackers. Specifically, we adapt from the elegant OpenAI Spinning Up \cite{SpinningUp2018} Implementation for PPO training algorithm. On top of the Spinning Up PPO implementation, we also keep track of the running average and standard deviation of the observation and normalize the observation. All experiments are conducted on NVIDIA GeForce RTX 2080 Ti GPUs.

For the policy network, we use a multi-layer perceptron (MLP) with two hidden layers of size 64. For a discrete action space, a categorical output distribution is used. For a continuous action space, since the valid action is bounded within a small range [-0.01,0.01], we parameterize the policy as a Beta distribution, which has been proposed in previous works to better solve reinforcement learning problems with bounded actions  \cite{pmlr-v70-chou17a}. In particular, we parameterize the Beta distribution by $\alpha_\theta$ and $\beta_\theta$, such that $\alpha=\log(1+e^{\alpha_{\theta}(s)})+1$ and $\beta=\log(1+e^{\beta_{\theta}(s)})+1$ (1 is added to make sure that $\alpha, \beta\geq 1$). Then, $\pi(a|s)=f(\frac{a-h}{2h};\alpha, \beta)$, where $h=0.01$, and $f(x;\alpha, \beta)=\frac{\Gamma(\alpha+\beta)}{\Gamma(\alpha)\Gamma(\beta)}x^{\alpha-1}(1-x)^{\beta-1}$ is the density function of the Beta Distribution.
For the value network, we also use an MLP with two hidden layers of size 64. 

In terms of other hyperparameters used in the experiments, we use a learning rate of 0.0003 for the policy network, and a learning rate of 0.001 is used for the value network. We use the Adam optimizer with $\beta_1=0.99$ and  $\beta_2 = 0.999$. For every training epoch, the PPO agent interacts with the environment for 4000 steps, and it is trained for 500 epochs in our experiments.

% \textcolor{purple}{PH: before describing the  type of attackers, should we mention what an attacker is training. For example, we say below that " The action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1." Perhaps we can state it here to make it more clear the attacker is learning a communication policy and not taking over the actions of agents?}


\textbf{Attacker}\quad
An attacker maps its own observation to the malicious communication messages that it will send to the victim agent. Thus, the action space of the attacker is the communication space of a benign agent, which is bounded between -1 and 1. 
% \vspace{-0.5cm}
\begin{itemize}
\item \emph{Non-adaptive Attacker}\quad
We implement a fast and naive attacking method for the adversary. At every dimension, the naive attacker randomly picks 1 or -1 as its action, and then sends the perturbed message which consists entirely of 1 or -1 to the victim agent. 
% \vspace{-0.2cm}
\item \emph{Adaptive RL Attacker}\quad
We use the PPO algorithm to train the attacker, where we set the reward of the attacker to be the negative reward of the victim. The attacker uses a Gaussian policy, where the action is clipped to be in the valid communication range. The network architecture and all other hyperparameter settings follow the exact same from the clean agent training.
\end{itemize}
% \vspace{-0.2cm}

\textbf{Implementation of Baselines}\quad
% \vspace{-0.2cm}
\begin{itemize}
\item \emph{Vanilla Learning}\quad
For Vanilla method, we train a shared policy network to map observations and communication to actions. 
% \vspace{-0.2cm}
\item \emph{Adversarial Training (AT)}\quad
For adversarial training, we alternate between the training of attacker and the training of the victim agent. Both the victim and attackers are trained by PPO. For every 200 training epochs, we switch the training, where we either fix the trained victim and train the attacker for the victim or fix the trained attacker and train the victim under attack. We continue this process for 10 iterations. 
% Similar to Vanilla, the victim also shuffles the communication messages to obtain higher reward and converge faster. 
\end{itemize}
% \vspace{-0.2cm}
% For Vanilla and AT, 
Note that the messages are symmetric (of the same format), we shuffle the messages before feeding them into the policy network for both Vanilla and AT, to reduce the bias caused by agent order. We find that shuffling the messages helps the agent converge much faster (50\% fewer total steps). Note that \ours randomly selects \ksamples and thus messages are also shuffled.

\subsubsection{\marketenv}
\label{app:exp_imple:market}


\textbf{Implementation of Trainer}\quad 
As in the FoodCollector experiments, we use the PPO algorithm to train all agent action policy as well as adversarial agent communication policies. We use the same MLP-based policy and value networks as the FoodCollector but parameterize the policy as a Gaussian distribution. The PPO agent interacts with the environment for $50$ steps, and it is trained for $10000$ episodes. The learning rate is set to be 0.0003 for the policy network, and 0.001 for the value network.
% All other hyper-parameters are set similar to the FoodCollector experiments.


\textbf{Attacker}\quad 
The attacker uses its observations to communicate malicious messages to  victim distributors, and its action space is the communication space of a benign agent.  We consider the following non-adaptive and adaptive attackers:
\begin{itemize}
    \item \textit{Non-adaptive Attacker}: The attacker's goal is to harm the victim agent by misreporting its observed demands so that the victim distributor under-estimates or over-estimates the restocking of products. In our experiments, we evaluate the effectiveness of defense strategies against the following attack strategies:
    \begin{itemize}
     \item{\permute}: The communication message is a random permutation of the true demand vector observed by the attacker.
    \item {\swap}: In order to construct a communication vector as different as possible from its observed demand, the attacker reports the most requested products as the least request ones and vice versa. Therefore, the highest demand among the products is interchanged with the lowest demand, the second highest demand is interchanged with the second lowest demand and so forth.
    \item{\flip:} Adversary $i$ modifies its observed demand $\mathbf{d}_i$ by mirroring it with respect to $\eta=\frac{1}{M}\sum_{j=1}^M d_{ij}$, such that products demanded less than $\eta$ are reported as being requested more, and conversely, highly demanded products are reported as less popular.
    \end{itemize}
   
    
    \item \textit{Adaptive Attacker}: The attacker communication policy is trained using the PPO algorithm, and its reward is set as the negative reward of the victim agent. The attacker uses a Gaussian policy with a softmax activation in the output layer to learn a adversarial probability distribution across products, which is then scaled by the total observed demands $\sum_{j=1}^M d_{ij}$ to construct the communication message.

\end{itemize} 


 

\textbf{Implementation of Baselines}\quad 
\begin{itemize}
    \item \textit{Vanilla Learning}: In the vanilla training method with no defense mechanism against adversarial  communication, we train a shared policy network using agents' local observations and their received communication messages.
     \item \textit{Adversarial Training (AT)}: We alternate between training the agent action policy and the victim communication policy, both using PPO. For the first iteration we train the policies for $10000$ episodes, and then use $1000$ episodes for $5$ additional training alteration iterations for both the action policy and the adversarial communication policy. For more efficient adversarial training, we first shuffle the received communication messages before feeding them into the policy network. Consequently, the trained policy  treats communications received from different agents in a similar manner, and we are able to only train the policy with a fixed set of adversarial agents rather than training the network on all possible combinations of adversarial agents. 
    %\ys{maybe mention the communication permuting here? and explain why permutation is not used for vanilla (performance no better than vanilla). }
\end{itemize}
For Vanilla and AT, we do not shuffle the communication messages being input to the policy, as we did not observe improved convergence, as in the FoodCollector environment. 

% \subsubsection{MNIST-Classification}
% \label{app:exp_imple:mnist}




\subsection{Additional Results}
\label{app:exp_results}

In addition to Figure \ref{fig:res_k_dist}, we also provide the plot for hyper-parameter tests in discrete-action FoodCollector and \marketenv in Figure \ref{fig:res_hyper} below. 
% \input{fig_food_k_dist}

\begin{figure}[h]
% \vspace{-1.5em}
% \hspace{-2em}
 \centering
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_cont}}
  \vspace{-1.5em}
  \caption{FoodCollector}
  \label{sfig:hyper_k_food}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}}
  \vspace{-1.5em}
  \caption{\marketenv}
  \label{sfig:hyper_k_market}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_sample_cont}}
  \vspace{-1.5em}
  \caption{FoodCollector}
  \label{sfig:hyper_d_food}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_K_sampleD}}
  \vspace{-1.5em}
  \caption{\marketenv}
  \label{sfig:hyper_d_market}
 \end{subfigure}
\vspace{-0.5em}
\caption{Hyper-parameter tests of ablation size $k$ and sample size $D$. 
We show how natural reward and attacked performance change with \textbf{(a)} various $k$ in continuous-action FoodCollector, \textbf{(b)} various $D$ in continuous-action FoodCollector, \textbf{(c)} various $k$ in \marketenv, and \textbf{(d)} various $D$ in \marketenv. \\
Dashed green lines refer to the performance of Vanilla agent under $C=2$ attacks. }
% \vspace{-1.5em}
\label{fig:res_hyper}
\end{figure}


\textbf{Adversarial Training does not improve agent's robust performance.}
As we observed in Figure \ref{fig:res_all}, adversarial training (AT) does not improve the robustness of the agent in both discrete and continuous action space, although AT achieves good robustness againt $\ell_p$ attacks in vision tasks~\cite{madry2018towards,zhang2019theoretically}, and against observation attacks~\cite{zhang2021robust,sun2021strongest} and action attacks~\cite{pinto2017robust} in RL.
We hypothesize that it is due to (1) the large number of total agents,  (2) the uncertainty of adversarial message channels, and (3) the relatively large perturbation length. 
To be more specific, in related works~\cite{pinto2017robust,zhang2021robust,sun2021strongest}, an agent and an attacker are alternately trained, during which the agent learns to adapt to the learned attacker. However, in the threat model we consider, there are $C$ out of $N$ messages significantly perturbed, which it is hard for the agent to adapt to attacks during alternate training.
% To be more specific, during the training of AT, we alternately train the agent and the attacker, and the attacker can change the channels it controls among iterations. As a result, the agent might not be able to distinguish adversarial messages and benign messages. 
% We hypothesize that it is due to the communication shuffling of the agent. In fact, this is also similar to another practical scenario where at different time steps, the attacker might hijack different agents. As a consequence, in both scenarios, malicious messages could randomly appear in any part of the agent's input vector. 
% Therefore, simply training the agent and attacker together cannot make the agent learn how to detect the malicious messages and ignore them. 

\textbf{Additional Results with QMIX}\quad 
\ours is a generic defense approach that can be used for any RL/MARL learning algorithm. In Figure~\ref{fig:res_qmix}, we show the results of \ours combined with an MARL algorithm QMIX~\cite{rashid2018qmix} in the discrete-action FoodCollector environment (QMIX does not work for continuous actions so it is not applicable in continuous-action FoodCollector and \marketenv). Compared to the vanilla QMIX algorithm, QMIX+\ours achieves much higher robustness and stable performance under various numbers of adversaries. 
\input{figs/QMIX_AME}



\section{Additional Experiment in MARL Image Classification}
\label{app:exp_mnist}

\subsection{Description of MARL-MNIST Environment}

We use the environment setup proposed by Mousavi et al.~\cite{mousavi2019multi}, where agents collaboratively classify an unknown image by their observations and inter-agent communication. 
More specifically, we use $N=9$ agents in the MNIST dataset of handwritten digits~\cite{lecun1998gradient}.  The dataset consists
of 60,000 training images and 10,000 testing images, where
each image has $28 \times 28$ pixels. 
There are $h=5$ steps in an episode. In the beginning, all agents start from a pre-determined spatial configuration. At every step, each agent observes a local $5 \times 5$ patch, performs some local data processing, and shares the result with neighboring agents (we use a fully connected communication graph). 
With given observation and communication, each agent outputs an action in $\{Up, Down, Left, Right\}$. By each movement, the agent is translated in the desired direction by $5$ pixels. In the end of an episode, agents make predictions, and all of them are rewarded by $- \mathrm{prediction\_loss}$. 


\subsection{Implementation Details}

We use the same network architecture and hyperparameter setting as Mousavi et al.~\cite{mousavi2019multi}, which are implemented in~\cite{mnistgithub}. 

\textbf{Network Architecture}\quad
Concretely, at every step, the input of every agent contains 3 components: (1) an encoded observation with two convolutional layers followed by vectorization and a fully connected layer; (2) the average of all communication messages from other agents; (3) a position encoding computed by feeding the current position into a single linear layer.
These 3 components are concatenated and passed to two independent LSTM modules, one is for an acting policy, another is for a message generator. 
In the end of an episode, every agent uses its final cell state to generate a prediction using a 2-layer MLP. Then we take the average of the output logits of all agents, and use a softmax function to obtain the final probabilistic label prediction. The reward is the opposite number of the L2 difference between the prediction and the one-hot encoding of true image label.

\textbf{Hyperparameters}\quad
In our experiments, we follow the default hyperparameter setting in~\cite{mnistgithub}. We use $N=9$ agents. The size of LSTM belief state is 128. The hidden layers have size 160. The message size is set to be 32. The state encoding has size 8. We use an Adam optimizer with learning rate 1e-3. We train the agents in the MNIST dataset for 40 epochs.

\textbf{Attackers}\quad
Since the communication messages are learned by neural networks, we perturb the $C$ messages received by each agent. To make sure that the messages are not obviously detectable, we clip every dimension of the perturbed message into the range of $[-3,3]$. The non-adaptive attacker randomly generates a new message. The adaptive attacker learns a new message generator based on its own belief state, which is trained with learning rate 1e-3 for 50 epochs.


\subsection{Experiment Results}
Figure~\ref{fig:res_all_mnist} demonstrates the robust performance of the MARL algorithm proposed by Mousavi et al.~\cite{mousavi2019multi} with our \ours defense or baseline defenses (Vanilla and AT). We set $N=9$ and $k=2$ for all experiments.
Under learned adaptive attackers, the original MARL classifier (Vanilla)~\cite{mousavi2019multi}  without \ours suffers from significant performance drop in terms of both precision and recall. Defending with adversarial training (AT) does not achieve good robustness, either. But \ours considerably improves the robustness of agents across different numbers of attackers. \\
Under random attacks, we find that the original MARL classifier~\cite{mousavi2019multi} is moderately robust when a few communication signals are randomly perturbed. However, when noise exists in many communication channels (e.g. $C=6$), the performance decreases a lot. In contrast, our \ours still achieves high performance when $C=6$ communication messages are corrupted, even if the guarantee of ablation size $k$ only holds for $C\leq 2$. Therefore, we again emphasize the the theoretical guarantee considers the worst-case strong attack, while under a relatively weak attack, we can achieve better robustness beyond what the theory suggests.

\begin{figure}[!t]
% \vspace{-1em}
\hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/mnist/MNIST_Adaptive_Attacker_Precision}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/mnist/MNIST_Adaptive_Attacker_Recall}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/mnist/MNIST_Random_Attacker_Precision}}
  \vspace{-1.5em}
  \caption{Non-adaptive Attack}
 \end{subfigure}
\hfill
 \begin{subfigure}[t]{0.24\textwidth}
 \centering
  \resizebox{\columnwidth}{!}{\input{figs/mnist/MNIST_Random_Attacker_Recall}}
  \vspace{-1.5em}
  \caption{Non-adaptive Attack}
 \end{subfigure}
\vspace{-0.5em}
\caption{\textbf{(MARL-MNIST)}: Precision and recall of MARL classification on MNIST without or with \ours, under learned adaptive attacks and non-adaptive random attacks. All results are averaged over 5 random seeds. }
% \vspace{-1.5em}
\label{fig:res_all_mnist}
\end{figure}

==> cmarl/neurips/a7_algo.tex <==
\section{Algorithm Pseudocode}
\label{app:algo}


Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test} demonstrate the procedures of \ours in training and defending phases, respectively. 
\input{algo_train}
\input{algo_test}




==> cmarl/neurips/a8_impact.tex <==
\section{Additional Discussion on Societal Impacts and Limitations}
\label{app:discuss}

This paper proposes a defense algorithm for multi-agent sequential decision making problems. The proposed algorithm, \ours, is certifiably robust during test-time under communication attacks that perturbs up to $C$ out of $N-1$ messages. Since our goal is to improve the robustness of any decision-making agent against corrupted communication, our algorithm will benefit many real-world applications. Therefore, the societal impacts of this work will be positive.

The method discussed in this paper is both theoretically grounded and empirically effective. But there are still some limitations. For example, the theoretical guarantee requires some conditions that may be broken in some challenging environments, as discussed in Appendix~\ref{app:hyper}, although the algorithm still performs well without these conditions in practice. Our future work includes relaxing these assumptions and conditions and obtain more universal certificates.
Moreover, we focus on the case where communication messages from different agents are symmetric, such that the \ablname can make decisions based on randomly sampled $k$ messages without considering the order of messages. But our algorithm can be extended to cover various message spaces (i.e., different agents may send messages with different formats).

==> cmarl/neurips/figs_all.tex <==


% \begin{figure}[!b]
% \vspace{-0.5em}
%  \centering
% %  \hspace{-1em}
%  \begin{subfigure}[t]{0.24\columnwidth}
%   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist_naive}}
%   \vspace{-1.5em}
%   \caption{Disc. \& Non-adaptive}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.24\columnwidth}
%   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist}}
%   \vspace{-1.5em}
%   \caption{Disc. \& Adaptive}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.24\columnwidth}
%   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Cont_naive}}
%   \vspace{-1.5em}
%   \caption{Cont. \& Non-adaptive}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.24\columnwidth}
%   \resizebox{\textwidth}{!}{ \input{figs/FoodCollector_Attacker_Cont}}
%   \vspace{-1.5em}
%   \caption{Cont. \& Adaptive}
%  \end{subfigure}
%  \vspace{-0.5em}
% \caption{\textbf{(FoodCollector)} Rewards of our \ours and baselines in FoodCollector with discrete/continuous action space, under no attacker or non-adaptive/adaptive attacks under varying numbers of adversaries. 
% % Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.
% }
% \vspace{-0.5em}
% \label{fig:res_all_food}
% \end{figure}


% \begin{figure}[!b]
% \vspace{-1em}
%  \centering
% %  \hspace{-1em}
%  \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
%  \centering
%   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_adaptive}}
%   \vspace{-1.5em}
%   \caption{Adaptive Attack}
%  \end{subfigure}
%  %\hfill
%  \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
%  \centering
%   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_permute}}
%   \vspace{-1.5em}
%   \caption{\permute}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
%  \centering
%   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_flip}}
%   \vspace{-1.5em}
%   \caption{\swap}
%  \end{subfigure}
%  %\hfill
%  \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
%  \centering
%   \resizebox{\linewidth}{!}{ \input{figs/MarketEnv/MarketEnv_Attacker_Dist_swap}}
%   \vspace{-1.5em}
%   \caption{\flip}
%  \end{subfigure}
%  \vspace{-0.5em}
% \caption{\textbf{(\marketenv)}: Rewards of our \ours and baselines with continuous action space, under no attacker and varying numbers of adversaries for (a) adaptive and (b), (c), (d) non-adaptive attacks. 
% % Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.
% }
% \vspace{-2em}
% \label{fig:res_all_market}
% \end{figure}

\begin{figure}[!b]
\vspace{-2em}
 \centering
%  \hspace{-1em}
\rotatebox{90}{\scriptsize{\qquad \quad \textbf{FoodCollector}}}
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist_naive}}
  \vspace{-1.5em}
  \caption{Disc. \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist}}
  \vspace{-1.5em}
  \caption{Disc. \& Adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Cont_naive}}
  \vspace{-1.5em}
  \caption{Cont. \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\textwidth}{!}{ \input{figs/FoodCollector_Attacker_Cont}}
  \vspace{-1.5em}
  \caption{Cont. \& Adaptive}
 \end{subfigure}
%  \vspace{-0.5em}
% \caption{\textbf{(FoodCollector)} Rewards of our \ours and baselines in FoodCollector with discrete/continuous action space, under no attacker or non-adaptive/adaptive attacks under varying numbers of adversaries. 
% % Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.
% }
% \vspace{-0.5em}
% \label{fig:res_all_food}
% \end{figure}
% \begin{figure}[!b]
% \vspace{-1em}
%  \centering
%  \hspace{-1em}

\rotatebox{90}{\scriptsize{\enspace\textbf{\marketenv}}}
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
  \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_adaptive}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_permute}}
  \vspace{-1.5em}
  \caption{\permute}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_flip}}
  \vspace{-1.5em}
  \caption{\swap}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.24\textwidth}%{0.49\columnwidth}
 \centering
  \resizebox{\linewidth}{!}{ \input{figs/MarketEnv/MarketEnv_Attacker_Dist_swap}}
  \vspace{-1.5em}
  \caption{\flip}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Rewards of our \ours and baselines in FoodCollector and \marketenv, under no attacker and varying numbers of adversaries for adaptive and various non-adaptive attacks. The dashed red lines stand for the average performance of a non-communicative agent. Results are averaged over 5 random seeds.
% Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.
}
\vspace{-2em}
\label{fig:res_all}
\end{figure}

==> cmarl/neurips/theory_cont.tex <==


\textbf{Action Certificate}\quad
As in the discrete action case, the continuous ensemble policy will output an action $\widetilde{a}$ that follows the consensus of benign messages. But in a continuous action space, it is hard to ensure that $\widetilde{a}$ is exactly in $\safeaction$. Instead, $\widetilde{a}$ is guaranteed to be within the range of $\safeaction$, as detailed in the following theorem.

\begin{theorem}[Action Certificate for Continuous Action Space]
\label{thm:main_cont}
Under Condition~\ref{cond:k}, the action $\widetilde{a} = \smpolicy(\his, \advmsg)$ generated by the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} satisfies
\begin{equation}
    \widetilde{a} \in \mathsf{Range}(\safeaction) := \{a: \forall 1\leq l \leq L, \exists \underline{a}, \overline{a} \in \safeaction \text{ s.t } \underline{a}_l \leq a_l \leq \overline{a}_l \}.
    \label{eq:cert_cont}
\end{equation}
% then any dimension $l$ of $\smpolicy$'s output satisfies
% \begin{equation*}
%     \inf_{\krv} [\hat{a}]_l  
%     \leq [\smpolicy(o, \advmsg, \{T_d\}_{d=1}^D)]_l 
%     \leq \sup_{\krv} [\hat{a}]_l.
% \end{equation*}
% where $\hat{a} := \ablpolicy(o, \mathsf{Ablate}(m, \krv))$.
\end{theorem}

In other words, if the \ensname takes an action $\widetilde{a}$, then at each dimension $l$, there must exist $a_1$ and $a_2$ suggested by some purely benign \ksamples such that the $l$-th dimension of $\widetilde{a}$ is lower and upper bounded by the $l$-th dimension of $a_1$ and $a_2$, respectively. 
Note that Theorem~\ref{thm:main_cont} certifies that the selected action is in a set of actions that are close to benign actions $\mathsf{Range}(\safeaction)$, but does not make any assumption on this set. Next we interpret this result in details.

\textbf{How to Understand $\mathsf{Range}(\safeaction)$?}\quad
Theoretically, $\mathsf{Range}(\safeaction)$ is a set of actions that are coordinate-wise bounded by base actions resulted from purely benign \ksamples. In many practical problems, it is reasonable to assume that actions in $\mathsf{Range}(\safeaction)$ are relatively safe, especially when benign actions in $\safeaction$ are concentrated. The following examples illustrate some scenarios where actions in $\mathsf{Range}(\safeaction)$ are relatively good.

\begin{enumerate}
    \item If the action denotes the price a seller sells its product in a market, and the communication messages are the transaction signals in an information pool, then $\mathsf{Range}(\safeaction)$ is a price range that is determined based on purely benign messages. Therefore, the seller will set a reasonable price without being influenced by a malicious message. 
    \item If the action denotes the driving speed, and benign message combinations have suggested driving at 40 mph or driving at 50 mph, then driving at 45 mph is also safe. 
    \item If the action is a vector denoting movements of all joints of a robot (as in many MuJoCo tasks), and two slightly different joint movements are suggested by two benign message combinations, then an action that does not exceed the range of the two benign movements at every joint is likely to be safe as well.
\end{enumerate}  

The above examples show by intuition why the \ensname can be regarded as a relatively robust policy. 
However, in extreme cases where there exists ``caveat'' in $\mathsf{Range}(\safeaction)$, taking an action in this set may also be unsafe. To quantify the influence of $\mathsf{Range}(\safeaction)$ on the long-term reward, we next analyze the cumulative reward of the \ensname in the continuous-action case.



\textbf{How Does $\mathsf{Range}(\safeaction)$ Lead to A Reward Certificate?}\quad
Different from the discrete-action case, the \ensname $\smpolicy$ in a continuous action space may take actions not in $\safeaction$ such that it generates trajectories not seen by the \ablname $\ablpolicy$. However, since the action of $\smpolicy$ is guaranteed to stay in $\mathsf{Range}(\safeaction)$, we can bound the difference between the value of $\smpolicy$ and the value of $\ablpolicy$, and how large the different is depends on some properties of $\mathsf{Range}(\safeaction)$.

Concretely, Let $R$ and $P$ be the reward function and transition probability function of the current agent when the other agents execute fixed policies. So $R(s,a)$ is the immediate reward of taking action $a$ at state $s$, and $P(s^\prime|s,a)$ is the probability of transitioning to state $s^\prime$ from $s$ by taking action $a$. (Note that $s$ is the underlying state which may not be observed by the agent.)
% Let $R_{\max}$ denote the supremum of the absolute value of $R$, i.e., $R_{\max}:=\sup_{s,a} |R(s,a)|$. 

\begin{definition}[Dynamics Discrepancy of $\ablpolicy$]
\label{def:disc}
A \ablname $\ablpolicy$ is called $\epsilon_R$,$\epsilon_P$-discrepant if $\epsilon_R$, $\epsilon_P$ are the smallest values such that for any $s\in\mathcal{S}$ and the corresponding \safename set $\safeaction$, we have $\forall a_1, a_2 \in \mathsf{Range}(\safeaction)$, 
\begin{align}
    & |R(s,a_1) - R(s,a_2)| \leq \epsilon_R, \\
    & \int | P(s^\prime| s, a_1) - P(s^\prime| s, a_2) | \mathrm{d}s^\prime \leq \epsilon_P. \label{eq:p_disc}
\end{align}
% Given a \ablname $\ablpolicy$, $\mathsf{Range}(\safeaction)$
% let $f_{\ablpolicy}$ be a mapping from state $s\in\mathcal{S}$ to the corresponding benign action range induced by $\ablpolicy$ at state $s$, i.e., $f_{\ablpolicy}(s)$ is 
\end{definition}

\textbf{Remarks.}
(1) Equation~\eqref{eq:p_disc} is equivalent to that the total variance distance between $P(\cdot| s, a_1)$ and $P(\cdot| s, a_2)$ is less than or equal to $\epsilon_P/2$.
(2) For any environment with bounded reward, $\epsilon_R$ and $\epsilon_P$ always exist. 
% (3) $\epsilon_R$ and $\epsilon_P$ are related to the \ablname, the communication quality, and the environment properties. When the reward function and transition function are smooth, and when the benign communications can reach some ``consensus'' of actions by propagating through $\ablpolicy$, $\epsilon_R$ and $\epsilon_P$ will be relatively small.



Definition~\ref{def:disc} characterizes how different the local dynamics of actions in $\mathsf{Range}(\safeaction)$ are, over all possible states. If $\mathsf{Range}(\safeaction)$ is small and the environment is relatively smooth, then taking different actions within this range will not result in very different future rewards. The theorem below shows a reward certificate for the \ensname $\smpolicy$.

% When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold at every step of execution, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} under adversarial communication is no lower than the lowest cumulative reward that the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
% \begin{equation}
% \begin{aligned}
%     \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta),
% \end{aligned}
% \end{equation}
% for any attacker $\nu$ satisfying Assumption~\ref{assum:num} ($C<\frac{N-1}{2}$).

\begin{theorem}[Reward Certificate for Continuous Action Space]
\label{thm:reward_cont}
Let $V^{\ablpolicy}(s)$ be the clean value (discounted cumulative reward) of $\ablpolicy$ starting from state $s$ under no attack; let $\tilde{V}^{\smpolicy}_\nu(s)$ be the value of $\smpolicy$ starting from state $s$ under attack algorithm $\nu$, where $\nu$ satisfies Assumption~\ref{assum:num}; let $k$ be an ablation size satisfying Condition~\ref{cond:k}.
If $\ablpolicy$ is $\epsilon_R$,$\epsilon_P$-discrepant, then for any state $s\in\mathcal{S}$, we have
\begin{equation}
    % \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta) - \frac{1}{1-\gamma}\epsilon_R - \frac{\gamma R_{\max}}{(1-\gamma)^2} \epsilon_P.
    \min_{\nu} \tilde{V}^{\smpolicy}_\nu(s) \geq V^{\ablpolicy}(s) - \frac{\epsilon_R+\gamma V_{\max}\epsilon_P}{1-\gamma},
\end{equation}
where $V_{\max} := \sup_{s,\pi}  |V^\pi(s)|$. 
% the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} is no lower than the lowest cumulative reward the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
% \begin{equation}
%     \min_{\advmsg^{(1)}, \advmsg^{(2)},\cdots} \advobj(\smpolicy) \geq \min_{[\goodmsg^{(1)}]_k,[\goodmsg^{(2)}]_k,\cdots} \natobj(\ablpolicy),
% \end{equation}
% where $[\goodmsg\step]_k\sim\mathrm{Uniform}(\mathcal{H}_{k}(\goodmsg\step))$.
\end{theorem}

\textbf{Remarks.}
(1) The certificate holds for any attack algorithm $\nu$ with $C<\frac{N-1}{2}$. 
(2) If $\epsilon_R$ and $\epsilon_P$ are small, then the performance of \ensname $\smpolicy$ under attacks is similar to the performance of the \ablname $\ablpolicy$ under no attack. 

It is important to note that $\epsilon_R$ and $\epsilon_P$ are intrinsic properties of $\ablpolicy$, independent of the attacker. Therefore, one can approximately measure $\epsilon_R$ and $\epsilon_P$ during training. 
Similar to Condition~\ref{cond:cons} required for a discrete action space, the gap between the attacked reward of $\smpolicy$ and the natural reward of $\ablpolicy$ depends on how well the benign messages are reaching a consensus. (Smaller $\epsilon_R$ and $\epsilon_P$ imply that the actions in $\safeaction$ are relatively concentrated and the environment dynamics are relatively smooth.)

Moreover, one can optimize $\ablpolicy$ during training such that $\epsilon_R$ and $\epsilon_P$ are as small as possible, to further improve the robustness guarantee of $\smpolicy$. This can be a future extension of this work.


Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.















% Therefore, in many cases we can expect the set $\mathsf{Range}(\safeaction)$ contain good actions. 
% Mathematically, the following assumption justifies when the set $\mathsf{Range}(\safeaction)$ is guaranteed to be safe, which rules out ``bad actions'' from this set. 

% \begin{assumption}
% \label{assump:order}
% Let $R: \mathcal{S} \times \mathcal{A} \to \mathbb{R}$ be the reward function of the current agent while the other agents are executing fixed policies. For any state $s\in\mathcal{S}$, let $\safeaction$ be the \safename set generated by the trained \ablname $\ablpolicy$, then we assume that for any action $a\in\mathsf{Range}(\safeaction)$, $R(s,a) \geq \min_{\hat{a}\in\mathsf{\safeaction}} R(s,\hat{a})$.
% \end{assumption} 

% \textbf{Remarks.} \\
% (1) Assumption~\ref{assump:order} suggests that there is no ``caveat'' in the safe action set. Note that without the assumption of reward structure, there may exist extreme cases where some actions in $\safeaction$ could lead to low reward, which makes the reward not certifiable. \\
% (2) This assumption holds in many real-life scenarios where actions have concrete meanings (e.g. price, speed, etc). In practice, we can expect this assumption to hold when the safe action range generated by the ablation policy is relatively narrow, i.e., the benign communication messages achieve agreements. \\
% (3) During training, we are able to compute the \safename set $\safeaction$ at every step, so \textit{we can check whether caveats can exist before deploying the policy to a real-world agent. } \\
% % For example, if driving at 40 mph and driving at 50 mph are both safe, then driving at 45 mph is also safe. 
% (4) Assumption~\ref{assump:order} assumes that the immediate reward of action $a\in\mathsf{Range}(\safeaction)$ is no lower than the actions in $\safeaction$. But it does not necessarily
% we can further relax this assumption such that the reward it as will be discussed later.


% \textbf{Reward Certificate}\quad
% % Theorem~\ref{thm:main_cont} shows how the ensemble policy outputs an action that is coordinate-wisely bounded by the range of benign actions. 
% % Under mild assumptions, it can also lead to a reward guarantee, as detailed in Appendix~\ref{app:theory_cont}.
% % Theorem~\ref{thm:main_cont} shows how the ensemble policy outputs an action bounded by safe actions. 
% With the notations defined in Appendix~\ref{app:theory_dist} and under Assumption~\ref{assump:order}, the following reward certificate holds.

% \begin{corollary}[Reward Certificate for Continuous Action Space]
% \label{cor:reward_cont}
% Under Condition~\ref{cond:k} and Assumption~\ref{assump:order}, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} is no lower than the lowest cumulative reward the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
% \begin{equation}
%     \min_{\advmsg^{(1)}, \advmsg^{(2)},\cdots} \advobj(\smpolicy) \geq \min_{[\goodmsg^{(1)}]_k,[\goodmsg^{(2)}]_k,\cdots} \natobj(\ablpolicy),
% \end{equation}
% where $[\goodmsg\step]_k\sim\mathrm{Uniform}(\mathcal{H}_{k}(\goodmsg\step))$.
% % \begin{equation}
% % \begin{aligned}
% %     \advobj(\smpolicy) \geq \min_{\msgk^{(1)},\msgk^{(2)},\cdots} \natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)
% %     % \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
% % \end{aligned}
% % \end{equation}
% % where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under arbitrary perturbations to up to $C$ communication messages, and $\natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ when the random \ksample in the first step is $\msgk^{(1)}$, the random \ksample in the second step is $\msgk^{(2)}$, etc.
% \end{corollary}


% \textbf{Relaxation of Assumption~\ref{assump:order}}\quad
% Assumption~\ref{assump:order} can hold in practice when the environment reward has ordered structures, or when benign actions are concentrated enough. As we have access to $\safeaction$ during training, one can estimate $\epsilon$ at every step and the worst-case reward drop. Then, the test-time performance can be lower bounded, and the agent will not be significantly reduced by any attacks. 
% In cases where Assumption~\ref{assump:order} does not hold, we can also relax it such that $R(s,a) \geq \min_{\hat{a}\in\mathsf{\safeaction}} R(s,\hat{a}) - \epsilon$ for some $\epsilon \geq 0$. Then the reward certificate in Theorem~\ref{thm:main_cont} can be relaxed to a softer version where the $\advobj(\smpolicy)$ is still lower bounded. 


% % \begin{corollary}[Reward Certificate for Continuous Action Space]
% % \label{cor:reward_cont}
% % Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If Assumption~\ref{assump:order} holds, and $D=\binom{N-1}{k}$, 
% % then the total reward of $\smpolicy$ satisfies
% % \begin{equation}
% % \label{eq:reward_cont}
% %     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy)
% % \end{equation}
% % where $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the sampled message indices used by $\ablpolicy$ at all steps.
% % \end{corollary}

==> fig_food_k_cont.tex <==
\begin{figure}[h]
 \centering
 \begin{subfigure}[t]{0.49\textwidth}
 \centering
  \input{figs/FoodCollector_Ablation_k_2adv_cont}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\textwidth}
 \centering
  \input{figs/FoodCollector_Ablation_k_sample_cont}
 \end{subfigure}
%  \vspace{-2em}
%  \subcaption{Continuous Action Space}
\vspace{-0.8em}
\caption{Hyper-parameter test in continuous-action FoodCollector. \textbf{Left:}  Natural and robust performance with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. Dashed green line refers to Vanilla under $C=2$ attacks.}
\vspace{-0.5em}
\label{fig:res_k_cont}
\end{figure}


==> fig_food_k_dist.tex <==
\begin{figure}[h]
\vspace{-0.5em}
\hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.49\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_dist}}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_sample_dist}}
 \end{subfigure}
%  \vspace{-1em}
%  \subcaption{Continuous Action Space}
% \vspace{-1em}
\caption{Hyper-parameter test in discrete-action FoodCollector. \textbf{Left:}  Natural and robust performance with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. Dashed green line refers to Vanilla under $C=2$ attacks.}
\vspace{-1.5em}
\label{fig:res_k_dist}
\end{figure}


==> fig_food_res.tex <==
\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.49\columnwidth}
  \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist_naive}}
  \vspace{-1.5em}
  \caption{Discrete \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Dist}}
  \vspace{-1.5em}
  \caption{Discrete \& Adaptive}
 \end{subfigure}
 \\
 %\hfill
 \begin{subfigure}[t]{0.49\columnwidth}
   \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Attacker_Cont_naive}}
  \vspace{-1.5em}
  \caption{Continuous \& Non-adaptive}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\columnwidth}
  \resizebox{\textwidth}{!}{ \input{figs/FoodCollector_Attacker_Cont}}
  \vspace{-1.5em}
  \caption{Continuous \& Adaptive}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Reward comparison between our \ours and baselines in FoodCollector with discrete/continuous action space, under no attacker or non-adaptive/adaptive attacks under varying numbers of adversaries. Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_all}
\end{figure}





==> fig_market_k_dist.tex <==

\begin{figure}[h]
 \centering
 \begin{subfigure}[t]{0.49\textwidth}
 \centering
  \input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.49\textwidth}
 \centering
  \input{figs/MarketEnv/MarketEnv_Ablation_K_sampleD}
 \end{subfigure}
%  \vspace{-2em}
%  \subcaption{Continuous Action Space}
\vspace{-0.8em}
\caption{\textbf{MarketEnv} Hyper-parameter test in continuous-action MarketEnv. \textbf{Left:}  Natural and robust performance with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. Dashed green line refers to Vanilla under $C=2$ attacks.}
\vspace{-0.5em}
\label{fig:res_k_cont_market}
\end{figure}




 

==> fig_market_res.tex <==
\begin{figure}[!h]
\vspace{-0.5em}
 \centering
%  \hspace{-1em}
 \begin{subfigure}[t]{0.35\textwidth}%{0.49\columnwidth}
  \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_adaptive}}
  \vspace{-1.5em}
  \caption{Adaptive Attack}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.35\textwidth}%{0.49\columnwidth}
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_permute}}
  \vspace{-1.5em}
  \caption{Non-adaptive (\permute)}
 \end{subfigure}
 \\
 %\hfill
 \begin{subfigure}[t]{0.35\textwidth}%{0.49\columnwidth}
   \resizebox{\linewidth}{!}{\input{figs/MarketEnv/MarketEnv_Attacker_Dist_flip}}
  \vspace{-1.5em}
  \caption{Non-adaptive (\swap)}
 \end{subfigure}
 %\hfill
 \begin{subfigure}[t]{0.35\textwidth}%{0.49\columnwidth}
  \resizebox{\linewidth}{!}{ \input{figs/MarketEnv/MarketEnv_Attacker_Dist_swap}}
  \vspace{-1.5em}
  \caption{Non-adaptive (\flip)}
 \end{subfigure}
 \vspace{-0.5em}
\caption{\textbf{MarketEnv}: Reward comparison between our \ours and baselines with continuous action space, under no attacker and varying numbers of adversaries for (a) adaptive and (b), (c) non-adaptive attacks. Dashed red line shows the performance without communication. For \ours, the ablation size $k$ is set as 2.}
\vspace{-0.5em}
\label{fig:res_all_market}
\end{figure}





==> figs/dist_n.tex <==
% This file was created with tikzplotlib v0.9.12.
\definecolor{color0}{rgb}{0.917647058823529,0.917647058823529,0.949019607843137}
\definecolor{color1}{rgb}{0.56078431372549,0.737254901960784,0.56078431372549}
\definecolor{color2}{rgb}{1,0.388235294117647,0.27843137254902}
 
\draw[draw=black,fill=color1] (axis cs:-0.1,0) rectangle (axis cs:0.1,86.55);
\draw[draw=black,fill=color1] (axis cs:0.9,0) rectangle (axis cs:1.1,31.58);
\draw[draw=black,fill=color1] (axis cs:1.9,0) rectangle (axis cs:2.1,14.73);
\draw[draw=black,fill=color1] (axis cs:2.9,0) rectangle (axis cs:3.1,12.56);
\draw[draw=black,fill=color2] (axis cs:0.1,0) rectangle (axis cs:0.3,74.19);
\draw[draw=black,fill=color2] (axis cs:1.1,0) rectangle (axis cs:1.3,73.72);
\draw[draw=black,fill=color2] (axis cs:2.1,0) rectangle (axis cs:2.3,71.91);
\draw[draw=black,fill=color2] (axis cs:3.1,0) rectangle (axis cs:3.3,43.27);
\addplot [semithick, green!50!black, mark=*, mark size=3, mark options={solid}]
table {%
0 86.55
1 31.58
2 14.73
3 12.56
};
\addlegendentry{vanilla training}
\addplot [semithick, red, mark=square*, mark size=3, mark options={solid}]
table {%
0.2 74.19
1.2 73.72
2.2 71.91
3.2 43.27
};
\addlegendentry{randomized ablation $(k=2)$}


==> neurips/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% \draft{We study the attacks and defenses in communicative multi-agent reinforcement learning.
% Our contributions:
% 1. formulate the adversarial problem in CMARL.
% 2. propose a certifiable defense algorithm
% 3. empirical study in a simulated game and a market environment.
% }
% Recent years have witnessed significant advances in reinforcement learning (RL), especially deep reinforcement learning (DRL). Although vanilla RL considers the interaction between a single agent and the environment, many real-world applications have multiple agents involved, such as autonomous driving~\cite{shalev2016safe}, robotics~\cite{dudek1996taxonomy}, etc. 
% \ys{start from decision making?}
% With the rapid improvement of deep reinforcement learning (DRL) techniques, neural network-based 
Neural network-based multi-agent reinforcement learning (MARL) has achieved significant advances in many real-world applications, such as autonomous driving~\cite{shalev2016safe,sallab2017deep}. In a multi-agent system, especially in a cooperative game, communication usually plays an important role. By feeding communication messages as additional inputs to the policy network, each agent can obtain more information about the environment and other agents, and thus can learn a better policy~\cite{foerster2016learning,hausknecht2016cooperation,sukhbaatar2016learning}. 
% Many recent works~\cite{foerster2016learning,hausknecht2016cooperation,sukhbaatar2016learning} have shown that feeding communication messages to RL networks can result in better decision makers.

However, neural networks are shown to be vulnerable to adversarial attacks~\cite{chakraborty2018adversarial}, i.e.,
% , especially network-based RL policies~\cite{huang2017adversarial} \fh{network-based RL policies are not a special case of neural networks. So the logic here is a bit unsmooth.}, 
a well-trained network may output a wrong answer if the input to the network is slightly perturbed~\cite{goodfellow2014explaining}.
% if the inputs to the network are slightly but deliberately perturbed, the network, although well-trained on clean datasets \fh{rather than datasets, shall we say unattacked environment or safe environment, since RL is not necessarily trained on a ``dataset''?}, may output a wrong answer. 
As a result, although a policy can obtain a high reward by taking in the messages sent by other agents, it may also get drastically misled by inaccurate information or even adversarial communication from malicious attackers. 
For example, when several drones execute pre-trained policies and exchange information via wireless communication, it is possible that messages get noisy in a hostile environment, or even some malicious attacker eavesdrops on their communication and intentionally perturbs some messages to a victim agent via cyber attacks. 
Moreover, even if the communication channel is protected by advanced encryption algorithms, an attacker may also hack some agents and alter the messages before they are sent out (e.g. hacking IoT devices that usually lack sufficient protection~\cite{naik2017cyber}). Figure~\ref{fig:diagram} shows an example of communication attacks, where the agents are trained with benign communication, but attackers may perturb the communication during the test time. The attacker may lure a well-trained agent to a dangerous location through malicious message propagation and cause fatal damage. 
Although our paper focuses on adversarial perturbations of the communication messages, it also includes unintentional perturbations, such as misinformation due to malfunctioning sensors or communication failures; these natural perturbations are no worse than adversarial attacks.

\begin{figure*}[!t]
\vspace{-3em}
    \centering
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{figs/marl.pdf}
         \vspace{-0.5em}
         \caption{Training time}
         \label{sfig:train}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{figs/marl_adv.pdf}
         \vspace{-0.5em}
         \caption{Test time (in deployment)}
         \label{sfig:test}
     \end{subfigure}
     \vspace{-0.5em}
    \caption{An example of test-time communication attacks in a communicative MARL system.  (a) During training, agents are trained collaboratively in a safe environment, such as a simulated environment. (b) In deployment, agents execute pre-trained policies in the real world, where malicious attackers may modify the benign ({\color{darkpastelgreen}{green}}) messages into adversarial ({\color{red}{red}}) signals to mislead some victim agent(s). 
    % \myst{In this figure, arrows denote communication channels among agents, {\color{darkpastelgreen}{green}} messages stand for benign communication, and {\color{red}{red}} messages stand for adversarial communication.}
    % \myst{Agents can be heterogeneous as depicted by various icons.}
    }
    \label{fig:diagram}
\vspace{-2em}
\end{figure*}

Although adversarial attacks and defenses have been extensively studied in supervised learning~\cite{madry2018towards,cohen2019certified,zhang2019theoretically} and reinforcement learning~\cite{zhang2020robust,zhang2021robust,oikarinen2020robust}, there has been little discussion on the robustness issue against adversarial communication in MARL problems. 
Therefore, to safely improve decision-making with communication in high-stakes multi-agent scenarios, it is crucial to robustify MARL policies against adversarial communication.  
% \textcolor{red}{Defending against the adversarial communication while still utilizing the benign communication}\fh{needs rewording. Maybe: Achieving high performance in a multi-agent cooperative game through inter-agent communication while remain robust to adversarial communication attacks} 
Achieving high performance in a multi-agent cooperative game through inter-agent communication while being robust to adversarial communication is a challenging problem due to the following reasons. 
\textbf{Challenge I}: 
% \myst{The attacker may construct malicious messages in various ways, so that they are hard to be distinguished from benign messages.} 
% \myst{For example, the malicious messages shown in Figure}~\ref{sfig:test} \myst{are in the same form as the benign messages and also make semantic sense.}
Sometimes communication attacks are stealthier as misleading
messages  (which share the form of benign messages and are semantically meaningful in Figure~\ref{sfig:test}) can be hard to recognize, while attacking by abnormal actions~\cite{gleave2020adversarial} can be easier for humans to notice.
\textbf{Challenge II}: A strong attacker can even be \textit{adaptive} to the victim agent and significantly reduce the victim's total reward. For instance, for a victim agent who moves according to the average of GPS coordinates sent by others, the attacker may learn to send extreme coordinates to influence the average.
% the attacker may learn an RL policy to send sequential misleading messages. \fh{This point is not very clear.}
\textbf{Challenge III}: There can be more than one attacker (or an attacker can perturb more than one message at one step), such that they can collaborate to mislead a victim agent.

Tu et al.~\cite{tu2021adversarial} apply adversarial training~\cite{madry2018towards} to improve model robustness against communication perturbations. But they focus on perturbations with small $\ell_p$ distances, which do not cover many attack scenarios as discussed in Section~\ref{sec:setup_adv}.
Some recent works~\cite{blumenkamp2020emergence,xue2021mis,mitchell2020gaussian} take the first step to investigate adversarial communications in MARL and propose several defending methods, such as a learned message filter~\cite{xue2021mis}. However, these empirical defenses do not fully address the aforementioned challenges, and are not guaranteed to be robust, especially under adaptive attacks. 
% \textcolor{purple}{PH: all communication attacks, any communication attack? YS: should be all, thanks} 
%\textcolor{purple}{PH: Is it clear what we mean by adaptive attacks? In challenge 2 we are kind of defining it. Would it make sense to make the \textit{adaptive} italic in challenge 2 to stand out? YS: Sure! Good point}
% Levine et al.~\cite{Levine_Feizi_2020} use randomized ablation to defend against sparse attacks in image classification, where a fraction of pixels may be corrupted. However, their high-probability guarantee is not suitable for sequential decision-making problems, as the guaranteed probability decreases along propagation over time. Moreover, their algorithm does not work when the policy takes continuous actions. 

In this paper, we address all aforementioned challenges by proposing {a certifiable defense, named \textbf{\oursfull (\ours)}, that can guarantee the performance of agents when a fraction of communication messages are perturbed}. 
The main idea of \ours is to make decisions based on multiple different subsets of communication messages (i.e., ablated messages). Specifically, for a list of messages coming from different agents, we train a \emph{\ablname} that takes in a subset of messages and outputs a \emph{base action}. Then, we construct an \emph{\ensname} by aggregating multiple base actions coming from multiple ablated message subsets. 
% The main idea of \ours is to construct an \emph{ensemble policy} which makes decisions based on multiple different subsets of communication messages (i.e., ablated messages). 
% Specifically, for a list of messages coming from different agents, we train a \emph{base ablation policy} that takes in a subset of messages and outputs a \emph{base action}. 
For a discrete action space, the ensemble policy takes the majority of the multiple base actions obtained, while for a continuous action space, the ensemble policy takes the median of these base actions. \ours is a generic framework that works for any agent that observes multiple messages from different sources, as long as the agent receives more benign communication messages than adversarial ones. We also show in Section~\ref{sec:algo_more} that \ours can be used in many other decision-making scenarios beyond defending against communication attacks. 
A similar randomized ablation idea is used by Levine et al.~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification. However, they provide high-probability guarantee for a single-step decision, which is not suitable for sequential decision-making problems, as the guaranteed probability decreases when it propagates over timesteps. Moreover, their algorithm does not work when the model has a continuous output space. 
In contrast, \ours has robustness guarantees for both the immediate action and the long-term reward, and for both discrete and continuous actions. 
% A similar randomized ablation idea is used by Levine et al.~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification. However, their high-probability guarantee is not suitable for RL \fh{sequential decision-making} problems, as the probability decreases along propagation over time. Moreover, their algorithm does not work for a continuous action space. In contrast, \ours has robustness guarantees for the long-term reward, and works on both discrete and continuous action spaces. 

% \ys{compare to Levine et al. high probability reduces along propagation of time / may not lead to reliable multi-step robustness due to the long horizon.}
% Therefore, \ours can be extended to defend against 
% \ys{flexibility, as discussed later}

Our contributions can be summarized as below:\\
\textbf{(1)} We formulate the problem of adversarial attacks and defenses in communicative MARL (CMARL). \\
% \fhc{Do we still use CMARL? If not, it is fine. If so, explain it.}.\\
\textbf{(2)} We propose a novel defense method, \ours, 
% \SF{perhaps introduce ``ablation" terminology in the previous paragraph so readers become familiar with it at this point}
% based on randomized ablation on communication messages. \ours 
that is certifiably robust against arbitrary perturbations of up to $C<\frac{N-1}{2}$ communications, where $N$ is the number of agents. \\
% both in discrete action space and in continuous action space. \fh{I feel the contribution is not that we include both discrete or continuous action space, but rather, we can achieve very strong results in the discrete space, as well as good results in the continuous space. I feel the current wording sounds a bit off the path.}\\
\textbf{(3)} Experiment in several multi-agent environments shows that \ours obtains significantly higher reward than baseline methods under both non-adaptive and adaptive attackers. 
% The agent trained with \ours achieves similar 
% \SF{add a bit more details here; what environments; discrete or cont; what gains do we achieve?}. 
% \fh{maybe some numbers in terms of performance improvement etc}



==> neurips/2_relate.tex <==
\vspace{-0.5em}
\section{Related Work}
\label{sec:relate}


\textbf{Adversarial Robustness of RL Agents}\quad
% As RL techniques have been applied to more and more applications, the robustness of agents under environment noise or adversarial attacks becomes an emerging research topic. 
Section~\ref{sec:setup_adv} introduces several adversarial attacks on single-agent and multi-agent problems.
To improve the robustness of agents, adversarial training (i.e., introducing adversarial agents to the system during training~\cite{pinto2017robust,phan2021resilient,zhang2021robust,sun2021strongest}) and network regularization~\cite{zhang2020robust,shen2020deep,oikarinen2020robust} are empirically shown to be effective under $\ell_p$ attacks, although such robustness is not theoretically guaranteed. 
Certifying the robustness of a network is an important research problem~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness}.
% There is an important line of work studying guaranteed robustness of neural networks~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness} when the input data is perturbed within an $\ell_p$ norm ball. 
In an effort to certify RL agents' robustness, some approaches~\cite{lutjens2020certified,zhang2020robust,oikarinen2020robust,fischer2019online} apply network certification tools to bound the Q networks and improve the worst-case value of the policy. Kumar et al.~\cite{kumar2021policy} and Wu et al.~\cite{wu2021crop} follow the idea of randomized smoothing~\cite{cohen2019certified} and smooth out the policy by adding Gaussian noise to the input.




\textbf{Adversarial Attacks and Defenses in CMARL}\quad
Appendix~\ref{app:related} discusses some related works on learning effective communication among agents~\cite{foerster2016learning,sukhbaatar2016learning,das2020tarmac}. 
Recently, the problem of adversarial communication in MARL has attracted increasing attention.  
Blumenkamp et al.~\cite{blumenkamp2020emergence} show that in a cooperative game, communication policies of some self-interest agents can hurt other agents' performance. 
% To accommodate multiple agent objectives, they propose \change{Aggregation}\fh{aggregated? is aggregation GNN a terminology? I've not heard of it.} Graph Neural Networks to model and learn an inter-agent communication policy. 
To achieve robust communication, Mitchell et al.~\cite{mitchell2020gaussian} adopt a Gaussian Process-based probabilistic model to compute the posterior probabilities that whether each partner is truthful. 
Tu et al.~\cite{tu2021adversarial} investigate the vulnerability of multi-agent autonomous systems against communication attacks, with a focus on vision tasks.
% \change{multiple aspects} \fh{?}.
Xue et al.~\cite{xue2021mis} propose an algorithm to defend against one adversarial communication message by an anomaly detector and a message reconstructor, which are trained with groundtruth labels and messages.

To the best of our knowledge, our \ours is the first certifiable defense in MARL against communication attacks. Moreover, we consider a strong threat model where up to half of the communication messages can be arbitrarily corrupted, capturing many realistic types of attacks.

% In comparison, we focus on a different and strong threat model where a fraction of communication messages are arbitrarily corrupted, capturing many realistic types of attacks. Our proposed defense has certifiable performance and achieves strong robustness in experiments.

% A similar randomized ablation defense is used to defend against $\ell_0$ attacks in image classification~\cite{Levine_Feizi_2020}.
% But our defensive mechanism is fundamentally different from the image classification defense~\cite{Levine_Feizi_2020} which provides a high-probability guarantee for discrete image label outputs, as our defense achieves both action and long-term reward certification (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output, which is non-trivial.

% Levine et al.~\cite{Levine_Feizi_2020} propose a similar defense based on randomized ablation against $\ell_0$ attacks in image classification.
% But our defense and theoretical results are fundamentally different and non-trivial extensions of this work~\cite{Levine_Feizi_2020}.
% Levine et al.~\cite{Levine_Feizi_2020} provide a high-probability guarantee for discrete image label outputs, while our defense achieves both action and reward certificates (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output.


% formulates adversarial attacks in a general \fh{are previous works not generic? Why?}communicative MARL (CMARL) setting, and 
% \fh{Is \cite{xue2021mis} attack agnostic? The current description doesn't answer this question.}.


% This threat model can cover many realistic attacking scenarios that the $\ell_p$ model does not solve.

% This paper \myst{is also closely related to} \fh{bears some similarities with}~\cite{gleave2020adversarial}, which studies the effects of adversarial actions in an MARL problem. In contrast, our work aims to defend against communication attacks that can be more stealthy in practice.
% Randomized ablation is proposed by~\cite{Levine_Feizi_2020} to defend against $\ell_0$ attacks in image classification problems, in which the classifier is trained by randomly ablating pixels of images. 
% We are the first to extend the idea of randomized ablation to MARL and to achieve action and reward certificates against communication attacks.
% Note that the number of pixels in an image and the number of agents in an MARL problem are in different scales. Also, a classifier outputs discrete labels, while a policy may have discrete or continuous output space. Therefore, our problem setup, methodology and theoretical results are significantly different from~\cite{Levine_Feizi_2020} and are novel.

% \textbf{parameter sharing} Sharing parameters are a common way to take advantage of centralized training \cite{lowe2017multi,foerster2016learning} by learning a single shared critic network for multiple agents. \cite{gupta2017cooperative} uses single-agent RL methods to learn policies in cooperative environments.

==> neurips/4_algo_short.tex <==
\section{Provably Robust Defense for CMARL}
\label{sec:algo}

In this section, we present our defense algorithm, \textit{\oursfull (\ours)}, against test-time communication attacks in CMARL. 
% \ours has two phases: the training phase where a base policy is trained for each agent we aim to robustify, and the defending phase where the base policy is used to make
% relatively safe
% decisions via message ablation and ensemble.  
We first introduce the algorithm design in Section~\ref{sec:algo_overview}, then present the theoretical analysis in Section~\ref{sec:algo_theory}.
Section~\ref{sec:algo_more} discusses several extensions of \ours.


\subsection{\oursfull (\ours)}
\label{sec:algo_overview}

% \SF{In the intro, we call the method ensemble policy; we should use the same terminology. I like AME} >> Sure, I added AME to the intro.
% As characterized in Section~\ref{sec:setup}, in a CMARL game, every agent makes decisions based on not only its own observations, but also all received messages. If an agent trusts the communication from all other agents, it may fail when some communication is maliciously corrupted.
% On the other hand, if an agent does not trust communication, it can not benefit from the useful information shared by other benign agents.
% Therefore, there is a trade-off between natural performance (i.e., reward under no attack) and robustness (i.e., reward under attacks).
% Our goal is to learn and execute a robust policy for any agent in the environment, so that the agent can perform well in both a non-adversarial environment and an adversarial environment.


% \textbf{Main Idea}\quad
% Intuitively, if an agent $i$ overly relies on the information given by agent $j$, then a strong adaptive attacker can easily mislead $i$ by perturbing the messages from $j$. On the other hand, if an agent does not trust communication, it can not benefit from the useful information shared by other benign agents.
% Therefore, there is a trade-off between natural performance (i.e., reward under no attack) and robustness (i.e., reward under attacks). 
% 
Our goal is to learn and execute a robust policy for any agent in the environment, so that the agent can perform well in both a non-adversarial environment and an adversarial environment. 
To ease the illustration, we focus on robustifying an arbitrary agent $i\in\agents$, and the same defense is applicable to all other agents.
We omit the agent subscript ${}_i$, and denote the agent's observation space, action space, and interaction history space as $\mathcal{O}$, $\mathcal{A}$, and $\hisspace$, respectively. 
% We aim to train a robust acting policy for the agent as $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$, where $\hisspace$ is the space of the interaction histories.

Let $\msg \in \mathcal{M}^{N-1}$ denote a set of $N-1$ messages received by the agent. Then, we can build an ablated message subset of $\msg$ with $k$ randomly selected messages, as defined below.

\begin{definition}[$\boldsymbol{k}$-Ablation Message Sample (k-Sample)]
For a message set $\msg \in \mathcal{M}^{N-1}$ and any integer $1 \leq k \leq N-1$, define a $k$-ablation message sample (or \ksample for short), $\msgk \in \mathcal{M}^k$, as a set of $k$ randomly sampled messages from $\msg$. Let $\allmsgk$ be the collection of all unique \ksamples of $\msg$, and thus $|\allmsgk|=\binom{N-1}{k}$.
\end{definition}


% \textbf{Notations}\quad
% % \textbf{(1) Agent and policy.} To ease the illustration, we focus on robustifying an arbitrary agent $i\in\agents$, and the same defense is applicable to all other agents.
% % We omit the agent subscript ${}_i$, and denote the agent's observation space and action space as $\mathcal{O}$ and $\mathcal{A}$. We aim to train a robust acting policy for the agent as $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$, where $\hisspace$ is the space of the interaction histories.  \\
% \textbf{(1) Ablated $k$ message samples (k-samples) $\boldsymbol{\msgk}$.} 
% Let $\msg \in \mathcal{M}^{N-1}$ denote a set of messages received by the agent with cardinality $N-1$. For any $1 \leq k \leq N-1$, define a $k$ message sample (or k-sample for short) $\msgk \in \mathcal{M}^k$ as a set of $k$ messages randomly sampled from $\msg$. \\
% \textbf{(2) All k-sample Combinations $\boldsymbol{\allmsgk}$.} 
% Among all $N-1$ messages in $\msg$, there are $\binom{N-1}{k}$ unique k-samples. Let $\allmsgk$ be the collection of all unique k-samples of $\msg$.

% Moreover, the benign messages sent from other agents usually contain redundant/overlapping information.
% \myst{, as the goal of communication is to provide the agent additional information and to help the agent make better decisions. }
Motivated by the fact that the benign messages sent from other agents usually contain overlapping information that may suggest similar decisions, the \textbf{main idea} of our defense is to make decisions based on the \emph{consensus} of the benign messages. 
To be more specific, we train a base policy that makes decisions with one \ksample at each step. During test time when communication messages can be perturbed, the agent collects multiple \ksamples at every step, and applies the trained base policy to each \ksample to get multiple resulting base actions. Then, the agent selects the action that reflects the majority opinion. By carefully designed ablation and ensemble strategies, we can ensure that the majority of these base actions is dominated by benign messages.
% , even if there exist $C$ adversarial messages.

% By a careful design of , the agent is guaranteed to make a ``good'' decision if it takes a collection of wisdom from the ensemble of all resulting actions, since the majority of these resulting actions are guaranteed to be dominated by benign messages.
% For a message set $\msg$, our proposed \ours 

% where a base policy is trained in a clean environment to act according under a random \ksample, and the testing/defending phase where the communications may be perturbed, uses the trained base policy by aggregating multiple \ksamples.



% % and the set has $N-1$ elements, each is a message received. 
% Our defense makes decisions based on multiple random subsets of this message set, called \emph{randomly-ablated message samples} (or \textit{m-samples} for short).
% Under a carefully designed ablation mechanism, benign m-samples can outweigh malicious ones.
% To be more specific, we train a \emph{base policy} that makes decisions with one 
% % \myst{randomly selected subset of the message set} 
% m-sample at each step. 
% Note that agents are trained without any attacks, such that the base policy learns to behave under purely-benign m-samples.
% Then, during test-time where communication messages can be perturbed, the agent generates multiple m-samples at every step.
% % One can design an ablation strategy which guarantees that a majority number of these m-samples contain no malicious messages.
% Then the agent applies the trained base policy to  
% % \myst{randomly ablated messages, and aggregate the base-policy actions by sampling multiple message combinations, so that the agent can make safe decisions with theoretical guarantees.}
% each of these m-samples, getting multiple resulting actions where the majority of them are generated based on benign messages only. 
% % The majority of these resulting actions are based on benign messages only and thus safe. 
% Therefore, the agent is guaranteed to make a ``good'' decision if it takes a collection of wisdom from the ensemble of all resulting actions, since the majority of these resulting actions are guaranteed to be dominated by benign messages.
% \myst{guided by} benign \myst{messages}.


% A similar randomized ablation defense is used to defend against $\ell_0$ attacks in image classification~\cite{Levine_Feizi_2020}. 
% But our defensive mechanism is fundamentally different from the image classification defense~\cite{Levine_Feizi_2020} which provides a high-probability guarantee for discrete image label outputs, as our defense achieves both action and long-term reward certification (i.e., robustness always holds rather than holding with high probability) for both discrete action output and continuous action output, which is non-trivial.


With the above intuition, we propose \oursfull (\ours), a generic defense framework that can be fused with any policy learning algorithm. 
% We first introduce some important notations for the algorithm.
% shown in Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test}, respectively, in Appendix~\ref{app:algo}. 
\ours has two phases: the training phase where agents are trained in a clean environment, and a testing/defending phase where communications may be perturbed. 
The training and defending strategies of \ours are illustrated below, and the pseudocode is shown by Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test} in Appendix~\ref{app:algo}.

\textbf{Training Phase with \ablnamecap $\boldsymbol\ablpolicy$ (Algorithm~\ref{alg:train})}\quad
During training time, the agent learns a \textit{\ablname} $\ablpolicy: \hisspace \times \mathcal{M}^k \to \mathcal{A}$ which maps its own interaction history $\his$ and a random \ksample $\msgk\sim \mathrm{Uniform}(\allmsgk)$ to an action, where $\mathrm{Uniform}(\allmsgk)$ is the uniform distribution over all \ksamples from the message set $\msg$ it receives.
% i.e., $a\step \sim \ablpolicy(\his\step,\msgk\step)$.
% $a\sim\ablpolicy(\his, \mathsf{Ablate}(\msg, T))$, where $T\in\mathcal{H}(N-1,k)$.
Here $k$ is a user-specified hyperparameter selected to satisfy certain conditions, as discussed in Section~\ref{sec:algo_theory}. 
The training objective is to maximize the cumulative reward of $\ablpolicy$ based on randomly sampled \ksamples in a non-adversarial environment. Any policy optimization algorithm can be used for training.
% Since all messages lie in the same message space $\mathcal{M}$, each agent only needs to learn a single ablation policy.
% which achieves as high reward as possible based on randomly sampled $k$ messages. 

% \fhc{Section 4.2 doesn't explain this specific hyperparameter.}
% Equation~\eqref{eq:k_cond} plays an important role in our robustness guarantees shown in Section~\ref{sec:algo_theory}.
% % Note that attacks do not exist during training.
% In every step, an agent randomly samples $k$ out of $N-1$ benign communication messages, and uses its current acting policy $\ablpolicy$ to take an action based on its observation history and the selected $k$ messages.
% react to its current observation and the selected $k$ messages (Line 7 in Algorithm~\ref{alg:train}). 
% Therefore, we optimize and make decisions via $\ablpolicy(\his, \mathsf{Ablate}(\msg, T))$, where $\mathsf{Ablate}(\msg, T)$ denotes the selected $k$ messages sent from other agents to agent $i$. 



\textbf{Defending Phase with \ensnamecap $\boldsymbol\smpolicy$ (Algorithm~\ref{alg:test})}\quad
Once we obtain a reasonable \ablname $\ablpolicy$, we can execute it with ablation and aggregation during test time to defend against adversarial communication. 
The main idea is to collect all possible \ksamples from $\allmsgk$, and select an action suggested by the majority of those \ksamples. 
Specifically, we construct a \textit{\ensname} $\smpolicy: \hisspace \times \mathcal{M}^{N-1} \to \mathcal{A}$ that outputs an action by aggregating the base actions produced by $\ablpolicy$ on multiple \ksamples (Line 5 in Algorithm~\ref{alg:test}). 
The construction of the \ensname depends on whether the agent's action space $\mathcal{A}$ is discrete or continuous, which is given below by Definition~\ref{def:ensemble_dist} and Definition~\ref{def:ensemble_cont}, respectively. 
% For notation simplicity, the definitions only focus on one agent (although our defense works for multiple agents) and omit the subscript $i$. We further use $\mathbf{m}$ to denote the message list $\mtoi$ received by the current agent at the current step. 
% The \ensname $\smpolicy_i$ depends on whether the action space $\mathcal{A}_i$ is discrete or continuous, 
% which will be detailed in Section~\ref{sec:algo_dist} and Section~\ref{sec:algo_cont}, with corresponding theoretical guarantees on actions and rewards.
% \textcolor{purple}{PH: would it help mentioning $\smpolicy_i: \mathcal{O}_i \times \mathcal{M}^{N-1} \to \mathcal{A}_i$?}

% \fhc{Shall we put the test algorithm back?}

\begin{definition}[\ensnamecap for Discrete Action Space]
\label{def:ensemble_dist}
For a \ablname $\ablpolicy$ with observation history $\his$ and received message set $\msg$, define the \ensname $\smpolicy$ as
\begin{equation}
\label{eq:ensemble_pi_dist}
    \smpolicy(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)=a].
\end{equation}
\end{definition}

% \begin{definition}[\textbf{\ensnamecap for Discrete Actions}]
% \label{def:ensemble_dist}
% For a \ablname $\ablpolicy$ with observation history $\his$, define $u_a$ as the number of times/votes such that the \ablname $\ablpolicy$ renders action $a$ when taking each of \ksamples in $\allmsgk$, i.e.,
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:vote}
%     u_a := \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)].
%     % u_a := \sum\nolimits_{T\in\mathcal{H}(N-1,k)} \mathbbm{1}[\ablpolicy(\his, \funabl(\mathbf{m}, T))=a].
% \end{equation}
% Then the \ensname $\smpolicy$ takes the action with the most votes, i.e.,
% \begin{equation}
% \label{eq:ensemble_pi_dist}
%     \smpolicy(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \; u_a
% \end{equation}
% % \fh{How about $\tilde{a} = \smpolicy\Big(o, \{\funabl(\mathbf{m}, T_d)\}_{d=1}^D\Big) := \mathrm{ argmax}_{a\in\mathcal{A}} \; u_a.$?}
% \end{definition}

\begin{definition}[\ensnamecap for Continuous Action Space]
\label{def:ensemble_cont}
For a \ablname $\ablpolicy$ with observation history $\his$ and received message set $\msg$, define the \ensname $\smpolicy$ as
\begin{equation}
\label{eq:ensemble_pi_cont}
    \tilde{\pi}(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \msgk): \msgk\in\allmsgk \},
    % \tilde{\pi}(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \funabl(\mathbf{m}, T): T\in\mathcal{H}(N-1,k) \},
\end{equation}
where $\funmed$ is a function that returns the element-wise median value of a set of vectors.
\end{definition}

% Recall that there are up to $C$ malicious messages out of $N-1$ total messages, and at least $N-1-C$ benign messages. 
Therefore, the \ensname $\smpolicy$ takes the action suggested by the consensus of all \ksamples (majority vote in a discrete action space, and median action for a continuous action space). We will show in the next section that, with some mild conditions, 
% the performance of $\smpolicy$ under adversarial communications is certifiable. 
$\smpolicy$ under adversarial communications works similarly as the \ablname $\ablpolicy$ under all-benign communications.
% , with mild assumptions \fhc{note}.

\textbf{Computation Complexity of \ours}\quad
Different from many model-ensemble methods~\cite{kurutach2018modelensemble,harutyunyan2014shaping} that learn multiple network models, \emph{we learn a single policy $\ablpolicy$ during training, and use a single policy $\smpolicy$ during testing.}
Therefore, the training process does not require extra computations compared to the original policy learning method.
In the defending phase, we aggregate decisions from $\binom{N-1}{k}$ \ksamples, which require $\binom{N-1}{k}$ forward passes through $\ablpolicy$. 
Note that $\binom{N-1}{k}$ is generally small, because the number of agents in practical multi-agent problems is usually small (e.g., the number of drones in an area). 
For example, when $N=10,k=2$, $\binom{N-1}{k}=36$.
In the case where $\binom{N-1}{k}$ is large, we provide a variant of the algorithm in Section~\ref{sec:algo_more}, which takes $D$ \ksamples for $D\leq\binom{N-1}{k}$.
Then the certificate of \ours becomes a high-probability guarantee, depending on the value of $D$.
% The defense objective is to make a \textit{\myst{safe} \fh{benign} decision} that is robust to malicious massages. 


% Note that the ensemble policy $\smpolicy$ takes the action suggested by the consensus of all size-$k$ message subsets (majority vote in a discrete action space, and median action for a continuous action space). 
% There are $\binom{N-1}{k}$ number of such size-$k$ subsets in total. In many practical multi-agent problems, $N$ is not very large, e.g., the number of drones in an area. Therefore, $\binom{N-1}{k}$ is relatively small and not expensive to compute. For example, when $N=10,k=2$, $\binom{N-1}{k}=36$.
% In the case where $\binom{N-1}{k}$ is large, we also provide a variant of the algorithm which takes $D<\binom{N-1}{k}$ samples of message subsets whose certification guarantee is provided in Section~\ref{sec:algo_more}.

\subsection{Robustness Certificates of \ours}
\label{sec:algo_theory}


% Our defense lets an agent make decisions based on multiple size-$k$ random subsets of all messages in $\mathbf{m}$. 
In this section, we provide theoretical guarantees for the robustness of \ours.
During test time, at any step, let $\his$ be the interaction history, $\goodmsg$ be the unperturbed benign message set, and $\advmsg$ be the perturbed message set. 
% $\goodmsg$ be the benign messages (before attack), and $\advmsg$ be the messages after attack (with up to $C$ messages being corrupted). 
Note that $\goodmsg$ and $\advmsg$ both have $N-1$ messages while they differ by up to $C$ messages. 
With the above notation, we define a set of actions rendered by purely benign \ksamples in Definition~\ref{def:safeact_dist}. As the agent using a well-trained \ablname is likely to take these actions in a non-adversarial environment, they can be regarded as ``good'' actions to take. 

\begin{definition}[Benign Action Set $\safeaction$]
\label{def:safeact_dist}
For the execution of the \ablname $\ablpolicy$ at any step, define $\safeaction \subseteq \mathcal{A}$ as a set of actions that $\ablpolicy$ may select under benign \ksamples.
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
\label{eq:safeact_dist}
    \safeaction := \cup_{\goodmsgk\in\goodallmsgk} \left\{\ablpolicy(\his, \goodmsgk) \right\}.
    %  \safeaction := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
\end{equation}
\end{definition}

% Since there are at most $C$ adversarial messages among the $N-1$ messages in $\advmsg$, we know that there are at least $\binom{N-1-C}{k}$ purely benign \ksamples in $\advallmsgk$. 
% For notation simplicity, let $n_1=\binom{N-1}{k}$ and $n_2=\binom{N-1-C}{k}$. That is, $n_1$ is the total number of \ksamples, while $n_2$ is the number of purely benign \ksamples. 
% In this section, we analyze the robustness guarantees of the proposed defense \ours. 
Next, we characterize a condition for the ablation size $k$, the extra hyperparameter introduced by \ours, which is important for our theoretical certificates to hold.
\begin{condition}[Dominating Benign Sample]
\label{cond:k}
The ablation size $k$ of \ours satisfies
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
    \label{eq:k_cond}
    \binom{N-1-C}{k} > \frac{1}{2} \binom{N-1}{k}.
\end{equation}
\end{condition}
\vspace{-0.5em}

\textbf{Remarks.}
(1) For the message set $\advmsg$ that has up to $C$ adversarial messages, Equation~\eqref{eq:k_cond} implies that among all \ksamples from $\advmsg$, there are more purely benign \ksamples than \ksamples that contain adversarial messages. 
(2) Under Assumption~\ref{assum:num}, this condition \textit{always has solutions }for $k$ as $C<\frac{N-1}{2}$, and $k=1$ is always a feasible solution. 
% (3) In practice, the value of $k$ is related to the trade-off between natural performance and robustness, as discussed in details in Section~\ref{sec:exp}.
% Condition~\ref{cond:k} is important for the 

In addition, for a discrete action space, the \ablname takes the action with the most votes from all \ksamples as suggested by Equation~\eqref{eq:ensemble_pi_dist}. To ensure that this action stands for the consensus of benign messages, the following condition is needed.

\begin{condition}[Confident Consensus (for discrete-action only)]
\label{cond:cons}
The highest number of votes among all actions $u_{\max}:=\max_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgk} \mathbbm{1}[\ablpolicy(\his, \msgk)=a]$ satisfies
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{0pt}
\begin{equation}
    \label{eq:u_cond}
    u_{\max} > {\small{\binom{N-1}{k} - \binom{N-1-C}{k}}} =: u_{\mathrm{adv}},
\end{equation}
where $u_{\mathrm{adv}}$ is the number of votes that adversarial messages may affect (number of \ksamples that contain at least one adversarial message). 
\end{condition}

\textbf{Remarks}.
(1) This condition ensures the consensus has more votes than the votes that adversarial messages are involved in. Therefore, when $\smpolicy$ takes an action, there must exist some purely-benign \ksamples voting for this action. 
(2) This condition is easy to satisfy when $C \ll N$ as $\binom{N-1}{k} \approx \binom{N-1-C}{k}$. 
(3) This condition can be easily checked at every step of execution. 

Condition~\ref{cond:cons} considers the worst-case scenario when the adversarial messages collaborate to vote for a malicious action and outweigh benign messages in all \ksamples. 
However, such a worst-case attack is uncommon in practice as attackers are usually not omniscient. Therefore, Condition~\ref{cond:cons} is sufficient but not necessary for the robustness of $\smpolicy$ during execution. 
In real-world problems, our algorithm achieves strong robustness without requiring this condition, as verified in experiments. 


We now provide both action and reward certificates for the ensemble policy $\smpolicy$ in the discrete-action case. The analysis for a continuous action space is provided in Appendix~\ref{app:theory_cont}.

\textbf{Action Certificate for Discrete Action Space}\quad
The following theorem suggests that the ensemble policy $\smpolicy$ always takes benign actions under the above conditions no matter whether attacks exist.
\begin{theorem}[Action Certificate for Discrete Action Space]
\label{thm:main_dist}
When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold, the ensemble policy $\smpolicy$ in Definition~\ref{def:ensemble_dist} produces benign actions under $\advmsg$, i.e.,
\begin{equation}
    \widetilde{a} = \smpolicy(\his, \advmsg) \in \safeaction.
    \label{eq:cert_dist}
\end{equation}
% if the majority votes $u_{\widetilde{a}}$ satisfies $u_{\widetilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$.
% where 
% \begin{equation}
%     \safeactiondist := \cup_{T\in\mathcal{H}(N-1,k)} \left\{\ablpolicy(o, \funabl(\goodmsg, T)) \right\}.
% \end{equation}
\end{theorem}
\vspace{-0.5em}

Under Condition~\ref{cond:k} and Condition~\ref{cond:cons} which are easy to check, Theorem~\ref{thm:main_dist} certifies that $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a benign action that is suggested by some benign message combinations, even when the malicious messages are not identified. 
Then, we can further derive a reward certificate as introduced below. 
% Note that a high-probability robustness guarantee~\cite{Levine_Feizi_2020} does not 

  
\textbf{Reward Certificate for Discrete Action Space}\quad
When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold, the \ensname $\smpolicy$'s action in every step falls into a benign action set, and thus \emph{its cumulative reward under adversarial communications is also guaranteed to be no lower than the worst natural reward the base policy $\ablpolicy$ can get under random benign message subsets.} Therefore, adversarial communication under Assumption~\ref{assum:num} cannot drop the reward of any agent trained with \ours. The formal reward certificate is shown in Corollary~\ref{cor:reward_dist} in Appendix~\ref{app:theory_dist}. 


\textbf{How to Select Ablation Size $k$: Trade-off between Performance and Robustness}\quad
The ablation size $k$ is an important hyperparameter for the guarantees to hold. For a fixed $C$, both Condition~\ref{cond:k} and Condition~\ref{cond:cons} prefer a relatively small $k$ as detailed in Appendix~\ref{app:hyper}. That is, a smaller $k$ can improve the robustness in general. Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
% Condition~\ref{cond:cons} is easier to be satisfied for a smaller $k$, because $u_{\mathrm{adv}}$ increases as $k$ (verified in Appendix~\ref{app:hyper}). 
However, we also point out that a smaller $k$ restricts the power of information sharing, as the \ablname can access fewer messages in one step. Therefore, the value of $k$ is related to the \emph{trade-off between robustness and natural performance}~\cite{tsipras2018robustness,zhang2019theoretically}. 
In experiments, we use \textit{the largest $k$ satisfying Equation~\eqref{eq:k_cond}}. 
In practice, one can also train several \ablnames with different $k$'s during training, and later adaptively select a \ablname to construct a \ensname during execution (decrease $k$ if higher robustness is needed). 
% Section~\ref{sec:exp} shows ablation experiments of $k$.

% % As pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}, there exists a \textit{trade-off between robustness and accuracy}. 
% Intuitively, the more an agent trusts communications from others, the more it may benefit from additional information, but it is more exposed to the risk of being attacked. Therefore, there exists a \textit{trade-off between robustness and accuracy}~\cite{tsipras2018robustness,zhang2019theoretically}. 
% We find that the ablation size $k$ directly controls such a trade-off: when $k$ is small, the \ensname is more robust since there are much more purely-benign \ksamples than adversarial \ksamples. However, the trained \ablname may not obtain a high reward with $k$ messages.
% % In general, if $k$ is smaller, the ensemble policy is more robust. However, the base ablation policy with a smaller $k$ could gain lower reward as it throws away many messages. Therefore, there is a \textit{trade-off between robustness and accuracy}, as is pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}. 
% Therefore, we can adjust $k$ based on our practical needs.
% If we know $C$ (or an upper bound of $C$), we can set $k$ to be the largest integer satisfying Condition~\ref{cond:k} such that the natural performance is not compromised much. 
% If $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Condition~\ref{cond:k}.
% % which shows how many adversarial messages the policy can tolerate. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Condition~\ref{cond:k}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
% Experiments in Section~\ref{sec:exp} verifies our claim by an ablation study of $k$.

% and when $C$ is small, we can use a larger $k$ such that the natural performance is not compromised much. 


\vspace{-0.5em}
\subsection{Extensions of \ours}
\label{sec:algo_more}

% In this section, we discuss the effects of hyperparameter $k$, the broader applications of \ours, and an extensions of \ours for scaling up to a large number of agents.

% \textbf{Discussion on Ablation Size $\boldsymbol k$}\quad 
% As an essential condition for the certificates in Section~\ref{sec:algo_theory} to hold, Equation~\eqref{eq:k_cond} implies that among all size-$k$ message subsets, there are more purely benign subsets than subsets that contain adversarial messages. This condition \textit{always has solutions }for $k$ as $C<\frac{N-1}{2}$, and $k=1$ is always a feasible solution. In general, if $k$ is smaller, the ensemble policy is more robust. However, the base ablation policy with a smaller $k$ could gain lower reward as it throws away many messages. Therefore, there is a \textit{trade-off between robustness and accuracy}, as is pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}.
% In practice, if we know $C$ in advance, we can set $k$ to be the largest integer satisfying Equation~\eqref{eq:k_cond}. On the other hand, if $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Equation~\eqref{eq:k_cond}, which shows how many adversarial messages the policy can tolerate. 
% % For example, when $N=10$, \ours can tolerate up to $C=4$ with $k=1$, and up to $C=2$ with $k=2$. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Equation~\eqref{eq:k_cond}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages, and when $C$ is small, we can use a larger $k$ such that the natural performance is not compromised much. 



\textbf{Scaling Up: Ensemble with Partial Samples}\quad
So far we have discussed the proposed \ours defense and the constructed ensemble policy that aggregates all $\binom{N-1}{k}$ number of \ksamples out of $N-1$ messages. 
However, if $N$ is large, sampling all $\binom{N-1}{k}$ combinations of message subsets could be expensive. In this case, a smaller number of \ksamples can be used. That is, given a sample size $0<D\leq\binom{N-1}{k}$, we randomly select $D$ number of \ksamples from $\allmsgk$ (without replacement), and then we aggregate the \ablname's decisions on selected \ksamples. 
In this way, we define a partial-sample version of the ensemble policy, namely \textit{$D$-ensemble policy} $\smpolicy_D$, whose formal definition is provided in Appendix~\ref{app:theory_sample}. In this case, the robustness guarantee holds with high probability that increases as $D$ gets larger, as detailed in Theorem~\ref{thm:sample_cont} in Appendix~\ref{app:theory_sample}. 
Decreasing the hyperparameter $D$ trades some robustness guarantee for higher computational efficiency.
In our experiments, we empirically show that \ours usually works well even for a small $D$ (e.g. $D=1$).


\textbf{More Applications of \ours}\quad
The central idea of \ours is to make decisions based on the consensus instead of each individual.
Therefore, \ours can be combined with any decision-making model to work with possibly-untrustworthy information sources, not only restricted to communication attacks in CMARL. 
For example, when one collects data from multiple sources (e.g., different websites, multiple questionnaires, etc.) and some sources may contain malicious information, \ours can be used to make decisions based on the collected statistics without being significantly misled by false data.
Moreover, the idea of \ours can also be extended to detect attackers, by measuring the difference between the action suggested by any specific communication message and the ensemble policy's action, as detailed and empirically verified in Appendix~\ref{app:exp_detect}. 












% formulated as below.
% , whose detailed definition is provided in Appendix~\ref{app:theory_sample}.
% define the $D$-ensemble policy $\smpolicy_D$ as the sampled version of $\smpolicy$
% \begin{equation}
% \label{eq:ensemble_pi_dist_d}
%     \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
% \end{equation}
% for a discrete action space, and
% \begin{equation}
% \label{eq:ensemble_pi_cont_d}
%     \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% for a continuous action space. 


% \subsection{Extension of \ours: Ensemble with Partial Samples}
% \label{sec:algo_partial}

% So far we have discussed the proposed \ours algorithm and the constructed ensemble policy that aggregates all $\binom{N-1}{k}$ number of message subsets out of $N-1$ messages. 
% However, if $N$ is large, sampling all $\binom{N-1}{k}$ combinations of message subsets could be expensive. In this case, a smaller number of message-subset combinations can be used. That is, given a sample size $0<D\leq\binom{N-1}{k}$, we randomly select $D$ samples $\{T_d\}_{d=1}^D$ from $\mathcal{H}(N-1,k)$ (without replacement), and then we aggregate the ablation policy's decision on $\{\funabl(\mathbf{m}, T_d)\}_{d=1}^D$. 
% In this way, we define a sampled version of the ensemble policy, namely \textit{$D$-ensemble policy} $\smpolicy_D$, formulated as below.
% % , whose detailed definition is provided in Appendix~\ref{app:theory_sample}.
% % define the $D$-ensemble policy $\smpolicy_D$ as the sampled version of $\smpolicy$
% \begin{equation}
% \label{eq:ensemble_pi_dist_d}
%     \smpolicy_D(o, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum\nolimits_{d=1}^D \mathbbm{1}[\ablpolicy(o, \funabl(\mathbf{m}, T_d))=a],
% \end{equation}
% for a discrete action space, and
% \begin{equation}
% \label{eq:ensemble_pi_cont_d}
%     \tilde{\pi}_D(o, \mathbf{m}) = \funmed \{\ablpolicy(o, \funabl(\mathbf{m}, T_d) \}_{d=1}^D.
% \end{equation}\normalsize
% for a continuous action space. 



% In this case, we can still provide a high-probability robustness guarantee. Theorem~\ref{thm:sample_cont} shows the theoretical result for a continuous action space, while the result for a discrete action space is slightly different and is provided in Appendix~\ref{app:theory_sample}.
% % in Theorem~\ref{thm:sample_dist} and Theorem~\ref{thm:sample_cont}. 

% \begin{theorem}[General Action Guarantee for Continuous Action Space]
% \label{thm:sample_cont}
% Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$,  under Assumption~\ref{assum:num}, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_cont_d} with ablation size $k$ satisfying Equation~\eqref{eq:k_cond}, relation~\eqref{eq:cert_cont} holds with probability at least
% \begin{equation}
% \label{eq:p_sample_cont}
%     p_D=\frac{\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n_1-n_2}{D-j}}{\binom{n_1}{D}},
% \end{equation}
% where $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$ and $\tilde{D} = {\lfloor \frac{D}{2} \rfloor}+1$. 
% \end{theorem}
% Therefore, for an arbitrary $D$, a benign action will be selected with high probability. The larger $D$ is, the higher the probability is. 
% In Theorem~\ref{thm:sample_cont}, when $D=\binom{N-1}{k}$,  the probability $p_D$ is 1 and the result matches Theorem~\ref{thm:main_cont}. 
% Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.


% \subsection{More Discussion on Applicability and Flexibility of \ours}

% \ys{general for any RL policy or decision-making model}

% \ys{how a policy is trained}



% \ys{training and testing hyperparameters}



==> neurips/5_exp_temp.tex <==
\vspace{-0.5em}
\section{Empirical Study}
\label{sec:exp}

\input{\texhome/figs_all}

In this section, we verify the robustness of our \ours in multiple different CMARL environments against various communication attack algorithms. % and evaluate the hyperparameters by ablation study.
Then, we conduct hyperparameter tests for the ablation size $k$ and the sample size $D$ (introduced in Section~\ref{sec:algo_more}).




\textbf{Environments}\quad 
To evaluate the effectiveness of \ours, we consider the following environments.\\
$\bullet$ \textit{FoodCollector}: a 2D particle environment adapted from the WaterWorld task in PettingZoo~\cite{terry2020pettingzoo}. In our experiment, there are $N=9$ agents with different colors searching for foods with the same colors. Agents use their limited-range sensors to observe the surrounding objects, while communicating with each other to share their observations. The action space can be either discrete (9 moving directions and 1 no-move action), or continuous (2-dimensional vector denoting acceleration). Agents are penalized for having leftover foods at every step, so they seek to find all foods as soon as possible. \\
$\bullet$ \textit{\marketenv}: a simulator of the real-world inventory management problem. There are $N=10$ cooperative distributors carrying inventory for $3$ products. Every of $300$ buyers requests each product from a randomly selected distributor agent according to a demand distribution. The distributor agents are penalized for mismatches between their inventory and the demand for each product. Distributors can take restocking actions (continuous) to adjust their inventory at every step, and communicate with each other by exchanging their own demand observations. \\
$\bullet$ \textit{MARL-MNIST}: an MARL image classification task proposed by Mousavi et al.~\cite{mousavi2019multi} in the MNIST dataset. $N=9$ agents aim to classify an image within a limited time horizon. At every step, each agent observes a patch of the image, and can take an action to move to an adjacent patch. Agents use learned communication policies to share their encoded local beliefs with each other.
% an MARL classification task in the MNIST dataset, which is proposed by Mousavi et al.~\cite{mousavi2019multi}
% $\bullet$ \textit{MNIST-Classification}: an MARL classification framework in the MNIST dataset, proposed by Mousavi et al.~\cite{mousavi2019multi}. $N=9$ agents aim to classify an image within a limited time horizon. At every step, each agent observes a patch of the image, and can take an action to move to an adjacent patch. In the meanwhile, agents are allowed to exchange information (encoded local beliefs) with other agents to update their own beliefs. \\
% Since our focus is to defend against adversarial communication over any communication policy, we let the benign agents communicate via fixed protocols detailed in Appendix~\ref{app:exp_env}. But our method also works for learned communications, as verified by additional experiments in Appendix~\ref{app:exp_mnist}. 
The detailed description of each environment is in Appendix~\ref{app:exp_env}, where we empirically show that agents benefit a lot from benign communications in these environments.
% Therefore, different from the hand-coded communication protocols used in FoodCollector and MarketEnv, agents in this MNIST classification task use learned communication.




\textbf{Implementation and Baselines}\quad
As discussed in Section~\ref{sec:algo}, our \ours is designed to defend against communication attacks, and can be fused with any policy learning algorithm. 
In FoodCollector and \marketenv, we use PPO~\cite{schulman2017proximal} with parameter sharing~\cite{terry2020parameter} as the base policy learning algorithm as it achieves relatively high natural performance. But other more advanced MARL algorithms can be used  
(see Appendix~\ref{app:exp_results} for results of QMIX~\cite{rashid2018qmix}). 
In \mnistenv, we use the LSTM policy architecture proposed by Mousavi et al~\cite{mousavi2019multi} following the existing implementation~\cite{mnistgithub}.
With the same policy learning method, we compare our \ours with two defense baselines: 
(1) \textbf{(Vanilla)}: vanilla training without defense, which learns a policy based on all benign messages. 
(2) \textbf{(AT)} adversarial training as in~\cite{zhang2021robust}, which alternatively trains an adaptive RL attacker and an agent. 
% As is common in related work~\cite{lowe2017multi,gupta2017cooperative}, we use parameter sharing and train a shared policy network for all agents.
% Due to the symmetricity of the agents, we train \ours and baselines using PPO~\cite{schulman2017proximal} with parameter sharing~\cite{terry2020parameter}. 
% For MNIST-Classification, our implementation is based on \cite{mnistgithub} that reproduces the results of~\cite{mousavi2019multi}. 
During training and defending, we set the ablation size \ours as $k=2$, as suggested by Equation~\eqref{eq:k_cond} for both $N=9$ (FoodCollector) and $N=10$ (\marketenv). For AT, we train the agent against $C=2$ learned adversaries. 
More implementation details are provided in Appendix~\ref{app:exp_imple}.

\textbf{Evaluation Metrics}\quad
To evaluate the effectiveness of our defense strategy, we test the performance of the trained policies under no attack and under various values of $C$ (for simplicity, we refer to $C$ as the \textit{number of adversaries}). 
Different from previous work~\cite{blumenkamp2020emergence} where the adversarial agent disrupts all the other agents, we consider the case where the attacker deliberately misleads a selected victim, which could evaluate the robustness of the victim under the harshest attacks. We report the victim's local reward under the following two types of attack methods: 
(1) \textit{Non-adaptive attack} that perturbs messages based on heuristics. In FoodCollector, we consider randomly generated messages within the valid range of communication messages. Note that this is already a strong attack since a randomly generated message could be arbitrary and far from the original benign message. For \marketenv where messages have clear physical meanings (demand of buyers), we consider 3 realistic attacks: \permute, \swap, \flip, which permute, swap or flip the demand observations, respectively, as detailed in Appendix~\ref{app:exp_imple:market}. 
(2) \textit{Learned adaptive attack} that learns the strongest/worst adversarial communication with an RL algorithm to minimize the victim's reward (a white-box attacker which knows the victim's reward). The learned attack can strategically mislead the victim.
As shown in prior works~\cite{zhang2020robust,zhang2021robust,sun2021strongest}, the theoretically optimal attack (which minimizes the victim's reward) can be formed as an RL problem and learned by RL algorithms. 
Therefore, we can regard this attack as a worst-case attack for the victim agents.
% Therefore, we train an RL attacker policy that maps adversarial agent's observations to adversarial communications. 
More details are in Appendix~\ref{app:exp_imple}.





\textbf{Experiment Results}\quad
The results are shown in Figure~\ref{fig:res_all}. 
We can see that the rewards of Vanilla and AT drastically drop under attacks. Under strong adaptive attackers, Vanilla and AT sometimes perform worse than a non-communicative agent shown by dashed red lines, which suggests that communication can be a double-edged sword. Although AT is usually effective for $\ell_p$ attacks~\cite{zhang2021robust}, we find that AT does not achieve better robustness than Vanilla, since it can not adapt to arbitrary perturbations to several messages.
% because the strong attacker we consider can arbitrarily perturb a subset of messages. 
(More analysis of AT is in Appendix~\ref{app:exp_imple}.)
In contrast, \textit{\ours can utilize benign communication well while being robust to adversarial communication. }
We use $k=2$ for our \ours, which in theory provides performance guarantees against up to $C=2$ adversaries for $N=9$ and $N=10$. 
We can see that the reward of \ours under $C=1$ or $C=2$ is similar to its reward under no attack, matching our theoretical analysis. 
Even under 3 adversaries where the theoretical guarantees no longer hold, \ours still obtains superior performance compared to Vanilla and AT.
Therefore, \textit{\ours makes agents robust under varying numbers of adversaries.} 
% Moreover, we find that AT does not achieve better robustness than Vanilla, although AT is usually effective for $\ell_p$ attacks~\cite{zhang2021robust}. One possible reason is that the message perturbation is relatively large, such that it is hard for AT to adapt to adversaries, as explained in Appendix~\ref{app:exp_imple}.

\begin{wrapfigure}{r}{0.3\textwidth}
\vspace{-1.5em}
\hspace{-1em}
 \centering
 \resizebox{0.28\columnwidth}{!}{\input{figs/mnist/MNIST_Adaptive_Attacker_Precision}}
 \vspace{-0.5em}
\caption{\textbf{(MARL-MNIST)}: Precision of MARL classification on MNIST without or with \ours, under learned adaptive attacks.}
\vspace{-1em}
\label{fig:res_mnist_sample}
\end{wrapfigure}

\textbf{Additional Results in MARL Image Classification}\quad
In addition to the above two environments, we also evaluate our proposed \ours defense in an MARL classification task in the MNIST dataset, which is proposed by Mousavi et al.~\cite{mousavi2019multi}. In this classification problem, every agent observes a local patch of an image and takes actions to move to adjacent patches. Agents are allowed to communicate with their encoded local beliefs which are \textit{learned} by LSTM networks~\cite{hochreiter1997long}. Figure~\ref{fig:res_mnist_sample} shows the classification precision of \ours and baselines under adaptive attacks. We can see that the attacks significantly mislead Vanilla and AT, while \ours stays robust.
% Results show that the original policies are vulnerable to adversarial attacks ($17.3\%$ reward drop under strong adaptive attacks), and applying \ours to the policies significantly improves their robustness (less than $3\%$ reward drop under strong adaptive attacks). 
More details and results of this task are provided in Appendix~\ref{app:exp_mnist}.

% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-1em}
% \centering
%     \begin{subfigure}[t]{0.24\columnwidth}
%         \centering
%         \resizebox{\textwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_cont}}
%         \vspace{-1.5em}
%         \caption{\small{FoodCollector (Cont.)}}
%         % \label{sfig:maxq}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\columnwidth}
%         \centering
%         \resizebox{\textwidth}{!}{\input{figs/MarketEnv/MarketEnv_Ablation_k_2adv}}
%         \vspace{-1.5em}
%         \caption{\small{MarketEnv}}
%         % \label{sfig:maxq}
%     \end{subfigure}
%     \vspace{-0.5em}
%     \caption{\small{Hyperparameter test of ablation size $k$ in (a) continuous-action FoodCollector and (b) MarketEnv.}}
%     \label{fig:hyper_k}
% \vspace{-1em}
% \end{wrapfigure}


\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2em}
% \hspace{-1em}
 \centering
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_2adv_dist}}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.24\columnwidth}
  \resizebox{\columnwidth}{!}{\input{figs/FoodCollector_Ablation_k_sample_dist}}
 \end{subfigure}
 \vspace{-0.5em}
\caption{Natural and robust performance of \ours with various values of \textbf{(left)} ablation size $k$ and \textbf{(right)} sample size $D$ in discrete-action FoodCollector under $C=2$. 
% \textbf{Left:}   with various ablation size $k$. \textbf{Right:} Robust performance with various sample size $D$. 
% Dashed green line refers to the robust performance of Vanilla under $C=2$ attacks.
}
\vspace{-1em}
\label{fig:res_k_dist}
\end{wrapfigure}



% \textbf{Ablation Size $k$: Balancing between Performance and Robustness}\quad
% As pointed out in literature~\cite{tsipras2018robustness,zhang2019theoretically}, there exists a \textit{trade-off between robustness and accuracy}. 
% In a CMARL problem, the more an agent trusts communications from others, the more it may benefit from additional information, but it is exposed to the risk of being attacked. 
% We find that the ablation size $k$ directly controls such a trade-off: when $k$ is small, the \ensname is more robust since there are much more purely-benign messages than adversarial messages. However, the trained \ablname may not obtain a high reward with $k$ messages.
% Therefore, we can adjust $k$ based on our practical needs.
% If we know $C$ (or an upper bound of $C$), we can set $k$ to be the largest integer satisfying Condition~\ref{cond:k} such that the natural performance is not compromised much. 
% If $C$ is unknown, any selection of $k$ can provide a certificate for the largest $C$ satisfying Condition~\ref{cond:k}.
% % which shows how many adversarial messages the policy can tolerate. 
% Figure~\ref{fig:ablation_cnk} in Appendix~\ref{app:hyper} demonstrates the numerical relationships among $C$, $k$ and $N$ with Condition~\ref{cond:k}, where we can see that a smaller $k$ enables guaranteed defense against more adversarial messages. 
\textbf{Hyperparameter Tests of Ablation Size $\boldsymbol k$}\quad
As discussed in Section~\ref{sec:algo_theory}, the ablation size $k$ controls the trade-off between natural performance and robustness. 
To see the empirical influence of $k$, we evaluate \ours's natural reward and reward under $C=2$ attacks with different ablation sizes $k$. 
The results in discrete-action FoodCollector is shown in Figure~\ref{fig:res_k_dist}(left), while results in other environments are similar and are put in Appendix~\ref{app:exp_results}.
We observe that a larger $k$ leads to higher natural performance since each agent could gather more information from others. However, raising $k$ also increases the risk of making decisions based on communication messages sent from an adversary. Therefore, \textit{increasing ablation size $k$ trades off robustness for natural performance.} On the other hand, $k=2$ as the largest solution to Equation~\eqref{eq:k_cond}, achieves a good balance between performance and robustness.
% there exist a ``sweet spot'' (e.g., $k=2$), where the performance and robustness are well-balanced.

\textbf{Hyper-parameter Test of Sample Size $\boldsymbol D$}\quad
We further evaluate the partial-sample variant of \ours introduced in Section~\ref{sec:algo_more} using $k=2$ under $C=2$ adversaries, with $D$ varying from $N-1 \choose k$ (the largest sample size) to 1 (the smallest sample size). Figure~\ref{fig:res_k_dist}(right) demonstrate the performance of different $D$'s in discrete-action FoodCollector, and Appendix~\ref{app:exp_results} shows other results. 
As $D$ goes down, \ours obtains lower reward under attackers, but it is still significantly more robust than baseline methods. For example, \ours in FoodCollector obtains much higher reward than Vanilla under attacks even when $D=1$ (using only 1 random \ksample). 
% which is both computationally efficient and robust.






==> neurips/6_discuss.tex <==
\vspace{-0.5em}
\section{Conclusion}
\label{sec:discuss}
\vspace{-0.5em}

This paper formulates communication attacks in MARL problems, and proposes a defense framework \ours, which is certifiably robust against multiple arbitrarily perturbed adversarial communication messages, based on randomized ablation and aggregation of messages. 
\ours can easily scale up and extend to many real-world tasks. 
Environments verify the effectiveness of \ours in different tasks.
% \ys{flexibility of different $k$'s in training and test.}

==> neurips/a1_related.tex <==
\section{Additional Related Work}
\label{app:related}

% \textbf{Adversarial Robustness of RL Agents}\quad
% As RL techniques have been applied to more and more applications, the robustness of agents under environment noise or adversarial attacks becomes an emerging research topic. 
% For a single-agent problem, there are many recent works on adversarial state perturbation~\cite{huang2017adversarial,zhang2020robust} and action perturbation~\cite{tan2020robustifying,tessler2019action}. In a multi-agent system, the interplay among agents introduces more uncertainty to the environment. \cite{gleave2020adversarial} point out that a well-trained agent can be completely misled by adversarial behaviors of another agent. Although adversarial training (i.e., introducing adversarial agents to the system during training~\cite{pinto2017robust,phan2021resilient}) can empirically improve agents' robustness, such robustness is not guaranteed to hold under all possible attackers.


% \textbf{Certifiable Defense}\quad
% There is an important line of work studying guaranteed robustness of neural networks~\cite{raghunathan2018certified,cohen2019certified,gowal2018effectiveness} while the input data is perturbed within an $\ell_p$ norm ball. In an effort to certify RL agents' robustness, \cite{lutjens2020certified} and \cite{oikarinen2020robust} utilize convex relaxation of Q networks to improve the worst-case performance of agents. \cite{kumar2021policy} and \cite{wu2021crop} follow the idea of randomized smoothing~\cite{cohen2019certified} and smooth out the policy by adding Gaussian noise to the input.
% To the best of our knowledge, our \ours is the first certifiable defense in MARL against communication attacks. Moreover, we consider a strong threat model where up to half of communication messages can be arbitrarily corrupted. 
% % \ys{flexibility}

\textbf{Communication in MARL}\quad
Communication is crucial in solving collaborative MARL problems. There are many existing studies learning communication protocols across multiple agents. Foerster et al. \cite{foerster2016learning} are the first to learn differentiable communication protocols that is end-to-end trainable across agents. Another work by Sukhbaatar et al. \cite{sukhbaatar2016learning} proposes an efficient permutation-invariant centralized learning algorithm which learns a large feed-forward neural network to map inputs of all agents to their actions. 
It is also important to communicate selectively, since some communication may be less informative or unnecessarily expensive. To tackle this challenge, Das et al. \cite{das2020tarmac} propose an attention mechanism for agents to adaptively select which other agents to send messages to. Liu et al. \cite{liu2020who2com} introduce a handshaking procedure so that the agents communicate only when needed. Our work assumes a pre-trained communication protocol and does not consider the problem of learning communication mechanisms.

==> neurips/a2_theory.tex <==
\section{Additional Theoretical Definitions and Analysis}
\label{app:theory}

\textbf{Relation between Communication Attack and $\boldsymbol \ell_0$ Observation Attack}\quad
The communication threat model described in Section~\ref{sec:setup_adv} is analogous to a constrained $\ell_0$ attack on policy inputs. When agent $i$ is attacked, the input space of its acting policy $\pi_i$ is $\mathcal{X}_i := \hisspace_i \times \mathcal{M}^{N-1}$. Therefore, when $C$ communication messages are corrupted, the original input $x_i$ gets perturbed to $\tilde{x}_i$. Let $d$ be the dimension of a communication message, then $x_i$ and $\tilde{x}_i$ differ by up to $dC$ dimensions, which is similar to an $\ell_0$ attack constrained in certain dimensions. 



\subsection{Additional Analysis of \ours in Discrete Action Space}
\label{app:theory_dist}

\textbf{Reward Certificate}\quad
Theorem~\ref{thm:main_dist} justifies that under sufficient majority votes, the \ensname $\smpolicy$ ignores the malicious messages in $\mathbf{m}_{\mathrm{adv}}$ and executes a benign action that is suggested by some benign message combinations, even when the malicious messages are not identified.
It is important to note that, when the \ensname $\smpolicy$ selects an action $\widetilde{a}$, there must exist at least one purely benign \ksample that let the \ablname $\ablpolicy$ produce $\widetilde{a}$. Therefore, as long as $\ablpolicy$ can obtain high reward with randomly selected benign \ksamples, $\smpolicy$ can also obtain high reward with ablated adversarial communication due to its design.

% Specifically, with ensemble policy $\smpolicy$, the agent's cumulative reward under adversarial communications would be similar to the natural reward of $\ablpolicy$ under no attacks, as justified in the following corollary.
% The corollary below shows the relationship between the attacked reward of $\smpolicy$ and the natural reward of $\ablpolicy$. Note that $\ablpolicy$ is the policy learned during training time in a clean (non-adversarial) environment, and it is easy for us to evaluate its natural cumulative reward. $\smpolicy$ is 
% \fh{I feel the current description doesn't make it easy to  distinguish between $\ablpolicy$ and $\smpolicy$.}
Specifically, we consider a specific agent with \ablname $\ablpolicy$ and \ensname $\smpolicy$ (suppose other agents are executing fixed policies). 
Let $\nu:\mathcal{M}^{N-1}\to\mathcal{M}^{N-1}$ be an attack algorithm that perturbs at most $C$ messages in a message set. 
Let $\zeta \sim Z(P,\ablpolicy)$ be a trajectory of policy $\ablpolicy$ under no attack, i.e., $\zeta=(o^{(0)},\msg^{(0)},a^{(0)},r^{(0)},o^{(1)},\msg^{(1)},a^{(0)},r^{(0)},\cdots)$. (Recall that a \ablname $\ablpolicy$ takes in a random size-$k$ subset of $\msg\step$ and outputs action $a\step$.)
When there exists attack with $\nu$, let $\zeta_\nu \sim Z(P,\smpolicy;\nu)$ be a trajectory of policy $\smpolicy$ under communication attacks, i.e., $\zeta_\nu=(o^{(0)},\nu(\msg^{(0)}),a^{(0)},r^{(0)},o^{(1)},\nu(\msg^{(1)}),a^{(0)},r^{(0)},\cdots)$. 
For any trajectory $\zeta$, let $r(\zeta)$ be the discounted cumulative reward of this trajectory.

% Let $\zeta=(o^{(0)},\msg^{(0)},a^{(0)},r^{(0)},o^{(1)},\msg^{(1)},a^{(0)},r^{(0)},\cdots)$ denote a trajectory. If \ablname is used, we have 
% $a\step = \ablpolicy(\his\step, \msgk)$ where $\msgk\sim\mathrm{Uniform}(\mathcal{H}_{k}(\msg\step))$. If \ensname is used, we have $a\step = \smpolicy(\his\step, \msg\step)$. 
% Let $\natobj(\zeta)$ denote the natural cumulative reward of a policy under no attack.
% Let $\advobj(\zeta)$ denote the cumulative reward of a policy under attacks, where at every step $t$, up to $C$ messages in the message set $\msg\step$ can be perturbed arbitrarily.

With the above notations, we propose the following reward certificate.
% let $\goodmsg\step$ and $\advmsg\step$ be the original benign message list and the perturbed message list the agent receives at step $t$, respectively. We use 
% \begin{equation}
%     \natobj(\pi) := J(\pi|\goodmsg^{(1)}, \goodmsg^{(2)},\cdots)
% \end{equation}
% to denote the expected cumulative reward of policy $\pi$ when it receives benign messages $\goodmsg^{(1)}, \goodmsg^{(2)},\cdots$, and use
% \begin{equation}
%     \advobj(\pi) := J(\pi|\advmsg^{(1)}, \advmsg^{(2)},\cdots)
% \end{equation}
% to denote the expected cumulative reward of policy $\pi$ when it receives perturbed messages $\advmsg^{(1)}, \advmsg^{(2)},\cdots$. Then, the following corollary presents the reward certificate of the \ensname when the agent's action space is discrete.

\begin{corollary}[Reward Certificate for Discrete Action Space]
\label{cor:reward_dist}
When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold at every step of execution, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} under adversarial communication is no lower than the lowest cumulative reward that the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
\begin{equation}
\begin{aligned}
    \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta),
    %  \min_{\advmsg^{(1)}, \advmsg^{(2)},\cdots} \advobj(\smpolicy) \geq \min_{[\goodmsg^{(1)}]_k,[\goodmsg^{(2)}]_k,\cdots} \natobj(\ablpolicy),
    % \advobj(\smpolicy) \geq \min_{\msgk^{(1)},\msgk^{(2)},\cdots} \natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)
    % \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
\end{aligned}
\end{equation}
for any attacker $\nu$ satisfying Assumption~\ref{assum:num} ($C<\frac{N-1}{2}$).
% where $[\goodmsg\step]_k\sim\mathrm{Uniform}(\mathcal{H}_{k}(\goodmsg\step))$.
% where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under arbitrary attacks to up to $C$ communication messages, and $\natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ when the random \ksample in the first step is $\msgk^{(1)}$, the random \ksample in the second step is $\msgk^{(2)}$, etc.
\end{corollary}

\textbf{Remarks.} 
(1) The certificate holds for any attack algorithm $\nu$ with $C<\frac{N-1}{2}$. 
(2) The \ablname $\ablpolicy$ has extra randomness from the sampling of \ksamples. That is, at every step, $\ablpolicy$ takes a uniformly randomly selected \ksample from $\allmsgk$. Therefore, the $\min_\zeta$ in the RHS considers the worst-case message sampling in the clean environment without attacks. Since $\smpolicy$ always takes actions selected by some purely-benign message combinations, the trajectory generated by $\smpolicy$ can also be produced by the \ablname.
(3) Note that the RHS ($\min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta)$) can be approximately estimated by executing $\ablpolicy$ during training time, so that the test-time performance of $\smpolicy$ is guaranteed to be no lower than this value, even if there are up to $C$ corrupted messages at every step.

% \begin{corollary}[Reward Certificate for Discrete Action Space]
% \label{cor:reward_dist}
% \fh{Under sample size $D=\binom{N-1}{k}$, the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} with a message subset size $k$ satisfying Equation~\eqref{eq:k_cond} obtains a total reward no worse than that obtained by the base ablation policy $\ablpolicy$ using benign messages:
% \begin{align}
%   & \advobj\Big(\smpolicy\big(o, \{\funabl(\advmsg, T_d)\}_{d=1}^D\big)\Big) \geq \nonumber \\
%   & \min_{T} \natobj\Big(\ablpolicy\big(o, \funabl(\goodmsg, T)\big)\Big) \label{eq:reward_dist}
% \end{align}
% if the majority votes $u_{\tilde{a}}$ satisfies $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step.
% }
% \textcolor{red}{Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If $D=\binom{N-1}{k}$, and the majority votes satisfy 
% $u_{\tilde{a}} > \binom{N-1}{k} - \binom{N-1-C}{k}$ at every step, 
% then the total reward of $\smpolicy$ satisfies
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \begin{equation}
% \label{eq:reward_dist}
%     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy),
% \end{equation}}
% Here $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the \textcolor{red}{sampled message indices}\fh{indices of the message subsets?} used by $\ablpolicy$ at all steps. \fh{What does this mean? My equation doesn't use $\tau$, rather I use $T$.}
% \end{corollary}


Appendix~\ref{app:proof} provides detailed proofs for the above theoretical results.


\subsection{Additional Analysis of \ours in Continuous Action Space}
\label{app:theory_cont}

\input{\texhome/theory_cont}



\subsection{Extension of \ours with Partial Samples}
\label{app:theory_sample}

As motivated in Section~\ref{sec:algo_more}, our \ours can be extended to a partial-sample version, where the ensemble policy is constructed by $D$ instead of $\binom{N-1}{k}$ samples. Let $\allmsgkd$ be a subset of $\allmsgk$ that contains $D$ random \ksamples from $\allmsgk$. Then the $D$-ensemble policy $\pi_D$ is defined as
\begin{equation}
\label{eq:ensemble_pi_dist_d}
    \smpolicy_D(\his, \mathbf{m}) := \mathrm{argmax}_{a\in\mathcal{A}} \sum_{\msgk\in\allmsgkd} \mathbbm{1}[\ablpolicy(o, \msgk)=a],
\end{equation}
for a discrete action space, and
\begin{equation}
\label{eq:ensemble_pi_cont_d}
    \tilde{\pi}_D(\his, \mathbf{m}) = \funmed \{\ablpolicy(\his, \msgk) \}_{\msgk\in\allmsgkd}.
\end{equation}\normalsize
for a continuous action space. 

In the partial-sample version of \ours, we can still provide high-probability robustness guarantees. 



For notation simplicity, let $n_1=\binom{N-1}{k}$, $n_2=\binom{N-C-1}{k}$. 
Define the majority vote as 
\begin{equation}
\label{eq:vote}
    u_{\max}:=\max_{a\in\mathcal{A}} \sum\nolimits_{\msgk\in\allmsgkd} \mathbbm{1}[\ablpolicy(\his, \msgk)=a].
\end{equation}
The following theorem shows a general guarantee for $D$-ensemble policy in a discrete action space. 

\begin{theorem}[General Action Guarantee for Discrete Action Space]
\label{thm:sample_dist}
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_dist_d} with an ablation size $k$ satisfying Condition~\ref{cond:k},
Relation~\eqref{eq:cert_dist} holds deterministically if the majority vote $u_{\max}>n_1-n_2$. 
Otherwise it holds with probability at least
%\vspace{-0.1cm}
\begin{equation}
\label{eq:p_sample_dist}
    p_D=\frac{\sum_{j=0}^{u_{\max}-1}\binom{n_1-n_2}{j}\binom{n_2}{D-j}}{\binom{n_1}{D}}.
\end{equation}
\end{theorem}
Note that Theorem~\ref{thm:main_dist} is a special case of Theorem~\ref{thm:sample_dist}, since it assumes $u_{\max}>n_1-n_2$. 


Theorem~\ref{thm:sample_cont} below further shows the theoretical result for a continuous action space.

\begin{theorem}[General Action Guarantee for Continuous Action Space]
\label{thm:sample_cont}
Given an arbitrary sample size $0<D\leq\binom{N-1}{k}$, for the $D$-ensemble policy $\smpolicy_D$ defined in Equation~\eqref{eq:ensemble_pi_cont_d} with an ablation size $k$ satisfying Condition~\ref{cond:k}, Relation~\eqref{eq:cert_cont} holds with probability at least
\begin{equation}
\label{eq:p_sample_cont}
    p_D=\frac{\sum_{j=\tilde{D}}^{D}\binom{n_2}{j}\binom{n_1-n_2}{D-j}}{\binom{n_1}{D}},
\end{equation}
where $\tilde{D} = {\lfloor \frac{D}{2} \rfloor}+1$. 
\end{theorem}

The larger $D$ is, the higher the probability $p_D$ is, the more likely that the \ensname selects an action in $\safeactioncont$.
In Theorem~\ref{thm:sample_cont}, when $D=\binom{N-1}{k}$,  the probability $p_D$ is 1 and the result matches Theorem~\ref{thm:main_cont}. 


Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.

==> neurips/a7_algo.tex <==
\section{Algorithm Pseudocode}
\label{app:algo}


Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test} demonstrate the procedures of \ours in training and defending phases, respectively. 
\input{algo_train}
\input{algo_test}




==> neurips/theory_cont.tex <==


\textbf{Action Certificate}\quad
As in the discrete action case, the continuous ensemble policy will output an action $\widetilde{a}$ that follows the consensus of benign messages. But in a continuous action space, it is hard to ensure that $\widetilde{a}$ is exactly in $\safeaction$. Instead, $\widetilde{a}$ is guaranteed to be within the range of $\safeaction$, as detailed in the following theorem.

\begin{theorem}[Action Certificate for Continuous Action Space]
\label{thm:main_cont}
Under Condition~\ref{cond:k}, the action $\widetilde{a} = \smpolicy(\his, \advmsg)$ generated by the ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} satisfies
\begin{equation}
    \widetilde{a} \in \mathsf{Range}(\safeaction) := \{a: \forall 1\leq l \leq L, \exists \underline{a}, \overline{a} \in \safeaction \text{ s.t } \underline{a}_l \leq a_l \leq \overline{a}_l \}.
    \label{eq:cert_cont}
\end{equation}
% then any dimension $l$ of $\smpolicy$'s output satisfies
% \begin{equation*}
%     \inf_{\krv} [\hat{a}]_l  
%     \leq [\smpolicy(o, \advmsg, \{T_d\}_{d=1}^D)]_l 
%     \leq \sup_{\krv} [\hat{a}]_l.
% \end{equation*}
% where $\hat{a} := \ablpolicy(o, \mathsf{Ablate}(m, \krv))$.
\end{theorem}

In other words, if the \ensname takes an action $\widetilde{a}$, then at each dimension $l$, there must exist $a_1$ and $a_2$ suggested by some purely benign \ksamples such that the $l$-th dimension of $\widetilde{a}$ is lower and upper bounded by the $l$-th dimension of $a_1$ and $a_2$, respectively. 
Note that Theorem~\ref{thm:main_cont} certifies that the selected action is in a set of actions that are close to benign actions $\mathsf{Range}(\safeaction)$, but does not make any assumption on this set. Next we interpret this result in details.

\textbf{How to Understand $\mathsf{Range}(\safeaction)$?}\quad
Theoretically, $\mathsf{Range}(\safeaction)$ is a set of actions that are coordinate-wise bounded by base actions resulted from purely benign \ksamples. In many practical problems, it is reasonable to assume that actions in $\mathsf{Range}(\safeaction)$ are relatively safe, especially when benign actions in $\safeaction$ are concentrated. The following examples illustrate some scenarios where actions in $\mathsf{Range}(\safeaction)$ are relatively good.

\begin{enumerate}
    \item If the action denotes the price a seller sells its product in a market, and the communication messages are the transaction signals in an information pool, then $\mathsf{Range}(\safeaction)$ is a price range that is determined based on purely benign messages. Therefore, the seller will set a reasonable price without being influenced by a malicious message. 
    \item If the action denotes the driving speed, and benign message combinations have suggested driving at 40 mph or driving at 50 mph, then driving at 45 mph is also safe. 
    \item If the action is a vector denoting movements of all joints of a robot (as in many MuJoCo tasks), and two slightly different joint movements are suggested by two benign message combinations, then an action that does not exceed the range of the two benign movements at every joint is likely to be safe as well.
\end{enumerate}  

The above examples show by intuition why the \ensname can be regarded as a relatively robust policy. 
However, in extreme cases where there exists ``caveat'' in $\mathsf{Range}(\safeaction)$, taking an action in this set may also be unsafe. To quantify the influence of $\mathsf{Range}(\safeaction)$ on the long-term reward, we next analyze the cumulative reward of the \ensname in the continuous-action case.



\textbf{How Does $\mathsf{Range}(\safeaction)$ Lead to A Reward Certificate?}\quad
Different from the discrete-action case, the \ensname $\smpolicy$ in a continuous action space may take actions not in $\safeaction$ such that it generates trajectories not seen by the \ablname $\ablpolicy$. However, since the action of $\smpolicy$ is guaranteed to stay in $\mathsf{Range}(\safeaction)$, we can bound the difference between the value of $\smpolicy$ and the value of $\ablpolicy$, and how large the different is depends on some properties of $\mathsf{Range}(\safeaction)$.

Concretely, Let $R$ and $P$ be the reward function and transition probability function of the current agent when the other agents execute fixed policies. So $R(s,a)$ is the immediate reward of taking action $a$ at state $s$, and $P(s^\prime|s,a)$ is the probability of transitioning to state $s^\prime$ from $s$ by taking action $a$. (Note that $s$ is the underlying state which may not be observed by the agent.)
% Let $R_{\max}$ denote the supremum of the absolute value of $R$, i.e., $R_{\max}:=\sup_{s,a} |R(s,a)|$. 

\begin{definition}[Dynamics Discrepancy of $\ablpolicy$]
\label{def:disc}
A \ablname $\ablpolicy$ is called $\epsilon_R$,$\epsilon_P$-discrepant if $\epsilon_R$, $\epsilon_P$ are the smallest values such that for any $s\in\mathcal{S}$ and the corresponding \safename set $\safeaction$, we have $\forall a_1, a_2 \in \mathsf{Range}(\safeaction)$, 
\begin{align}
    & |R(s,a_1) - R(s,a_2)| \leq \epsilon_R, \\
    & \int | P(s^\prime| s, a_1) - P(s^\prime| s, a_2) | \mathrm{d}s^\prime \leq \epsilon_P. \label{eq:p_disc}
\end{align}
% Given a \ablname $\ablpolicy$, $\mathsf{Range}(\safeaction)$
% let $f_{\ablpolicy}$ be a mapping from state $s\in\mathcal{S}$ to the corresponding benign action range induced by $\ablpolicy$ at state $s$, i.e., $f_{\ablpolicy}(s)$ is 
\end{definition}

\textbf{Remarks.}
(1) Equation~\eqref{eq:p_disc} is equivalent to that the total variance distance between $P(\cdot| s, a_1)$ and $P(\cdot| s, a_2)$ is less than or equal to $\epsilon_P/2$.
(2) For any environment with bounded reward, $\epsilon_R$ and $\epsilon_P$ always exist. 
% (3) $\epsilon_R$ and $\epsilon_P$ are related to the \ablname, the communication quality, and the environment properties. When the reward function and transition function are smooth, and when the benign communications can reach some ``consensus'' of actions by propagating through $\ablpolicy$, $\epsilon_R$ and $\epsilon_P$ will be relatively small.



Definition~\ref{def:disc} characterizes how different the local dynamics of actions in $\mathsf{Range}(\safeaction)$ are, over all possible states. If $\mathsf{Range}(\safeaction)$ is small and the environment is relatively smooth, then taking different actions within this range will not result in very different future rewards. The theorem below shows a reward certificate for the \ensname $\smpolicy$.

% When Condition~\ref{cond:k} and Condition~\ref{cond:cons} hold at every step of execution, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_dist} under adversarial communication is no lower than the lowest cumulative reward that the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
% \begin{equation}
% \begin{aligned}
%     \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta),
% \end{aligned}
% \end{equation}
% for any attacker $\nu$ satisfying Assumption~\ref{assum:num} ($C<\frac{N-1}{2}$).

\begin{theorem}[Reward Certificate for Continuous Action Space]
\label{thm:reward_cont}
Let $V^{\ablpolicy}(s)$ be the clean value (discounted cumulative reward) of $\ablpolicy$ starting from state $s$ under no attack; let $\tilde{V}^{\smpolicy}_\nu(s)$ be the value of $\smpolicy$ starting from state $s$ under attack algorithm $\nu$, where $\nu$ satisfies Assumption~\ref{assum:num}; let $k$ be an ablation size satisfying Condition~\ref{cond:k}.
If $\ablpolicy$ is $\epsilon_R$,$\epsilon_P$-discrepant, then for any state $s\in\mathcal{S}$, we have
\begin{equation}
    % \min_{\zeta_\nu\sim Z(P,\smpolicy;\nu)} r(\zeta_\nu) \geq \min_{\zeta\sim Z(P,\ablpolicy)} r(\zeta) - \frac{1}{1-\gamma}\epsilon_R - \frac{\gamma R_{\max}}{(1-\gamma)^2} \epsilon_P.
    \min_{\nu} \tilde{V}^{\smpolicy}_\nu(s) \geq V^{\ablpolicy}(s) - \frac{\epsilon_R+\gamma V_{\max}\epsilon_P}{1-\gamma},
\end{equation}
where $V_{\max} := \sup_{s,\pi}  |V^\pi(s)|$. 
% the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} is no lower than the lowest cumulative reward the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
% \begin{equation}
%     \min_{\advmsg^{(1)}, \advmsg^{(2)},\cdots} \advobj(\smpolicy) \geq \min_{[\goodmsg^{(1)}]_k,[\goodmsg^{(2)}]_k,\cdots} \natobj(\ablpolicy),
% \end{equation}
% where $[\goodmsg\step]_k\sim\mathrm{Uniform}(\mathcal{H}_{k}(\goodmsg\step))$.
\end{theorem}

\textbf{Remarks.}
(1) The certificate holds for any attack algorithm $\nu$ with $C<\frac{N-1}{2}$. 
(2) If $\epsilon_R$ and $\epsilon_P$ are small, then the performance of \ensname $\smpolicy$ under attacks is similar to the performance of the \ablname $\ablpolicy$ under no attack. 

It is important to note that $\epsilon_R$ and $\epsilon_P$ are intrinsic properties of $\ablpolicy$, independent of the attacker. Therefore, one can approximately measure $\epsilon_R$ and $\epsilon_P$ during training. 
Similar to Condition~\ref{cond:cons} required for a discrete action space, the gap between the attacked reward of $\smpolicy$ and the natural reward of $\ablpolicy$ depends on how well the benign messages are reaching a consensus. (Smaller $\epsilon_R$ and $\epsilon_P$ imply that the actions in $\safeaction$ are relatively concentrated and the environment dynamics are relatively smooth.)

Moreover, one can optimize $\ablpolicy$ during training such that $\epsilon_R$ and $\epsilon_P$ are as small as possible, to further improve the robustness guarantee of $\smpolicy$. This can be a future extension of this work.


Technical proofs of all theoretical results can be found in Appendix~\ref{app:proof}.















% Therefore, in many cases we can expect the set $\mathsf{Range}(\safeaction)$ contain good actions. 
% Mathematically, the following assumption justifies when the set $\mathsf{Range}(\safeaction)$ is guaranteed to be safe, which rules out ``bad actions'' from this set. 

% \begin{assumption}
% \label{assump:order}
% Let $R: \mathcal{S} \times \mathcal{A} \to \mathbb{R}$ be the reward function of the current agent while the other agents are executing fixed policies. For any state $s\in\mathcal{S}$, let $\safeaction$ be the \safename set generated by the trained \ablname $\ablpolicy$, then we assume that for any action $a\in\mathsf{Range}(\safeaction)$, $R(s,a) \geq \min_{\hat{a}\in\mathsf{\safeaction}} R(s,\hat{a})$.
% \end{assumption} 

% \textbf{Remarks.} \\
% (1) Assumption~\ref{assump:order} suggests that there is no ``caveat'' in the safe action set. Note that without the assumption of reward structure, there may exist extreme cases where some actions in $\safeaction$ could lead to low reward, which makes the reward not certifiable. \\
% (2) This assumption holds in many real-life scenarios where actions have concrete meanings (e.g. price, speed, etc). In practice, we can expect this assumption to hold when the safe action range generated by the ablation policy is relatively narrow, i.e., the benign communication messages achieve agreements. \\
% (3) During training, we are able to compute the \safename set $\safeaction$ at every step, so \textit{we can check whether caveats can exist before deploying the policy to a real-world agent. } \\
% % For example, if driving at 40 mph and driving at 50 mph are both safe, then driving at 45 mph is also safe. 
% (4) Assumption~\ref{assump:order} assumes that the immediate reward of action $a\in\mathsf{Range}(\safeaction)$ is no lower than the actions in $\safeaction$. But it does not necessarily
% we can further relax this assumption such that the reward it as will be discussed later.


% \textbf{Reward Certificate}\quad
% % Theorem~\ref{thm:main_cont} shows how the ensemble policy outputs an action that is coordinate-wisely bounded by the range of benign actions. 
% % Under mild assumptions, it can also lead to a reward guarantee, as detailed in Appendix~\ref{app:theory_cont}.
% % Theorem~\ref{thm:main_cont} shows how the ensemble policy outputs an action bounded by safe actions. 
% With the notations defined in Appendix~\ref{app:theory_dist} and under Assumption~\ref{assump:order}, the following reward certificate holds.

% \begin{corollary}[Reward Certificate for Continuous Action Space]
% \label{cor:reward_cont}
% Under Condition~\ref{cond:k} and Assumption~\ref{assump:order}, the cumulative reward of ensemble policy $\smpolicy$ defined in Equation~\eqref{eq:ensemble_pi_cont} is no lower than the lowest cumulative reward the ablation policy $\ablpolicy$ can obtain with randomly selected \ksamples under no attacks, i.e.,
% \begin{equation}
%     \min_{\advmsg^{(1)}, \advmsg^{(2)},\cdots} \advobj(\smpolicy) \geq \min_{[\goodmsg^{(1)}]_k,[\goodmsg^{(2)}]_k,\cdots} \natobj(\ablpolicy),
% \end{equation}
% where $[\goodmsg\step]_k\sim\mathrm{Uniform}(\mathcal{H}_{k}(\goodmsg\step))$.
% % \begin{equation}
% % \begin{aligned}
% %     \advobj(\smpolicy) \geq \min_{\msgk^{(1)},\msgk^{(2)},\cdots} \natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)
% %     % \min_{T_1\in\mathcal{H}(N-1,k),T_2\in\mathcal{H}(N-1,k),\cdots} \natobj(\ablpolicy|T_1,T_2,\cdots)
% % \end{aligned}
% % \end{equation}
% % where $\advobj(\smpolicy)$ is the cumulative reward obtained by $\smpolicy$ under arbitrary perturbations to up to $C$ communication messages, and $\natobj(\ablpolicy|\msgk^{(1)},\msgk^{(2)},\cdots)$ is the natural cumulative reward obtained by $\ablpolicy$ when the random \ksample in the first step is $\msgk^{(1)}$, the random \ksample in the second step is $\msgk^{(2)}$, etc.
% \end{corollary}


% \textbf{Relaxation of Assumption~\ref{assump:order}}\quad
% Assumption~\ref{assump:order} can hold in practice when the environment reward has ordered structures, or when benign actions are concentrated enough. As we have access to $\safeaction$ during training, one can estimate $\epsilon$ at every step and the worst-case reward drop. Then, the test-time performance can be lower bounded, and the agent will not be significantly reduced by any attacks. 
% In cases where Assumption~\ref{assump:order} does not hold, we can also relax it such that $R(s,a) \geq \min_{\hat{a}\in\mathsf{\safeaction}} R(s,\hat{a}) - \epsilon$ for some $\epsilon \geq 0$. Then the reward certificate in Theorem~\ref{thm:main_cont} can be relaxed to a softer version where the $\advobj(\smpolicy)$ is still lower bounded. 


% % \begin{corollary}[Reward Certificate for Continuous Action Space]
% % \label{cor:reward_cont}
% % Assume that $k$ and $\smpolicy$ satisfy Equation~\eqref{eq:k_cond} and~\eqref{eq:ensemble_pi_dist}. If Assumption~\ref{assump:order} holds, and $D=\binom{N-1}{k}$, 
% % then the total reward of $\smpolicy$ satisfies
% % \begin{equation}
% % \label{eq:reward_cont}
% %     \advobj(\smpolicy) \geq \min_{\tau} \natobj(\ablpolicy)
% % \end{equation}
% % where $\tau=[\krv_{k,N-1}^{(1)}, \krv_{k,N-1}^{(2)}, \cdots]$ denotes the sampled message indices used by $\ablpolicy$ at all steps.
% % \end{corollary}
